Interventional Speech Noise Injection for ASR Generalizable Spoken Language Understanding

Recently, pre-trained language models (PLMs) have been increasingly adopted in spoken language understanding (SLU). However, automatic speech recognition (ASR) systems frequently produce inaccurate transcriptions, leading to noisy inputs for SLU models, which can significantly degrade their performance. To address this, our objective is to train SLU models to withstand ASR errors by exposing them to noises commonly observed in ASR systems, referred to as ASR-plausible noises. Speech noise injection (SNI) methods have pursued this objective by introducing ASR-plausible noises, but we argue that these methods are inherently biased towards specific ASR systems, or ASR-specific noises. In this work, we propose a novel and less biased augmentation method of introducing the noises that are plausible to any ASR system, by cutting off the non-causal effect of noises. Experimental results and analyses demonstrate the effectiveness of our proposed methods in enhancing the robustness and generalizability of SLU models against unseen ASR systems by introducing more diverse and plausible ASR noises in advance.

==> backup/230703/0_abs.tex <==
\begin{abstract}
This paper proposes ASR-generalizable speech noise injection (SNI) for improving spoken language understanding (SLU) models in the presence of ASR errors. Pretrained language models (PLMs) trained on written language struggle to adapt to the differences in spoken language, especially due to phonetic misunderstanding and misspelling errors introduced by ASR systems. While previous works have explored SNI, the generalizability of SLU models to different ASR systems remains understudied. We factorize ASR errors into two steps: phonetic misunderstanding and misspelling, and demonstrate that misspelling errors are more model generalizable compared to phonetic misunderstanding. To explicitly model these steps, we propose constrained generation, focusing on regenerating ASR-noised words. The approach enables targeted generation and improves the robustness and generalizability of SLU models. Experimental results and analysis are provided to support the effectiveness of ASR-generalizable SNI.
\end{abstract}

==> backup/230703/1_intro.tex <==
\section{Introduction}
Starting from ELMo~\cite{peters-etal-2018-deep} to recent GPT4~\cite{openai2023gpt4}, pretrained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
As such abilities are essential for spoken language understanding (SLU)~\cite{broscheit-etal-2022-distributionally, 8907842}, PLMs are widely adopted in speech-enabled systems such as voice assistants.
Specifically,  PLMS are adopted in a  pipeline  process of such speech-enabled systems. 
First, audio is converted into textual transcription by an automatic speech recognition (ASR) system. 
Then, the transcription is fed into PLMs to conduct various tasks. 


As PLMs are trained in the different modality of written text, they suffer to adapt to the difference between the transcription and text.
The key difference disturbing PLMs in SLU is the errors of the ASR systems.
Specifically, ASR systems confuse to generate phonetically similar and semantically different words, ASR error words~\cite{ruan20_interspeech,9054689}.
Blinded to such phonetic similarities, PLMs suffer to understand the semantics from such corrupted input.
Previous works show that even a small corruption made by ASR systems could disturb PLMs~\cite{belinkov2018synthetic}.

%데이터
Adopting subword tokenization such as byte pair encoding, previous work showed that PLMs could robustly understand the semantics under such corruption when they are trained on transcriptions~\cite{heigold-etal-2018-robust}.
However, collecting sufficient SLU corpora to train PLMs is more demanding than the written corpora.
Specifically, collecting SLU corpora requires the additional step from collected written corpora, Recording and Transcription, where human annotators read the collected written corpora, and their readings are recorded as audio.
Then, the audio recordings are then transcribed using ASR systems.


Due to the additional effort of the recording step, data augmentation methods of corrupting the written corpora have been widely researched, which we call speech noise injection (SNI).
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, SNI aims to corrupt $X$ to pseudo-ASR transcription, $X^{\prime}=\{x^{\prime}_{i}\}_{i=1}^{n^{\prime}}$ which contains phonetically similar but semantically different ASR error words.
Then, generated pseudo-ASR, $X^{\prime}$, is used to train downstream models.
Trained on pseudo-ASR, downstream models can robustly understand the transcriptions with ASR errors.

Previous works in SNI can be categorized into two methods. 
The most intuitive method is the TTS-ASR pipeline, where the TTS engine (text-to-speech) converts the text into audio, and the ASR system transcribes the audio.
While ASR errors are generated by TTS engines and ASR systems, they are both computationally expensive.
Additionally, they cannot generate sufficient ASR errors as the noise engaged during human reading does not exist in the audio converted by TTS.
In contrast, generative SNI supervises the autoregressive language model $M$ to generate the pseudo-ASR given the text as the following:
\begin{equation}
    X^{\prime} = M(X)
\end{equation}
As generative SNI is shown to be effective in various situations~\cite{asrglue}, we focus on generative SNI.

While many previous works studied generative SNI~\cite{feng22c_interspeech, noisygen}, ASR-generalizability, the ability of an SLU model to perform robustly across different ASR systems,  is not well studied.
However, such generalizability has been focused on diverse SLU tasks~\cite{blackbox1} as ASR systems are often adopted in SLU as black-box models, meaning that their internal state is not accessible or transparent~\cite{blackbox1}.
Also, training PLMs for numerous ASR systems is intractable.

For ASR generalizable SNI, we factorize the generation of ASR errors into two distinct steps: phonetic misunderstanding and misspelling.
In the phonetic misunderstanding step, the ASR system misinterprets the spoken phonemes, leading to inaccuracies in the resulting transcription. 
Consequently, the subsequent step, misspelling, arises as a result of the ASR system generating misspelled words based on its flawed understanding of the original speech. 
Misspelling errors occur when the ASR system incorrectly converts the misunderstood phonemes into different characters, further deviating from the intended transcription. 

\input{table/asr_cer}

Among two distinct steps, we argue that  
while the phonetic misunderstanding is ASR-specific noise, the misspelling step is ASR-generalizable.
Specifically, phonetic misunderstanding can be largely influenced by training data and acoustic modeling.
For example, ASR systems with distinct acoustic feature extractors and different accented training audio would exhibit distinct susceptibility to phonetic misunderstanding.
In contrast, we argue that the phenomenon of misspelling is more ASR-generalizable. 
This is because a language possesses specific spelling conventions that are shared across different ASR models regardless of training data or acoustic modeling techniques. 

To demonstrate the generalizability of misspelling errors among ASR models, we present the Character Error Rate (CER) between different open-source ASR models, DeepSpeech and Leopard, and ground-truth transcription in Table~\ref{tab:cer}. 
In Table~\ref{tab:cer}, we observe that the CER values for the different ASR models are smaller than that of each ASR model and ground-truth transcription. 
This indicates that, despite the differences in model-specific factors, the misspelling errors generated by these models are more similar to each other than ground-truth transcription.

Toward ASR-generalizable SNI, we consider alignable characteristics of the ASR-error words.
That is, the words in the ground-truth text can be easily aligned to their corresponding words in ASR transcription.
When the words are correctly transcribed, the words in the ASR and its ground-truth text would be easily aligned.
However, such alignment is not limited to the correctly transcribed words.
As ASR systems misspell the words of the ground-truth text into phonetically, also graphemically, similar words, even inaccurately transcribed words can be easily aligned to their corresponding words.

Considering such alignment, we propose to break down SNI from generating entire pseudo-ASR transcription $X^{\prime}$ given written text $X$ into the finer-grained generation of ASR error words $w^{\prime}\in X^{\prime}$ given written word $w \in X$ adopting constrained generation which can be formulated as follows:
\begin{equation}
    w^{\prime} = M(w)
\end{equation}
Directly conditioned on the cleanly written word $w$, not the entire text $X$, such fine-grained SNI can better supervise the SNI model of how the written words $w$ are corrupted to ASR error words $w^{\prime}$ by misspelling. 
By better supervising misspelling with fine-grained SNI, we enhance its ability to generalize across different ASR systems, as ASR misspelling is generalizable to different written words, regardless of the ASR systems.

In addition to misspellings, fine-grained SNI can also contribute to a more ASR-generalizable approach in the context of phoneme misunderstanding.
In previous generative SNI, whether the cleanly written word $w$ would be corrupted is implicitly determined by SNI model $M$.
Biased by the phoneme misunderstanding pattern of the ASR system used to transcribe the training set, the SNI model tends to corrupt only the words that the specific ASR system would phonetically misunderstand.
Compared to sentence-level SNI, our word-level SNI gives more control in selecting which words to corrupt to ASR error words.
For ASR-generalizable SNI, we propose to randomly select the words to corrupt, so that the resulting pseudo-ASRs would contain diverse ASR-error words.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose a word-level SNI approach adopting constrained generation
2) propose a random word selection in the proposed word-level SNI 
and 3) show that the proposed word-level SNI improves the ASR-generalizability of downstream models.




%factorize the two distinct steps involved in ASR errors: phonetic misunderstanding and misspelling. 
%By doing so, we isolate the phonetic misunderstanding step where the ASR system misinterprets the spoken phonemes, and the subsequent misspelling step where it generates incorrect spellings based on the misunderstood speech.
%In contrast to previous approaches that treat SNI as a unified sequence-to-sequence generation task, our proposed constrained generation method allows us to focus solely on regenerating the ASR-noised words, while preserving the original written words. 
%This factorization enables us to address each step independently and develop targeted strategies to mitigate phonetic misunderstanding and improve the accuracy of misspelling generation.
%By adopting constrained generation and explicitly considering the phonetic misunderstanding and misspelling steps, our approach offers a novel perspective and potential advancements in the field of ASR-generalizable SNI. 
%It allows for more fine-grained control and targeted interventions, ultimately leading to improved performance and robustness in the generation of ASR-corrupted data.




==> backup/230703/2_related_works.tex <==
\section{Related Works}
\subsection{Robustness }
In recent years, large-scale PLMs have demonstrated remarkable performance in Natural Language Understanding (NLU) tasks~\cite{openai2023gpt4}. 
To evaluate their robustness, several studies have employed human-crafted adversarial examples or generated examples through adversarial attacks~\cite{wang2021adversarial}. 
Another approach involves projecting input data into a latent space using Generative Adversarial Networks and then retrieving adversaries that closely resemble the original instance in the latent space~\cite{zhao2017generating}.
Additionally, controlled paraphrase networks are proposed to generate syntactically adversarial examples~\cite{iyyer2018adversarial}. 
These examples not only deceive PLMs but also enhance their resilience to syntactic variations when used for training data augmentation. 
However, the extent to which PLMs exhibit robustness against ASR errors in real-world conditions has been under-explored.
\subsection{SNI}
%SNI 정의, 
Recently, a few works showed that training with ASR-noised samples can robustify PLMs so that they can be adapted for SLU.
To bridge the gap between written and spoken conversations, many works attempt SNI, a data augmentation method of converting the written text $X$ into pseudo-ASR $X^{\prime}$ by imitating ASR errors.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow X^{\prime}$.
The most intuitive method is the TTS-ASR pipeline, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio.
In addition to the exhaustive cost of the TTS engine and ASR system, they cannot fully simulate ASR errors as the audio generated by the TTS and the human recording have different error distributions.~\cite{asrglue}


Another category of SNI, text-level SNI,  simulates ASR errors by perturbing the written text $X$ so that the resulting pseudo-ASR $X^{\prime}$ contains ASR errors.
Text-level SNI can be subdivided into confusion matrix and generative SNI.
In the confusion matrix method,  first, the word-level confusion matrix between written text and its paired ASR transcription is built. 
Then, ASR error is added to the written text according to the frequencies in the confusion matrix.

Another method of text-level SNI and our main baseline is the generative SNI which supervises the pre-trained auto-regressive language model as $F$.
Specifically, the pre-trained auto-regressive language model such as GPT-2 and BART is supervised to generate pseudo-ASR $X^{\prime}$ containing ASR errors given the written text $X$.
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.

We argue that the pseudo-ASR by the generative SNI is not generalizable across the different ASR systems.
That is, different ASR systems generate different error distributions, thus, the downstream task model robust for one ASR system's error would not be robust to the other ASR systems.
While such generalization scenario has been widely studied in the other SLU tasks, it has been understudied for SNI.
Previous works in generative SNI used identical ASR systems for both training SNI models and transcribing SLU downstream tasks.



%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsection{ASR Correction}
The other category of minimizing the gap between ASR transcription and written text is ASR correction, which conducts the inverse functional mapping of SNI $F^{-1} X^{\prime} \rightarrow X$ of converting ASR transcription to the written text $X$ by removing the ASR error.
%While it has distinct strength for making 

==> backup/230703/3_ours.tex <==
\section{Ours}
The task of SNI can be treated as a functional mapping $F:X \rightarrow X^{\prime}$ between the written text $X$ and the pseudo-ASR transcription $X^{\prime}$,  where $X=\{x_1, ..., x_n\}$ denotes ground truth transcription which is a sequence of n words and  $X^{\prime}=\{x^{\prime}_1, ..., x^{\prime}_{n^{\prime}}\}$ is the ASR transcription of a sequence of $n^{\prime}$ words.  


Previous works model SNI as trivial sequence-to-sequence problem of generating $X^{\prime}$ given $X$ using vocabulary $V$ as followed:
\begin{equation}
    x^{\prime}_i = argmax P(V|X, x^{\prime}_{1}, ... x^{\prime}_{i-1}).
\end{equation}
In this formulation, noise target phrase selection and noise phrase generation are implicitly done at once.
Thus, the resulting SNI sentences can be biased toward specific ASR systems as distinct ASR systems have different phoneme misunderstanding patterns.
Also, unlike other sequence-to-sequence tasks such as question answering, which may have radically different inputs and outputs, it is observed that the input, and output of SNI, ground-truth transcription $X$, and ASR transcription $T$, are nearly identical.
Moreover, ASR noise phrases $W^{\prime} = \{w^{\prime}_1...,w^{\prime}_p\} \subset T$ can be easily aligned to their clean written form $W = \{w_1...,w_q\}\subset X$, the sequence-to-sequence formulation of SNI does not reflect such easy-to-align nature of ASR errors.
Without noticing such easy-to-align nature, the SNI model can rather generate entirely different sentences than corrupt the clean sentences into ASR-like sentences.
Thus, requiring additional heuristic filtering of noised samples~\cite{noisygen}.



Our key idea is to explicitly factorize SNI as two-step procedure similar to the two steps of the ASR-noise generation process. 
Specifically, we formulate SNI as following two subsequent steps: noise target phrase selection and noise phrase generation.
Noise target phrase selection aims to select noise target phrase $W \subset X$ which is replaced in ASR transcription as noise phrase $W^{\prime} \in T$.
Then, given a noise target phrase $W$, noise phrase generation aims to generate noise phrase $W^{\prime} \in T$.

In our training setting for noise target phrase selection, our objective is to identify potential ASR noise phrases from the ground-truth transcription so that identified phrases can be corrupted. 
To accomplish this, we used the phrases noised in the ASR transcription as our noise target phrases during the training phase. 
In inference time of conducting SNI on written text, we randomly selected phrases from the input text to serve as the noise target phrases.
This approach was motivated by the fact that different ASR systems can exhibit varying patterns of phoneme misunderstanding, making it challenging to generalize the selection of noise target phrases across different ASR systems. 
By randomly selecting noise-target phrases during inference, we ensure that the resulting noised sentences are not biased towards any specific ASR system. 
This allows downstream task models trained with our SNI data to simulate the diverse phonetic misunderstandings that can occur across different ASR systems, enhancing the robustness and generalizability of our approach in handling ASR-induced errors in real-world scenarios.

Then our next step is noise phrase generation, which aims to generate noise phrase $W^{\prime} \in T$ given noise target phrase $W  \subset X$ modeled as follows:
\begin{equation}
    w^{\prime}_i = argmax P(V|W, w^{\prime}_1, ... w^{\prime}_{i-1}).
\end{equation}
Generating noise phrases given only selected noise target phrases, our SNI model focuses on generating ASR-like sentences and does not require heuristic filtering in previous works.



%Specifically, we propose to fractionize SNI into more fine-grained mapping $f:W \rightarrow W^{\prime}$ between the noise target phrases and the noised phrases. 

%We design an end-to-end architecture consisting of an encoder, a decoder, and an operation predictor to constrain the decoding process to the desired part of the input sequence.  
%The encoder produces sequence embeddings from the word embeddings of the ASR output texts and related positional embeddings.  
%The operation predictor is a fully-connected layer trained to identify the above-mentioned“K”, “D” and “C” input sequence embeddings.  
%The model can reduce inference latency significantly by restricting the decoding process to the “C” tokens

%For the change position, the transformed-based decoder inputs at timestep t are calculated as follows: \begin{equation}
%    Eyt,k=Wp[(WE(wyt,k) + PE(wyt,k))exk], 
%\end{equation}
%where $WE$ and $PE$ are the same word and position embedding functions as in equation.
%$exk$ is the encoded token representation mentioned before. 
%$Wp$ is the trainable parameters.
%Then, a standard transformer decoder is employed to fuse all relevant information:
%\begin{align}
%    hkt+1= TransformerDecoder(Q,K,V),\\
%    Q=Eyt,k,K=Ex,V=Ex,
%\end{align}
%where  the decoder  input $Eyt,k$ works  as query (“Q”),  and  encoded model input $Ex$ works as key (“K”) and value (“V”) in the transformer decoder.
%$hkt+1$ is the fused vector.
%Finally, the target output is predicted as follows:
%\begin{equation}
%    p(ˆωyt+1,k) = softmax(Wyhkt+1+by), 
%\end{equation}
%where $Wy$ and $by$ are trained parameters.   
%Then, generation loss is defined as followed:
%\begin{equation}
%   lossdec=tlog(p(ˆωyt,k)).
%\end{equation}

==> backup/230703/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

~\input{table/dataset_statistics}

For training SNI model, we followed the settings from the previous work~\cite{noisygen}, which used to popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, DeepSpeech, and get recognized results. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2}, which models task-oriented dialogue systems with unstructured knowledge access.
The key reason for adopting DSTC10 Track2 dataset is that its sentences are the transcription of human-spoken task-oriented dialogue by an unknown ASR model.
Specifically, it includes three subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG).
In DSTC10 Tack 2 dataset, task-oriented dialogue systems are modeled as sequence of three subtasks.
First, determine whether the dialogue turn requires external knowledge access or not. 
Once determined to require external knowledge, then the second step is to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the whole knowledge base.
Finally, the response should be generated based on the dialogue context and the selected knowledge snippet. 
We choose DSTC10 Track2 dataset as it contains major tasks in NLP, classification and retrieval, generation as SLU.



\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

We followed settings for downstream task DSTC10 Track2 from previous works~\cite{dstc10_2, tian2021tod-da}.
We conducted SNI on the written form of each subtask dataset in a task-oriented dialogue system dataset and used the resulting noised sentence for training downstream models.
For the downstream task model, we followed the baseline model setting of DSTC10 Track2~\cite{dstc10_2} and trained GPT2-small on each subtask.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2}.



==> backup/230703/5_results.tex <==
\section{Results}
\input{table/result}
%We present the result on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
%The downstream model trained with our method outperformed baselines with a large margin in KS and RG subtasks and comparable results in KTD.
In this section, we first present the results of our proposed method for on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
Specifically, we report the results of all subtasks, the knowledge turn detection subtask and the knowledge selection, and response generation.
The results demonstrate the superiority of our approach in knowledge selection and response generation, while also achieving comparable performance in knowledge turn detection.

For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


In the response generation subtask, our method outperformed the baseline methods in every metric. 
However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
This indicates that our SNI method can better robustify the PLMs on generation task.


Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.

Overall, our proposed method demonstrated superior performance in the knowledge selection and response generation subtasks of the task-oriented dialogue dataset. 
Additionally, it showcased competitive results in the knowledge turn detection subtask. 
These findings highlight the effectiveness of our approach in enhancing the capabilities of task-oriented dialogue systems and improving their performance in understanding user queries, selecting relevant knowledge, and generating appropriate responses.


==> backup/230703/6_conclusion.tex <==
\section{Conclusion}
In this paper, we first showed that among two ASR noise procedures, the misspelling step is generalizable between different ASR models while the phoneme misunderstanding does not.
Based on such findings, we proposed a new SNI method that formulated SNI as a constrained generation problem that fractionize SNI as a phrase-to-phrase problem.
From such formulation, we could attain an ASR-generalizable SNI model by randomizing noise target word selection and better supervising the noise word generation.

==> backup/230706/1_intro.tex <==
\section{Introduction}
Starting from ELMo~\cite{peters-etal-2018-deep} to recent GPT4~\cite{openai2023gpt4}, pretrained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
As such abilities are essential for spoken language understanding (SLU)~\cite{broscheit-etal-2022-distributionally, 8907842}, PLMs are widely adopted in speech-enabled systems such as voice assistants.
Specifically,  PLMS are adopted in a  pipeline  process of such speech-enabled systems. 
First, audio is converted into textual transcription by an automatic speech recognition (ASR) system. 
Then, the transcription is fed into PLMs to conduct various tasks. 


%As PLMs are trained in the different modality of written text, they suffer to adapt to the difference between the transcription and text.
%이 문단에서 하고 싶은 말은 PLM들이 SLU에서 ASR noise 때문에 못하지만 ASR noise를 포함하는 데이터를 학습하면 robust해짐
While PLMs suffer from the noise in the spoken transcription, ASR errors, they can be robustified when trained on the SLU corpora corrupted by noise.
That is, ASR systems fail to generate the correct transcription and confuse to generate phonetically similar but wrong ASR error words~\cite{ruan20_interspeech,9054689}.
%The key difference disturbing PLMs in SLU is the errors of the ASR systems. 
%Specifically, ASR systems confuse to generate phonetically similar and semantically different words, ASR error words~\cite{ruan20_interspeech,9054689}.
As the ASR error words are mapped to different tokens, the input sequence different from the written text is fed to PLMs.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original spoken language and makes an incorrect prediction on SLU~\cite{belinkov2018synthetic}.


%데이터
%SLU copora 모으는거 어렵기 때문에 SNi 함
The data augmentation method of the speech noise injection (SNI) of converting the written text into pseudo transcription has been widely studied to reduce the human annotation required for SLU corpora.
An SLU corpus requires two additional steps following after collecting the written corpus.
The collected written language corpus is first recorded in audio by human annotators, then transcribed into text using ASR systems.
SNI can convert a written corpus without the additional human annotation into a pseudo-SLU corpus by injecting the ASR errors into the written text.

%여기는 previous SNI 들이 다 ASR specific 하다는 내용 위주로 고치기.
%Previous works in SNI can be categorized into two methods. 
%The most intuitive method is the TTS-ASR pipeline, where the TTS engine (text-to-speech) converts the text into audio, and the ASR system transcribes the audio.
%While ASR errors are generated by TTS engines and ASR systems, they are both computationally expensive.
%Additionally, they cannot generate sufficient ASR errors as the noise engaged during human reading does not exist in the audio converted by TTS.
%In contrast, generative SNI supervises the autoregressive language model $M$ to generate the pseudo-ASR given the text as the following:
%\begin{equation}
%    X^{\prime} = M(X)
%\end{equation}
%As generative SNI is shown to be effective in various situations~\cite{asrglue}, we focus on generative SNI.

While many previous works studied SNI~\cite{feng22c_interspeech, noisygen}, ASR-generalizability, the ability of an SLU model to perform robustly across different ASR systems, is not well studied for SNI.
Such generalizability has been focused on diverse SLU tasks as different ASR systems can be used in SLU pipeline~\cite{blackbox1}.
%ASR-generalizability has been important as different ASR systems have distinct error distributions and SLU trained on one error distribution suffers to generalize on different error distribution.
However, previous works in SNI confirmed their effectiveness using identical ASR systems for both SNI and downstream tasks, where the ASR generalizability still remains unveiled~\cite{noisygen,tts_asr}.
We argue that ASR-generalizability is also crucial in SNI as the resulting pseudo-ASR would follow the error distribution of an individual ASR system.



For ASR generalizable SNI, we factorize the generation of ASR errors into two distinct steps: phonetic misunderstanding and misspelling.
In the phonetic misunderstanding step, the ASR system misinterprets the spoken phonemes, leading to inaccuracies in the resulting transcription. 
Consequently, the subsequent step, misspelling, arises as a result of the ASR system generating misspelled words based on its flawed understanding of the original speech. 
Misspelling errors occur when the ASR system incorrectly converts the misunderstood phonemes into different characters, further deviating from the intended transcription. 

\input{table/asr_cer}

Among two distinct steps, we argue that  
while the phonetic misunderstanding is ASR-specific noise, the misspelling step is ASR-generalizable.
Specifically, phonetic misunderstanding can be largely influenced by training data and acoustic modeling.
For example, ASR systems with distinct acoustic feature extractors and different accented training audio would exhibit distinct susceptibility to phonetic misunderstanding.
In contrast, we argue that the phenomenon of misspelling is more ASR-generalizable. 
This is because a language possesses specific spelling conventions that are shared across different ASR models regardless of training data or acoustic modeling techniques. 

To demonstrate the generalizability of misspelling errors among ASR models, we present the Character Error Rate (CER) between different open-source ASR models, DeepSpeech and Leopard, and ground-truth transcription in Table~\ref{tab:cer}. 
In Table~\ref{tab:cer}, we observe that the CER values for the different ASR models are smaller than that of each ASR model and ground-truth transcription. 
This indicates that, despite the differences in model-specific factors, the misspelling errors generated by these models are more similar to each other than ground-truth transcription.

Toward ASR-generalizable SNI, we consider alignable characteristics of the ASR-error words.
That is, the words in the ground-truth text can be easily aligned to their corresponding words in ASR transcription.
When the words are correctly transcribed, the words in the ASR and its ground-truth text would be easily aligned.
However, such alignment is not limited to the correctly transcribed words.
As ASR systems misspell the words of the ground-truth text into phonetically, also graphemically, similar words, even inaccurately transcribed words can be easily aligned to their corresponding words.

Considering such alignment, we propose to break down SNI from generating entire pseudo-ASR transcription $X^{\prime}$ given written text $X$ into the finer-grained generation of ASR error words $w^{\prime}\in X^{\prime}$ given written word $w \in X$ adopting constrained generation which can be formulated as follows:
\begin{equation}
    w^{\prime} = M(w)
\end{equation}
Directly conditioned on the cleanly written word $w$, not the entire text $X$, such fine-grained SNI can better supervise the SNI model of how the written words $w$ are corrupted to ASR error words $w^{\prime}$ by misspelling. 
By better supervising misspelling with fine-grained SNI, we enhance its ability to generalize across different ASR systems, as ASR misspelling is generalizable to different written words, regardless of the ASR systems.

In addition to misspellings, fine-grained SNI can also contribute to a more ASR-generalizable approach in the context of phoneme misunderstanding.
In previous generative SNI, whether the cleanly written word $w$ would be corrupted is implicitly determined by SNI model $M$.
Biased by the phoneme misunderstanding pattern of the ASR system used to transcribe the training set, the SNI model tends to corrupt only the words that the specific ASR system would phonetically misunderstand.
Compared to sentence-level SNI, our word-level SNI gives more control in selecting which words to corrupt to ASR error words.
For ASR-generalizable SNI, we propose to randomly select the words to corrupt, so that the resulting pseudo-ASRs would contain diverse ASR-error words.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose a word-level SNI approach adopting constrained generation
2) propose a random word selection in the proposed word-level SNI 
and 3) show that the proposed word-level SNI improves the ASR-generalizability of downstream models.




%factorize the two distinct steps involved in ASR errors: phonetic misunderstanding and misspelling. 
%By doing so, we isolate the phonetic misunderstanding step where the ASR system misinterprets the spoken phonemes, and the subsequent misspelling step where it generates incorrect spellings based on the misunderstood speech.
%In contrast to previous approaches that treat SNI as a unified sequence-to-sequence generation task, our proposed constrained generation method allows us to focus solely on regenerating the ASR-noised words, while preserving the original written words. 
%This factorization enables us to address each step independently and develop targeted strategies to mitigate phonetic misunderstanding and improve the accuracy of misspelling generation.
%By adopting constrained generation and explicitly considering the phonetic misunderstanding and misspelling steps, our approach offers a novel perspective and potential advancements in the field of ASR-generalizable SNI. 
%It allows for more fine-grained control and targeted interventions, ultimately leading to improved performance and robustness in the generation of ASR-corrupted data.




==> backup/230708/1_intro.tex <==
\section{Introduction}
Starting from ELMo~\cite{peters-etal-2018-deep} to recent GPT4~\cite{openai2023gpt4}, pretrained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
As such abilities are essential for spoken language understanding (SLU)~\cite{broscheit-etal-2022-distributionally, 8907842}, PLMs are widely adopted in speech-enabled systems such as voice assistants.
Specifically,  PLMS are adopted in a  pipeline  process of such speech-enabled systems. 
First, audio is converted into textual transcription by an automatic speech recognition (ASR) system. 
Then, the transcription is fed into PLMs to conduct various tasks. 


%As PLMs are trained in the different modality of written text, they suffer to adapt to the difference between the transcription and text.
%이 문단에서 하고 싶은 말은 PLM들이 SLU에서 ASR noise 때문에 못하지만 ASR noise를 포함하는 데이터를 학습하면 robust해짐
While PLMs suffer from the noise in the spoken transcription, ASR errors, they can be robustified when trained on the SLU corpora corrupted by noise.
That is, ASR systems fail to generate the correct transcription and confuse to generate phonetically similar but wrong ASR error words~\cite{ruan20_interspeech,9054689}.
%The key difference disturbing PLMs in SLU is the errors of the ASR systems. 
%Specifically, ASR systems confuse to generate phonetically similar and semantically different words, ASR error words~\cite{ruan20_interspeech,9054689}.
As the ASR error words are mapped to different tokens, the input sequence different from the written text is fed to PLMs.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original spoken language and makes an incorrect prediction on SLU~\cite{belinkov2018synthetic}.


%데이터
%SLU copora 모으는거 어렵기 때문에 SNi 함
The data augmentation method of the speech noise injection (SNI) of converting the written text into pseudo transcription has been widely studied to reduce the human annotation required for SLU corpora.
An SLU corpus requires two additional steps following after collecting the written corpus.
The collected written language corpus is first recorded in audio by human annotators, then transcribed into text using ASR systems.
SNI can convert a written corpus without the additional human annotation into a pseudo-SLU corpus by injecting the ASR errors into the written text.

%여기는 previous SNI 들이 다 ASR specific 하다는 내용 위주로 고치기.
%Previous works in SNI can be categorized into two methods. 
%The most intuitive method is the TTS-ASR pipeline, where the TTS engine (text-to-speech) converts the text into audio, and the ASR system transcribes the audio.
%While ASR errors are generated by TTS engines and ASR systems, they are both computationally expensive.
%Additionally, they cannot generate sufficient ASR errors as the noise engaged during human reading does not exist in the audio converted by TTS.
%In contrast, generative SNI supervises the autoregressive language model $M$ to generate the pseudo-ASR given the text as the following:
%\begin{equation}
%    X^{\prime} = M(X)
%\end{equation}
%As generative SNI is shown to be effective in various situations~\cite{asrglue}, we focus on generative SNI.

While many previous works studied SNI~\cite{feng22c_interspeech, noisygen}, ASR-generalizability, the ability of an SLU model to perform robustly across different ASR systems, is not well studied for SNI.
Such generalizability has been focused on diverse SLU tasks as different ASR systems can be used in SLU pipeline~\cite{blackbox1}.
%ASR-generalizability has been important as different ASR systems have distinct error distributions and SLU trained on one error distribution suffers to generalize on different error distribution.
However, previous works in SNI confirmed their effectiveness using identical ASR systems for both SNI and downstream tasks, where the ASR generalizability still remains unveiled~\cite{noisygen,tts_asr}.
We argue that ASR-generalizability is also crucial in SNI as the resulting pseudo-ASR would follow the error distribution of an individual ASR system.



Toward ASR generalizable SNI, we first propose to intervene SNI process based on do-calculus~\cite{glymour2016causal} so that the resulting pseudo-ASR would not follow the error distribution of an individual ASR system. 
%factorize the generation of ASR errors into two distinct steps: phonetic misunderstanding and misspelling.
For such goal, we train SNI model to generate the ASR-noised words constrained on its written words, the noise target words.
Previous works supervised SNI model to maximize the likelihood of the entire ASR transcription given its written sentence~\cite{asrglue, noisygen}.
During such supervision, the SNI model is biased to select the noise target words following the error distribution of the ASR system adopted for training.
Thus, the resulting pseudo-ASR would contain biased ASR errors, such as containing errors for specific phonemes.
In contrast, our SNI model randomly selects the noise target words. 
This random selection serves as an intervention to the error distribution of the ASR system and debias the resulting pseudo-ASR to diversify the error distribution.
Trained on the pseudo-ASR with more diverse ASR errors, downstream task models can more robustly conduct downstream tasks.
%As a result
%, similar to interventions performed in do-calculus, where we actively modify the values of certain variables to observe the effects on the overall system.
%By randomly selecting the words, we remove the bias associated with specific ASR systems and ensure a more diverse set of corrupted words.

In addition to intervention in the error distribution, we propose to correct the generation of ASR noise words using phonetic information. 
While ASR systems generate phonetically similar words as ASR error words, SNI models are optimized to maximize the likelihood of the grapheme-based tokens corresponding to ASR error words.
Blinded to phonetic similarity, the existing SNI model fails to generate phonetically similar pseudo-ASR and requires additional phonetic similarity based heuristic to filter out such failing pseudo-ASR.
Instead of such heuristic, we propose to supervise and incorporate phonetic similarity to correct the noise word generation.
Specifically, we propose a phoneme head, another language model head that generates ASR noise words based on their phonemes.
This phoneme head is used with trivial language model head of SNI models and ensures to generate the phonetically similar ASR error words.

%Powerful generation models of ten meet most of the task requirements, yet miss a few (e.g.,omittinga subset of keywords), or generate incorrect hypotheses that nevertheless provide useful structure (e.g.,a correct problem solving strategy with a missing step). However, after generatingevenaslightlysub-optimalsequence,thesingle-passparadigmrequiresmodelsto“startfrom scratch”,effectivelydiscardingworkalreadydone.Amorenatural,intuitiveapproachisleveraging thegenerationasausefulstartingpointtorefineintoahigherqualityoutput.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose to correct the generation of ASR error words with phoneme head
and 3) show that the proposed methods improves the ASR-generalizability of downstream models.

\begin{comment}
In the phonetic misunderstanding step, the ASR system misinterprets the spoken phonemes, leading to inaccuracies in the resulting transcription. 
Consequently, the subsequent step, misspelling, arises as a result of the ASR system generating misspelled words based on its flawed understanding of the original speech. 
Misspelling errors occur when the ASR system incorrectly converts the misunderstood phonemes into different characters, further deviating from the intended transcription. 

\input{table/asr_cer}

Among two distinct steps, we argue that  
while the phonetic misunderstanding is ASR-specific noise, the misspelling step is ASR-generalizable.
Specifically, phonetic misunderstanding can be largely influenced by training data and acoustic modeling.
For example, ASR systems with distinct acoustic feature extractors and different accented training audio would exhibit distinct susceptibility to phonetic misunderstanding.
In contrast, we argue that the phenomenon of misspelling is more ASR-generalizable. 
This is because a language possesses specific spelling conventions that are shared across different ASR models regardless of training data or acoustic modeling techniques. 

To demonstrate the generalizability of misspelling errors among ASR models, we present the Character Error Rate (CER) between different open-source ASR models, DeepSpeech and Leopard, and ground-truth transcription in Table~\ref{tab:cer}. 
In Table~\ref{tab:cer}, we observe that the CER values for the different ASR models are smaller than that of each ASR model and ground-truth transcription. 
This indicates that, despite the differences in model-specific factors, the misspelling errors generated by these models are more similar to each other than ground-truth transcription.

Toward ASR-generalizable SNI, we consider alignable characteristics of the ASR-error words.
That is, the words in the ground-truth text can be easily aligned to their corresponding words in ASR transcription.
When the words are correctly transcribed, the words in the ASR and its ground-truth text would be easily aligned.
However, such alignment is not limited to the correctly transcribed words.
As ASR systems misspell the words of the ground-truth text into phonetically, also graphemically, similar words, even inaccurately transcribed words can be easily aligned to their corresponding words.

Considering such alignment, we propose to break down SNI from generating entire pseudo-ASR transcription $X^{\prime}$ given written text $X$ into the finer-grained generation of ASR error words $w^{\prime}\in X^{\prime}$ given written word $w \in X$ adopting constrained generation which can be formulated as follows:
\begin{equation}
    w^{\prime} = M(w)
\end{equation}
Directly conditioned on the cleanly written word $w$, not the entire text $X$, such fine-grained SNI can better supervise the SNI model of how the written words $w$ are corrupted to ASR error words $w^{\prime}$ by misspelling. 
By better supervising misspelling with fine-grained SNI, we enhance its ability to generalize across different ASR systems, as ASR misspelling is generalizable to different written words, regardless of the ASR systems.

In addition to misspellings, fine-grained SNI can also contribute to a more ASR-generalizable approach in the context of phoneme misunderstanding.
In previous generative SNI, whether the cleanly written word $w$ would be corrupted is implicitly determined by SNI model $M$.
Biased by the phoneme misunderstanding pattern of the ASR system used to transcribe the training set, the SNI model tends to corrupt only the words that the specific ASR system would phonetically misunderstand.
Compared to sentence-level SNI, our word-level SNI gives more control in selecting which words to corrupt to ASR error words.
For ASR-generalizable SNI, we propose to randomly select the words to corrupt, so that the resulting pseudo-ASRs would contain diverse ASR-error words.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose a word-level SNI approach adopting constrained generation
2) propose a random word selection in the proposed word-level SNI 
and 3) show that the proposed word-level SNI improves the ASR-generalizability of downstream models.




%factorize the two distinct steps involved in ASR errors: phonetic misunderstanding and misspelling. 
%By doing so, we isolate the phonetic misunderstanding step where the ASR system misinterprets the spoken phonemes, and the subsequent misspelling step where it generates incorrect spellings based on the misunderstood speech.
%In contrast to previous approaches that treat SNI as a unified sequence-to-sequence generation task, our proposed constrained generation method allows us to focus solely on regenerating the ASR-noised words, while preserving the original written words. 
%This factorization enables us to address each step independently and develop targeted strategies to mitigate phonetic misunderstanding and improve the accuracy of misspelling generation.
%By adopting constrained generation and explicitly considering the phonetic misunderstanding and misspelling steps, our approach offers a novel perspective and potential advancements in the field of ASR-generalizable SNI. 
%It allows for more fine-grained control and targeted interventions, ultimately leading to improved performance and robustness in the generation of ASR-corrupted data.

\end{comment}


==> backup/230708/3_ours.tex <==
\section{Ours}
The task of SNI can be treated as a functional mapping $F:X \rightarrow X^{\prime}$ between the written text $X$ and the pseudo-ASR transcription $X^{\prime}$,  where $X=\{x_1, ..., x_n\}$ denotes ground truth transcription which is a sequence of n words and  $X^{\prime}=\{x^{\prime}_1, ..., x^{\prime}_{n^{\prime}}\}$ is the ASR transcription of a sequence of $n^{\prime}$ words.  

We now propose our methods for ASR-generalizable SNI.
Mimicking the ASR error generation process, we explicitly decompose the SNI as two consecutive steps of the noise target word selection and noise word generation.
By explicitly 
 Previous works model SNI as trivial sequence-to-sequence problem of generating $X^{\prime}$ given $X$ using vocabulary $V$ as followed:
\begin{equation}
    x^{\prime}_i = argmax P(V|X, x^{\prime}_{1}, ... x^{\prime}_{i-1}).
\end{equation}
In this formulation, noise target phrase selection and noise phrase generation are implicitly done at once.
Thus, the resulting SNI sentences can be biased toward specific ASR systems as distinct ASR systems have different phoneme misunderstanding patterns.
Also, unlike other sequence-to-sequence tasks such as question answering, which may have radically different inputs and outputs, it is observed that the input, and output of SNI, ground-truth transcription $X$, and ASR transcription $T$, are nearly identical.
Moreover, ASR noise phrases $W^{\prime} = \{w^{\prime}_1...,w^{\prime}_p\} \subset T$ can be easily aligned to their clean written form $W = \{w_1...,w_q\}\subset X$, the sequence-to-sequence formulation of SNI does not reflect such easy-to-align nature of ASR errors.
Without noticing such easy-to-align nature, the SNI model can rather generate entirely different sentences than corrupt the clean sentences into ASR-like sentences.
Thus, requiring additional heuristic filtering of noised samples~\cite{noisygen}.



Our key idea is to explicitly factorize SNI as two-step procedure similar to the two steps of the ASR-noise generation process. 
Specifically, we formulate SNI as following two subsequent steps: noise target phrase selection and noise phrase generation.
Noise target phrase selection aims to select noise target phrase $W \subset X$ which is replaced in ASR transcription as noise phrase $W^{\prime} \in T$.
Then, given a noise target phrase $W$, noise phrase generation aims to generate noise phrase $W^{\prime} \in T$.

In our training setting for noise target phrase selection, our objective is to identify potential ASR noise phrases from the ground-truth transcription so that identified phrases can be corrupted. 
To accomplish this, we used the phrases noised in the ASR transcription as our noise target phrases during the training phase. 
In inference time of conducting SNI on written text, we randomly selected phrases from the input text to serve as the noise target phrases.
This approach was motivated by the fact that different ASR systems can exhibit varying patterns of phoneme misunderstanding, making it challenging to generalize the selection of noise target phrases across different ASR systems. 
By randomly selecting noise-target phrases during inference, we ensure that the resulting noised sentences are not biased towards any specific ASR system. 
This allows downstream task models trained with our SNI data to simulate the diverse phonetic misunderstandings that can occur across different ASR systems, enhancing the robustness and generalizability of our approach in handling ASR-induced errors in real-world scenarios.

Then our next step is noise phrase generation, which aims to generate noise phrase $W^{\prime} \in T$ given noise target phrase $W  \subset X$ modeled as follows:
\begin{equation}
    w^{\prime}_i = argmax P(V|W, w^{\prime}_1, ... w^{\prime}_{i-1}).
\end{equation}
Generating noise phrases given only selected noise target phrases, our SNI model focuses on generating ASR-like sentences and does not require heuristic filtering in previous works.



%Specifically, we propose to fractionize SNI into more fine-grained mapping $f:W \rightarrow W^{\prime}$ between the noise target phrases and the noised phrases. 

%We design an end-to-end architecture consisting of an encoder, a decoder, and an operation predictor to constrain the decoding process to the desired part of the input sequence.  
%The encoder produces sequence embeddings from the word embeddings of the ASR output texts and related positional embeddings.  
%The operation predictor is a fully-connected layer trained to identify the above-mentioned“K”, “D” and “C” input sequence embeddings.  
%The model can reduce inference latency significantly by restricting the decoding process to the “C” tokens

%For the change position, the transformed-based decoder inputs at timestep t are calculated as follows: \begin{equation}
%    Eyt,k=Wp[(WE(wyt,k) + PE(wyt,k))exk], 
%\end{equation}
%where $WE$ and $PE$ are the same word and position embedding functions as in equation.
%$exk$ is the encoded token representation mentioned before. 
%$Wp$ is the trainable parameters.
%Then, a standard transformer decoder is employed to fuse all relevant information:
%\begin{align}
%    hkt+1= TransformerDecoder(Q,K,V),\\
%    Q=Eyt,k,K=Ex,V=Ex,
%\end{align}
%where  the decoder  input $Eyt,k$ works  as query (“Q”),  and  encoded model input $Ex$ works as key (“K”) and value (“V”) in the transformer decoder.
%$hkt+1$ is the fused vector.
%Finally, the target output is predicted as follows:
%\begin{equation}
%    p(ˆωyt+1,k) = softmax(Wyhkt+1+by), 
%\end{equation}
%where $Wy$ and $by$ are trained parameters.   
%Then, generation loss is defined as followed:
%\begin{equation}
%   lossdec=tlog(p(ˆωyt,k)).
%\end{equation}

==> backup/230714/0_abs.tex <==
\begin{abstract}
This paper proposes ASR-generalizable speech noise injection (SNI) for improving spoken language understanding (SLU) models in the presence of ASR errors. Pretrained language models (PLMs) trained on written language struggle to adapt to the differences in spoken language, especially due to phonetic misunderstanding and misspelling errors introduced by ASR systems. While previous works have explored SNI, the generalizability of SLU models to different ASR systems remains understudied. We factorize ASR errors into two steps: phonetic misunderstanding and misspelling, and demonstrate that misspelling errors are more model generalizable compared to phonetic misunderstanding. To explicitly model these steps, we propose constrained generation, focusing on regenerating ASR-noised words. The approach enables targeted generation and improves the robustness and generalizability of SLU models. Experimental results and analysis are provided to support the effectiveness of ASR-generalizable SNI.
\end{abstract}

==> backup/230714/1_intro.tex <==
\section{Introduction}
Starting from ELMo~\cite{peters-etal-2018-deep} to recent GPT4~\cite{openai2023gpt4}, pretrained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
As such abilities are essential for spoken language understanding (SLU)~\cite{broscheit-etal-2022-distributionally, 8907842}, PLMs are widely adopted in speech-enabled systems such as voice assistants.
Specifically,  PLMS are adopted in a  pipeline  process of such speech-enabled systems. 
First, audio is converted into textual transcription by an automatic speech recognition (ASR) system. 
Then, the transcription is fed into PLMs to conduct various tasks. 


%As PLMs are trained in the different modality of written text, they suffer to adapt to the difference between the transcription and text.
%이 문단에서 하고 싶은 말은 PLM들이 SLU에서 ASR noise 때문에 못하지만 ASR noise를 포함하는 데이터를 학습하면 robust해짐
While PLMs suffer from the noise in the spoken transcription, ASR errors, they can be robustified when trained on the SLU corpora corrupted by noise.
That is, ASR systems fail to generate the correct transcription and confuse to generate phonetically similar but wrong ASR error words~\cite{ruan20_interspeech,9054689}.
%The key difference disturbing PLMs in SLU is the errors of the ASR systems. 
%Specifically, ASR systems confuse to generate phonetically similar and semantically different words, ASR error words~\cite{ruan20_interspeech,9054689}.
As the ASR error words are mapped to different tokens, the input sequence different from the written text is fed to PLMs.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original spoken language and makes an incorrect prediction on SLU~\cite{belinkov2018synthetic}.


%데이터
%SLU copora 모으는거 어렵기 때문에 SNi 함
The data augmentation method of the speech noise injection (SNI) of converting the written text into pseudo transcription has been widely studied to reduce the human annotation required for SLU corpora.
An SLU corpus requires two additional steps following after collecting the written corpus.
The collected written language corpus is first recorded in audio by human annotators, then transcribed into text using ASR systems.
SNI can convert a written corpus without the additional human annotation into a pseudo-SLU corpus by injecting the ASR errors into the written text.

%여기는 previous SNI 들이 다 ASR specific 하다는 내용 위주로 고치기.
%Previous works in SNI can be categorized into two methods. 
%The most intuitive method is the TTS-ASR pipeline, where the TTS engine (text-to-speech) converts the text into audio, and the ASR system transcribes the audio.
%While ASR errors are generated by TTS engines and ASR systems, they are both computationally expensive.
%Additionally, they cannot generate sufficient ASR errors as the noise engaged during human reading does not exist in the audio converted by TTS.
%In contrast, generative SNI supervises the autoregressive language model $M$ to generate the pseudo-ASR given the text as the following:
%\begin{equation}
%    X^{\prime} = M(X)
%\end{equation}
%As generative SNI is shown to be effective in various situations~\cite{asrglue}, we focus on generative SNI.

While many previous works studied SNI~\cite{feng22c_interspeech, noisygen}, ASR-generalizability, the ability of an SLU model to perform robustly across different ASR systems, is not well studied for SNI.
Such generalizability has been focused on diverse SLU tasks as different ASR systems can be used in SLU pipeline~\cite{blackbox1}.
%ASR-generalizability has been important as different ASR systems have distinct error distributions and SLU trained on one error distribution suffers to generalize on different error distribution.
However, previous works in SNI confirmed their effectiveness using identical ASR systems for both SNI and downstream tasks, where the ASR generalizability still remains unveiled~\cite{noisygen,tts_asr}.
We argue that ASR-generalizability is also crucial in SNI as the resulting pseudo-ASR would follow the error distribution of an individual ASR system.



Toward ASR generalizable SNI, we first propose to intervene SNI process based on do-calculus~\cite{glymour2016causal} so that the resulting pseudo-ASR would not follow the error distribution of an individual ASR system. 
%factorize the generation of ASR errors into two distinct steps: phonetic misunderstanding and misspelling.
For such goal, we train SNI model to generate the ASR-noised words constrained on its written words, the noise target words.
Previous works supervised SNI model to maximize the likelihood of the entire ASR transcription given its written sentence~\cite{asrglue, noisygen}.
During such supervision, the SNI model is biased to select the noise target words following the error distribution of the ASR system adopted for training.
Thus, the resulting pseudo-ASR would contain biased ASR errors, such as containing errors for specific phonemes.
In contrast, our SNI model randomly selects the noise target words. 
This random selection serves as an intervention to the error distribution of the ASR system and debias the resulting pseudo-ASR to diversify the error distribution.
Trained on the pseudo-ASR with more diverse ASR errors, downstream task models can more robustly conduct downstream tasks.
%As a result
%, similar to interventions performed in do-calculus, where we actively modify the values of certain variables to observe the effects on the overall system.
%By randomly selecting the words, we remove the bias associated with specific ASR systems and ensure a more diverse set of corrupted words.

In addition to intervention in the error distribution, we propose to correct the generation of ASR noise words using phonetic information. 
While ASR systems generate phonetically similar words as ASR error words, SNI models are optimized to maximize the likelihood of the grapheme-based tokens corresponding to ASR error words.
Blinded to phonetic similarity, the existing SNI model fails to generate phonetically similar pseudo-ASR and requires additional phonetic similarity based heuristic to filter out such failing pseudo-ASR.
Instead of such heuristic, we propose to supervise and incorporate phonetic similarity to correct the noise word generation.
Specifically, we propose a phoneme head, another language model head that generates ASR noise words based on their phonemes.
This phoneme head is used with trivial language model head of SNI models and ensures to generate the phonetically similar ASR error words.

%Powerful generation models of ten meet most of the task requirements, yet miss a few (e.g.,omittinga subset of keywords), or generate incorrect hypotheses that nevertheless provide useful structure (e.g.,a correct problem solving strategy with a missing step). However, after generatingevenaslightlysub-optimalsequence,thesingle-passparadigmrequiresmodelsto“startfrom scratch”,effectivelydiscardingworkalreadydone.Amorenatural,intuitiveapproachisleveraging thegenerationasausefulstartingpointtorefineintoahigherqualityoutput.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose to correct the generation of ASR error words with phoneme head
and 3) show that the proposed methods improves the ASR-generalizability of downstream models.

\begin{comment}
In the phonetic misunderstanding step, the ASR system misinterprets the spoken phonemes, leading to inaccuracies in the resulting transcription. 
Consequently, the subsequent step, misspelling, arises as a result of the ASR system generating misspelled words based on its flawed understanding of the original speech. 
Misspelling errors occur when the ASR system incorrectly converts the misunderstood phonemes into different characters, further deviating from the intended transcription. 

\input{table/asr_cer}

Among two distinct steps, we argue that  
while the phonetic misunderstanding is ASR-specific noise, the misspelling step is ASR-generalizable.
Specifically, phonetic misunderstanding can be largely influenced by training data and acoustic modeling.
For example, ASR systems with distinct acoustic feature extractors and different accented training audio would exhibit distinct susceptibility to phonetic misunderstanding.
In contrast, we argue that the phenomenon of misspelling is more ASR-generalizable. 
This is because a language possesses specific spelling conventions that are shared across different ASR models regardless of training data or acoustic modeling techniques. 

To demonstrate the generalizability of misspelling errors among ASR models, we present the Character Error Rate (CER) between different open-source ASR models, DeepSpeech and Leopard, and ground-truth transcription in Table~\ref{tab:cer}. 
In Table~\ref{tab:cer}, we observe that the CER values for the different ASR models are smaller than that of each ASR model and ground-truth transcription. 
This indicates that, despite the differences in model-specific factors, the misspelling errors generated by these models are more similar to each other than ground-truth transcription.

Toward ASR-generalizable SNI, we consider alignable characteristics of the ASR-error words.
That is, the words in the ground-truth text can be easily aligned to their corresponding words in ASR transcription.
When the words are correctly transcribed, the words in the ASR and its ground-truth text would be easily aligned.
However, such alignment is not limited to the correctly transcribed words.
As ASR systems misspell the words of the ground-truth text into phonetically, also graphemically, similar words, even inaccurately transcribed words can be easily aligned to their corresponding words.

Considering such alignment, we propose to break down SNI from generating entire pseudo-ASR transcription $X^{\prime}$ given written text $X$ into the finer-grained generation of ASR error words $w^{\prime}\in X^{\prime}$ given written word $w \in X$ adopting constrained generation which can be formulated as follows:
\begin{equation}
    w^{\prime} = M(w)
\end{equation}
Directly conditioned on the cleanly written word $w$, not the entire text $X$, such fine-grained SNI can better supervise the SNI model of how the written words $w$ are corrupted to ASR error words $w^{\prime}$ by misspelling. 
By better supervising misspelling with fine-grained SNI, we enhance its ability to generalize across different ASR systems, as ASR misspelling is generalizable to different written words, regardless of the ASR systems.

In addition to misspellings, fine-grained SNI can also contribute to a more ASR-generalizable approach in the context of phoneme misunderstanding.
In previous generative SNI, whether the cleanly written word $w$ would be corrupted is implicitly determined by SNI model $M$.
Biased by the phoneme misunderstanding pattern of the ASR system used to transcribe the training set, the SNI model tends to corrupt only the words that the specific ASR system would phonetically misunderstand.
Compared to sentence-level SNI, our word-level SNI gives more control in selecting which words to corrupt to ASR error words.
For ASR-generalizable SNI, we propose to randomly select the words to corrupt, so that the resulting pseudo-ASRs would contain diverse ASR-error words.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose a word-level SNI approach adopting constrained generation
2) propose a random word selection in the proposed word-level SNI 
and 3) show that the proposed word-level SNI improves the ASR-generalizability of downstream models.




%factorize the two distinct steps involved in ASR errors: phonetic misunderstanding and misspelling. 
%By doing so, we isolate the phonetic misunderstanding step where the ASR system misinterprets the spoken phonemes, and the subsequent misspelling step where it generates incorrect spellings based on the misunderstood speech.
%In contrast to previous approaches that treat SNI as a unified sequence-to-sequence generation task, our proposed constrained generation method allows us to focus solely on regenerating the ASR-noised words, while preserving the original written words. 
%This factorization enables us to address each step independently and develop targeted strategies to mitigate phonetic misunderstanding and improve the accuracy of misspelling generation.
%By adopting constrained generation and explicitly considering the phonetic misunderstanding and misspelling steps, our approach offers a novel perspective and potential advancements in the field of ASR-generalizable SNI. 
%It allows for more fine-grained control and targeted interventions, ultimately leading to improved performance and robustness in the generation of ASR-corrupted data.

\end{comment}


==> backup/230714/2_related_works.tex <==
\section{Preliminaries}
\subsection{Problem Formulation}
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, SNI aims to corrupt $X$ to pseudo-ASR transcription, $T=\{t_{i^{\prime}}\}_{i^{\prime}=1}^{n^{\prime}}$ which contains phonetically similar but semantically different ASR error words.
Then, generated pseudo-ASR, $T$, is used to train downstream models.
Trained on pseudo-ASR, downstream models can robustly understand the transcriptions with ASR errors.
\subsection{Related Works}
%\subsubsection{Robustness }
%In recent years, large-scale PLMs have demonstrated remarkable performance in Natural Language Understanding (NLU) tasks~\cite{openai2023gpt4}. 
%To evaluate their robustness, several studies have employed human-crafted adversarial examples or generated examples through adversarial attacks~\cite{wang2021adversarial}. 
%Another approach involves projecting input data into a latent space using Generative Adversarial Networks and then retrieving adversaries that closely resemble the original instance in the latent space~\cite{zhao2017generating}.
%Additionally, controlled paraphrase networks are proposed to generate syntactically adversarial examples~\cite{iyyer2018adversarial}. 
%These examples not only deceive PLMs but also enhance their resilience to syntactic variations when used for training data augmentation. 
%However, the extent to which PLMs exhibit robustness against ASR errors in real-world conditions has been under-explored.
\subsubsection{SNI}
%SNI 정의, 
Recently, a few works showed that training with ASR-noised samples can robustify PLMs so that they can be adapted for SLU.
To bridge the gap between written and spoken conversations, many works attempt SNI, a data augmentation method of converting the written text $X$ into pseudo-ASR $T$ by imitating ASR errors.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$.


The most intuitive method is the TTS-ASR pipeline, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio.
In addition to the exhaustive cost of the TTS engine and ASR system, they cannot fully simulate ASR errors as the audio generated by the TTS and the human recording have different error distributions.~\cite{asrglue}


Another category of SNI, text-level SNI,  simulates ASR errors by perturbing the written text $X$ so that the resulting pseudo-ASR $T$ contains ASR errors.
Text-level SNI can be subdivided into confusion matrix and generative SNI.
In the confusion matrix method,  first, the word-level confusion matrix between written text and its paired ASR transcription is built. 
Then, ASR error is added to the written text according to the frequencies in the confusion matrix.

Another method of text-level SNI and our main baseline is the generative SNI which supervises the pre-trained auto-regressive language model as $F$.
Specifically, the pre-trained auto-regressive language model such as GPT-2 and BART is supervised to generate pseudo-ASR $T$ containing ASR errors given the written text $X$ using the probability distribution modeled as follows:
\begin{equation}
    t_{i^{\prime}} = argmax_{w \in W} P(W|X, t_{1}, ... t_{i^{\prime}-1}).
\end{equation}
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.

We argue that the pseudo-ASR by the generative SNI is not generalizable across the different ASR systems.
That is, different ASR systems generate different error distributions, thus, the downstream task model robust for one ASR system's error would not be robust to the other ASR systems.
While such generalization scenario has been widely studied in the other SLU tasks, it has been understudied for SNI.
Previous works in generative SNI used identical ASR systems for both training SNI models and transcribing SLU downstream tasks.



%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
The other category of minimizing the gap between ASR transcription and written text is ASR correction, which conducts the inverse functional mapping of SNI $F^{-1} X^{\prime} \rightarrow X$ of converting ASR transcription to the written text $X$ by removing the ASR error.
%While it has distinct strength for making 

==> backup/230714/3_ours.tex <==
\section{Ours}
We now propose our SNI model, which aims to generate pseudo-ASR which is not biased toward an individual ASR system and robustifies downstream task models against diverse ASR errors.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method for ASR generalizable SNI is to intervene in the noise word selection process, where the word to corrupt is chosen.
It is widely known that an ASR system is biased to make errors on certain phonemes more frequently and training settings such as training data can cause such error distribution~\cite{feng2021quantifying}.
As a result of such biased error distribution of the ASR system, SNI models supervised to mimic ASR errors are also vulnerable to generating pseudo-ASR following such biased error distribution.

We blame such bias on the noise word selection process in SNI, where the word to corrupt is chosen.
Let us consider whether the word $x_{i}\in X$ is corrupted or not in pseudo-ASR $T$ as the variable $z_i$.
Then, the SNI process can be written as follows:
\begin{equation}
     P(t_{i^{\prime}}|x_{i}) = \sum_{z_{i}}P(t_{i^{\prime}}|x_{i})\cdot P(z_{i}|x_{i}).
\end{equation}
Trained to mimic ASR error of specific ASR error system, the SNI model would have biased noise word selection probability for different phonemes, $P(z|x_{i})$.
That is, the SNI model would be biased to corrupt the words $x_{i}$ which is frequently corrupted by the ASR system used for training the SNI model.
Specifically, we observed that the noisygen model tends to make more errors on the phonemes, such as S and R, while rarely corrupting the phonemes IH0 and AA1 following ASR system used for training.

In order to debias SNI model to generate ASR generalizable pseudo-ASR, we propose to intervene in the noise word selection process.
Intervening the noise word selection process, we aim to attain pseudo-ASR which has more diverse corrupted phonemes. 
For such goal, we propose to adopt do-calculus and intervene in the noise word selection process.
Specifically, using the do-calculus to remove any influence from the intervened variable, $x_{i}$, on $z$ and we have the SNI modeled as follows:
\begin{align}
    P(t_{i^{\prime}}|do(x_{i})) &= \sum_{z}P(t_{i^{\prime}}, z|x_{i})\\
                                &= \sum_{z}P(t_{i^{\prime}}|x_{i},z) \cdot P(z|do(x_{i}))\\
                                &= \sum_{z}P(t_{i^{\prime}}|x_{i},z) \cdot P(z).
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In our interventional SNI, we aim to conduct the noise word selection process without the effect of $x_{i}$ so it does not follow the error distribution of any individual ASR system.
For such purpose, we propose to conduct the noise words selection process explicitly. 
Specifically, for each word $x_i$, we sample random variable $v_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, we decide whether the word $x_{i}$ will be corrupted, which is determined as the value of $z$ as follows:
\begin{align}
    z = 
    \begin{cases}
        1, \quad \text{if} \quad v_i \leq P(z) \\
        0, \quad \text{else}
    \end{cases}
\end{align}
where the word $x_{i}$ will be corrupted if $z$ is set to 1 or not if $z$ is set to 0.
Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

In this paper, we propose to model $P(t_{i^{\prime}}|x_{i},z)$ as sequence-to-sequence generation constrained on $x_{i}$.
The key characteristic of ASR error is that the ASR noise word $t_{i^{\prime}}$ can be easily aligned to its cleanly written form $x_{i}$.
To model $P(t_{i^{\prime}}|x_{i},z)$, we use such easy-to-align characteristic.
Specifically, if $z$ is set to 0, $t_{i^{\prime}}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, we constrain the generation of the ASR noise word $t^{\prime}_{i}$ to $x_{i}$ so that the generated ASR noise word $t^{\prime}_{i}$ to be phonetically similar to the cleanly written word $x_{i}$.
Replacing $x_{i}$ to the generated ASR noise word $t^{\prime}_{i}$, $X$ is corrupted into pseudo-ASR $X^{\prime}$.

To generate pseudo-ASR $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the ASR noise word $t_{i^{\prime}}$.
To generate $k$-th token for the $t_{i^{\prime}}$, the input for the decoder, the encoder representation of the cleanly written word $e^{encoder}_{i}$ and the previously generated tokens $D^{k}_{i} = \{d^{1}_{i},...d^{k-1}_{i}\}$, is formulated as follows:     
\begin{equation}
    E^{decoder}{i,k}=W_{d}[e^{encoder}_{i}; WE(D^{k}_{i}) + PE(D^{k}_{i})],
\end{equation}
where $WE$ and $PE$ are the same word and position embeddings in Eq.~\ref{eq:encoder} and $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate $k$-th token from the input and outputs the hidden representation $h^{k}_{i}$ as following:
\begin{align}
    h^{k}_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder}_{i,k},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution  for the $k$-th token is evaluated as follows:
\begin{equation}
    P_{gen}(d^{k}_{i}) = softmax(WE \cdot h^{k}_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

In training, We used the ASR transcription $T$.
Specifically, our SNI model is supervised to maximize the log-likelihood of the tokens $D_{i}$ corresponding to the ASR noise word $t_{i^{\prime}}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(d^{k}_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method for ASR generalizable SNI is to correct the phonetically differently generated ASR noise word considering the phonetic similarity.
Pure text-based generation lacks useful information like pronunciation and prosody~\cite{wang2022building} and results in phonetically different pseudo-ASR, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
Thus, we propose to evaluate phonetic similarity-based generation probability $P_{phoneme}(d^{k}_{i})$ and correct the generation probability in Eq.~\ref{eq:gen_prob} so that the phonetically similar ASR noise words can be generated as followed:
\begin{equation}
    P_{correct}(d^{k}_{i}) = P_{gen}(d^{k}_{i}) \cdot P_{phoneme}(d^{k}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


The main difficulty in the generation of phonetically similar ASR noise words is that PLMs are supervised to understand semantic context, not phonetic information.
Thus, their input, word embedding, lacks phonetic information.
Our first proposal to generate phonetically similar ASR noise words is to provide phonetic information using phoneme embedding $PHE$.
The phoneme embedding $PHE$ aims to deliver the phonetic information of tokens in the vocabulary.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The phoneme embedding is fed to the decoder similar to the encoder as follows:
\begin{multline}
    E^{decoder}_{i,k}=W_{d}[e^{encoder}_{i};  \lambda_{w}\cdot WE(X)+\lambda_{p}\cdot PHE(X) \\+ PE(D^{k}_{i})].
\end{multline}


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(d^{k}_{i}) = softmax(PHE \cdot h^{k}_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob},  $P_{phoneme}(d^{k}_{i})$ can evaluate the generation probability based on the phonetic information.

Without proper supervision of the phonetic information, $P_{phoneme}(d^{k}_{i})$ cannot correct the generation of the phonetically different ASR noise words.
For the supervision of the phonetic information, we propose to distill the phonetic information from the phonetic edit distance~\cite{9662078}.
The phoneme edit distance measures the similarity between the given two words $w_i$ and $w_j$ by two consecutive steps.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}

In order to correct the generation probability as in Eq.~\ref{eq:phoneme_correction_prob}, the phonetic information should be evaluated as the probability distribution. 
For such purpose, we convert the phoneme edit distance to the phoneme probability distribution $\textbf{Q}(d^{k}_{i})$, which will be used as the label for $P_{phoneme}(d^{k}_{i})$.
First, the phoneme edit distance is converted into the phoneme similarity score $PS$ which is defined as follows
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.
For the ground-truth token, $d^{k}_{i}$, the phoneme probability distribution $\textbf{Q}(d^{k}_{i})$ is evaluated for each token $w$ in vocabulary as followed:
\begin{equation}
    Q^{j}(d^{k}_{i}) = \frac{PS(d^{k}_{i},w)}{\sum_{w^{\prime}\in W}PS(d^{k}_{i},w^{\prime} )}.
 \end{equation}
 The phoneme probability distribution  $\textbf{Q}(d^{k}_{i})$ is used as a label to supervise the phoneme information to evaluate loss as followed:
 \begin{equation}
     l_p = KLD(P_{phoneme}(d^{k}_{i}),  Q(d^{k}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(d^{k}_{i})$ can correct the generation of the phonetically different words.
 

 



\begin{comment}
phonemeisconsideredasacleanform1ofspeechrepresentationcomplementarytotext. ~\cite{wang2022building}

    TheauxiliaryBERTencoderextractsadditionaltext featuresforcharacter-basedunits(e.g.,character[21],subword [19,22]),whichenablestheTTSsystemtogeneratespeechwith betterpronunciationandexpressiveness.Thosemethodshave tofacethechallengethatthepre-trainingwiththecharacterbasedunitsisinconsistentwiththeTTSfine-tuningtakingpure phonemeastheinput.Theinconsistencywillbringseveral problems:1)Thealignmentbetweenphonemeandcharacterinformationmightbeunstable(e.g.,misalignmentbetween phonemeandcharactersequence),makingtheTTSphoneme encoderfailtoleveragethepre-trainedtextfeatures.~\cite{zhang2022mixedphoneme}
\end{comment}
\begin{comment}
    
The task of SNI can be treated as a functional mapping $F:X \rightarrow X^{\prime}$ between the written text $X$ and the pseudo-ASR transcription $X^{\prime}$,  where $X=\{x_1, ..., x_n\}$ denotes ground truth transcription which is a sequence of n words and  $X^{\prime}=\{x^{\prime}_1, ..., x^{\prime}_{n^{\prime}}\}$ is the ASR transcription of a sequence of $n^{\prime}$ words.  

We now propose our methods for ASR-generalizable SNI.
Mimicking the ASR error generation process, we explicitly decompose the SNI as two consecutive steps of the noise target word selection and noise word generation.
By explicitly 
 Previous works model SNI as trivial sequence-to-sequence problem of generating $X^{\prime}$ given $X$ using vocabulary $V$ as followed:
\begin{equation}
    x^{\prime}_i = argmax P(V|X, x^{\prime}_{1}, ... x^{\prime}_{i-1}).
\end{equation}
In this formulation, noise target phrase selection and noise phrase generation are implicitly done at once.
Thus, the resulting SNI sentences can be biased toward specific ASR systems as distinct ASR systems have different phoneme misunderstanding patterns.
Also, unlike other sequence-to-sequence tasks such as question answering, which may have radically different inputs and outputs, it is observed that the input, and output of SNI, ground-truth transcription $X$, and ASR transcription $T$, are nearly identical.
Moreover, ASR noise phrases $W^{\prime} = \{w^{\prime}_1...,w^{\prime}_p\} \subset T$ can be easily aligned to their clean written form $W = \{w_1...,w_q\}\subset X$, the sequence-to-sequence formulation of SNI does not reflect such easy-to-align nature of ASR errors.
Without noticing such easy-to-align nature, the SNI model can rather generate entirely different sentences than corrupt the clean sentences into ASR-like sentences.
Thus, requiring additional heuristic filtering of noised samples~\cite{noisygen}.



Our key idea is to explicitly factorize SNI as two-step procedure similar to the two steps of the ASR-noise generation process. 
Specifically, we formulate SNI as following two subsequent steps: noise target phrase selection and noise phrase generation.
Noise target phrase selection aims to select noise target phrase $W \subset X$ which is replaced in ASR transcription as noise phrase $W^{\prime} \in T$.
Then, given a noise target phrase $W$, noise phrase generation aims to generate noise phrase $W^{\prime} \in T$.

In our training setting for noise target phrase selection, our objective is to identify potential ASR noise phrases from the ground-truth transcription so that identified phrases can be corrupted. 
To accomplish this, we used the phrases noised in the ASR transcription as our noise target phrases during the training phase. 
In inference time of conducting SNI on written text, we randomly selected phrases from the input text to serve as the noise target phrases.
This approach was motivated by the fact that different ASR systems can exhibit varying patterns of phoneme misunderstanding, making it challenging to generalize the selection of noise target phrases across different ASR systems. 
By randomly selecting noise-target phrases during inference, we ensure that the resulting noised sentences are not biased towards any specific ASR system. 
This allows downstream task models trained with our SNI data to simulate the diverse phonetic misunderstandings that can occur across different ASR systems, enhancing the robustness and generalizability of our approach in handling ASR-induced errors in real-world scenarios.

Then our next step is noise phrase generation, which aims to generate noise phrase $W^{\prime} \in T$ given noise target phrase $W  \subset X$ modeled as follows:
\begin{equation}
    w^{\prime}_i = argmax P(V|W, w^{\prime}_1, ... w^{\prime}_{i-1}).
\end{equation}
Generating noise phrases given only selected noise target phrases, our SNI model focuses on generating ASR-like sentences and does not require heuristic filtering in previous works.



%Specifically, we propose to fractionize SNI into more fine-grained mapping $f:W \rightarrow W^{\prime}$ between the noise target phrases and the noised phrases. 

%We design an end-to-end architecture consisting of an encoder, a decoder, and an operation predictor to constrain the decoding process to the desired part of the input sequence.  
%The encoder produces sequence embeddings from the word embeddings of the ASR output texts and related positional embeddings.  
%The operation predictor is a fully-connected layer trained to identify the above-mentioned“K”, “D” and “C” input sequence embeddings.  
%The model can reduce inference latency significantly by restricting the decoding process to the “C” tokens

%For the change position, the transformed-based decoder inputs at timestep t are calculated as follows: \begin{equation}
%    Eyt,k=Wp[(WE(wyt,k) + PE(wyt,k))exk], 
%\end{equation}
%where $WE$ and $PE$ are the same word and position embedding functions as in equation.
%$exk$ is the encoded token representation mentioned before. 
%$Wp$ is the trainable parameters.
%Then, a standard transformer decoder is employed to fuse all relevant information:
%\begin{align}
%    hkt+1= TransformerDecoder(Q,K,V),\\
%    Q=Eyt,k,K=Ex,V=Ex,
%\end{align}
%where  the decoder  input $Eyt,k$ works  as query (“Q”),  and  encoded model input $Ex$ works as key (“K”) and value (“V”) in the transformer decoder.
%$hkt+1$ is the fused vector.
%Finally, the target output is predicted as follows:
%\begin{equation}
%    p(ˆωyt+1,k) = softmax(Wyhkt+1+by), 
%\end{equation}
%where $Wy$ and $by$ are trained parameters.   
%Then, generation loss is defined as followed:
%\begin{equation}
%   lossdec=tlog(p(ˆωyt,k)).
%\end{equation}

\end{comment}

==> backup/230714/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

~\input{table/dataset_statistics}

For training SNI model, we followed the settings from the previous work~\cite{noisygen}, which used to popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, DeepSpeech, and get recognized results. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2}, which models task-oriented dialogue systems with unstructured knowledge access.
The key reason for adopting DSTC10 Track2 dataset is that its sentences are the transcription of human-spoken task-oriented dialogue by an unknown ASR model.
Specifically, it includes three subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG).
In DSTC10 Tack 2 dataset, task-oriented dialogue systems are modeled as sequence of three subtasks.
First, determine whether the dialogue turn requires external knowledge access or not. 
Once determined to require external knowledge, then the second step is to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the whole knowledge base.
Finally, the response should be generated based on the dialogue context and the selected knowledge snippet. 
We choose DSTC10 Track2 dataset as it contains major tasks in NLP, classification and retrieval, generation as SLU.



\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

We followed settings for downstream task DSTC10 Track2 from previous works~\cite{dstc10_2, tian2021tod-da}.
We conducted SNI on the written form of each subtask dataset in a task-oriented dialogue system dataset and used the resulting noised sentence for training downstream models.
For the downstream task model, we followed the baseline model setting of DSTC10 Track2~\cite{dstc10_2} and trained GPT2-small on each subtask.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2}.



==> backup/230714/5_results.tex <==
\section{Results}
\input{table/result}
%We present the result on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
%The downstream model trained with our method outperformed baselines with a large margin in KS and RG subtasks and comparable results in KTD.
In this section, we first present the results of our proposed method for on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
Specifically, we report the results of all subtasks, the knowledge turn detection subtask and the knowledge selection, and response generation.
The results demonstrate the superiority of our approach in knowledge selection and response generation, while also achieving comparable performance in knowledge turn detection.

For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


In the response generation subtask, our method outperformed the baseline methods in every metric. 
However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
This indicates that our SNI method can better robustify the PLMs on generation task.


Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.

Overall, our proposed method demonstrated superior performance in the knowledge selection and response generation subtasks of the task-oriented dialogue dataset. 
Additionally, it showcased competitive results in the knowledge turn detection subtask. 
These findings highlight the effectiveness of our approach in enhancing the capabilities of task-oriented dialogue systems and improving their performance in understanding user queries, selecting relevant knowledge, and generating appropriate responses.


==> backup/230714/6_conclusion.tex <==
\section{Conclusion}
In this paper, we first showed that among two ASR noise procedures, the misspelling step is generalizable between different ASR models while the phoneme misunderstanding does not.
Based on such findings, we proposed a new SNI method that formulated SNI as a constrained generation problem that fractionize SNI as a phrase-to-phrase problem.
From such formulation, we could attain an ASR-generalizable SNI model by randomizing noise target word selection and better supervising the noise word generation.

==> backup/230720/0_abs.tex <==
\begin{abstract}
This paper proposes ASR-generalizable speech noise injection (SNI) for improving spoken language understanding (SLU) models in the presence of ASR errors. Pretrained language models (PLMs) trained on written language struggle to adapt to the differences in spoken language, especially due to phonetic misunderstanding and misspelling errors introduced by ASR systems. While previous works have explored SNI, the generalizability of SLU models to different ASR systems remains understudied. We factorize ASR errors into two steps: phonetic misunderstanding and misspelling, and demonstrate that misspelling errors are more model generalizable compared to phonetic misunderstanding. To explicitly model these steps, we propose constrained generation, focusing on regenerating ASR-noised words. The approach enables targeted generation and improves the robustness and generalizability of SLU models. Experimental results and analysis are provided to support the effectiveness of ASR-generalizable SNI.
\end{abstract}

==> backup/230720/1_intro.tex <==
\section{Introduction}
Starting from ELMo~\cite{peters-etal-2018-deep} to recent GPT4~\cite{openai2023gpt4}, pretrained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
As such abilities are essential for spoken language understanding (SLU)~\cite{broscheit-etal-2022-distributionally, 8907842}, PLMs are widely adopted in speech-enabled systems such as voice assistants.
Specifically,  PLMS are adopted in a  pipeline  process of such speech-enabled systems. 
First, audio is converted into textual transcription by an automatic speech recognition (ASR) system. 
Then, the transcription is fed into PLMs to conduct downstream SLU tasks. 


%As PLMs are trained in the different modality of written text, they suffer to adapt to the difference between the transcription and text.
%이 문단에서 하고 싶은 말은 PLM들이 SLU에서 ASR noise 때문에 못하지만 ASR noise를 포함하는 데이터를 학습하면 robust해짐
While PLMs suffer from the noise in the spoken transcription, ASR errors, they can be robustified when trained on the SLU corpora containing such noises..
That is, ASR systems fail to generate the correct transcription and confuse to generate phonetically similar but wrong ASR error words~\cite{ruan20_interspeech,9054689}.
%The key difference disturbing PLMs in SLU is the errors of the ASR systems. 
%Specifically, ASR systems confuse to generate phonetically similar and semantically different words, ASR error words~\cite{ruan20_interspeech,9054689}.
As the ASR error words are mapped to different tokens, the input sequence different from the written text is fed to PLMs.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original spoken language and makes an incorrect prediction on SLU~\cite{belinkov2018synthetic}.


%데이터
%SLU copora 모으는거 어렵기 때문에 SNi 함
As collecting such SLU corpora requires additional human annotations, the data augmentation method of the speech noise injection (SNI) has been introduced.
An SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
SNI aims to reduce the additional effort in collecting SLU corpora by removing human annotation in recording and transcribing.
Specifically, SNI corrupts the written corpora by mimicking how the ASR systems make incorrect transcriptions.

%여기는 previous SNI 들이 다 ASR specific 하다는 내용 위주로 고치기.
%Previous works in SNI can be categorized into two methods. 
%The most intuitive method is the TTS-ASR pipeline, where the TTS engine (text-to-speech) converts the text into audio, and the ASR system transcribes the audio.
%While ASR errors are generated by TTS engines and ASR systems, they are both computationally expensive.
%Additionally, they cannot generate sufficient ASR errors as the noise engaged during human reading does not exist in the audio converted by TTS.
%In contrast, generative SNI supervises the autoregressive language model $M$ to generate the pseudo-ASR given the text as the following:
%\begin{equation}
%    X^{\prime} = M(X)
%\end{equation}
%As generative SNI is shown to be effective in various situations~\cite{asrglue}, we focus on generative SNI.
However, as different ASR systems can be used in SLU pipeline, pseudo-ASR should not be biased toward individual ASR and generalizable across different ASR systems.
While such ASR-generalizability has been widely studied in diverse SLU tasks, previous works in SNI is limited to only individual ASR system.
We argue that ASR-generalizability is also crucial in SNI.
For ASR- generalizability, the ASR systems should be trained on ASR noise generated from diverse error distributions~\cite{7178796}.
However, previous works in SNI cannot generate such diverse ASR errors and follows the individual ASR system.
%While many previous works studied SNI~\cite{feng22c_interspeech, noisygen}, ASR-generalizability, the ability of an SLU model to perform robustly across different ASR systems, is not well studied for SNI.
%Such generalizability has been focused on diverse SLU tasks as different ASR systems can be used in SLU pipeline~\cite{blackbox1}.
%ASR-generalizability has been important as different ASR systems have distinct error distributions and SLU trained on one error distribution suffers to generalize on different error distribution.
%However, previous works in SNI confirmed their effectiveness using identical ASR systems for both SNI and downstream tasks, where the ASR generalizability still remains unveiled~\cite{noisygen,tts_asr}.
%We argue that ASR-generalizability is also crucial in SNI as the resulting pseudo-ASR would follow the error distribution of an individual ASR system.


\input{figure_latex/figure1}
%Toward ASR generalizable SNI, we first propose to intervene SNI process based on do-calculus~\cite{glymour2016causal} so that the resulting pseudo-ASR would not follow the error distribution of an individual ASR system. 
Toward ASR generalizable SNI containing diverse ASR noises, we first propose to intervene SNI based on do-calculus~\cite{glymour2016causal}.
%factorize the generation of ASR errors into two distinct steps: phonetic misunderstanding and misspelling.
%For such goal, we train SNI model to generate the ASR-noised words constrained on its written words, the noise target words.
%Previous works supervised SNI model to maximize the likelihood of the entire ASR transcription given its written sentence~\cite{asrglue, noisygen}.
Due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to follow the error distribution of individual ASR systems.
%During such supervision, the SNI model is biased to select the noise target words following the error distribution of the ASR system adopted for training.
Thus, the resulting pseudo-ASR would contain biased ASR errors, such as containing errors for specific phonemes.
To remove such bias, we propose to implement the intervention in SNI by factorizing it into the two processes of noise word selection and noise word generation.
In the noise word selection, the noise target word, the word to be corrupted in the pseudo-ASR, is randomly selected without bias. Then, by constraining the noise target word, a phonetically similar ASR noise word is generated.
As the bias from the ASR system is removed, the resulting pseudo-ASR contains diverse ASR errors and can robustify the downstream model against the diverse ASR systems.
%In contrast, our SNI model randomly selects the noise target words. 
%This random selection serves as an intervention to the error distribution of the ASR system and debias the resulting pseudo-ASR to diversify the error distribution.
%Trained on the pseudo-ASR with more diverse ASR errors, downstream task models can more robustly conduct downstream tasks.
%As a result
%, similar to interventions performed in do-calculus, where we actively modify the values of certain variables to observe the effects on the overall system.
%By randomly selecting the words, we remove the bias associated with specific ASR systems and ensure a more diverse set of corrupted words.

Our second contribution toward ASR generalizable SNI is to correct the generation of phonetically different ASR noise words. 
The key characteristic of ASR errors is that the ASR systems incorrectly transcript into phonetically similar words.
However, existing SNI models generate the ASR error words under ignorance of the phonemes.
We argue that  such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems and fails to generate phonetically different ASR noise words.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Understanding phonemes, the resulting pseudo-ASR become more phonetically similar to cleanly written sentences.

%In addition to intervention in the error distribution, we propose to correct the generation of ASR noise words using phonetic information. 
%While ASR systems generate phonetically similar words as ASR error words, SNI models are optimized to maximize the likelihood of the grapheme-based tokens corresponding to ASR error words.
%Blinded to phonetic similarity, the existing SNI model fails to generate phonetically similar pseudo-ASR and requires additional phonetic similarity based heuristic to filter out such failing pseudo-ASR.
%Instead of such heuristic, we propose to supervise and incorporate phonetic similarity to correct the noise word generation.
%Specifically, we propose a phoneme head, another language model head that generates ASR noise words based on their phonemes.
%This phoneme head is used with trivial language model head of SNI models and ensures to generate the phonetically similar ASR error words.

%Powerful generation models of ten meet most of the task requirements, yet miss a few (e.g.,omittinga subset of keywords), or generate incorrect hypotheses that nevertheless provide useful structure (e.g.,a correct problem solving strategy with a missing step). However, after generatingevenaslightlysub-optimalsequence,thesingle-passparadigmrequiresmodelsto“startfrom scratch”,effectivelydiscardingworkalreadydone.Amorenatural,intuitiveapproachisleveraging thegenerationasausefulstartingpointtorefineintoahigherqualityoutput.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of phonetically different ASR noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

\begin{comment}
In the phonetic misunderstanding step, the ASR system misinterprets the spoken phonemes, leading to inaccuracies in the resulting transcription. 
Consequently, the subsequent step, misspelling, arises as a result of the ASR system generating misspelled words based on its flawed understanding of the original speech. 
Misspelling errors occur when the ASR system incorrectly converts the misunderstood phonemes into different characters, further deviating from the intended transcription. 

\input{table/asr_cer}

Among two distinct steps, we argue that  
while the phonetic misunderstanding is ASR-specific noise, the misspelling step is ASR-generalizable.
Specifically, phonetic misunderstanding can be largely influenced by training data and acoustic modeling.
For example, ASR systems with distinct acoustic feature extractors and different accented training audio would exhibit distinct susceptibility to phonetic misunderstanding.
In contrast, we argue that the phenomenon of misspelling is more ASR-generalizable. 
This is because a language possesses specific spelling conventions that are shared across different ASR models regardless of training data or acoustic modeling techniques. 

To demonstrate the generalizability of misspelling errors among ASR models, we present the Character Error Rate (CER) between different open-source ASR models, DeepSpeech and Leopard, and ground-truth transcription in Table~\ref{tab:cer}. 
In Table~\ref{tab:cer}, we observe that the CER values for the different ASR models are smaller than that of each ASR model and ground-truth transcription. 
This indicates that, despite the differences in model-specific factors, the misspelling errors generated by these models are more similar to each other than ground-truth transcription.

Toward ASR-generalizable SNI, we consider alignable characteristics of the ASR-error words.
That is, the words in the ground-truth text can be easily aligned to their corresponding words in ASR transcription.
When the words are correctly transcribed, the words in the ASR and its ground-truth text would be easily aligned.
However, such alignment is not limited to the correctly transcribed words.
As ASR systems misspell the words of the ground-truth text into phonetically, also graphemically, similar words, even inaccurately transcribed words can be easily aligned to their corresponding words.

Considering such alignment, we propose to break down SNI from generating entire pseudo-ASR transcription $X^{\prime}$ given written text $X$ into the finer-grained generation of ASR error words $w^{\prime}\in X^{\prime}$ given written word $w \in X$ adopting constrained generation which can be formulated as follows:
\begin{equation}
    w^{\prime} = M(w)
\end{equation}
Directly conditioned on the cleanly written word $w$, not the entire text $X$, such fine-grained SNI can better supervise the SNI model of how the written words $w$ are corrupted to ASR error words $w^{\prime}$ by misspelling. 
By better supervising misspelling with fine-grained SNI, we enhance its ability to generalize across different ASR systems, as ASR misspelling is generalizable to different written words, regardless of the ASR systems.

In addition to misspellings, fine-grained SNI can also contribute to a more ASR-generalizable approach in the context of phoneme misunderstanding.
In previous generative SNI, whether the cleanly written word $w$ would be corrupted is implicitly determined by SNI model $M$.
Biased by the phoneme misunderstanding pattern of the ASR system used to transcribe the training set, the SNI model tends to corrupt only the words that the specific ASR system would phonetically misunderstand.
Compared to sentence-level SNI, our word-level SNI gives more control in selecting which words to corrupt to ASR error words.
For ASR-generalizable SNI, we propose to randomly select the words to corrupt, so that the resulting pseudo-ASRs would contain diverse ASR-error words.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose a word-level SNI approach adopting constrained generation
2) propose a random word selection in the proposed word-level SNI 
and 3) show that the proposed word-level SNI improves the ASR-generalizability of downstream models.




%factorize the two distinct steps involved in ASR errors: phonetic misunderstanding and misspelling. 
%By doing so, we isolate the phonetic misunderstanding step where the ASR system misinterprets the spoken phonemes, and the subsequent misspelling step where it generates incorrect spellings based on the misunderstood speech.
%In contrast to previous approaches that treat SNI as a unified sequence-to-sequence generation task, our proposed constrained generation method allows us to focus solely on regenerating the ASR-noised words, while preserving the original written words. 
%This factorization enables us to address each step independently and develop targeted strategies to mitigate phonetic misunderstanding and improve the accuracy of misspelling generation.
%By adopting constrained generation and explicitly considering the phonetic misunderstanding and misspelling steps, our approach offers a novel perspective and potential advancements in the field of ASR-generalizable SNI. 
%It allows for more fine-grained control and targeted interventions, ultimately leading to improved performance and robustness in the generation of ASR-corrupted data.

\end{comment}


==> backup/230720/2_prelim.tex <==
\section{Preliminaries}
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into the pseudo-ASR, which an ASR system would transcribe into given the recording of the written corpora.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo-ASR transcription, $T=\{t_{i^{\prime}}\}_{i^{\prime}=1}^{n^{\prime}}$.
Then, the resulting pseudo-ASR, $T$, is used to train downstream models.
Trained on pseudo-ASR $T$ containing ASR errors, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
%\subsubsection{Robustness }
%In recent years, large-scale PLMs have demonstrated remarkable performance in Natural Language Understanding (NLU) tasks~\cite{openai2023gpt4}. 
%To evaluate their robustness, several studies have employed human-crafted adversarial examples or generated examples through adversarial attacks~\cite{wang2021adversarial}. 
%Another approach involves projecting input data into a latent space using Generative Adversarial Networks and then retrieving adversaries that closely resemble the original instance in the latent space~\cite{zhao2017generating}.
%Additionally, controlled paraphrase networks are proposed to generate syntactically adversarial examples~\cite{iyyer2018adversarial}. 
%These examples not only deceive PLMs but also enhance their resilience to syntactic variations when used for training data augmentation. 
%However, the extent to which PLMs exhibit robustness against ASR errors in real-world conditions has been under-explored.
\subsubsection{SNI}

Previous works pointed out that the key distinction of the incorrect transcription $t_{i^{\prime}}\in T$ from different noise is phonetically similar to its written word $x_{i}\in X$~\cite{9721159, asrglue, tian2021tod-da}.
Specifically, each word $t_{i^{\prime}}\in T$ would be either identical or different to its corresponding written word $x_{i}\in X$ as a simulation of correct or incorrect transcription of an ASR system.
Therefore, previous works proposed various corrupting methods to reflect such phonetic characteristics in the pseudo-ASR.
Previously proposed methods can be summarized as 3 categories of textual perturbation and TTS-ASR pipeline, auto-regressive generation.

The most intuitive method of SNI is textual perturbation which simulates ASR errors by perturbing the written text $X$ so that the resulting pseudo-ASR $T$ contains ASR errors~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, the pseudo-ASR $X$ is generated by replacing the written word $x_i$ with its phonetically similar word $t_{i^{\prime}}$ which is determined as follows: 
\begin{equation}
   t_{i^{\prime}} = argmax_{w \in W} P(W|x_{i}),
\end{equation}
where $P(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $P(W|x_{i})$. 
Specifically, $P(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo-ASR efficiently, they cannot generate diverse ASR noises as $P(W|x_{i})$ is pre-defined.



Another category of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio.
During the conversion between the text and audio, the errors of the TTS engines and the ASR systems are expected to corrupt the written word into its phonetically similar word.
The exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora.
Also, they cannot fully simulate ASR errors as the audio generated by the TTS and the human recording have different error distributions~\cite{asrglue}, thus the resulting pseudo-ASR would have different error distribution from the ASR transcription.




The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to implement $F$~\cite{asrglue, noisygen}.
Specifically, the auto-regressive PLMs such as GPT-2 or BART is supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$.
During such supervision, the SNI model is expected to generate pseudo-ASR following the error distribution of the ASR system. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.

We argue that the pseudo-ASR generated by auto-regressive generation is not generalizable across the different ASR systems.
That is, different ASR systems generate different error distributions, thus, the downstream task model robust for one ASR system's error would not be robust to the other ASR systems.
While such generalization scenario has been widely studied in the other SLU tasks, it has been understudied for SNI.
Previous works in generative SNI used identical ASR systems for both training SNI models and transcribing SLU downstream tasks.



%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F^{-1} X^{\prime} \rightarrow X$ of converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which generates the written words constrained on the ASR noise words was proposed~\cite{constdecoder}
However, due to the innate robustness of PLMs against to noises~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

==> backup/230720/3_ours.tex <==
\section{Ours}
We now propose our SNI model, which aims to generate pseudo-ASR which is not biased toward an individual ASR system and robustifies downstream task models against diverse ASR errors.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method for ASR generalizable SNI is to intervene in the noise word selection process, where the word to corrupt is chosen.
It is widely known that an ASR system is biased to make errors on certain phonemes more frequently and training settings such as training data can cause such error distribution~\cite{feng2021quantifying}.
As a result of such biased error distribution of the ASR system, SNI models supervised to mimic ASR errors are also vulnerable to generating pseudo-ASR following such biased error distribution.

We blame such bias on the noise word selection process in SNI, where the word to corrupt is chosen.
Let us consider whether the word $x_{i}\in X$ is corrupted or not in pseudo-ASR $T$ as the variable $z_i$.
Then, the SNI process can be written as follows:
\begin{equation}
     P(t_{i^{\prime}}|x_{i}) = \sum_{z_{i}}P(t_{i^{\prime}}|x_{i})\cdot P(z_{i}|x_{i}).
\end{equation}
Trained to mimic ASR error of specific ASR error system, the SNI model would have biased noise word selection probability for different phonemes, $P(z|x_{i})$.
That is, the SNI model would be biased to corrupt the words $x_{i}$ which is frequently corrupted by the ASR system used for training the SNI model.
Specifically, we observed that the noisygen model tends to make more errors on the phonemes, such as S and R, while rarely corrupting the phonemes IH0 and AA1 following ASR system used for training.

In order to debias SNI model to generate ASR generalizable pseudo-ASR, we propose to intervene in the noise word selection process.
Intervening the noise word selection process, we aim to attain pseudo-ASR which has more diverse corrupted phonemes. 
For such goal, we propose to adopt do-calculus and intervene in the noise word selection process.
Specifically, using the do-calculus to remove any influence from the intervened variable, $x_{i}$, on $z$ and we have the SNI modeled as follows:
\begin{align}
    P(t_{i^{\prime}}|do(x_{i})) &= \sum_{z}P(t_{i^{\prime}}, z|x_{i})\\
                                &= \sum_{z}P(t_{i^{\prime}}|x_{i},z) \cdot P(z|do(x_{i}))\\
                                &= \sum_{z}P(t_{i^{\prime}}|x_{i},z) \cdot P(z).
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In our interventional SNI, we aim to conduct the noise word selection process without the effect of $x_{i}$ so it does not follow the error distribution of any individual ASR system.
For such purpose, we propose to conduct the noise words selection process explicitly. 
Specifically, for each word $x_i$, we sample random variable $v_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, we decide whether the word $x_{i}$ will be corrupted, which is determined as the value of $z$ as follows:
\begin{align}
    z = 
    \begin{cases}
        1, \quad \text{if} \quad v_i \leq P(z) \\
        0, \quad \text{else}
    \end{cases}
\end{align}
where the word $x_{i}$ will be corrupted if $z$ is set to 1 or not if $z$ is set to 0.
Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

In this paper, we propose to model $P(t_{i^{\prime}}|x_{i},z)$ as sequence-to-sequence generation constrained on $x_{i}$.
The key characteristic of ASR error is that the ASR noise word $t_{i^{\prime}}$ can be easily aligned to its cleanly written form $x_{i}$.
To model $P(t_{i^{\prime}}|x_{i},z)$, we use such easy-to-align characteristic.
Specifically, if $z$ is set to 0, $t_{i^{\prime}}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, we constrain the generation of the ASR noise word $t^{\prime}_{i}$ to $x_{i}$ so that the generated ASR noise word $t^{\prime}_{i}$ to be phonetically similar to the cleanly written word $x_{i}$.
Replacing $x_{i}$ to the generated ASR noise word $t^{\prime}_{i}$, $X$ is corrupted into pseudo-ASR $X^{\prime}$.

To generate pseudo-ASR $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the ASR noise word $t_{i^{\prime}}$.
To generate $k$-th token for the $t_{i^{\prime}}$, the input for the decoder, the encoder representation of the cleanly written word $e^{encoder}_{i}$ and the previously generated tokens $D^{k}_{i} = \{d^{1}_{i},...d^{k-1}_{i}\}$, is formulated as follows:     
\begin{equation}
    E^{decoder}{i,k}=W_{d}[e^{encoder}_{i}; WE(D^{k}_{i}) + PE(D^{k}_{i})],
\end{equation}
where $WE$ and $PE$ are the same word and position embeddings in Eq.~\ref{eq:encoder} and $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate $k$-th token from the input and outputs the hidden representation $h^{k}_{i}$ as following:
\begin{align}
    h^{k}_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder}_{i,k},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution  for the $k$-th token is evaluated as follows:
\begin{equation}
    P_{gen}(d^{k}_{i}) = softmax(WE \cdot h^{k}_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

In training, We used the ASR transcription $T$.
Specifically, our SNI model is supervised to maximize the log-likelihood of the tokens $D_{i}$ corresponding to the ASR noise word $t_{i^{\prime}}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(d^{k}_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method for ASR generalizable SNI is to correct the phonetically differently generated ASR noise word considering the phonetic similarity.
Pure text-based generation lacks useful information like pronunciation and prosody~\cite{wang2022building} and results in phonetically different pseudo-ASR, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
Thus, we propose to evaluate phonetic similarity-based generation probability $P_{phoneme}(d^{k}_{i})$ and correct the generation probability in Eq.~\ref{eq:gen_prob} so that the phonetically similar ASR noise words can be generated as followed:
\begin{equation}
    P_{correct}(d^{k}_{i}) = P_{gen}(d^{k}_{i}) \cdot P_{phoneme}(d^{k}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


The main difficulty in the generation of phonetically similar ASR noise words is that PLMs are supervised to understand semantic context, not phonetic information.
Thus, their input, word embedding, lacks phonetic information.
Our first proposal to generate phonetically similar ASR noise words is to provide phonetic information using phoneme embedding $PHE$.
The phoneme embedding $PHE$ aims to deliver the phonetic information of tokens in the vocabulary.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The phoneme embedding is fed to the decoder similar to the encoder as follows:
\begin{multline}
    E^{decoder}_{i,k}=W_{d}[e^{encoder}_{i};  \lambda_{w}\cdot WE(X)+\lambda_{p}\cdot PHE(X) \\+ PE(D^{k}_{i})].
\end{multline}


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(d^{k}_{i}) = softmax(PHE \cdot h^{k}_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob},  $P_{phoneme}(d^{k}_{i})$ can evaluate the generation probability based on the phonetic information.

Without proper supervision of the phonetic information, $P_{phoneme}(d^{k}_{i})$ cannot correct the generation of the phonetically different ASR noise words.
For the supervision of the phonetic information, we propose to distill the phonetic information from the phonetic edit distance~\cite{9662078}.
The phoneme edit distance measures the similarity between the given two words $w_i$ and $w_j$ by two consecutive steps.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}

In order to correct the generation probability as in Eq.~\ref{eq:phoneme_correction_prob}, the phonetic information should be evaluated as the probability distribution. 
For such purpose, we convert the phoneme edit distance to the phoneme probability distribution $\textbf{Q}(d^{k}_{i})$, which will be used as the label for $P_{phoneme}(d^{k}_{i})$.
First, the phoneme edit distance is converted into the phoneme similarity score $PS$ which is defined as follows
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.
For the ground-truth token, $d^{k}_{i}$, the phoneme probability distribution $\textbf{Q}(d^{k}_{i})$ is evaluated for each token $w$ in vocabulary as followed:
\begin{equation}
    Q^{j}(d^{k}_{i}) = \frac{PS(d^{k}_{i},w)}{\sum_{w^{\prime}\in W}PS(d^{k}_{i},w^{\prime} )}.
 \end{equation}
 The phoneme probability distribution  $\textbf{Q}(d^{k}_{i})$ is used as a label to supervise the phoneme information to evaluate loss as followed:
 \begin{equation}
     l_p = KLD(P_{phoneme}(d^{k}_{i}),  Q(d^{k}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(d^{k}_{i})$ can correct the generation of the phonetically different words.
 

 



\begin{comment}
phonemeisconsideredasacleanform1ofspeechrepresentationcomplementarytotext. ~\cite{wang2022building}

    TheauxiliaryBERTencoderextractsadditionaltext featuresforcharacter-basedunits(e.g.,character[21],subword [19,22]),whichenablestheTTSsystemtogeneratespeechwith betterpronunciationandexpressiveness.Thosemethodshave tofacethechallengethatthepre-trainingwiththecharacterbasedunitsisinconsistentwiththeTTSfine-tuningtakingpure phonemeastheinput.Theinconsistencywillbringseveral problems:1)Thealignmentbetweenphonemeandcharacterinformationmightbeunstable(e.g.,misalignmentbetween phonemeandcharactersequence),makingtheTTSphoneme encoderfailtoleveragethepre-trainedtextfeatures.~\cite{zhang2022mixedphoneme}
\end{comment}
\begin{comment}
    
The task of SNI can be treated as a functional mapping $F:X \rightarrow X^{\prime}$ between the written text $X$ and the pseudo-ASR transcription $X^{\prime}$,  where $X=\{x_1, ..., x_n\}$ denotes ground truth transcription which is a sequence of n words and  $X^{\prime}=\{x^{\prime}_1, ..., x^{\prime}_{n^{\prime}}\}$ is the ASR transcription of a sequence of $n^{\prime}$ words.  

We now propose our methods for ASR-generalizable SNI.
Mimicking the ASR error generation process, we explicitly decompose the SNI as two consecutive steps of the noise target word selection and noise word generation.
By explicitly 
 Previous works model SNI as trivial sequence-to-sequence problem of generating $X^{\prime}$ given $X$ using vocabulary $V$ as followed:
\begin{equation}
    x^{\prime}_i = argmax P(V|X, x^{\prime}_{1}, ... x^{\prime}_{i-1}).
\end{equation}
In this formulation, noise target phrase selection and noise phrase generation are implicitly done at once.
Thus, the resulting SNI sentences can be biased toward specific ASR systems as distinct ASR systems have different phoneme misunderstanding patterns.
Also, unlike other sequence-to-sequence tasks such as question answering, which may have radically different inputs and outputs, it is observed that the input, and output of SNI, ground-truth transcription $X$, and ASR transcription $T$, are nearly identical.
Moreover, ASR noise phrases $W^{\prime} = \{w^{\prime}_1...,w^{\prime}_p\} \subset T$ can be easily aligned to their clean written form $W = \{w_1...,w_q\}\subset X$, the sequence-to-sequence formulation of SNI does not reflect such easy-to-align nature of ASR errors.
Without noticing such easy-to-align nature, the SNI model can rather generate entirely different sentences than corrupt the clean sentences into ASR-like sentences.
Thus, requiring additional heuristic filtering of noised samples~\cite{noisygen}.



Our key idea is to explicitly factorize SNI as two-step procedure similar to the two steps of the ASR-noise generation process. 
Specifically, we formulate SNI as following two subsequent steps: noise target phrase selection and noise phrase generation.
Noise target phrase selection aims to select noise target phrase $W \subset X$ which is replaced in ASR transcription as noise phrase $W^{\prime} \in T$.
Then, given a noise target phrase $W$, noise phrase generation aims to generate noise phrase $W^{\prime} \in T$.

In our training setting for noise target phrase selection, our objective is to identify potential ASR noise phrases from the ground-truth transcription so that identified phrases can be corrupted. 
To accomplish this, we used the phrases noised in the ASR transcription as our noise target phrases during the training phase. 
In inference time of conducting SNI on written text, we randomly selected phrases from the input text to serve as the noise target phrases.
This approach was motivated by the fact that different ASR systems can exhibit varying patterns of phoneme misunderstanding, making it challenging to generalize the selection of noise target phrases across different ASR systems. 
By randomly selecting noise-target phrases during inference, we ensure that the resulting noised sentences are not biased towards any specific ASR system. 
This allows downstream task models trained with our SNI data to simulate the diverse phonetic misunderstandings that can occur across different ASR systems, enhancing the robustness and generalizability of our approach in handling ASR-induced errors in real-world scenarios.

Then our next step is noise phrase generation, which aims to generate noise phrase $W^{\prime} \in T$ given noise target phrase $W  \subset X$ modeled as follows:
\begin{equation}
    w^{\prime}_i = argmax P(V|W, w^{\prime}_1, ... w^{\prime}_{i-1}).
\end{equation}
Generating noise phrases given only selected noise target phrases, our SNI model focuses on generating ASR-like sentences and does not require heuristic filtering in previous works.



%Specifically, we propose to fractionize SNI into more fine-grained mapping $f:W \rightarrow W^{\prime}$ between the noise target phrases and the noised phrases. 

%We design an end-to-end architecture consisting of an encoder, a decoder, and an operation predictor to constrain the decoding process to the desired part of the input sequence.  
%The encoder produces sequence embeddings from the word embeddings of the ASR output texts and related positional embeddings.  
%The operation predictor is a fully-connected layer trained to identify the above-mentioned“K”, “D” and “C” input sequence embeddings.  
%The model can reduce inference latency significantly by restricting the decoding process to the “C” tokens

%For the change position, the transformed-based decoder inputs at timestep t are calculated as follows: \begin{equation}
%    Eyt,k=Wp[(WE(wyt,k) + PE(wyt,k))exk], 
%\end{equation}
%where $WE$ and $PE$ are the same word and position embedding functions as in equation.
%$exk$ is the encoded token representation mentioned before. 
%$Wp$ is the trainable parameters.
%Then, a standard transformer decoder is employed to fuse all relevant information:
%\begin{align}
%    hkt+1= TransformerDecoder(Q,K,V),\\
%    Q=Eyt,k,K=Ex,V=Ex,
%\end{align}
%where  the decoder  input $Eyt,k$ works  as query (“Q”),  and  encoded model input $Ex$ works as key (“K”) and value (“V”) in the transformer decoder.
%$hkt+1$ is the fused vector.
%Finally, the target output is predicted as follows:
%\begin{equation}
%    p(ˆωyt+1,k) = softmax(Wyhkt+1+by), 
%\end{equation}
%where $Wy$ and $by$ are trained parameters.   
%Then, generation loss is defined as followed:
%\begin{equation}
%   lossdec=tlog(p(ˆωyt,k)).
%\end{equation}

\end{comment}

==> backup/230720/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

~\input{table/dataset_statistics}

For training SNI model, we followed the settings from the previous work~\cite{noisygen}, which used to popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, DeepSpeech, and get recognized results. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2}, which models task-oriented dialogue systems with unstructured knowledge access.
The key reason for adopting DSTC10 Track2 dataset is that its sentences are the transcription of human-spoken task-oriented dialogue by an unknown ASR model.
Specifically, it includes three subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG).
In DSTC10 Tack 2 dataset, task-oriented dialogue systems are modeled as sequence of three subtasks.
First, determine whether the dialogue turn requires external knowledge access or not. 
Once determined to require external knowledge, then the second step is to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the whole knowledge base.
Finally, the response should be generated based on the dialogue context and the selected knowledge snippet. 
We choose DSTC10 Track2 dataset as it contains major tasks in NLP, classification and retrieval, generation as SLU.



\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

We followed settings for downstream task DSTC10 Track2 from previous works~\cite{dstc10_2, tian2021tod-da}.
We conducted SNI on the written form of each subtask dataset in a task-oriented dialogue system dataset and used the resulting noised sentence for training downstream models.
For the downstream task model, we followed the baseline model setting of DSTC10 Track2~\cite{dstc10_2} and trained GPT2-small on each subtask.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2}.



==> backup/230720/5_results.tex <==
\section{Results}
\input{table/dstc_result}
%We present the result on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
%The downstream model trained with our method outperformed baselines with a large margin in KS and RG subtasks and comparable results in KTD.
In this section, we first present the results of our proposed method for on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
Specifically, we report the results of all subtasks, the knowledge turn detection subtask and the knowledge selection, and response generation.
The results demonstrate the superiority of our approach in knowledge selection and response generation, while also achieving comparable performance in knowledge turn detection.

For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


In the response generation subtask, our method outperformed the baseline methods in every metric. 
However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
This indicates that our SNI method can better robustify the PLMs on generation task.


Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.

\input{table/asrglue_result}
Overall, our proposed method demonstrated superior performance in the knowledge selection and response generation subtasks of the task-oriented dialogue dataset. 
Additionally, it showcased competitive results in the knowledge turn detection subtask. 
These findings highlight the effectiveness of our approach in enhancing the capabilities of task-oriented dialogue systems and improving their performance in understanding user queries, selecting relevant knowledge, and generating appropriate responses.


==> backup/230720/6_conclusion.tex <==
\section{Conclusion}
In this paper, we first showed that among two ASR noise procedures, the misspelling step is generalizable between different ASR models while the phoneme misunderstanding does not.
Based on such findings, we proposed a new SNI method that formulated SNI as a constrained generation problem that fractionize SNI as a phrase-to-phrase problem.
From such formulation, we could attain an ASR-generalizable SNI model by randomizing noise target word selection and better supervising the noise word generation.

==> backup/230731/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
Trained in written language, PLMs may struggle to adapt to the differences in spoken language.
The main obstacle to such adaptation is the errors introduced by ASR systems.
ASR systems incorrectly transcribe the spoken language into phonetically similar but semantically different words.
PLMs struggle to understand semantics from such erroneous transcriptions.
The most effective and intuitive method to robustify PLMs for SLU is to expose PLMs to such erroneous transcriptions during training, for which we propose to augment the written language into pseudo transcription.
For such goal, pseudo transcription should contain the errors which diverse ASR systems would make in practice.
Unless, the robustness of the trained PLMs would not be generalizable to individual ASR system.
Therefore, motivated by do-calculus, we first propose to intervene in the augmentation for diversity adopting constrained generation.
For plausibility, we propose to correct the augmentation based on the phonetic information with which the ASR systems transcribe.
The proposed approaches result in the diversity and plausibility of the pseudo transcription and improve the robustness and generalizability of SLU models.
Experimental results and analysis are provided to support the effectiveness of our proposed methods.
\end{abstract}

==> backup/230731/1_intro.tex <==
\section{Introduction}
Starting from ELMo~\cite{peters-etal-2018-deep} to recent GPT4~\cite{openai2023gpt4}, pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription  is fed into PLMs to conduct downstream SLU tasks. 


%As PLMs are trained in the different modality of written text, they suffer to adapt to the difference between the transcription and text.
%이 문단에서 하고 싶은 말 ASR error의 특징 : phonetically similar but semantically different + PLMs cannot understand semantics from noised input
As ASR systems incorrectly transcribe the speech into phonetically similar but wrong words~\cite{ruan20_interspeech,9054689}, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
Pronounced similarly, the ASR systems struggle to accurately distinguish phonetically similar words from speech such as wait and weight in Fig.~\ref{fig:example}.
Confusing such words, the ASR systems fail to distinguish them and generate incorrect transcription containing phonetically similar words, ASR error words, instead of the correct words~\cite{ruan20_interspeech,9054689}.
For example, confusing between wait and weight, cereal and serial, the ASR systems generate incorrect transcription of ``I cannot weight to eat serieal''  as depicted in Fig.~\ref{fig:example}.
In contrast to the similarity in pronunciation, the semantics of ASR error words differ from the correct words, thus, it is hard to understand the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.


%데이터
%학습시 aSR error 노출시키면 robust 가능, 그래서 asr error augmentation, SNI 할거
However, PLMs can be robustified if they are trained with incorrect transcription~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}, for which the data augmentation method of converting the written sentence into pseudo transcription containing ASR errors, speech noise injection (SNI), has been introduced.
Though training PLMs with incorrection transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
An SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
SNI aims to reduce  human annotation of recording and transcribing in collecting SLU corpora by generating pseudo transcription.
Specifically, given the written sentence, SNI mimics the confusion of the ASR systems and corrupts the words in the written sentence with ASR-plausible error words which are phonetically similar.

\input{figure_latex/figure1}
%여기는 previous SNI 들이 다 ASR specific 하다는 내용 위주로 고치기.
%Previous works in SNI can be categorized into two methods. 
%The most intuitive method is the TTS-ASR pipeline, where the TTS engine (text-to-speech) converts the text into audio, and the ASR system transcribes the audio.
%While ASR errors are generated by TTS engines and ASR systems, they are both computationally expensive.
%Additionally, they cannot generate sufficient ASR errors as the noise engaged during human reading does not exist in the audio converted by TTS.
%In contrast, generative SNI supervises the autoregressive language model $M$ to generate the pseudo-ASR given the text as the following:
%\begin{equation}
%    X^{\prime} = M(X)
%\end{equation}
%As generative SNI is shown to be effective in various situations~\cite{asrglue}, we focus on generative SNI.
%이 문단에서  하교 싶은 얘기 ASR generalizble 하려면 어떻게 ASR error 를 만들어야 하나
In order for the PLM trained with pseudo transcription to be generally used with different ASR systems, they should be trained on pseudo transcription containing diverse ASR-plausible error words~\cite{7178796}.
%However, previous works in SNI follow the individual ASR system and cannot generate such diverse ASR-plausible error words.
Due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to follow the error distribution of an individual ASR system.
As a result, only the phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
Such bias even degrades the plausibility of the resulting pseudo transcription when SNI model is blinded to the phonetic information
For example, as depicted in Fig.~\ref{fig:example}, following the incorrect transcription of the ASR system on `c' to `s' such as `cereal' to `serial' and `cease' to `sees', SNI is biased to corrupt the words containing `c' while leaving the words with `w'.
Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-unplausible error words. 

%While many previous works studied SNI~\cite{feng22c_interspeech, noisygen}, ASR-generalizability, the ability of an SLU model to perform robustly across different ASR systems, is not well studied for SNI.
%Such generalizability has been focused on diverse SLU tasks as different ASR systems can be used in SLU pipeline~\cite{blackbox1}.
%ASR-generalizability has been important as different ASR systems have distinct error distributions and SLU trained on one error distribution suffers to generalize on different error distribution.
%However, previous works in SNI confirmed their effectiveness using identical ASR systems for both SNI and downstream tasks, where the ASR generalizability still remains unveiled~\cite{noisygen,tts_asr}.
%We argue that ASR-generalizability is also crucial in SNI as the resulting pseudo-ASR would follow the error distribution of an individual ASR system.


%Toward ASR generalizable SNI, we first propose to intervene SNI process based on do-calculus~\cite{glymour2016causal} so that the resulting pseudo-ASR would not follow the error distribution of an individual ASR system. 
In order to increase the diversity of the ASR-plausible error words, we first propose to intervene SNI based on do-calculus~\cite{glymour2016causal}.
Adopting Do-calculus in SNI enables such diversification by cutting off the probability to corrupt the frequently incorrectly transcribed phonemes and increasing such probability of the other phonemes as contrasted by $P(z|x_i)$ and $P(z)$ in Fig~\ref{fig:example}. 
%Adopting Do-calculus in SNI enables such diversification by intervening in the corruption of the phonemes so that infrequently corrupted phonemes are more corrupted while frequently corrupted phonemes are less corrupted. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-plausible error words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to ASR-plausible errors by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as 'wait` and 'cue` as depicted in Fig.~\ref{fig:example} as a result of such diversification.
%factorize the generation of ASR errors into two distinct steps: phonetic misunderstanding and misspelling.
%For such goal, we train SNI model to generate the ASR-noised words constrained on its written words, the noise target words.
%Previous works supervised SNI model to maximize the likelihood of the entire ASR transcription given its written sentence~\cite{asrglue, noisygen}.
%
%During such supervision, the SNI model is biased to select the noise target words following the error distribution of the ASR system adopted for training.
%Thus, the resulting pseudo-ASR would contain biased ASR errors, such as containing errors for specific phonemes.
%As a result, we intervene in the choice of the word to corrupt so that diverse phonemes can be corrupted.
%implemen the intervention in SNI by factorizing it into the two processes of noise word selection and noise word generation.
%In the noise word selection, the noise target word, the word to be corrupted in the pseudo-ASR, is randomly selected without bias. Then, by constraining the noise target word, a phonetically similar ASR noise word is generated.
%As the bias from the ASR system is removed, the resulting pseudo-ASR contains diverse ASR errors and can robustify the downstream model against the diverse ASR systems.
%In contrast, our SNI model randomly selects the noise target words. 
%This random selection serves as an intervention to the error distribution of the ASR system and debias the resulting pseudo-ASR to diversify the error distribution.
%Trained on the pseudo-ASR with more diverse ASR errors, downstream task models can more robustly conduct downstream tasks.
%As a result
%, similar to interventions performed in do-calculus, where we actively modify the values of certain variables to observe the effects on the overall system.
%By randomly selecting the words, we remove the bias associated with specific ASR systems and ensure a more diverse set of corrupted words.

Our second contribution to increase the plausibility of ASR plausible error words is to correct the generation of phonetically different ASR plausible error words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as 'choir` to 'quire`.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting 'c`  to 's`.
Fed only the words, not their phonetic information, previous SNI models confuse 'c` in the word 'cue` to be pronounced as 's` and generate the unplausible ASR error word 'sue`.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that 'c` is pronounced as phoneme 'k`, our SNI model corrupts into the phonetically similar ASR-plausible error word 'queue`.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-plausible.

%In addition to intervention in the error distribution, we propose to correct the generation of ASR noise words using phonetic information. 
%While ASR systems generate phonetically similar words as ASR error words, SNI models are optimized to maximize the likelihood of the grapheme-based tokens corresponding to ASR error words.
%Blinded to phonetic similarity, the existing SNI model fails to generate phonetically similar pseudo-ASR and requires additional phonetic similarity based heuristic to filter out such failing pseudo-ASR.
%Instead of such heuristic, we propose to supervise and incorporate phonetic similarity to correct the noise word generation.
%Specifically, we propose a phoneme head, another language model head that generates ASR noise words based on their phonemes.
%This phoneme head is used with trivial language model head of SNI models and ensures to generate the phonetically similar ASR error words.

%Powerful generation models of ten meet most of the task requirements, yet miss a few (e.g.,omittinga subset of keywords), or generate incorrect hypotheses that nevertheless provide useful structure (e.g.,a correct problem solving strategy with a missing step). However, after generatingevenaslightlysub-optimalsequence,thesingle-passparadigmrequiresmodelsto“startfrom scratch”,effectivelydiscardingworkalreadydone.Amorenatural,intuitiveapproachisleveraging thegenerationasausefulstartingpointtorefineintoahigherqualityoutput.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of phonetically different ASR noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

\begin{comment}
In the phonetic misunderstanding step, the ASR system misinterprets the spoken phonemes, leading to inaccuracies in the resulting transcription. 
Consequently, the subsequent step, misspelling, arises as a result of the ASR system generating misspelled words based on its flawed understanding of the original speech. 
Misspelling errors occur when the ASR system incorrectly converts the misunderstood phonemes into different characters, further deviating from the intended transcription. 

\input{table/asr_cer}

Among two distinct steps, we argue that  
while the phonetic misunderstanding is ASR-specific noise, the misspelling step is ASR-generalizable.
Specifically, phonetic misunderstanding can be largely influenced by training data and acoustic modeling.
For example, ASR systems with distinct acoustic feature extractors and different accented training audio would exhibit distinct susceptibility to phonetic misunderstanding.
In contrast, we argue that the phenomenon of misspelling is more ASR-generalizable. 
This is because a language possesses specific spelling conventions that are shared across different ASR models regardless of training data or acoustic modeling techniques. 

To demonstrate the generalizability of misspelling errors among ASR models, we present the Character Error Rate (CER) between different open-source ASR models, DeepSpeech and Leopard, and ground-truth transcription in Table~\ref{tab:cer}. 
In Table~\ref{tab:cer}, we observe that the CER values for the different ASR models are smaller than that of each ASR model and ground-truth transcription. 
This indicates that, despite the differences in model-specific factors, the misspelling errors generated by these models are more similar to each other than ground-truth transcription.

Toward ASR-generalizable SNI, we consider alignable characteristics of the ASR-error words.
That is, the words in the ground-truth text can be easily aligned to their corresponding words in ASR transcription.
When the words are correctly transcribed, the words in the ASR and its ground-truth text would be easily aligned.
However, such alignment is not limited to the correctly transcribed words.
As ASR systems misspell the words of the ground-truth text into phonetically, also graphemically, similar words, even inaccurately transcribed words can be easily aligned to their corresponding words.

Considering such alignment, we propose to break down SNI from generating entire pseudo-ASR transcription $X^{\prime}$ given written text $X$ into the finer-grained generation of ASR error words $w^{\prime}\in X^{\prime}$ given written word $w \in X$ adopting constrained generation which can be formulated as follows:
\begin{equation}
    w^{\prime} = M(w)
\end{equation}
Directly conditioned on the cleanly written word $w$, not the entire text $X$, such fine-grained SNI can better supervise the SNI model of how the written words $w$ are corrupted to ASR error words $w^{\prime}$ by misspelling. 
By better supervising misspelling with fine-grained SNI, we enhance its ability to generalize across different ASR systems, as ASR misspelling is generalizable to different written words, regardless of the ASR systems.

In addition to misspellings, fine-grained SNI can also contribute to a more ASR-generalizable approach in the context of phoneme misunderstanding.
In previous generative SNI, whether the cleanly written word $w$ would be corrupted is implicitly determined by SNI model $M$.
Biased by the phoneme misunderstanding pattern of the ASR system used to transcribe the training set, the SNI model tends to corrupt only the words that the specific ASR system would phonetically misunderstand.
Compared to sentence-level SNI, our word-level SNI gives more control in selecting which words to corrupt to ASR error words.
For ASR-generalizable SNI, we propose to randomly select the words to corrupt, so that the resulting pseudo-ASRs would contain diverse ASR-error words.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose a word-level SNI approach adopting constrained generation
2) propose a random word selection in the proposed word-level SNI 
and 3) show that the proposed word-level SNI improves the ASR-generalizability of downstream models.




%factorize the two distinct steps involved in ASR errors: phonetic misunderstanding and misspelling. 
%By doing so, we isolate the phonetic misunderstanding step where the ASR system misinterprets the spoken phonemes, and the subsequent misspelling step where it generates incorrect spellings based on the misunderstood speech.
%In contrast to previous approaches that treat SNI as a unified sequence-to-sequence generation task, our proposed constrained generation method allows us to focus solely on regenerating the ASR-noised words, while preserving the original written words. 
%This factorization enables us to address each step independently and develop targeted strategies to mitigate phonetic misunderstanding and improve the accuracy of misspelling generation.
%By adopting constrained generation and explicitly considering the phonetic misunderstanding and misspelling steps, our approach offers a novel perspective and potential advancements in the field of ASR-generalizable SNI. 
%It allows for more fine-grained control and targeted interventions, ultimately leading to improved performance and robustness in the generation of ASR-corrupted data.

\end{comment}


==> backup/230731/2_prelim.tex <==
\section{Preliminaries}
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into a pseudo transcription.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo transcription, $T=\{t_{i}\}_{i=1}^{n}$.
Then, the resulting pseudo transcription, $T$, is used to train downstream models.
Trained on pseudo transcription $T$ containing ASR plausible errors, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
%\subsubsection{Robustness }
%In recent years, large-scale PLMs have demonstrated remarkable performance in Natural Language Understanding (NLU) tasks~\cite{openai2023gpt4}. 
%To evaluate their robustness, several studies have employed human-crafted adversarial examples or generated examples through adversarial attacks~\cite{wang2021adversarial}. 
%Another approach involves projecting input data into a latent space using Generative Adversarial Networks and then retrieving adversaries that closely resemble the original instance in the latent space~\cite{zhao2017generating}.
%Additionally, controlled paraphrase networks are proposed to generate syntactically adversarial examples~\cite{iyyer2018adversarial}. 
%These examples not only deceive PLMs but also enhance their resilience to syntactic variations when used for training data augmentation. 
%However, the extent to which PLMs exhibit robustness against ASR errors in real-world conditions has been under-explored.
\subsubsection{SNI}

Previous works pointed out that the key distinction of the incorrect transcription $t_{i^{\prime}}\in T$ from different noise is phonetically similar to its written word $x_{i}\in X$~\cite{9721159, asrglue, tian2021tod-da}.
Specifically, each word $t_{i}\in T$ would be either identical or different to its corresponding written word $x_{i}\in X$.
When the word $t_i$ is different from the written word $x_i$,  the ASR error word $t_i$ is phonetically similar to the written word $x_i$.
Therefore, previous works proposed various methods to generate the pseudo transcription containing the ASR plausible error word $t_i$ which is phonetically similar to the written word $x_i$.
Previously proposed methods can be summarized as 3 categories of TTS-ASR pipeline and textual perturbation, auto-regressive generation.

The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio. 
During the conversion between the text and audio, the written word $x_i$ is expected to be corrupted into the ASR plausible error word $t_i$.
However, due to different error distribution between the human recording and the audio generated by TTS,  the resulting pseudo transcription would have different
error distribution from the ASR transcription~\cite{asrglue}.
 In addition, the exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora. 




Another category of SNI is textual perturbation which generates the pseudo transcription $T$ by replacing words $x_i \in X$ to its phonetically similar word $t_i$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, phonetically similar word $t_i$ is determined as the word which is  phonetically similar to the word $x_i$ as followed:
\begin{equation}
   t_{i^{\prime}} = argmax_{w \in W} P(W|x_{i}),
\end{equation}
where $P(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $P(W|x_{i})$. 
Specifically, $P(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo transcription efficiently, they cannot generate diverse ASR plausible error words as $P(W|x_{i})$ is pre-defined.

The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to
implement~\cite{asrglue,noisygen}. 
Specifically, the auto-regressive PLMs such as GPT-2 or BART is supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.
We argue that the pseudo-ASR generated by auto-regressive generation is not generalizable across the different ASR systems.
That is, during such supervision, the SNI model is biased to follow the error distribution of the ASR system and cannot generate diverse ASR plausible errors. 




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F^{-1} T \rightarrow X$ of converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which generates the written words constrained on the ASR noise words was proposed~\cite{constdecoder}
However, due to the innate robustness of PLMs against to noises~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

==> backup/230731/3_ours.tex <==
\section{Ours}
We now propose our SNI model, which aims to generate pseudo-ASR which is not biased toward an individual ASR system and robustifies downstream task models against diverse ASR errors.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method for ASR generalizable SNI is to intervene in the SNI so that the resulting pseudo transcriptions contain the ASR plausible error words of diverse phonemes.
For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted or not in the resulting pseudo transcript.
Using the variable $z_i$, the SNI process can be written as follows:
\begin{equation}
     P(t_{i^{\prime}}|x_{i}) = \sum_{z_{i}}P(t_{i}|x_{i})\cdot P(z_{i}|x_{i}).
     \label{eq:sni_definition}
\end{equation}
An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
Therefore, the SNI model following such an ASR system would have a similar distribution of $P(z_{i}|x_{i})$.
%It is widely known that an ASR system is biased to make errors on certain phonemes more frequently and training settings such as training data can cause such error distribution~\cite{feng2021quantifying}.
%As a result of such biased error distribution of the ASR system, SNI models supervised to mimic ASR errors are also vulnerable to generating pseudo-ASR following such biased error distribution.

%We blame such bias on the noise word selection process in SNI, where the word to corrupt is chosen.
%Let us consider whether the word $x_{i}\in X$ is corrupted or not in pseudo-ASR $T$ as the variable $z_i$.
%Then, the SNI process can be written as follows:
%\begin{equation}
%     P(t_{i^{\prime}}|x_{i}) = \sum_{z_{i}}P(t_{i^{\prime}}|x_{i})\cdot P(z_{i}|x_{i}).
%\end{equation}
%Trained to mimic ASR error of specific ASR error system, the SNI model would have biased noise word selection probability for different phonemes, $P(z|x_{i})$.
%That is, the SNI model would be biased to corrupt the words $x_{i}$ which is frequently corrupted by the ASR system used for training the SNI model.
%Specifically, we observed that the noisygen model tends to make more errors on the phonemes, such as S and R, while rarely corrupting the phonemes IH0 and AA1 following ASR system used for training.

In order to generate ASR generalizable pseudo transcription, we propose to intervene $z_i$.
Intervening $z_i$, we aim to manipulate $P(z_{i}|x_{i})$ so that $P(z_{i}|x_{i})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
As a result of such manipulation, resulting pseudo transcription would contain more diverse ASR-plausible errors.
Specifically, we remove any influence from the intervened variable, $x_{i}$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{align}
    P(t_{i^{\prime}}|do(x_{i})) &= \sum_{z}P(t_{i}, z|x_{i})\\
                                &= \sum_{z}P(t_{i}|x_{i},z) \cdot P(z|do(x_{i}))\\
                                &= \sum_{z}P(t_{i}|x_{i},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
To implement Eq.~\ref{eq:do-calculus}, we propose to conduct such determination explicitly. 
Specifically, for each word $x_i$, we sample random variable $d_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, we decide whether the word $x_{i}$ will be corrupted, which is determined as the value of $z_i$ as follows:
\begin{align}
    z_i = 
    \begin{cases}
        1, \quad \text{if} \quad d_i \leq P(z) \\
        0, \quad \text{else}
    \end{cases}
    \label{eq:random_selection}
\end{align}
where the word $x_{i}$ will be corrupted if $z$ is set to 1 or not if $z$ is set to 0.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

When $x_{i}$ is determined to be corrupted, the ASR plausible error word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t_{i}|x_{i},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t_{i} \in T$ is phonetically similar to its cleanly written form $x_{i} in X$.
Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$
Specifically, if $z$ is set to 0, $t_{i}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, we constrain the generation of the ASR noise word $t_{i}$ to $x_{i}$ so that the generated ASR noise word $t_{i}$ is phonetically similar to the cleanly written word $x_{i}$.
Replacing $x_{i}$ to the generated ASR noise word $t_{i}$, $X$ is corrupted into pseudo-ASR $T$.

To generate pseudo transcription $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the ASR plausible error word $t_{i}$ constrained on the written word $x_i$.
Specifically, the encoder representation of the written word $e^{encoder}_{i}$ and the special embedding vector $BOS$ representing the begin of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E^{decoder}_{i}=W_{d}[e^{encoder}_{i}; BOS],
    \label{eq:decoder_input}
\end{equation}
where  $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate ASR plausible error word $t_i$ from the inputs and outputs the hidden representation $h^{k}_{i}$ as follows:
\begin{align}
    h_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder}_{i},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution of ASR plausible error word $t_i$ is predicted as follows:
\begin{equation}
    P_{gen}(\hat{t}_{i}) = softmax(WE \cdot h_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

In training, we used the ASR transcription $T$.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t_{i}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(t_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method for ASR generalizable SNI is to correct the phonetically differently generated ASR noise word considering the phonetic similarity.
Pure text-based generation lacks useful information like pronunciation and prosody~\cite{wang2022building} and results in phonetically different pseudo-ASR, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
Thus, we propose to evaluate phonetic similarity-based generation probability $P_{phoneme}(\hat{t}_{i})$ and correct the generation probability in Eq.~\ref{eq:gen_prob} so that the phonetically similar ASR noise words can be generated as followed:
\begin{equation}
    P_{correct}(\hat{t}_{i}) = P_{gen}(\hat{t}_{i}) \cdot P_{phoneme}(\hat{t}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


The main difficulty in the generation of phonetically similar ASR noise words is that PLMs are supervised to understand semantic context, not phonetic information.
Thus, their input, word embedding, lacks phonetic information.
Our first proposal to generate phonetically similar ASR noise words is to provide phonetic information using phoneme embedding $PHE$.
The phoneme embedding $PHE$ aims to deliver the phonetic information of tokens in the vocabulary.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
%The phoneme embedding is fed to the decoder similar to the encoder as follows:
%\begin{multline}
%    E^{decoder}_{i,k}=W_{d}[e^{encoder}_{i};  \lambda_{w}\cdot WE(X)+\lambda_{p}\cdot PHE(X) \\+ PE(D^{k}_{i})].
%\end{multline}
The input for decoder is formulated similar to Eq.~\ref{eq:decoder_input}

Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(\hat{t}_{i}) = softmax(PHE \cdot h_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob},  $P_{phoneme}(\hat{t}_{i})$ can evaluate the generation probability based on the phonetic information.

Without proper supervision of the phonetic information, $P_{phoneme}(\hat{t}_{i}$ cannot correct the generation of the phonetically different ASR noise words.
For the supervision of the phonetic information, we propose to distill the phonetic information from the phonetic edit distance~\cite{9662078}.
The phoneme edit distance measures the similarity between the given two words $w_i$ and $w_j$ by two consecutive steps.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}

In order to correct the generation probability as in Eq.~\ref{eq:phoneme_correction_prob}, the phonetic information should be evaluated as the probability distribution. 
For such purpose, we convert the phoneme edit distance to the phoneme probability distribution $R(\hat{t}_{i})$, which will be used as the label for $P_{phoneme}(\hat{t}_{i})$.
First, the phoneme edit distance is converted into the phoneme similarity score $PS$ which is defined as follows
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.
For the ground-truth ASR error word, $t_{i}$, the phoneme probability distribution $R(\hat{t}_{i})$ is evaluated for each token $w$ in vocabulary as followed:
\begin{equation}
    R(\hat{t}_{i}) = \frac{PS(t_{i},w)}{\sum_{w^{\prime}\in W}PS(t_{i},w^{\prime} )}.
 \end{equation}
 The phoneme probability distribution  $R(\hat{t}_{i})$ is used as a label to supervise the phoneme information to evaluate loss as followed:
 \begin{equation}
     l_p = KLD(P_{phoneme}(\hat{t}_{i}),  R(\hat{t}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(\hat{t}_{i})$ can correct the generation of the phonetically different words.
 

 




==> backup/230731/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset.
DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG), where human responses are ASR transcription generated from an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it requires ASR generalizability as transcriptions of human responses are generated by unknown ASR and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the famous NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which DSTC10 Track2 dataset does not contain.




\input{table/dstc_result}
\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset.


As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
To show ASR generalizability of our proposed methods, we adopt both task-agnostic and specific baselines.
Our main task-agnostic baseline which we used for both DSTC Track 2 dataset and ASR GLUE benchmark is Noisy-Gen, the SNI model of auto-regressive generation.
Noisy-Gen and ours used identical ASR transcriptions for training.
We adopt task-specific baselines which were proven to improve the robustness against ASR errors in each task.
For DSTC10 Track2 dataset, we adopt TOD-DA~\cite{tian2021tod-da}, SNI method based on both the TTS-ASR pipeline and textual perturbation.
For ASR GLUE dataset, we adopt GPT2 based SNI model similar to Noisy-Gen provided by ASR GLUE benchmark which we call Noisy-Gen (Kaldi).
Training set for Noisy-Gen (Kaldi) is constructed by transcribing the libriSpeech corpus with Kaldi based ASR system.
Compared to Noisy-Gen, Noisy-Gen (Kaldi) is trained with smaller corpus but used identical ASR system to transcribe the test set.







==> backup/230731/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme correction robustify the downstream task models on ASR errors? 


\noindent \textbf{RQ2:}Does our proposed interventional SNI and phoneme correction increase ASR generalizability?



\subsection{RQ1: Effectiveness of our proposed methods on robustifying downstream SLU tasks.}
In this section, we show the effectiveness of our proposed methods in robustifying downstream SLU tasks.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines without ASR generalizability struggle to robustify against ASR errors generated by unknown ASR system, showing R@1 score below 60.
In contrast to the observations made by adopting an identical ASR system for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
This result shows that pseudo transcription following individual ASR system struggles to robustify against ASR errors generated by unknown ASR systems.
In contrast, ours outperforms baselines in every metric in KS with a large margin, showing that ours can robustify against ASR errors made by unknown ASR system.

Results in Table~\ref{tab:dstc_results} shows that robustification of our proposed methods is not limited in KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed 
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.

To confirm that our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methdos in turn.
We report the result without the phoneme correction in fouth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme correction showed the decreased score in every subtasks, showing that the importance of ASR plausibility of psuedo transcription to robustify against ASR errors.


\input{table/asrglue_result}
To conduct the ablation on the intervention itself, we trained constrained decoding based SNI model without do-calculus based random corruption as in Eq.~\ref{eq:random_selection}.
Specifically, as constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x_i$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z_i|x_i)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of the Table~\ref{tab:dstc_results}. 
Decreased performance of last row shows that intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.


\subsection{RQ2: ASR generalizability of our proposed methods. }

Then, we now study ASR generalizability of our proposed methods with ASR GLUE benchmark.
We report the results on ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
First, we show that autoregressive generation based SNI models are not generalizable across ASR systems.
For such purpose, we compare Noisy-Gen and Noisy-Gen (Kaldi).
While Noisy-Gen used larger training corpus, Noisy-Gen (Kaldi) outperformed Noisy-Gen in every tasks.
Interestingly, in QNLI, accuracy of Noisy-Gen (Kaldi) in high noise level was highger than that of Nosiy-Gen in medium noise level.
This result shows that autoregressive generation based SNI models struggles to generalize across the ASR errors.

In contrast, ours showed comparable results to Noisy-Gen (Kaldi), even though we used different ASR system to construct training set of SNI models.
Specifically, ours outperformed Noisy-Gen (Kaldi) in QNLI of high and medium noise level and in SST of low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtasks.
These results shows that our proposed methods can generate pseudo transcription which can generalize across different ASR systems.


==> backup/230731/6_conclusion.tex <==
\section{Conclusion}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.



==> backup/230804/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
Trained in written language, PLMs may struggle to adapt to the differences in spoken language.
ASR systems incorrectly transcribe the spoken language into phonetically similar but semantically different words.
The most effective and intuitive method to robustify PLMs for SLU is to expose PLMs to such erroneous transcriptions during training, for which we propose to augment the written language into pseudo transcription.
For such goal, pseudo transcription should cover the errors which diverse ASR systems would make in practice.
%Unless, the robustness of the trained PLMs would not be generalizable to individual ASR system.
Therefore, we  propose a causal perspective that utilizes do-calculus and intervenes in the augmentation for diversity adopting constrained generation.
For plausibility, we propose to correct the augmentation based on the phonetic information with which the ASR systems transcribe.
The proposed approaches result in the diversity and plausibility of the pseudo transcription and improve the robustness and generalizability of SLU models.
Experimental results and analysis show the effectiveness of our proposed methods.
\end{abstract}

==> backup/230804/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 




As ASR systems incorrectly transcribe the speech into phonetically similar but wrong words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', the ASR systems generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
In contrast to the similarity in pronunciation, the semantics of ASR error words differ from the correct words, thus, it is hard to understand the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce the additional annotation of recording and transcription, the data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be corrupted as noise words in the pseudo transcription, which ASR systems would probably confuse the ground-truth word into, due to the phonetic similarity.  

\input{figure_latex/figure1}
In order for the PLM trained to be generally used with different ASR systems, noise words in the pseudo transcription should be diverse and ASR probable~\cite{7178796}.
That is, ASR systems have different error distributions, such as phoneme or accents~\cite{different_error_distribution}.
For example, different from ASR 1 of corrupting `c' to `s', ASR 2 would confuse `r' and generate the error word `walkers' instead of the correct word `workers'.
Due to the difference in errors, PLMs robust against ASR 1 would be fragile to the errors made by ASR 2.

However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to follow the error distribution of an individual ASR system.
Such bias results in the following two problems: 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
To show such bias explicitly, we introduce the variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



To overcome, we propose Interventional Speech Noise Injection (ISNI). For the narrowed noise problem,
We propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the frequently corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as 'reading` and 'cue` as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to make noise words more ASR probable, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of ASR improbable noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.



==> backup/230804/2_prelim.tex <==
\section{Preliminaries}
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into a pseudo transcription.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo transcription, $T=\{t_{i}\}_{i=1}^{n}$.
Then, the resulting pseudo transcription, $T$, is used to train downstream models.
Trained on pseudo transcription $T$ containing noise words, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
%\subsubsection{Robustness }
%In recent years, large-scale PLMs have demonstrated remarkable performance in Natural Language Understanding (NLU) tasks~\cite{openai2023gpt4}. 
%To evaluate their robustness, several studies have employed human-crafted adversarial examples or generated examples through adversarial attacks~\cite{wang2021adversarial}. 
%Another approach involves projecting input data into a latent space using Generative Adversarial Networks and then retrieving adversaries that closely resemble the original instance in the latent space~\cite{zhao2017generating}.
%Additionally, controlled paraphrase networks are proposed to generate syntactically adversarial examples~\cite{iyyer2018adversarial}. 
%These examples not only deceive PLMs but also enhance their resilience to syntactic variations when used for training data augmentation. 
%However, the extent to which PLMs exhibit robustness against ASR errors in real-world conditions has been under-explored.
\subsubsection{SNI}

%Previous works pointed out that the key distinction of the incorrect transcription $t_{i^{\prime}}\in T$ from different noise is phonetically similar to its written word $x_{i}\in X$~\cite{9721159, asrglue, tian2021tod-da}.
%Specifically, each word $t_{i}\in T$ would be either identical or different to its corresponding written word $x_{i}\in X$.
%When the ASR system incorrectly transcribed the word $t_i$, the error word $t_i$ is different but phonetically similar to the written word $x_i$.
%Therefore, previous works proposed various methods to generate the pseudo transcription containing the ASR probable error word $t_i$ which is phonetically similar to the written word $x_i$.
Previously proposed methods can be summarized as 3 categories of TTS-ASR pipeline and textual perturbation, auto-regressive generation, which differs in how to generate the noise word $t_i$ of the word $x_i$.

The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio. 
During the conversion between the text and audio, the written word $x_i$ is expected to be corrupted into the ASR probable noise word $t_i$.
However, due to different error distribution between the human recording and the audio generated by TTS, the resulting pseudo transcription would have different error distribution from the ASR transcription~\cite{asrglue}.
 In addition, the exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora. 




Another category of SNI is textual perturbation which generates the pseudo transcription $T$ by replacing words $x_i \in X$ to its phonetically similar noise word $t_i$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, the noise word $t_i$ is determined as the word which is phonetically similar to the word $x_i$ as followed:
\begin{equation}
   t_{i} = argmax_{w \in W} S(W|x_{i}),
\end{equation}
where $S(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $S(W|x_{i})$. 
Specifically, $S(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo transcription efficiently, they cannot generate diverse error words as $S(W|x_{i})$ is pre-defined.

The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to
implement~\cite{asrglue,noisygen}. 
Specifically, the auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.
We argue that auto-regressive generation suffers from narrow noise problem and ASR improbable noise problem due to following individual ASR system.




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F$, $F^{-1} : T \rightarrow X$, converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which generates the written words constrained on the ASR noise words was proposed~\cite{constdecoder}
However, due to the innate robustness of PLMs against to errors~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

\subsubsection{Do-calculus}
Do-calculus aims to understand the causal effect of variable $X$ on another variable $Y$ more robustly.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
That is, when a specific value of $X$ is strongly correlated to $z$ and has large $P(z|X)$, resulting $P(Y|X)$ would be influenced by the value of $P(Y|X,z)$, even when the other value of $X$ would have different $P(Y|X,z)$.
Do-calculus removes such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no more influenced by $X$, thus influence of $X$ on $Y$ through the mediator $z$ is removed.



==> backup/230804/3_ours.tex <==
\section{Methods}
We now propose our SNI model, which aims to generate pseudo transcription containing diverse and ASR probable noises resolving narrow noise problem and ASR improbable noise problem.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method to remedy the narrowed noise problem is to intervene in the SNI so that the resulting pseudo transcriptions contain the noise words of diverse phonemes.
For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Using the variable $z_i$, the SNI process can be written as follows:
\begin{equation}
     P(t_{i}|x_{i}) = \sum_{z_{i}}P(t_{i}|x_{i},z_{i})\cdot P(z_{i}|x_{i}).
     \label{eq:sni_definition}
\end{equation}
An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


In order to generate ASR generalizable pseudo transcription, we propose to intervene $z_i$.
Intervening $z_i$, we aim to manipulate $P(z_{i}|x_{i})$ so that $P(z_{i}|x_{i})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
As a result of such manipulation, resulting pseudo transcription would contain more diverse noise words.
Specifically, we remove any influence from the intervened variable, $x_{i}$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t_{i^{\prime}}|do(x_{i})) = \sum_{z}P(t_{i}|x_{i},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
To implement Eq.~\ref{eq:do-calculus}, we propose to conduct such determination explicitly. 
Specifically, for each word $x_i$, we sample random variable $d_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, the value of $z_i$ is determined as 1 if $d_i\leq P(z)$ else 0.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t_{i}|x_{i},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t_{i} \in T$ is phonetically similar to its cleanly written form $x_{i} \in X$.
Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$.
Specifically, if $z$ is set to 0, $t_{i}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, the noise word $t_{i}$ is generated under the constraint on $x_{i}$ so that the generated noise word $t_{i}$ is phonetically similar to the cleanly written word $x_{i}$.
Replacing $x_{i}$ to the generated noise word $t_{i}$, $X$ is corrupted into pseudo transcription $T$.

To generate pseudo transcription $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the noise word $t_{i}$ constrained on the written word $x_i$.
Specifically, the encoder representation of the written word $e^{encoder}_{i}$ and the special embedding vector $BOS$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E^{decoder}_{i}=W_{d}[e^{encoder}_{i}; BOS],
    \label{eq:decoder_input}
\end{equation}
where  $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate noise word $t_i$ from the inputs and outputs the hidden representation $h^{k}_{i}$ as follows:
\begin{align}
    h_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder}_{i},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution of noise word $t_i$ is predicted as follows:
\begin{equation}
    P_{gen}(\hat{t}_{i}) = softmax(WE \cdot h_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

For training our interventional SNI model, we used the ASR transcription $T$.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t_{i}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(t_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method is to make ASR improbable noise words more probable by correcting the noise word generation based on the phonetic information.
Toward our goal of more ASR probable noise words, we propose to correct the generation probability $P_{gen}(\hat{t}_{i})$ with the phoneme-based generation probability $P_{phoneme}(\hat{t}_{i})$ so that the ASR probable noise words can be generated as followed:
\begin{equation}
    P_{correct}(\hat{t}_{i}) = P_{gen}(\hat{t}_{i}) \cdot P_{phoneme}(\hat{t}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $P_{phoneme}(\hat{t}_{i})$ is to provide phonetic information via phoneme embedding $PHE$.
The main difficulty of evaluating $P_{phoneme}(\hat{t}_{i})$ is that PLMs are not aware of how the written sentences are pronounced.
%Conventional text generation is not aware of how the words are pronounced~\cite{wang2022building} and results in ASR improbable noise %words, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
%Thus, their input, word embedding, lacks phonetic information.
Our proposed phoneme embedding $PHE$ is designed to have the phonetic information of each token in the vocabulary.
Thus, feeding the phoneme embedding $PHE$ can deliver how each word in written sentences is pronounced.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(\hat{t}_{i}) = softmax(PHE \cdot h_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob}, $P_{phoneme}(\hat{t}_{i})$ can be evaluated based on the phonetic information.


Our second proposal for $P_{phoneme}(\hat{t}_{i})$ is to distill the phonetic information from phonetic similarity.
To generate ASR probable noise words, $P_{phoneme}(\hat{t}_{i})$ should evaluate how phonetically similar the words are to the $x_i$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $P_{phoneme}(\hat{t}_{i})$.
Specifically, phonetic similarity $PS$ is evaluated using the phoneme edit distance $PD$~\cite{9662078}.
The phoneme edit distance $PD$ measures the difference of the phonetic code between the given two words $w_i$ and $w_j$.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}
Then, phonetic similarity $PS$ can be defined as follows:
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.

To supervise $P_{phoneme}(\hat{t}_{i})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $R(\hat{t}_{i})$ as follows:
\begin{equation}
    R(\hat{t}_{i}) = \frac{PS(t_{i},w)}{\sum_{w^{\prime}\in W}PS(t_{i},w^{\prime} )}.
 \end{equation}
Then, $P_{phoneme}(\hat{t}_{i})$ is supervised by loss defined as follows:
 \begin{equation}
     l_p = KLD(P_{phoneme}(\hat{t}_{i}),  R(\hat{t}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(\hat{t}_{i})$ can correct the generation of ASR improbable words.
 

 




==> backup/230804/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\input{table/dstc_result}
As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset.
DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG), where human responses are ASR transcription generated from an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it requires ASR generalizability as transcriptions of human responses are generated by unknown ASR and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the famous NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.




\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset.


As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
To show ASR generalizability of our proposed methods, we adopt both task-agnostic and specific baselines.
Our main task-agnostic baseline which we used for both DSTC Track 2 dataset and ASR GLUE benchmark is Noisy-Gen, the SNI model of auto-regressive generation.
Noisy-Gen and ours used identical ASR transcriptions for training.
We adopt task-specific baselines which were proven to improve the robustness against ASR errors in each task.
For DSTC10 Track2 dataset, we adopt TOD-DA~\cite{tian2021tod-da}, SNI method based on both the TTS-ASR pipeline and textual perturbation.
For ASR GLUE dataset, we adopt GPT2 based SNI model similar to Noisy-Gen provided by ASR GLUE benchmark which we call Noisy-Gen (Kaldi).
Training set for Noisy-Gen (Kaldi) is constructed by transcribing the libriSpeech corpus with Kaldi based ASR system.
Compared to Noisy-Gen, Noisy-Gen (Kaldi) is trained with smaller corpus but used identical ASR system to transcribe the test set.







==> backup/230804/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme correction robustify the downstream task models on ASR errors? 


\noindent \textbf{RQ2:} Does our proposed interventional SNI and phoneme correction increase ASR generalizability?



\input{table/asrglue_result}
\subsection{RQ1: Effectiveness of our proposed methods on robustifying downstream SLU tasks.}
In this section, we show the effectiveness of our proposed methods in robustifying downstream SLU tasks.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines without ASR generalizability struggle to robustify against ASR errors generated by unknown ASR system, showing R@1 score below 60.
In contrast to the observations made by adopting an identical ASR system for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
This result shows that pseudo transcription following individual ASR system struggles to robustify against ASR errors generated by unknown ASR systems.
In contrast, ours outperforms baselines in every metric in KS with a large margin, showing that ours can robustify against ASR errors made by unknown ASR system.

Results in Table~\ref{tab:dstc_results} shows that robustification of our proposed methods is not limited in KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed 
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.

To confirm that our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methdos in turn.
We report the result without the phoneme correction in fouth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme correction showed the decreased score in every subtasks, showing that the importance of ASR plausibility of psuedo transcription to robustify against ASR errors.


To conduct the ablation on the intervention itself, we trained constrained decoding based SNI model without do-calculus based random corruption as in Eq.~\ref{eq:random_selection}.
Specifically, as constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x_i$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z_i|x_i)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of the Table~\ref{tab:dstc_results}. 
Decreased performance of last row shows that intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.


\subsection{RQ2: ASR generalizability of our proposed methods. }

Then, we now study ASR generalizability of our proposed methods with ASR GLUE benchmark.
We report the results on ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
First, we show that autoregressive generation based SNI models are not generalizable across ASR systems.
For such purpose, we compare Noisy-Gen and Noisy-Gen (Kaldi).
While Noisy-Gen used larger training corpus, Noisy-Gen (Kaldi) outperformed Noisy-Gen in every tasks.
Interestingly, in QNLI, accuracy of Noisy-Gen (Kaldi) in high noise level was highger than that of Nosiy-Gen in medium noise level.
This result shows that autoregressive generation based SNI models struggles to generalize across the ASR errors.

In contrast, ours showed comparable results to Noisy-Gen (Kaldi), even though we used different ASR system to construct training set of SNI models.
Specifically, ours outperformed Noisy-Gen (Kaldi) in QNLI of high and medium noise level and in SST of low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtasks.
These results shows that our proposed methods can generate pseudo transcription which can generalize across different ASR systems.


==> backup/230804/6_conclusion.tex <==
\section{Conclusion}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.



==> backup/230805/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
Trained in written language, PLMs may struggle to adapt to the differences in spoken language.
ASR systems incorrectly transcribe the spoken language into phonetically similar but semantically different words.
The most effective and intuitive method to robustify PLMs for SLU is to expose PLMs to such erroneous transcriptions during training, for which we propose to augment the written language into pseudo transcription.
For such goal, pseudo transcription should cover the errors which diverse ASR systems would make in practice.
%Unless, the robustness of the trained PLMs would not be generalizable to individual ASR system.
Therefore, we  propose a causal perspective that utilizes do-calculus and intervenes in the augmentation for diversity adopting constrained generation.
For plausibility, we propose to correct the augmentation based on the phonetic information with which the ASR systems transcribe.
The proposed approaches result in the diversity and plausibility of the pseudo transcription and improve the robustness and generalizability of SLU models.
Experimental results and analysis show the effectiveness of our proposed methods.
\end{abstract}

==> backup/230805/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', the ASR systems generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
In contrast to the similarity in pronunciation, the semantics of ASR error words differ from the correct words, thus, it is hard to understand the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce the additional annotation of recording and transcription, the data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
 As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, noise words in the pseudo transcription should be diverse and ASR probable~\cite{7178796}.
That is, ASR systems have different error distributions, such as phoneme or accents~\cite{different_error_distribution}.
For example, different from ASR 1 of corrupting `c' to `s', ASR 2 would confuse `r' and generate the error word `walkers' instead of the correct word `workers', where both errors are ASR probable.
Due to the difference in errors, PLMs robust against ASR 1 would be fragile to the errors made by ASR 2.

However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to follow the error distribution of an individual ASR system.
Such bias results in the following two problems
1) Narrowed noise problem: Only the narrow range of phonemes that are favored by an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



To overcome, we propose Interventional Speech Noise Injection (ISNI). For the narrowed noise problem,
We propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to make noise words more ASR probable, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of ASR improbable noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.



==> backup/230805/2_prelim.tex <==
\section{Preliminaries}
Before we present our proposed ISNI, we formulate our task of SNI. Then, we introduce related works in SNI, our main task, and ASR correction, another method of adapting PLM for SLU, where we adopt the constrained decoding method to implement ISNI. Finally, we introduce do-calculus, the theoretical background of our proposed ISNI.
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into a pseudo transcription.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo transcription, $T=\{t_{i}\}_{i=1}^{n}$.
Then, the resulting pseudo transcription, $T$, is used to train downstream models.
Trained on pseudo transcription $T$ containing noise words, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
\subsubsection{SNI}


Previously proposed methods can be summarized as 3 categories of TTS-ASR pipeline and textual perturbation, auto-regressive generation, which differs in how to generate the noise word $t_i$ of the word $x_i$.

The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio. 
During the conversion between the text and audio, the written word $x_i$ is expected to be corrupted into the ASR probable noise word $t_i$.
However, due to different error distribution between the human recording and the audio generated by TTS, the resulting pseudo transcription would have different error distribution from the ASR transcription~\cite{asrglue}.
 In addition, the exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora. 




Another category of SNI is textual perturbation which generates the pseudo transcription $T$ by replacing words $x_i \in X$ to its phonetically similar noise word $t_i$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, the noise word $t_i$ is determined as the word which is phonetically similar to the word $x_i$ as followed:
\begin{equation}
   t_{i} = argmax_{w \in W} S(W|x_{i}),
\end{equation}
where $S(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $S(W|x_{i})$. 
Specifically, $S(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo transcription efficiently, they cannot generate diverse error words as $S(W|x_{i})$ is pre-defined.

The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to
implement~\cite{asrglue,noisygen}. 
Specifically, the auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.
We argue that auto-regressive generation suffers from narrow noise problem and ASR improbable noise problem due to following individual ASR system.




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F$, $F^{-1} : T \rightarrow X$, converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors and then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, due to the innate robustness of PLMs against to errors~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

\subsubsection{Do-calculus}
Do-calculus aims to understand the causal effect of variable $X$ on another variable $Y$ more robustly.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
That is, when a specific value of $X$ is strongly correlated to $z$ and has large $P(z|X)$, resulting $P(Y|X)$ would be influenced by the value of $P(Y|X,z)$, even when the other value of $X$ would have different $P(Y|X,z)$.
Do-calculus removes such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no more influenced by $X$, thus influence of $X$ on $Y$ through the mediator $z$ is removed.



==> backup/230805/3_ours.tex <==
\section{Methods}
We now propose our SNI model, which aims to generate pseudo transcription containing diverse and ASR probable noises resolving narrow noise problem and ASR improbable noise problem.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method to remedy the narrowed noise problem is to intervene in the SNI so that the resulting pseudo transcriptions contain the noise words of diverse phonemes.
For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Using the variable $z_i$, the SNI process can be written as follows:
\begin{equation}
     P(t_{i}|x_{i}) = \sum_{z_{i}}P(t_{i}|x_{i},z_{i})\cdot P(z_{i}|x_{i}).
     \label{eq:sni_definition}
\end{equation}
An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


In order to generate ASR generalizable pseudo transcription, we propose to intervene $z_i$.
Intervening $z_i$, we aim to manipulate $P(z_{i}|x_{i})$ so that $P(z_{i}|x_{i})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
As a result of such manipulation, resulting pseudo transcription would contain more diverse noise words.
Specifically, we remove any influence from the intervened variable, $x_{i}$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t_{i}|do(x_{i})) = \sum_{z}P(t_{i}|x_{i},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
To implement Eq.~\ref{eq:do-calculus}, we propose to conduct such determination explicitly. 
Specifically, for each word $x_i$, we sample random variable $d_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, the value of $z_i$ is determined as 1 if $d_i\leq P(z)$ else 0.
If $z$ is set to 0, $t_{i}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, $t_{i}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t_{i}|x_{i},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t_{i} \in T$ is phonetically similar to its cleanly written form $x_{i} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
Generated under the constraint on $x_{i}$, the noise word $t_{i}$ can be phonetically similar to the cleanly written word $x_{i}$ by using such characteristic.
Replacing $x_{i}$ to the generated noise word $t_{i}$, $X$ is corrupted into pseudo transcription $T$.

To generate pseudo transcription $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the noise word $t_{i}$ constrained on the written word $x_i$.
Specifically, the encoder representation of the written word $e^{encoder}_{i}$ and the special embedding vector $BOS$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E^{decoder}_{i}=W_{d}[e^{encoder}_{i}; BOS],
    \label{eq:decoder_input}
\end{equation}
where  $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate noise word $t_i$ from the inputs and outputs the hidden representation $h^{k}_{i}$ as follows:
\begin{align}
    h_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution $P_{gen}(\hat{t}_{i})$ measures the probability of each token in vocabulary to be noise word $t_i$ is predicted as follows:
\begin{equation}
    P_{gen}(\hat{t}_{i}) = softmax(WE \cdot h_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t_{i}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(t_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method is to make ASR improbable noise words more probable by correcting the noise word generation based on the phonetic information.
Toward our goal of more ASR probable noise words, we propose to correct the generation probability $P_{gen}(\hat{t}_{i})$ with the phoneme-based generation probability $P_{phoneme}(\hat{t}_{i})$ so that the ASR probable noise words can be generated as followed:
\begin{equation}
    P_{correct}(\hat{t}_{i}) = P_{gen}(\hat{t}_{i}) \cdot P_{phoneme}(\hat{t}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $P_{phoneme}(\hat{t}_{i})$ is to provide phonetic information via phoneme embedding $PHE$.
The main difficulty of evaluating $P_{phoneme}(\hat{t}_{i})$ is that PLMs are not aware of how the written sentences are pronounced.
%Conventional text generation is not aware of how the words are pronounced~\cite{wang2022building} and results in ASR improbable noise %words, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
%Thus, their input, word embedding, lacks phonetic information.
Our proposed phoneme embedding $PHE$ is designed to have the phonetic information of each token in the vocabulary.
Thus, feeding the phoneme embedding $PHE$ can deliver how each word in written sentences is pronounced.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(\hat{t}_{i}) = softmax(PHE \cdot h_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob}, $P_{phoneme}(\hat{t}_{i})$ can be evaluated based on the phonetic information.


Our second proposal for $P_{phoneme}(\hat{t}_{i})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR probable noise words, $P_{phoneme}(\hat{t}_{i})$ should evaluate how phonetically similar the words are to the $x_i$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $P_{phoneme}(\hat{t}_{i})$.
Specifically, phonetic similarity $PS$ is evaluated using the phoneme edit distance $PD$~\cite{9662078}.
The phoneme edit distance $PD$ measures the difference of the phonetic code between the given two words $w_i$ and $w_j$.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}
Then, phonetic similarity $PS$ can be defined as follows:
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.

To supervise $P_{phoneme}(\hat{t}_{i})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $R(\hat{t}_{i})$ as follows:
\begin{equation}
    R(\hat{t}_{i}) = \frac{PS(t_{i},w)}{\sum_{w^{\prime}\in W}PS(t_{i},w^{\prime} )}.
 \end{equation}
Then, $P_{phoneme}(\hat{t}_{i})$ is supervised by loss defined as follows:
 \begin{equation}
     l_p = KLD(P_{phoneme}(\hat{t}_{i}),  R(\hat{t}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(\hat{t}_{i})$ can correct the generation of ASR improbable words.
 

 




==> backup/230805/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\input{table/dstc_result}
As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset.
DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG), where human responses are ASR transcription generated from an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it requires ASR generalizability as transcriptions of human responses are generated by unknown ASR and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the famous NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.




\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset.


As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
To show ASR generalizability of our proposed methods, we adopt both task-agnostic and specific baselines.
Our main task-agnostic baseline which we used for both DSTC Track 2 dataset and ASR GLUE benchmark is Noisy-Gen, the SNI model of auto-regressive generation.
Noisy-Gen and ours used identical ASR transcriptions for training.
We adopt task-specific baselines which were proven to improve the robustness against ASR errors in each task.
For DSTC10 Track2 dataset, we adopt TOD-DA~\cite{tian2021tod-da}, SNI method based on both the TTS-ASR pipeline and textual perturbation.
For ASR GLUE dataset, we adopt GPT2 based SNI model similar to Noisy-Gen provided by ASR GLUE benchmark which we call Noisy-Gen (Kaldi).
Training set for Noisy-Gen (Kaldi) is constructed by transcribing the libriSpeech corpus with Kaldi based ASR system.
Compared to Noisy-Gen, Noisy-Gen (Kaldi) is trained with smaller corpus but used identical ASR system to transcribe the test set.







==> backup/230805/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme correction robustify the downstream task models on ASR errors? 


\noindent \textbf{RQ2:} Does our proposed interventional SNI and phoneme correction increase ASR generalizability?



\input{table/asrglue_result}
\subsection{RQ1: Effectiveness of our proposed methods on robustifying downstream SLU tasks.}
In this section, we show the effectiveness of our proposed methods in robustifying downstream SLU tasks.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines without ASR generalizability struggle to robustify against ASR errors generated by an unknown ASR system, showing R@1 score below 60.
In contrast to the observations made by adopting an identical ASR system for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
This result shows that pseudo transcription following an individual ASR system struggles to robustify against ASR errors generated by unknown ASR systems.
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed 
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.

To confirm that our proposed methods contribute to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.
We report the result without the phoneme correction in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme correction showed a decreased score in every subtask, showing that the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.


To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:random_selection}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x_i$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z_i|x_i)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Decreased performance of the last row shows that the intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.


\subsection{RQ2: ASR generalizability of our proposed methods. }

Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
First, we show that autoregressive generation-based SNI models are not generalizable across ASR systems.
For such purposes, we compare Noisy-Gen and Noisy-Gen (Kaldi).
While Noisy-Gen used a larger training corpus, Noisy-Gen (Kaldi) outperformed Noisy-Gen in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (Kaldi) in the high noise level was higher than that of Nosiy-Gen in the medium noise level.
This result shows that autoregressive generation-based SNI models struggle to generalize across the ASR errors.

In contrast, ours showed comparable results to Noisy-Gen (Kaldi), even though we used a different ASR system to construct a training set of SNI models.
Specifically, ours outperformed Noisy-Gen (Kaldi) in QNLI of the high and medium noise level and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can generate pseudo transcription which can generalize across different ASR systems.


==> backup/230805/6_conclusion.tex <==
\section{Conclusion}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.



==> backup/230806/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
Trained in written language, PLMs may struggle to adapt to the differences in spoken language.
ASR systems incorrectly transcribe the spoken language into phonetically similar but semantically different words.
The most effective and intuitive method to robustify PLMs for SLU is to expose PLMs to such erroneous transcriptions during training, for which we propose to augment the written language into pseudo transcription.
For such goal, pseudo transcription should cover the errors which diverse ASR systems would make in practice.
%Unless, the robustness of the trained PLMs would not be generalizable to individual ASR system.
Therefore, we  propose a causal perspective that utilizes do-calculus and intervenes in the augmentation for diversity adopting constrained generation.
For plausibility, we propose to correct the augmentation based on the phonetic information with which the ASR systems transcribe.
The proposed approaches result in the diversity and plausibility of the pseudo transcription and improve the robustness and generalizability of SLU models.
Experimental results and analysis show the effectiveness of our proposed methods.
\end{abstract}

==> backup/230806/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
 As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, noise words in the pseudo transcription should ASR probable. 
 However, this notion of ASR probability is specific to ASR system.~\cite{7178796}.
That is, ASR systems have different error distributions, such as phoneme or accents~\cite{different_error_distribution}.
For example, different from ASR 1 of corrupting `c' to `s', ASR 2 would confuse `r' and generate the error word `walkers' instead of the correct word `workers', where both errors are ASR probable.
Due to the difference in errors, PLMs robust against ASR 1 would be fragile to the errors made by ASR 2.

However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to follow the error distribution of an individual ASR system.
Such bias results in the following two problems
1) Narrowed noise problem: Only the narrow range of phonemes that are favored by an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



Meanwhile, we pursue ASR-generality: we propose Interventional Speech Noise Injection (ISNI). 
For the narrowed noise problem,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to make noise words more ASR probable, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of ASR improbable noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.



==> backup/230806/2_prelim.tex <==
\section{Preliminaries}
Before we present our proposed ISNI, we formulate our task of SNI. Then, we introduce related works in SNI, our main task, and ASR correction, another method of adapting PLM for SLU, where we adopt the constrained decoding method to implement ISNI. Finally, we introduce do-calculus, the theoretical background of our proposed ISNI.
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into a pseudo transcription.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo transcription, $T=\{t_{i}\}_{i=1}^{n}$.
Then, the resulting pseudo transcription, $T$, is used to train downstream models.
Trained on pseudo transcription $T$ containing noise words, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
\subsubsection{SNI}


Previously proposed methods can be summarized as 3 categories of TTS-ASR pipeline and textual perturbation, auto-regressive generation, which differs in how to generate the noise word $t_i$ of the word $x_i$.

The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio. 
During the conversion between the text and audio, the written word $x_i$ is expected to be corrupted into the ASR probable noise word $t_i$.
However, due to different error distribution between the human recording and the audio generated by TTS, the resulting pseudo transcription would have different error distribution from the ASR transcription~\cite{asrglue}.
 In addition, the exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora. 




Another category of SNI is textual perturbation which generates the pseudo transcription $T$ by replacing words $x_i \in X$ to its phonetically similar noise word $t_i$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, the noise word $t_i$ is determined as the word which is phonetically similar to the word $x_i$ as followed:
\begin{equation}
   t_{i} = argmax_{w \in W} S(W|x_{i}),
\end{equation}
where $S(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $S(W|x_{i})$. 
Specifically, $S(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo transcription efficiently, they cannot generate diverse error words as $S(W|x_{i})$ is pre-defined.

The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to
implement~\cite{asrglue,noisygen}. 
Specifically, the auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.
We argue that auto-regressive generation suffers from narrow noise problem and ASR improbable noise problem due to following individual ASR system.




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F$, $F^{-1} : T \rightarrow X$, converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors and then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, due to the innate robustness of PLMs against to errors~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

\subsubsection{Do-calculus}
Do-calculus aims to understand the causal effect of variable $X$ on another variable $Y$ more robustly.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
That is, when a specific value of $X$ is strongly correlated to $z$ and has large $P(z|X)$, resulting $P(Y|X)$ would be influenced by the value of $P(Y|X,z)$, even when the other value of $X$ would have different $P(Y|X,z)$.
Do-calculus removes such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no more influenced by $X$, thus influence of $X$ on $Y$ through the mediator $z$ is removed.



==> backup/230806/3_ours.tex <==
\section{Methods}
We now propose our SNI model, which aims to generate pseudo transcription containing diverse and ASR probable noises resolving narrow noise problem and ASR improbable noise problem.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method to remedy the narrowed noise problem is to intervene in the SNI so that the resulting pseudo transcriptions contain the noise words of diverse phonemes.
For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Using the variable $z_i$, the SNI process can be written as follows:
\begin{equation}
     P(t_{i}|x_{i}) = \sum_{z_{i}}P(t_{i}|x_{i},z_{i})\cdot P(z_{i}|x_{i}).
     \label{eq:sni_definition}
\end{equation}
An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


In order to generate ASR generalizable pseudo transcription, we propose to intervene $z_i$.
Intervening $z_i$, we aim to manipulate $P(z_{i}|x_{i})$ so that $P(z_{i}|x_{i})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
As a result of such manipulation, resulting pseudo transcription would contain more diverse noise words.
Specifically, we remove any influence from the intervened variable, $x_{i}$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t_{i}|do(x_{i})) = \sum_{z}P(t_{i}|x_{i},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
To implement Eq.~\ref{eq:do-calculus}, we propose to conduct such determination explicitly. 
Specifically, for each word $x_i$, we sample random variable $d_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, the value of $z_i$ is determined as 1 if $d_i\leq P(z)$ else 0.
If $z$ is set to 0, $t_{i}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, $t_{i}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t_{i}|x_{i},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t_{i} \in T$ is phonetically similar to its cleanly written form $x_{i} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
Generated under the constraint on $x_{i}$, the noise word $t_{i}$ can be phonetically similar to the cleanly written word $x_{i}$ by using such characteristic.
Replacing $x_{i}$ to the generated noise word $t_{i}$, $X$ is corrupted into pseudo transcription $T$.

To generate pseudo transcription $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the noise word $t_{i}$ constrained on the written word $x_i$.
Specifically, the encoder representation of the written word $e^{encoder}_{i}$ and the special embedding vector $BOS$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E^{decoder}_{i}=W_{d}[e^{encoder}_{i}; BOS],
    \label{eq:decoder_input}
\end{equation}
where  $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate noise word $t_i$ from the inputs and outputs the hidden representation $h^{k}_{i}$ as follows:
\begin{align}
    h_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution $P_{gen}(\hat{t}_{i})$ measures the probability of each token in vocabulary to be noise word $t_i$ is predicted as follows:
\begin{equation}
    P_{gen}(\hat{t}_{i}) = softmax(WE \cdot h_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t_{i}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(t_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method is to make ASR improbable noise words more probable by correcting the noise word generation based on the phonetic information.
Toward our goal of more ASR probable noise words, we propose to correct the generation probability $P_{gen}(\hat{t}_{i})$ with the phoneme-based generation probability $P_{phoneme}(\hat{t}_{i})$ so that the ASR probable noise words can be generated as followed:
\begin{equation}
    P_{correct}(\hat{t}_{i}) = P_{gen}(\hat{t}_{i}) \cdot P_{phoneme}(\hat{t}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $P_{phoneme}(\hat{t}_{i})$ is to provide phonetic information via phoneme embedding $PHE$.
The main difficulty of evaluating $P_{phoneme}(\hat{t}_{i})$ is that PLMs are not aware of how the written sentences are pronounced.
%Conventional text generation is not aware of how the words are pronounced~\cite{wang2022building} and results in ASR improbable noise %words, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
%Thus, their input, word embedding, lacks phonetic information.
Our proposed phoneme embedding $PHE$ is designed to have the phonetic information of each token in the vocabulary.
Thus, feeding the phoneme embedding $PHE$ can deliver how each word in written sentences is pronounced.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(\hat{t}_{i}) = softmax(PHE \cdot h_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob}, $P_{phoneme}(\hat{t}_{i})$ can be evaluated based on the phonetic information.


Our second proposal for $P_{phoneme}(\hat{t}_{i})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR probable noise words, $P_{phoneme}(\hat{t}_{i})$ should evaluate how phonetically similar the words are to the $x_i$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $P_{phoneme}(\hat{t}_{i})$.
Specifically, phonetic similarity $PS$ is evaluated using the phoneme edit distance $PD$~\cite{9662078}.
The phoneme edit distance $PD$ measures the difference of the phonetic code between the given two words $w_i$ and $w_j$.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}
Then, phonetic similarity $PS$ can be defined as follows:
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.

To supervise $P_{phoneme}(\hat{t}_{i})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $R(\hat{t}_{i})$ as follows:
\begin{equation}
    R(\hat{t}_{i}) = \frac{PS(t_{i},w)}{\sum_{w^{\prime}\in W}PS(t_{i},w^{\prime} )}.
 \end{equation}
Then, $P_{phoneme}(\hat{t}_{i})$ is supervised by loss defined as follows:
 \begin{equation}
     l_p = KLD(P_{phoneme}(\hat{t}_{i}),  R(\hat{t}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(\hat{t}_{i})$ can correct the generation of ASR improbable words.
 

 




==> backup/230806/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\input{table/dstc_result}
As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset.
DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG), where human responses are ASR transcription generated from an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it requires ASR generalizability as transcriptions of human responses are generated by unknown ASR and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the famous NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.




\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset.


As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
To show ASR generalizability of our proposed methods, we adopt both task-agnostic and specific baselines.
Our main task-agnostic baseline which we used for both DSTC Track 2 dataset and ASR GLUE benchmark is Noisy-Gen, the SNI model of auto-regressive generation.
Noisy-Gen and ours used identical ASR transcriptions for training.
We adopt task-specific baselines which were proven to improve the robustness against ASR errors in each task.
For DSTC10 Track2 dataset, we adopt TOD-DA~\cite{tian2021tod-da}, SNI method based on both the TTS-ASR pipeline and textual perturbation.
For ASR GLUE dataset, we adopt GPT2 based SNI model similar to Noisy-Gen provided by ASR GLUE benchmark which we call Noisy-Gen (Kaldi).
Training set for Noisy-Gen (Kaldi) is constructed by transcribing the libriSpeech corpus with Kaldi based ASR system.
Compared to Noisy-Gen, Noisy-Gen (Kaldi) is trained with smaller corpus but used identical ASR system to transcribe the test set.







==> backup/230806/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme correction robustify the downstream task models on ASR errors? 


\noindent \textbf{RQ2:} Does our proposed interventional SNI and phoneme correction increase ASR generalizability?



\input{table/asrglue_result}
\subsection{RQ1: Effectiveness of our proposed methods on robustifying downstream SLU tasks.}
In this section, we show the effectiveness of our proposed methods in robustifying downstream SLU tasks.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines without ASR generalizability struggle to robustify against ASR errors generated by an unknown ASR system, showing R@1 score below 60.
In contrast to the observations made by adopting an identical ASR system for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
This result shows that pseudo transcription following an individual ASR system struggles to robustify against ASR errors generated by unknown ASR systems.
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed 
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.

To confirm that our proposed methods contribute to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.
We report the result without the phoneme correction in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme correction showed a decreased score in every subtask, showing that the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.


To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:random_selection}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x_i$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z_i|x_i)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Decreased performance of the last row shows that the intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.


\subsection{RQ2: ASR generalizability of our proposed methods. }

Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
First, we show that autoregressive generation-based SNI models are not generalizable across ASR systems.
For such purposes, we compare Noisy-Gen and Noisy-Gen (Kaldi).
While Noisy-Gen used a larger training corpus, Noisy-Gen (Kaldi) outperformed Noisy-Gen in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (Kaldi) in the high noise level was higher than that of Nosiy-Gen in the medium noise level.
This result shows that autoregressive generation-based SNI models struggle to generalize across the ASR errors.

In contrast, ours showed comparable results to Noisy-Gen (Kaldi), even though we used a different ASR system to construct a training set of SNI models.
Specifically, ours outperformed Noisy-Gen (Kaldi) in QNLI of the high and medium noise level and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can generate pseudo transcription which can generalize across different ASR systems.


==> backup/230806/6_conclusion.tex <==
\section{Conclusion}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.



==> backup/230808/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
Trained in written language, PLMs may struggle to adapt to the differences in spoken language.
The main obstacle to such adaptation is the errors introduced by ASR systems.
ASR systems incorrectly transcribe the spoken language into phonetically similar but semantically different words.
PLMs struggle to understand semantics from such erroneous transcriptions.
The most effective and intuitive method to robustify PLMs for SLU is to expose PLMs to such erroneous transcriptions during training, for which we propose to augment the written language into pseudo transcription.
For such goal, pseudo transcription should contain the errors which diverse ASR systems would make in practice.
Unless, the robustness of the trained PLMs would not be generalizable to individual ASR system.
Therefore, motivated by do-calculus, we first propose to intervene in the augmentation for diversity adopting constrained generation.
For plausibility, we propose to correct the augmentation based on the phonetic information with which the ASR systems transcribe.
The proposed approaches result in the diversity and plausibility of the pseudo transcription and improve the robustness and generalizability of SLU models.
Experimental results and analysis are provided to support the effectiveness of our proposed methods.
\end{abstract}

==> backup/230808/1_intro.tex <==
\section{Introduction}
Starting from ELMo~\cite{peters-etal-2018-deep} to recent GPT4~\cite{openai2023gpt4}, pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription  is fed into PLMs to conduct downstream SLU tasks. 


%As PLMs are trained in the different modality of written text, they suffer to adapt to the difference between the transcription and text.
%이 문단에서 하고 싶은 말 ASR error의 특징 : phonetically similar but semantically different + PLMs cannot understand semantics from noised input
As ASR systems incorrectly transcribe the speech into phonetically similar but wrong words~\cite{ruan20_interspeech,9054689}, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
Pronounced similarly, the ASR systems struggle to accurately distinguish phonetically similar words from speech such as wait and weight in Fig.~\ref{fig:example}.
Confusing such words, the ASR systems fail to distinguish them and generate incorrect transcription containing phonetically similar words, ASR error words, instead of the correct words~\cite{ruan20_interspeech,9054689}.
For example, confusing between wait and weight, cereal and serial, the ASR systems generate incorrect transcription of ``I cannot weight to eat serieal''  as depicted in Fig.~\ref{fig:example}.
In contrast to the similarity in pronunciation, the semantics of ASR error words differ from the correct words, thus, it is hard to understand the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.


%데이터
%학습시 aSR error 노출시키면 robust 가능, 그래서 asr error augmentation, SNI 할거
However, PLMs can be robustified if they are trained with incorrect transcription~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}, for which the data augmentation method of converting the written sentence into pseudo transcription containing ASR errors, speech noise injection (SNI), has been introduced.
Though training PLMs with incorrection transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
An SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
SNI aims to reduce  human annotation of recording and transcribing in collecting SLU corpora by generating pseudo transcription.
Specifically, given the written sentence, SNI mimics the confusion of the ASR systems and corrupts the words in the written sentence with ASR-plausible error words which are phonetically similar.

\input{figure_latex/figure1}
%여기는 previous SNI 들이 다 ASR specific 하다는 내용 위주로 고치기.
%Previous works in SNI can be categorized into two methods. 
%The most intuitive method is the TTS-ASR pipeline, where the TTS engine (text-to-speech) converts the text into audio, and the ASR system transcribes the audio.
%While ASR errors are generated by TTS engines and ASR systems, they are both computationally expensive.
%Additionally, they cannot generate sufficient ASR errors as the noise engaged during human reading does not exist in the audio converted by TTS.
%In contrast, generative SNI supervises the autoregressive language model $M$ to generate the pseudo-ASR given the text as the following:
%\begin{equation}
%    X^{\prime} = M(X)
%\end{equation}
%As generative SNI is shown to be effective in various situations~\cite{asrglue}, we focus on generative SNI.
%이 문단에서  하교 싶은 얘기 ASR generalizble 하려면 어떻게 ASR error 를 만들어야 하나
In order for the PLM trained with pseudo transcription to be generally used with different ASR systems, they should be trained on pseudo transcription containing diverse ASR-plausible error words~\cite{7178796}.
%However, previous works in SNI follow the individual ASR system and cannot generate such diverse ASR-plausible error words.
Due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to follow the error distribution of an individual ASR system.
As a result, only the phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
Such bias even degrades the plausibility of the resulting pseudo transcription when SNI model is blinded to the phonetic information
For example, as depicted in Fig.~\ref{fig:example}, following the incorrect transcription of the ASR system on `c' to `s' such as `cereal' to `serial' and `cease' to `sees', SNI is biased to corrupt the words containing `c' while leaving the words with `w'.
Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-unplausible error words. 

%While many previous works studied SNI~\cite{feng22c_interspeech, noisygen}, ASR-generalizability, the ability of an SLU model to perform robustly across different ASR systems, is not well studied for SNI.
%Such generalizability has been focused on diverse SLU tasks as different ASR systems can be used in SLU pipeline~\cite{blackbox1}.
%ASR-generalizability has been important as different ASR systems have distinct error distributions and SLU trained on one error distribution suffers to generalize on different error distribution.
%However, previous works in SNI confirmed their effectiveness using identical ASR systems for both SNI and downstream tasks, where the ASR generalizability still remains unveiled~\cite{noisygen,tts_asr}.
%We argue that ASR-generalizability is also crucial in SNI as the resulting pseudo-ASR would follow the error distribution of an individual ASR system.


%Toward ASR generalizable SNI, we first propose to intervene SNI process based on do-calculus~\cite{glymour2016causal} so that the resulting pseudo-ASR would not follow the error distribution of an individual ASR system. 
In order to increase the diversity of the ASR-plausible error words, we first propose to intervene SNI based on do-calculus~\cite{glymour2016causal}.
Adopting Do-calculus in SNI enables such diversification by cutting off the probability to corrupt the frequently incorrectly transcribed phonemes and increasing such probability of the other phonemes as contrasted by $P(z|x_i)$ and $P(z)$ in Fig~\ref{fig:example}. 
%Adopting Do-calculus in SNI enables such diversification by intervening in the corruption of the phonemes so that infrequently corrupted phonemes are more corrupted while frequently corrupted phonemes are less corrupted. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-plausible error words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to ASR-plausible errors by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as 'wait` and 'cue` as depicted in Fig.~\ref{fig:example} as a result of such diversification.
%factorize the generation of ASR errors into two distinct steps: phonetic misunderstanding and misspelling.
%For such goal, we train SNI model to generate the ASR-noised words constrained on its written words, the noise target words.
%Previous works supervised SNI model to maximize the likelihood of the entire ASR transcription given its written sentence~\cite{asrglue, noisygen}.
%
%During such supervision, the SNI model is biased to select the noise target words following the error distribution of the ASR system adopted for training.
%Thus, the resulting pseudo-ASR would contain biased ASR errors, such as containing errors for specific phonemes.
%As a result, we intervene in the choice of the word to corrupt so that diverse phonemes can be corrupted.
%implemen the intervention in SNI by factorizing it into the two processes of noise word selection and noise word generation.
%In the noise word selection, the noise target word, the word to be corrupted in the pseudo-ASR, is randomly selected without bias. Then, by constraining the noise target word, a phonetically similar ASR noise word is generated.
%As the bias from the ASR system is removed, the resulting pseudo-ASR contains diverse ASR errors and can robustify the downstream model against the diverse ASR systems.
%In contrast, our SNI model randomly selects the noise target words. 
%This random selection serves as an intervention to the error distribution of the ASR system and debias the resulting pseudo-ASR to diversify the error distribution.
%Trained on the pseudo-ASR with more diverse ASR errors, downstream task models can more robustly conduct downstream tasks.
%As a result
%, similar to interventions performed in do-calculus, where we actively modify the values of certain variables to observe the effects on the overall system.
%By randomly selecting the words, we remove the bias associated with specific ASR systems and ensure a more diverse set of corrupted words.

Our second contribution to increase the plausibility of ASR plausible error words is to correct the generation of phonetically different ASR plausible error words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as 'choir` to 'quire`.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting 'c`  to 's`.
Fed only the words, not their phonetic information, previous SNI models confuse 'c` in the word 'cue` to be pronounced as 's` and generate the unplausible ASR error word 'sue`.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that 'c` is pronounced as phoneme 'k`, our SNI model corrupts into the phonetically similar ASR-plausible error word 'queue`.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-plausible.

%In addition to intervention in the error distribution, we propose to correct the generation of ASR noise words using phonetic information. 
%While ASR systems generate phonetically similar words as ASR error words, SNI models are optimized to maximize the likelihood of the grapheme-based tokens corresponding to ASR error words.
%Blinded to phonetic similarity, the existing SNI model fails to generate phonetically similar pseudo-ASR and requires additional phonetic similarity based heuristic to filter out such failing pseudo-ASR.
%Instead of such heuristic, we propose to supervise and incorporate phonetic similarity to correct the noise word generation.
%Specifically, we propose a phoneme head, another language model head that generates ASR noise words based on their phonemes.
%This phoneme head is used with trivial language model head of SNI models and ensures to generate the phonetically similar ASR error words.

%Powerful generation models of ten meet most of the task requirements, yet miss a few (e.g.,omittinga subset of keywords), or generate incorrect hypotheses that nevertheless provide useful structure (e.g.,a correct problem solving strategy with a missing step). However, after generatingevenaslightlysub-optimalsequence,thesingle-passparadigmrequiresmodelsto“startfrom scratch”,effectivelydiscardingworkalreadydone.Amorenatural,intuitiveapproachisleveraging thegenerationasausefulstartingpointtorefineintoahigherqualityoutput.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of phonetically different ASR noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

\begin{comment}
In the phonetic misunderstanding step, the ASR system misinterprets the spoken phonemes, leading to inaccuracies in the resulting transcription. 
Consequently, the subsequent step, misspelling, arises as a result of the ASR system generating misspelled words based on its flawed understanding of the original speech. 
Misspelling errors occur when the ASR system incorrectly converts the misunderstood phonemes into different characters, further deviating from the intended transcription. 

\input{table/asr_cer}

Among two distinct steps, we argue that  
while the phonetic misunderstanding is ASR-specific noise, the misspelling step is ASR-generalizable.
Specifically, phonetic misunderstanding can be largely influenced by training data and acoustic modeling.
For example, ASR systems with distinct acoustic feature extractors and different accented training audio would exhibit distinct susceptibility to phonetic misunderstanding.
In contrast, we argue that the phenomenon of misspelling is more ASR-generalizable. 
This is because a language possesses specific spelling conventions that are shared across different ASR models regardless of training data or acoustic modeling techniques. 

To demonstrate the generalizability of misspelling errors among ASR models, we present the Character Error Rate (CER) between different open-source ASR models, DeepSpeech and Leopard, and ground-truth transcription in Table~\ref{tab:cer}. 
In Table~\ref{tab:cer}, we observe that the CER values for the different ASR models are smaller than that of each ASR model and ground-truth transcription. 
This indicates that, despite the differences in model-specific factors, the misspelling errors generated by these models are more similar to each other than ground-truth transcription.

Toward ASR-generalizable SNI, we consider alignable characteristics of the ASR-error words.
That is, the words in the ground-truth text can be easily aligned to their corresponding words in ASR transcription.
When the words are correctly transcribed, the words in the ASR and its ground-truth text would be easily aligned.
However, such alignment is not limited to the correctly transcribed words.
As ASR systems misspell the words of the ground-truth text into phonetically, also graphemically, similar words, even inaccurately transcribed words can be easily aligned to their corresponding words.

Considering such alignment, we propose to break down SNI from generating entire pseudo-ASR transcription $X^{\prime}$ given written text $X$ into the finer-grained generation of ASR error words $w^{\prime}\in X^{\prime}$ given written word $w \in X$ adopting constrained generation which can be formulated as follows:
\begin{equation}
    w^{\prime} = M(w)
\end{equation}
Directly conditioned on the cleanly written word $w$, not the entire text $X$, such fine-grained SNI can better supervise the SNI model of how the written words $w$ are corrupted to ASR error words $w^{\prime}$ by misspelling. 
By better supervising misspelling with fine-grained SNI, we enhance its ability to generalize across different ASR systems, as ASR misspelling is generalizable to different written words, regardless of the ASR systems.

In addition to misspellings, fine-grained SNI can also contribute to a more ASR-generalizable approach in the context of phoneme misunderstanding.
In previous generative SNI, whether the cleanly written word $w$ would be corrupted is implicitly determined by SNI model $M$.
Biased by the phoneme misunderstanding pattern of the ASR system used to transcribe the training set, the SNI model tends to corrupt only the words that the specific ASR system would phonetically misunderstand.
Compared to sentence-level SNI, our word-level SNI gives more control in selecting which words to corrupt to ASR error words.
For ASR-generalizable SNI, we propose to randomly select the words to corrupt, so that the resulting pseudo-ASRs would contain diverse ASR-error words.



Our major contributions to ASR-generalizable SNI are threefold:
1) propose a word-level SNI approach adopting constrained generation
2) propose a random word selection in the proposed word-level SNI 
and 3) show that the proposed word-level SNI improves the ASR-generalizability of downstream models.




%factorize the two distinct steps involved in ASR errors: phonetic misunderstanding and misspelling. 
%By doing so, we isolate the phonetic misunderstanding step where the ASR system misinterprets the spoken phonemes, and the subsequent misspelling step where it generates incorrect spellings based on the misunderstood speech.
%In contrast to previous approaches that treat SNI as a unified sequence-to-sequence generation task, our proposed constrained generation method allows us to focus solely on regenerating the ASR-noised words, while preserving the original written words. 
%This factorization enables us to address each step independently and develop targeted strategies to mitigate phonetic misunderstanding and improve the accuracy of misspelling generation.
%By adopting constrained generation and explicitly considering the phonetic misunderstanding and misspelling steps, our approach offers a novel perspective and potential advancements in the field of ASR-generalizable SNI. 
%It allows for more fine-grained control and targeted interventions, ultimately leading to improved performance and robustness in the generation of ASR-corrupted data.

\end{comment}


==> backup/230808/2_prelim.tex <==
\section{Preliminaries}
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into a pseudo transcription.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo transcription, $T=\{t_{i}\}_{i=1}^{n}$.
Then, the resulting pseudo transcription, $T$, is used to train downstream models.
Trained on pseudo transcription $T$ containing ASR plausible errors, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
%\subsubsection{Robustness }
%In recent years, large-scale PLMs have demonstrated remarkable performance in Natural Language Understanding (NLU) tasks~\cite{openai2023gpt4}. 
%To evaluate their robustness, several studies have employed human-crafted adversarial examples or generated examples through adversarial attacks~\cite{wang2021adversarial}. 
%Another approach involves projecting input data into a latent space using Generative Adversarial Networks and then retrieving adversaries that closely resemble the original instance in the latent space~\cite{zhao2017generating}.
%Additionally, controlled paraphrase networks are proposed to generate syntactically adversarial examples~\cite{iyyer2018adversarial}. 
%These examples not only deceive PLMs but also enhance their resilience to syntactic variations when used for training data augmentation. 
%However, the extent to which PLMs exhibit robustness against ASR errors in real-world conditions has been under-explored.
\subsubsection{SNI}

Previous works pointed out that the key distinction of the incorrect transcription $t_{i^{\prime}}\in T$ from different noise is phonetically similar to its written word $x_{i}\in X$~\cite{9721159, asrglue, tian2021tod-da}.
Specifically, each word $t_{i}\in T$ would be either identical or different to its corresponding written word $x_{i}\in X$.
When the word $t_i$ is different from the written word $x_i$,  the ASR error word $t_i$ is phonetically similar to the written word $x_i$.
Therefore, previous works proposed various methods to generate the pseudo transcription containing the ASR plausible error word $t_i$ which is phonetically similar to the written word $x_i$.
Previously proposed methods can be summarized as 3 categories of TTS-ASR pipeline and textual perturbation, auto-regressive generation.

The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio. 
During the conversion between the text and audio, the written word $x_i$ is expected to be corrupted into the ASR plausible error word $t_i$.
However, due to different error distribution between the human recording and the audio generated by TTS,  the resulting pseudo transcription would have different
error distribution from the ASR transcription~\cite{asrglue}.
 In addition, the exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora. 




Another category of SNI is textual perturbation which generates the pseudo transcription $T$ by replacing words $x_i \in X$ to its phonetically similar word $t_i$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, phonetically similar word $t_i$ is determined as the word which is  phonetically similar to the word $x_i$ as followed:
\begin{equation}
   t_{i^{\prime}} = argmax_{w \in W} P(W|x_{i}),
\end{equation}
where $P(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $P(W|x_{i})$. 
Specifically, $P(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo transcription efficiently, they cannot generate diverse ASR plausible error words as $P(W|x_{i})$ is pre-defined.

The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to
implement~\cite{asrglue,noisygen}. 
Specifically, the auto-regressive PLMs such as GPT-2 or BART is supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.
We argue that the pseudo-ASR generated by auto-regressive generation is not generalizable across the different ASR systems.
That is, during such supervision, the SNI model is biased to follow the error distribution of the ASR system and cannot generate diverse ASR plausible errors. 




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F^{-1} T \rightarrow X$ of converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which generates the written words constrained on the ASR noise words was proposed~\cite{constdecoder}
However, due to the innate robustness of PLMs against to noises~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

==> backup/230808/3_ours.tex <==
\section{Ours}
We now propose our SNI model, which aims to generate pseudo-ASR which is not biased toward an individual ASR system and robustifies downstream task models against diverse ASR errors.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method for ASR generalizable SNI is to intervene in the SNI so that the resulting pseudo transcriptions contain the ASR plausible error words of diverse phonemes.
For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted or not in the resulting pseudo transcript.
Using the variable $z_i$, the SNI process can be written as follows:
\begin{equation}
     P(t_{i^{\prime}}|x_{i}) = \sum_{z_{i}}P(t_{i}|x_{i})\cdot P(z_{i}|x_{i}).
     \label{eq:sni_definition}
\end{equation}
An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
Therefore, the SNI model following such an ASR system would have a similar distribution of $P(z_{i}|x_{i})$.
%It is widely known that an ASR system is biased to make errors on certain phonemes more frequently and training settings such as training data can cause such error distribution~\cite{feng2021quantifying}.
%As a result of such biased error distribution of the ASR system, SNI models supervised to mimic ASR errors are also vulnerable to generating pseudo-ASR following such biased error distribution.

%We blame such bias on the noise word selection process in SNI, where the word to corrupt is chosen.
%Let us consider whether the word $x_{i}\in X$ is corrupted or not in pseudo-ASR $T$ as the variable $z_i$.
%Then, the SNI process can be written as follows:
%\begin{equation}
%     P(t_{i^{\prime}}|x_{i}) = \sum_{z_{i}}P(t_{i^{\prime}}|x_{i})\cdot P(z_{i}|x_{i}).
%\end{equation}
%Trained to mimic ASR error of specific ASR error system, the SNI model would have biased noise word selection probability for different phonemes, $P(z|x_{i})$.
%That is, the SNI model would be biased to corrupt the words $x_{i}$ which is frequently corrupted by the ASR system used for training the SNI model.
%Specifically, we observed that the noisygen model tends to make more errors on the phonemes, such as S and R, while rarely corrupting the phonemes IH0 and AA1 following ASR system used for training.

In order to generate ASR generalizable pseudo transcription, we propose to intervene $z_i$.
Intervening $z_i$, we aim to manipulate $P(z_{i}|x_{i})$ so that $P(z_{i}|x_{i})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
As a result of such manipulation, resulting pseudo transcription would contain more diverse ASR-plausible errors.
Specifically, we remove any influence from the intervened variable, $x_{i}$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{align}
    P(t_{i^{\prime}}|do(x_{i})) &= \sum_{z}P(t_{i}, z|x_{i})\\
                                &= \sum_{z}P(t_{i}|x_{i},z) \cdot P(z|do(x_{i}))\\
                                &= \sum_{z}P(t_{i}|x_{i},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
To implement Eq.~\ref{eq:do-calculus}, we propose to conduct such determination explicitly. 
Specifically, for each word $x_i$, we sample random variable $d_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, we decide whether the word $x_{i}$ will be corrupted, which is determined as the value of $z_i$ as follows:
\begin{align}
    z_i = 
    \begin{cases}
        1, \quad \text{if} \quad d_i \leq P(z) \\
        0, \quad \text{else}
    \end{cases}
    \label{eq:random_selection}
\end{align}
where the word $x_{i}$ will be corrupted if $z$ is set to 1 or not if $z$ is set to 0.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

When $x_{i}$ is determined to be corrupted, the ASR plausible error word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t_{i}|x_{i},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t_{i} \in T$ is phonetically similar to its cleanly written form $x_{i} in X$.
Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$
Specifically, if $z$ is set to 0, $t_{i}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, we constrain the generation of the ASR noise word $t_{i}$ to $x_{i}$ so that the generated ASR noise word $t_{i}$ is phonetically similar to the cleanly written word $x_{i}$.
Replacing $x_{i}$ to the generated ASR noise word $t_{i}$, $X$ is corrupted into pseudo-ASR $T$.

To generate pseudo transcription $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the ASR plausible error word $t_{i}$ constrained on the written word $x_i$.
Specifically, the encoder representation of the written word $e^{encoder}_{i}$ and the special embedding vector $BOS$ representing the begin of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E^{decoder}_{i}=W_{d}[e^{encoder}_{i}; BOS],
    \label{eq:decoder_input}
\end{equation}
where  $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate ASR plausible error word $t_i$ from the inputs and outputs the hidden representation $h^{k}_{i}$ as follows:
\begin{align}
    h_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder}_{i},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution of ASR plausible error word $t_i$ is predicted as follows:
\begin{equation}
    P_{gen}(\hat{t}_{i}) = softmax(WE \cdot h_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

In training, we used the ASR transcription $T$.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t_{i}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(t_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method for ASR generalizable SNI is to correct the phonetically differently generated ASR noise word considering the phonetic similarity.
Pure text-based generation lacks useful information like pronunciation and prosody~\cite{wang2022building} and results in phonetically different pseudo-ASR, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
Thus, we propose to evaluate phonetic similarity-based generation probability $P_{phoneme}(\hat{t}_{i})$ and correct the generation probability in Eq.~\ref{eq:gen_prob} so that the phonetically similar ASR noise words can be generated as followed:
\begin{equation}
    P_{correct}(\hat{t}_{i}) = P_{gen}(\hat{t}_{i}) \cdot P_{phoneme}(\hat{t}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


The main difficulty in the generation of phonetically similar ASR noise words is that PLMs are supervised to understand semantic context, not phonetic information.
Thus, their input, word embedding, lacks phonetic information.
Our first proposal to generate phonetically similar ASR noise words is to provide phonetic information using phoneme embedding $PHE$.
The phoneme embedding $PHE$ aims to deliver the phonetic information of tokens in the vocabulary.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
%The phoneme embedding is fed to the decoder similar to the encoder as follows:
%\begin{multline}
%    E^{decoder}_{i,k}=W_{d}[e^{encoder}_{i};  \lambda_{w}\cdot WE(X)+\lambda_{p}\cdot PHE(X) \\+ PE(D^{k}_{i})].
%\end{multline}
The input for decoder is formulated similar to Eq.~\ref{eq:decoder_input}

Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(\hat{t}_{i}) = softmax(PHE \cdot h_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob},  $P_{phoneme}(\hat{t}_{i})$ can evaluate the generation probability based on the phonetic information.

Without proper supervision of the phonetic information, $P_{phoneme}(\hat{t}_{i}$ cannot correct the generation of the phonetically different ASR noise words.
For the supervision of the phonetic information, we propose to distill the phonetic information from the phonetic edit distance~\cite{9662078}.
The phoneme edit distance measures the similarity between the given two words $w_i$ and $w_j$ by two consecutive steps.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}

In order to correct the generation probability as in Eq.~\ref{eq:phoneme_correction_prob}, the phonetic information should be evaluated as the probability distribution. 
For such purpose, we convert the phoneme edit distance to the phoneme probability distribution $R(\hat{t}_{i})$, which will be used as the label for $P_{phoneme}(\hat{t}_{i})$.
First, the phoneme edit distance is converted into the phoneme similarity score $PS$ which is defined as follows
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.
For the ground-truth ASR error word, $t_{i}$, the phoneme probability distribution $R(\hat{t}_{i})$ is evaluated for each token $w$ in vocabulary as followed:
\begin{equation}
    R(\hat{t}_{i}) = \frac{PS(t_{i},w)}{\sum_{w^{\prime}\in W}PS(t_{i},w^{\prime} )}.
 \end{equation}
 The phoneme probability distribution  $R(\hat{t}_{i})$ is used as a label to supervise the phoneme information to evaluate loss as followed:
 \begin{equation}
     l_p = KLD(P_{phoneme}(\hat{t}_{i}),  R(\hat{t}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(\hat{t}_{i})$ can correct the generation of the phonetically different words.
 

 




==> backup/230808/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset.
DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG), where human responses are ASR transcription generated from an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it requires ASR generalizability as transcriptions of human responses are generated by unknown ASR and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the famous NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which DSTC10 Track2 dataset does not contain.




\input{table/dstc_result}
\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset.


As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
To show ASR generalizability of our proposed methods, we adopt both task-agnostic and specific baselines.
Our main task-agnostic baseline which we used for both DSTC Track 2 dataset and ASR GLUE benchmark is Noisy-Gen, the SNI model of auto-regressive generation.
Noisy-Gen and ours used identical ASR transcriptions for training.
We adopt task-specific baselines which were proven to improve the robustness against ASR errors in each task.
For DSTC10 Track2 dataset, we adopt TOD-DA~\cite{tian2021tod-da}, SNI method based on both the TTS-ASR pipeline and textual perturbation.
For ASR GLUE dataset, we adopt GPT2 based SNI model similar to Noisy-Gen provided by ASR GLUE benchmark which we call Noisy-Gen (Kaldi).
Training set for Noisy-Gen (Kaldi) is constructed by transcribing the libriSpeech corpus with Kaldi based ASR system.
Compared to Noisy-Gen, Noisy-Gen (Kaldi) is trained with smaller corpus but used identical ASR system to transcribe the test set.







==> backup/230808/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme correction robustify the downstream task models on ASR errors? 


\noindent \textbf{RQ2:}Does our proposed interventional SNI and phoneme correction increase ASR generalizability?



\subsection{RQ1: Effectiveness of our proposed methods on robustifying downstream SLU tasks.}
In this section, we show the effectiveness of our proposed methods in robustifying downstream SLU tasks.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines without ASR generalizability struggle to robustify against ASR errors generated by unknown ASR system, showing R@1 score below 60.
In contrast to the observations made by adopting an identical ASR system for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
This result shows that pseudo transcription following individual ASR system struggles to robustify against ASR errors generated by unknown ASR systems.
In contrast, ours outperforms baselines in every metric in KS with a large margin, showing that ours can robustify against ASR errors made by unknown ASR system.

Results in Table~\ref{tab:dstc_results} shows that robustification of our proposed methods is not limited in KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed 
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.

To confirm that our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methdos in turn.
We report the result without the phoneme correction in fouth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme correction showed the decreased score in every subtasks, showing that the importance of ASR plausibility of psuedo transcription to robustify against ASR errors.


\input{table/asrglue_result}
To conduct the ablation on the intervention itself, we trained constrained decoding based SNI model without do-calculus based random corruption as in Eq.~\ref{eq:random_selection}.
Specifically, as constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x_i$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z_i|x_i)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of the Table~\ref{tab:dstc_results}. 
Decreased performance of last row shows that intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.


\subsection{RQ2: ASR generalizability of our proposed methods. }

Then, we now study ASR generalizability of our proposed methods with ASR GLUE benchmark.
We report the results on ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
First, we show that autoregressive generation based SNI models are not generalizable across ASR systems.
For such purpose, we compare Noisy-Gen and Noisy-Gen (Kaldi).
While Noisy-Gen used larger training corpus, Noisy-Gen (Kaldi) outperformed Noisy-Gen in every tasks.
Interestingly, in QNLI, accuracy of Noisy-Gen (Kaldi) in high noise level was highger than that of Nosiy-Gen in medium noise level.
This result shows that autoregressive generation based SNI models struggles to generalize across the ASR errors.

In contrast, ours showed comparable results to Noisy-Gen (Kaldi), even though we used different ASR system to construct training set of SNI models.
Specifically, ours outperformed Noisy-Gen (Kaldi) in QNLI of high and medium noise level and in SST of low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtasks.
These results shows that our proposed methods can generate pseudo transcription which can generalize across different ASR systems.


==> backup/230808/6_conclusion.tex <==
\section{Conclusion}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.



==> backup/230811/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR probability is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
% As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, noise words in the pseudo transcription should ASR probable. 
 %However, this notion of ASR probability is specific to ASR system.~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
Such bias results in the following two problems blocking the generalization of ASR probability:
1) Narrowed noise problem: Only the narrow range of phonemes that are favored by an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



Meanwhile, we pursue ASR-generality: we propose Interventional Speech Noise Injection (ISNI). 
For the narrowed noise problem,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to make noise words more ASR probable, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of ASR improbable noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/230812/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
Trained in written language, PLMs may struggle to adapt to the differences in spoken language.
ASR systems incorrectly transcribe the spoken language into phonetically similar but semantically different words.
The most effective and intuitive method to robustify PLMs for SLU is to expose PLMs to such erroneous transcriptions during training.
For such goal, pseudo transcription should cover the errors which diverse ASR systems would make in practice.
%Unless, the robustness of the trained PLMs would not be generalizable to individual ASR system.
Therefore, we propose a causal perspective that utilizes do-calculus and intervenes in the augmentation for diversity adopting constrained generation.
For plausibility, we propose to correct the augmentation based on the phonetic information with which the ASR systems transcribe.
The proposed approaches result in the diversity and plausibility of the pseudo transcription and improve the robustness and generalizability of SLU models.
Experimental results and analysis show the effectiveness of our proposed methods.
\end{abstract}

==> backup/230812/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR probability is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
% As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, noise words in the pseudo transcription should ASR probable. 
 %However, this notion of ASR probability is specific to ASR system.~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
Such bias results in the following two problems blocking the generalization of ASR probability:
1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



Meanwhile, we pursue ASR-generality: we propose Interventional Speech Noise Injection (ISNI). 
For the narrowed noise problem,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to make noise words more ASR probable, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method for ASR generalizable SNI
2) propose phoneme correction which corrects the generation of ASR improbable noise words
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/230812/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/230812/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/230812/2_prelim.tex <==
\section{Preliminaries}
Before we present our proposed ISNI, we formulate our task of SNI. Then, we introduce related works in SNI, our main task, and ASR correction, another method of adapting PLM for SLU, where we adopt the constrained decoding method to implement ISNI. Finally, we introduce do-calculus, the theoretical background of our proposed ISNI.
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into a pseudo transcription.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo transcription, $T=\{t_{i}\}_{i=1}^{n}$.
Then, the resulting pseudo transcription, $T$, is used to train downstream models.
Trained on pseudo transcription $T$ containing noise words, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
\subsubsection{SNI}


Previously proposed methods can be summarized as 3 categories of TTS-ASR pipeline and textual perturbation, auto-regressive generation, which differs in how to generate the noise word $t_i$ of the word $x_i$.

The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio. 
During the conversion between the text and audio, the written word $x_i$ is expected to be corrupted into the ASR plausible noise word $t_i$.
However, due to different error distribution between the human recording and the audio generated by TTS, the resulting pseudo transcription would have different error distribution from the ASR transcription~\cite{asrglue}.
 In addition, the exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora. 




Another category of SNI is textual perturbation which generates the pseudo transcription $T$ by replacing words $x_i \in X$ to its phonetically similar noise word $t_i$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, the noise word $t_i$ is determined as the word which is phonetically similar to the word $x_i$ as followed:
\begin{equation}
   t_{i} = argmax_{w \in W} S(W|x_{i}),
\end{equation}
where $S(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $S(W|x_{i})$. 
Specifically, $S(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo transcription efficiently, they cannot generate diverse error words as $S(W|x_{i})$ is pre-defined.

The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to
implement~\cite{asrglue,noisygen}. 
Specifically, the auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.
We argue that auto-regressive generation suffers from distribution bias and ASR implausible noise words due to following individual ASR system.




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F$, $F^{-1} : T \rightarrow X$, converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors and then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, due to the innate robustness of PLMs against to errors~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

\subsubsection{Do-calculus}
Do-calculus aims to understand the causal effect of variable $X$ on another variable $Y$ more robustly.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
That is, when a specific value of $X$ is strongly correlated to $z$ and has large $P(z|X)$, resulting $P(Y|X)$ would be influenced by the value of $P(Y|X,z)$, even when the other value of $X$ would have different $P(Y|X,z)$.
Do-calculus removes such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no more influenced by $X$, thus influence of $X$ on $Y$ through the mediator $z$ is removed.



==> backup/230812/3_ours.tex <==
\section{Methods}
We now propose our SNI model, which aims to generate pseudo transcription generated by true ASR error distribution without ASR implausible noise words.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method to remove distribution bias is to intervene in the SNI so that the resulting pseudo transcriptions contain the noise words of diverse phonemes.
For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Using the variable $z_i$, the SNI process can be written as follows:
\begin{equation}
     P(t_{i}|x_{i}) = \sum_{z_{i}}P(t_{i}|x_{i},z_{i})\cdot P(z_{i}|x_{i}).
     \label{eq:sni_definition}
\end{equation}
An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


In order to generate ASR generalizable pseudo transcription, we propose to intervene $z_i$.
Intervening $z_i$, we aim to manipulate $P(z_{i}|x_{i})$ so that $P(z_{i}|x_{i})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
As a result of such manipulation, resulting pseudo transcription would contain more diverse noise words.
Specifically, we remove any influence from the intervened variable, $x_{i}$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t_{i}|do(x_{i})) = \sum_{z}P(t_{i}|x_{i},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
To implement Eq.~\ref{eq:do-calculus}, we propose to conduct such determination explicitly. 
Specifically, for each word $x_i$, we sample random variable $d_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, the value of $z_i$ is determined as 1 if $d_i\leq P(z)$ else 0.
If $z$ is set to 0, $t_{i}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, $t_{i}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t_{i}|x_{i},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t_{i} \in T$ is phonetically similar to its cleanly written form $x_{i} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
Generated under the constraint on $x_{i}$, the noise word $t_{i}$ can be phonetically similar to the cleanly written word $x_{i}$ by using such characteristic.
Replacing $x_{i}$ to the generated noise word $t_{i}$, $X$ is corrupted into pseudo transcription $T$.

To generate pseudo transcription $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the noise word $t_{i}$ constrained on the written word $x_i$.
Specifically, the encoder representation of the written word $e^{encoder}_{i}$ and the special embedding vector $BOS$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E^{decoder}_{i}=W_{d}[e^{encoder}_{i}; BOS],
    \label{eq:decoder_input}
\end{equation}
where  $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate noise word $t_i$ from the inputs and outputs the hidden representation $h^{k}_{i}$ as follows:
\begin{align}
    h_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution $P_{gen}(\hat{t}_{i})$ measures the probability of each token in vocabulary to be noise word $t_i$ is predicted as follows:
\begin{equation}
    P_{gen}(\hat{t}_{i}) = softmax(WE \cdot h_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t_{i}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(t_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method is to make noise words more ASR plausible by correcting the generation of ASR implausible noise words based on the phonetic information.
Toward our goal of more ASR plausible noise words, we propose to correct the generation probability $P_{gen}(\hat{t}_{i})$ with the phoneme-based generation probability $P_{phoneme}(\hat{t}_{i})$ so that the ASR plausible noise words can be generated as followed:
\begin{equation}
    P_{correct}(\hat{t}_{i}) = P_{gen}(\hat{t}_{i}) \cdot P_{phoneme}(\hat{t}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $P_{phoneme}(\hat{t}_{i})$ is to provide phonetic information via phoneme embedding $PHE$.
The main difficulty of evaluating $P_{phoneme}(\hat{t}_{i})$ is that PLMs are not aware of how the written sentences are pronounced.
%Conventional text generation is not aware of how the words are pronounced~\cite{wang2022building} and results in ASR improbable noise %words, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
%Thus, their input, word embedding, lacks phonetic information.
Our proposed phoneme embedding $PHE$ is designed to have the phonetic information of each token in the vocabulary.
Thus, feeding the phoneme embedding $PHE$ can deliver how each word in written sentences is pronounced.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(\hat{t}_{i}) = softmax(PHE \cdot h_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob}, $P_{phoneme}(\hat{t}_{i})$ can be evaluated based on the phonetic information.


Our second proposal for $P_{phoneme}(\hat{t}_{i})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR probable noise words, $P_{phoneme}(\hat{t}_{i})$ should evaluate how phonetically similar the words are to the $x_i$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $P_{phoneme}(\hat{t}_{i})$.
Specifically, phonetic similarity $PS$ is evaluated using the phoneme edit distance $PD$~\cite{9662078}.
The phoneme edit distance $PD$ measures the difference of the phonetic code between the given two words $w_i$ and $w_j$.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}
Then, phonetic similarity $PS$ can be defined as follows:
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.

To supervise $P_{phoneme}(\hat{t}_{i})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $R(\hat{t}_{i})$ as follows:
\begin{equation}
    R(\hat{t}_{i}) = \frac{PS(t_{i},w)}{\sum_{w^{\prime}\in W}PS(t_{i},w^{\prime} )}.
 \end{equation}
Then, $P_{phoneme}(\hat{t}_{i})$ is supervised by loss defined as follows:
 \begin{equation}
     l_p = KLD(P_{phoneme}(\hat{t}_{i}),  R(\hat{t}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(\hat{t}_{i})$ can correct the generation of ASR implausible words.
 

 




==> backup/230812/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\input{table/dstc_result}
As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset.
DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG), where human responses are ASR transcription generated from an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it requires ASR generalizability as transcriptions of human responses are generated by unknown ASR and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the famous NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.




\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset.


As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
\input{table/asr_dataset}
To show ASR generalizability of our proposed methods, we adopt both task-agnostic and specific baselines.
Our main task-agnostic baseline which we used for both DSTC Track 2 dataset and ASR GLUE benchmark is Noisy-Gen, the SNI model of auto-regressive generation.
Noisy-Gen and ours used identical ASR transcriptions for training.
We adopt task-specific baselines which were proven to improve the robustness against ASR errors in each task.
For DSTC10 Track2 dataset, we adopt TOD-DA~\cite{tian2021tod-da}, SNI method based on both the TTS-ASR pipeline and textual perturbation.
For ASR GLUE dataset, we adopt GPT2 based SNI model similar to Noisy-Gen provided by ASR GLUE benchmark which we call Noisy-Gen (Kaldi).
Training set for Noisy-Gen (Kaldi) is constructed by transcribing the libriSpeech corpus with Kaldi based ASR system.
Compared to Noisy-Gen, Noisy-Gen (Kaldi) is trained with smaller corpus but used identical ASR system to transcribe the test set.







==> backup/230812/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme correction robustify the downstream task models on ASR errors? 


\noindent \textbf{RQ2:} Does our proposed interventional SNI and phoneme correction increase ASR generalizability?



\input{table/asrglue_result}
\subsection{RQ1: Effectiveness of our proposed methods on robustifying downstream SLU tasks.}
In this section, we show the effectiveness of our proposed methods in robustifying downstream SLU tasks.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines without ASR generalizability struggle to robustify against ASR errors generated by an unknown ASR system, showing R@1 score below 60.
In contrast to the observations made by adopting an identical ASR system for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
This result shows that pseudo transcription following an individual ASR system struggles to robustify against ASR errors generated by unknown ASR systems.
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed 
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.

To confirm that our proposed methods contribute to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.
We report the result without the phoneme correction in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme correction showed a decreased score in every subtask, showing that the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.


To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x_i$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z_i|x_i)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Decreased performance of the last row shows that the intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.


\subsection{RQ2: ASR generalizability of our proposed methods. }

Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
First, we show that autoregressive generation-based SNI models are not generalizable across ASR systems.
For such purposes, we compare Noisy-Gen and Noisy-Gen (Kaldi).
While Noisy-Gen used a larger training corpus, Noisy-Gen (Kaldi) outperformed Noisy-Gen in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (Kaldi) in the high noise level was higher than that of Nosiy-Gen in the medium noise level.
This result shows that autoregressive generation-based SNI models struggle to generalize across the ASR errors.

In contrast, ours showed comparable results to Noisy-Gen (Kaldi), even though we used a different ASR system to construct a training set of SNI models.
Specifically, ours outperformed Noisy-Gen (Kaldi) in QNLI of the high and medium noise level and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can generate pseudo transcription which can generalize across different ASR systems.


==> backup/230812/6_conclusion.tex <==
\section{Conclusion}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.



==> backup/230813/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
Trained in written language, PLMs may struggle to adapt to the differences in spoken language.
ASR systems incorrectly transcribe the spoken language into phonetically similar but semantically different words.
The most effective and intuitive method to robustify PLMs for SLU is to expose PLMs to such erroneous transcriptions during training.
For such goal, pseudo transcription should cover the errors which diverse ASR systems would make in practice.
%Unless, the robustness of the trained PLMs would not be generalizable to individual ASR system.
Therefore, we propose a causal perspective that utilizes do-calculus and intervenes in the augmentation for diversity adopting constrained generation.
For plausibility, we propose to correct the augmentation based on the phonetic information with which the ASR systems transcribe.
The proposed approaches result in the diversity and plausibility of the pseudo transcription and improve the robustness and generalizability of SLU models.
Experimental results and analysis show the effectiveness of our proposed methods.
\end{abstract}

==> backup/230813/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes which were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts which are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/230813/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/230813/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/230813/2_prelim.tex <==
\section{Preliminaries}
Before we present our proposed ISNI, we formulate our task of SNI. Then, we introduce related works in SNI, our main task, and ASR correction, another method of adapting PLM for SLU, where we adopt the constrained decoding method to implement ISNI. Finally, we introduce do-calculus, the theoretical background of our proposed ISNI.
\subsection{Problem Formulation}
The goal of SNI is to robustify the PLMs against ASR errors so that they can adapt to downstream SLU tasks without additional human annotation of recording and transcription.
For such goal, SNI aims to corrupt the written corpora into a pseudo transcription.
Specifically, SNI can be formulated as a functional mapping $F: X \rightarrow T$ between the cleanly written text $X$ and the ASR transcription $T$.
Given the cleanly written text $X=\{x_{i}\}_{i=1}^{n}$, an SNI model is expected to output the pseudo transcription, $T=\{t_{i}\}_{i=1}^{n}$.
Then, the resulting pseudo transcription, $T$, is used to train downstream models.
Trained on pseudo transcription $T$ containing noise words, downstream models can robustly understand the semantics of the ASR transcriptions and conduct the downstream SLU as in the written corpus.
\subsection{Related Works}
\subsubsection{SNI}


Previously proposed methods can be summarized as 3 categories of TTS-ASR pipeline and textual perturbation, auto-regressive generation, which differs in how to generate the noise word $t_i$ of the word $x_i$.

The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS (Text-To-Speech) engine converts the written text into audio, then an ASR system transcribes the audio. 
During the conversion between the text and audio, the written word $x_i$ is expected to be corrupted into the ASR plausible noise word $t_i$.
However, due to different error distribution between the human recording and the audio generated by TTS, the resulting pseudo transcription would have different error distribution from the ASR transcription~\cite{asrglue}.
 In addition, the exhaustive cost of the TTS engine and ASR system makes such methods hard to be adopted for large-scale corpora. 




Another category of SNI is textual perturbation which generates the pseudo transcription $T$ by replacing words $x_i \in X$ to its phonetically similar noise word $t_i$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, the noise word $t_i$ is determined as the word which is phonetically similar to the word $x_i$ as followed:
\begin{equation}
   t_{i} = argmax_{w \in W} S(W|x_{i}),
\end{equation}
where $S(W|x_{i})$ evaluates the phonetic similarity between the words in vocabulary $W$ and the written word $x_{i}$.
Previous works in textual perturbation differ in evaluating $S(W|x_{i})$. 
Specifically, $S(W|x_{i})$ can be evaluated by the confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
While textual perturbation methods can generate pseudo transcription efficiently, they cannot generate diverse error words as $S(W|x_{i})$ is pre-defined.

The most recent method is the auto-regressive generation which adopts the auto-regressive PLMs as an SNI model to
implement~\cite{asrglue,noisygen}. 
Specifically, the auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T$ given the written text $X$. 
The key strength of the generative SNI is that it can consider contextual information~\cite{noisygen}, similar to the language model in ASR systems.
We argue that auto-regressive generation suffers from distribution bias and ASR implausible noise words due to following individual ASR system.




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
ASR correction bridges the gap between the ASR transcription $T$ and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
Specifically, it can be considered as an inverse functional mapping of SNI $F$, $F^{-1} : T \rightarrow X$, converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model to output the corrected transcription.
As the ASR errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.
Due to the similarity between SNI and ASR correction, methods similar to textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were proposed.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors and then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, due to the innate robustness of PLMs against to errors~\cite{heigold-etal-2018-robust}, SNI outperformed ASR correction~\cite{asrglue}.



%While it has distinct strength for making 

\subsubsection{Do-calculus}
Do-calculus aims to understand the causal effect of variable $X$ on another variable $Y$ more robustly.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
That is, when a specific value of $X$ is strongly correlated to $z$ and has large $P(z|X)$, resulting $P(Y|X)$ would be influenced by the value of $P(Y|X,z)$, even when the other value of $X$ would have different $P(Y|X,z)$.
Do-calculus removes such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(x_{i}))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no more influenced by $X$, thus influence of $X$ on $Y$ through the mediator $z$ is removed.



==> backup/230813/3_ours.tex <==
\section{Methods}
We now propose our SNI model, which aims to generate pseudo transcription generated by true ASR error distribution without ASR implausible noise words.
\subsection{Interventional SNI}
\label{interventional_sni}
Our first method to remove distribution bias is to intervene in the SNI so that the resulting pseudo transcriptions contain the noise words of diverse phonemes.
For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Using the variable $z_i$, the SNI process can be written as follows:
\begin{equation}
     P(t_{i}|x_{i}) = \sum_{z_{i}}P(t_{i}|x_{i},z_{i})\cdot P(z_{i}|x_{i}).
     \label{eq:sni_definition}
\end{equation}
An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


In order to generate ASR generalizable pseudo transcription, we propose to intervene $z_i$.
Intervening $z_i$, we aim to manipulate $P(z_{i}|x_{i})$ so that $P(z_{i}|x_{i})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
As a result of such manipulation, resulting pseudo transcription would contain more diverse noise words.
Specifically, we remove any influence from the intervened variable, $x_{i}$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t_{i}|do(x_{i})) = \sum_{z}P(t_{i}|x_{i},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x_{i}$, which we set as a hyperparameter.

In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
To implement Eq.~\ref{eq:do-calculus}, we propose to conduct such determination explicitly. 
Specifically, for each word $x_i$, we sample random variable $d_i$ from the continuous uniform distribution of interval $[0,1]$.
Then, the value of $z_i$ is determined as 1 if $d_i\leq P(z)$ else 0.
If $z$ is set to 0, $t_{i}$ would be identical to $x_{i}$ which simulates the successful transcription of the ASR system.
If $z$ is set to 1, $t_{i}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t_{i}|x_{i},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t_{i} \in T$ is phonetically similar to its cleanly written form $x_{i} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
Generated under the constraint on $x_{i}$, the noise word $t_{i}$ can be phonetically similar to the cleanly written word $x_{i}$ by using such characteristic.
Replacing $x_{i}$ to the generated noise word $t_{i}$, $X$ is corrupted into pseudo transcription $T$.

To generate pseudo transcription $T$, following constrained decoding method~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written text $X$ into the vector representation $E$ of $X$ as follows:
\begin{equation}
    E^{encoder} = BERT(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e^{encoder}_{i} \in E^{encoder}$ is the encoder representation of the token $x_{i}\in X$ and $WE$ and $PE$ are word and position embeddings.

Then, the standard transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the noise word $t_{i}$ constrained on the written word $x_i$.
Specifically, the encoder representation of the written word $e^{encoder}_{i}$ and the special embedding vector $BOS$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E^{decoder}_{i}=W_{d}[e^{encoder}_{i}; BOS],
    \label{eq:decoder_input}
\end{equation}
where  $W_d$ is the linear transformation.
Then, a standard transformer decoder aggregates the information required to generate noise word $t_i$ from the inputs and outputs the hidden representation $h^{k}_{i}$ as follows:
\begin{align}
    h_{i}= TransformerDecoder(Q,K,V),\\
    Q=E^{decoder},K=E^{encoder},V=E^{encoder},
    \label{eq:decoder}
\end{align}
where the decoder input $E^{decoder}_{i,k}$ is used as query $Q$, and  encoder representation $E^{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution $P_{gen}(\hat{t}_{i})$ measures the probability of each token in vocabulary to be noise word $t_i$ is predicted as follows:
\begin{equation}
    P_{gen}(\hat{t}_{i}) = softmax(WE \cdot h_{i}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t_{i}$ as follows:
\begin{equation}
    l =-\sum_{k} log(P_{gen}(t_{i})).
\end{equation}


\subsection{Phonetic Correction}
\label{phoneme_head}
Our second method is to make noise words more ASR plausible by correcting the generation of ASR implausible noise words based on the phonetic information.
Toward our goal of more ASR plausible noise words, we propose to correct the generation probability $P_{gen}(\hat{t}_{i})$ with the phoneme-based generation probability $P_{phoneme}(\hat{t}_{i})$ so that the ASR plausible noise words can be generated as followed:
\begin{equation}
    P_{correct}(\hat{t}_{i}) = P_{gen}(\hat{t}_{i}) \cdot P_{phoneme}(\hat{t}_{i})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $P_{phoneme}(\hat{t}_{i})$ is to provide phonetic information via phoneme embedding $PHE$.
The main difficulty of evaluating $P_{phoneme}(\hat{t}_{i})$ is that PLMs are not aware of how the written sentences are pronounced.
%Conventional text generation is not aware of how the words are pronounced~\cite{wang2022building} and results in ASR improbable noise %words, which requires additional phoneme-based filtering heuristics~\cite{noisygen}.
%Thus, their input, word embedding, lacks phonetic information.
Our proposed phoneme embedding $PHE$ is designed to have the phonetic information of each token in the vocabulary.
Thus, feeding the phoneme embedding $PHE$ can deliver how each word in written sentences is pronounced.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E^{encoder} = BERT(\lambda_{w}\cdot WE(X)+(1-\lambda_{w})\cdot PHE(X)\\+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}_{i}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^{k}_i$ to evaluate the phoneme based generation probability $P_{phoneme}(d^{k}_{i})$ as follows:
\begin{equation}
    P_{phoneme}(\hat{t}_{i}) = softmax(PHE \cdot h_{i}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob}, $P_{phoneme}(\hat{t}_{i})$ can be evaluated based on the phonetic information.


Our second proposal for $P_{phoneme}(\hat{t}_{i})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR probable noise words, $P_{phoneme}(\hat{t}_{i})$ should evaluate how phonetically similar the words are to the $x_i$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $P_{phoneme}(\hat{t}_{i})$.
Specifically, phonetic similarity $PS$ is evaluated using the phoneme edit distance $PD$~\cite{9662078}.
The phoneme edit distance $PD$ measures the difference of the phonetic code between the given two words $w_i$ and $w_j$.
First, two words are converted into phonetic code $C_i=\{c_{i}^{k}\}_{k=1}^{|C_i|}$ and $C_j=\{c_{j}^{k}\}_{k=1}^{|C_j|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $PD(w_i, w_j)$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    PD(w_i, w_j) = Levenshtein(C_i,C_j).
\end{equation}
Then, phonetic similarity $PS$ can be defined as follows:
\begin{equation}
    PS(w_i, w_j) = min(|C_i|-PD(w_i ,w_j ), 0),
\end{equation}
so that $PS(w_i, w_j)$ is larger when $w_i$ and $w_j$ are phonetically similar and 0 when they are phonetically different.

To supervise $P_{phoneme}(\hat{t}_{i})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $R(\hat{t}_{i})$ as follows:
\begin{equation}
    R(\hat{t}_{i}) = \frac{PS(t_{i},w)}{\sum_{w^{\prime}\in W}PS(t_{i},w^{\prime} )}.
 \end{equation}
Then, $P_{phoneme}(\hat{t}_{i})$ is supervised by loss defined as follows:
 \begin{equation}
     l_p = KLD(P_{phoneme}(\hat{t}_{i}),  R(\hat{t}_{i})),
 \end{equation}
 where KLD is the kl divergence loss.
 Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $P_{phoneme}(\hat{t}_{i})$ can correct the generation of ASR implausible words.
 

 




==> backup/230813/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio and LJSpeech-1.1, to collect ASR noise samples.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR transcriptions containing ASR errors remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\input{table/dstc_result}
As a downstream task to show ASR-noise robustness, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset.
DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS) and Knowledge-grounded Response Generation (RG), where human responses are ASR transcription generated from an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it requires ASR generalizability as transcriptions of human responses are generated by unknown ASR and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the famous NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.




\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset.


As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
\input{table/asr_dataset}
To show ASR generalizability of our proposed methods, we adopt both task-agnostic and specific baselines.
Our main task-agnostic baseline which we used for both DSTC Track 2 dataset and ASR GLUE benchmark is Noisy-Gen, the SNI model of auto-regressive generation.
Noisy-Gen and ours used identical ASR transcriptions for training.
We adopt task-specific baselines which were proven to improve the robustness against ASR errors in each task.
For DSTC10 Track2 dataset, we adopt TOD-DA~\cite{tian2021tod-da}, SNI method based on both the TTS-ASR pipeline and textual perturbation.
For ASR GLUE dataset, we adopt GPT2 based SNI model similar to Noisy-Gen provided by ASR GLUE benchmark which we call Noisy-Gen (Kaldi).
Training set for Noisy-Gen (Kaldi) is constructed by transcribing the libriSpeech corpus with Kaldi based ASR system.
Compared to Noisy-Gen, Noisy-Gen (Kaldi) is trained with smaller corpus but used identical ASR system to transcribe the test set.







==> backup/230813/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme correction robustify the downstream task models on ASR errors? 


\noindent \textbf{RQ2:} Does our proposed interventional SNI and phoneme correction increase ASR generalizability?



\input{table/asrglue_result}
\subsection{RQ1: Effectiveness of our proposed methods on robustifying downstream SLU tasks.}
In this section, we show the effectiveness of our proposed methods in robustifying downstream SLU tasks.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines without ASR generalizability struggle to robustify against ASR errors generated by an unknown ASR system, showing R@1 score below 60.
In contrast to the observations made by adopting an identical ASR system for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
This result shows that pseudo transcription following an individual ASR system struggles to robustify against ASR errors generated by unknown ASR systems.
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed 
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.

To confirm that our proposed methods contribute to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.
We report the result without the phoneme correction in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme correction showed a decreased score in every subtask, showing that the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.


To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x_i$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z_i|x_i)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Decreased performance of the last row shows that the intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.


\subsection{RQ2: ASR generalizability of our proposed methods. }

Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
First, we show that autoregressive generation-based SNI models are not generalizable across ASR systems.
For such purposes, we compare Noisy-Gen and Noisy-Gen (Kaldi).
While Noisy-Gen used a larger training corpus, Noisy-Gen (Kaldi) outperformed Noisy-Gen in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (Kaldi) in the high noise level was higher than that of Nosiy-Gen in the medium noise level.
This result shows that autoregressive generation-based SNI models struggle to generalize across the ASR errors.

In contrast, ours showed comparable results to Noisy-Gen (Kaldi), even though we used a different ASR system to construct a training set of SNI models.
Specifically, ours outperformed Noisy-Gen (Kaldi) in QNLI of the high and medium noise level and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can generate pseudo transcription which can generalize across different ASR systems.


==> backup/230813/6_conclusion.tex <==
\section{Conclusion}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.



==> backup/231211/4_experiment.tex <==
\section{Experiments}
\subsection{Dataset}

\input{table/dataset_statistics}

For training the SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1, to collect ASR error transcriptions.
Specifically, we put the audio recordings of the above corpora into the open-source commercial ASR system, Mozilla DeepSpeech, and get ASR transcriptions. 
Then,  we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR error transcriptions would remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\input{table/dstc_result}
As a downstream task to show the robustification of the pseudo transcriptions, we adopted DSTC10 Track2 dataset~\cite{dstc10_2} and QNLI and RTE, SST2 from ASR GLUE Benchmark dataset~\cite{asrglue}, which requires zero-shot generalization ability against ASR systems.
We formulate both datasets as the ASR zero-shot setting where the SNI model is trained with transcriptions generated by DeepSpeech and the SLU task model is tested with the transcriptions generated by either unknown or private ASR systems.

DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken conversational manner.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS), and Knowledge-grounded Response Generation (RG), where human responses are transcribed by an unknown ASR system.
The reason for adopting DSTC10 Track2 dataset is that it can measure the ASR generalizability of the SNI model as an unknown ASR system is used to generate transcriptions and contains major tasks in NLP, classification and retrieval, generation as SLU.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a textual classification task. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet from the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 

ASR GLUE benchmark is an SLU version of the widely adopted NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which the DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.




\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{attention_is_all} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.

Using the trained SNI model, the written sentences in DSTC10 Track2 dataset and ASR GLUE benchmark dataset are converted into pseudo transcription.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset based on the validation set result of downstream SLU tasks.
Also, we set $\lambda_{w}$ and $\lambda_{phoneme}$ as 0.5 to balance the semantic and phonetic information. 



As downstream task models, we adopted the GPT2 small model for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}.
For further details on downstream task models, we refer to previous work~\cite{dstc10_2,asrglue}.

\subsection{Baselines}
Our main baseline is NoisyGen, the GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
NoisyGen is trained with a training set identical to ours.
Pseudo-transcriptions generated by NoisyGen are filtered by phoneme-based heuristics. 


For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
TOD-DA is an SNI method based on both the TTS-ASR pipeline and textual perturbation.
Specifically, TOD-DA adopted the TTS engine from Google Translate and wave2vec ASR system.
Also, it conducted character-level perturbation of substitution and insertion and deletion and swap and split.


For ASR GLUE benchmark, we adopt another baseline Noisy-Gen (In Domain)~\cite{asrglue}.
NoisyGen and NoisyGen (In Domain) are similar in that they are both gpt2-based SNI models.
Though NoisyGen (In Domain) is trained in a smaller training set of LibriSpeech corpus, the ASR system transcribed the test set is used for the training set, which is improbable in the ASR zero-shot setting.
Comparing with NoisyGen (In Domain) can show how SNI models are successful in ASR generalizability.





==> backup/231213/5_results.tex <==
\section{Results}
We now present our experimental results, 
aiming to address each of the following research questions:

\noindent \textbf{RQ1:} Can our proposed interventional SNI and phoneme-aware generation robustify the SLU tasks in ASR zero-shot setting? 

\noindent \textbf{RQ2:} Does each of interventional SNI and phoneme-aware generation contributes to robustification?

\yj{\noindent \textbf{RQ3:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?}

\noindent \textbf{RQ4:} How well do our proposed methods generalize in the ASR zero-shot setting?



\subsection{RQ1: Robustification of our proposed methods on downstream SLU tasks.}
In this section, we show that our proposed methods can better robustify SLU tasks in ASR zero-shot setting.
As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
In contrast to the previous observations where the identical ASR system is used for training and testing~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed the increase of the BLEU score by 2-3x times for RG.
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.



\subsection{RQ2: Importance of each component to the robustification. }
To confirm that each of our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.

We report the result without the phoneme-aware generation in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme-aware generation showed a decreased score in every subtask, showing the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.


To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Decreased performance of the last row shows that the intervention itself contributes to robustification.


%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.
\yj{
\subsection{RQ3:Phoneme-aware generation for ASR$_*$-plausiblity. }
}
\input{table/phoneme_edit_distance}
\yj{
In this section, we show that PLMs are insufficient to generate the ASR$_*$-plausible pseudo transcriptions.
The noise words would be ASR$_*$-plausible if it is phonetically similar to its written form as an ASR system would incorrectly transcribe into phonetically similar noise words.
Therefore, we compared the phoneme edit distance defined in Eq.~\ref{eq:phoneme_edit_distance} between the written GT and the pseudo transcriptions.
For a fair comparison, we set identical $P(z)$ for the noise word generation to ensure that the noise words are generated for identical words.}

\yj{Table~\ref{tab4:phoneme_edit_distance} shows that the pseudo transcriptions without phoneme-aware generation show 17\% larger phonetic distance.
This result shows that PLMs are not enough to generate the ASR$_*$-plausible pseudo transcriptions and ignorance of phonetic information is the obstacle to generating ASR$_*$-lausible pseudo transcriptions.}


\input{table/asrglue_result}
\subsection{RQ4: Generalization of our proposed methods on ASR$_*$. }

%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.

\yj{
First, we show that existing auto-regressive generation-based SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation-based SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Nosiy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.}

%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ours showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
Specifically, ours outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can make SLU models ASR generalizable in the ASR zero-shot setting.


==> backup/231215/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs thus have gained widespread acceptance and employment within the realm of spoken language understanding (SLU) as applied in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
A concrete instance of this application involves a pipeline leveraging PLMs subsequent to the automatic speech recognition system (ASR) transcribing audio inputs. The resulting transcriptions are input to PLMs to facilitate downstream SLU tasks.


However, such pipeline would encounter challenges when confronted with inaccuracies stemming from ASR systems incorrectly transcribing speech into phonetically akin yet semantically unrelated terms~\cite{ruan20_interspeech,9054689}, which we denote as, ASR error words.
%, PLMs suffer to understand semantics from such erroneous transcription.
This inherent issue undermines the capacity of PLMs to discern meaningful semantics from such flawed transcriptions. To illustrate, consider Fig.~\ref{fig:example}, 
where ASR systems, confused between  ``cereal'' and ``serial'', ``quarry'' and ``carry'', may generate an incorrect transcription such as ``workers eat serial in the carry''.
These ASR error words, despite the phonetic resemblance, convey unintended meanings, thereby obstructing the coherent semantics of the spoken content in the downstream SLU tasks~\cite{belinkov2018synthetic}.




A well-known solution is annotating likely incorrect transcriptions, known as speech noise injection, or, SNI~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
%in addition to correct ground-truth (GT).
%Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
%The collected written language corpus is first recorded in audio by human annotators.
%Then they are transcribed into text using ASR systems.
%Such additional annotation steps obstruct collecting the %large-scale SLU corpora.
An SLU corpus annotation typically starts from a corpus of written 
text as a ground-truth (GT), recorded into audio recording, then
transcribed into text using ASR systems.
%the transcriptions are generated from the audio recordings using ASR systems. However, these supplemental annotation procedures impede the efficient aggregation of extensive SLU corpora.
A more efficient alternative is, skipping the recording and transcription,
to directly corrupt the written GT, to
%To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, 
 %In essence, SNI 
 introduce noise to the original written sentence, creating a pseudo transcription that closely aligns with the expected output of an ASR system.
 Desirably, SNI noise should be ``ASR-plausible'', indicating the pseudo transcription is likely to be generated by ASR systems.

\input{figure_latex/figure1}


However, by definition, ASR plausibility is 
%limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
%As ASR systems have different error distributions, such as phonemes or accents, ASR plausibility 
conditional to a particular ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may be implausible in another ASR~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR$_1$ would be implausible to ASR$_2$ which generates the correct transcript on `cerial' while confusing `r' and generating the error word `walkers'. 
In contrast,
%Due to the difference in ASR plausibility, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.
%For PLMs to be used with arbitrary ASR systems,ㅁ
we propose to generate pseudo transcription  that
generalizes beyond a particular ASR system.


%Our distinctions are two-fold: 
Our distinctions are two steps: 
First, after generating noises conditional to ASR$_i$,
we debias its dependence on ASR$_i$.
%First, we propose not to exactly follow an individual ASR system.
%As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes which were frequently corrupted by such ASR system.
%To show such mimicking explicitly, we 
We generate  ASR$_i$-plausible noises, by introducing a binary variable $z$, which determines whether the word $x$ in the written GT would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
\yj{For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR$_1$ would corrupt the word `cue' and `ceiling' with character `c', %following the ASR$_1$.
and training with such pseudo transcripts
can only robustify against errors from ASR$_1$,
but may fail to robustify against those from ASR$_2$.}
%would only robustify against the errors by ASR$_1$.
%Therefore, our proposed SNI model would have corrupting probability $P(z|x)$ different from an individual ASR system. 
To mitigate such bias,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 

To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-plausible noise words given the words in the written sentences, with do-calculus implemented by evenly corrupting the words in the written sentences.
\yj{For example, as depicted in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR 2 but not in ASR 1, in addition to the ones corrupted by baseline SNI,  as a result of such diversification.}
%\yj{For example, our SNI corrupts words which were with phonemes such as `reading', in addition to the ones corrupted by baseline SNI such as `cue' and `ceiling', as depicted in Fig.~\ref{fig:example} as a result of such diversification.}

Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$.
%Second, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$.
%common in that they are phonetically similar to their ground truth words.
For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
`serial'.
However, `c' can sound differently in another word, `cue' with k sound,
where replacing c with s (or, replacing `cue' with `sue') is not plausible for any ASR system.
To ensure noise generation to aware of such ASR-generic characteristics, we provide additional phoneme information that
`c' is pronounced as the phoneme `k',
%our SNI model 
%corrupts into the phonetically similar, thus ASR plausible, noise word 
to more ASR-plausible word `queue', regardless of the ASR system used, or ASR$_*$-plausible.
%Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.


Experiments are conducted in ASR zero-shot setting where SNI models are trained on ASR$_i$ and the SLU task is tested on another ASR$_j$ on DSTC10 Track2 and ASR GLUE benchmark.
Results show that our proposed methods are effective in ASR generalization with comparable or even outperforming performance compared to the in-domain setting where ASR$_j$ is used to train the SNI model.

Our major contributions to ASR-generalizable SNI are threefold:
1) We propose an interventional method in SNI to debias the dependence on a particular ASR system, ASR$_i$,
2) We propose phoneme-aware generation which ensures the generated pseudo transcriptions ASR$_*$-plausible
and 3) We show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/231215/2_prelim.tex <==
\section{Preliminaries}

Before we present our proposed Interventional SNI (ISNI), we formally define SNI and introduce related work as preliminaries.
%our task of SNI. Then, we introduce related works in SNI, our main task, and ASR correction, another method of adapting PLM for SLU, where we adopt the constrained decoding method to implement ISNI.
%Finally, we introduce do-calculus, the theoretical background of our proposed ISNI.

\subsection{Problem Formulation}
%\sw{we generate i-plausible pseudo transcription T$_i$ (existing work), then eliminate its bias to i. second step is ensuring asr-*}
%Our goal is to robustify PLMs so that they can be used with ASR$_*$.
%For such goal, we propose to generalize SNI such that the resulting pseudo transcriptions are ASR$_*$ plausible.
%Conditional to ASR$_i$, previous works formulated
SNI model can be formally defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Specifically, given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
Then, the resulting pseudo transcription, $T_i$, is used to train downstream SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ASR$_*$ plausible pseudo transcription $T_*$


\subsection{Related Work}
\subsubsection{SNI}
Previously proposed methods can be summarized as three categories, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 



Another category of SNI is textual perturbation which generates the pseudo transcription $T_i$ by replacing words $x^k \in X$ to noise word $t_{i}^{k}$.~\cite{li-specia-2019-improving, tian2021tod-da,tsvetkov-etal-2014-augmenting, wang-etal-2020-data}.
In textual perturbation, the noise word $t_{i}^{k}$ is replaced to the noise word $x^k$ which is selected as followed:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
Despite the efficiency of these textual perturbation methods, such scoring
cannot reflect contextual information and thus is outperformed by auto-regressive PLMs we introduce next~\cite{noisygen}.
%can generate pseudo transcription efficiently, their ignorance of contextual information makes the resulting pseudo transcription sub-optimal~\cite{noisygen}.

The most recent and effective method is  the auto-regressive PLMs as an SNI model~\cite{asrglue,noisygen}, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$ plausible noise words~\cite{noisygen}.

We adopt the third category as our baseline reporting the most competitive results in various SLU tasks~\cite{noisygen,asrglue}.
Our distinction is, while auto-regressive generation 
%fails to generalized for ASR$_*$ as they are supervised to generate 
is biased to ASR$_i$ plausible noise words,
%Our distinction is to 
generalizing SNI models so that the SLU tasks can be conducted with ASR$_*$. 
%\sw{we adopt the third category as a baseline because their reported results are best--but our distinction is distribution bias...overcome}




%To inject recognition noises, confusion-matrix-based ASR error simulators~\cite{confusion_matrix,confusion_matrix2} and
%TTS-ASR pipelines~\cite{tts_asr} are applied to the original data. 
%To imitate the disfluencies during speaking, some works~\cite{zayats2016disfluency,wang2020multi} interrupt the original dialogues by inserting or deleting words and phrases. 
%These works concentrate on word or sentence-level simulations.
%Our key baseline is ~\citet{tian2021tod-da} which aggregated the above-mentioned methods, TTS-ASR pipeline, and word or phrase insertion and deletion.

%Also, there exists another line of works adopting PLMs for SNI~\cite{noisygen,asrglue}.
%Specifically, they formulated SNI as a sequence-to-sequence problem which aims to generate a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
As an alternative direction to robustify SLU models for ASR errors, ASR correction %bridges the gap between the 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$,
%and the written corpus $X$ by correcting the ASR errors in the ASR transcription.
%Specifically, it 
which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
%converting ASR transcription to the written text $X$ by removing the ASR error.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which outputs the corrected transcription.
With errors are corrected, the resulting corrected transcriptions are fed to downstream models trained with the written corpus.

Due to this similarity between SNI and ASR correction, methods used for SNI, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart} were used.
In ASR correction, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors and then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, due to the innate robustness of PLMs against to errors~\cite{heigold-etal-2018-robust}, SNI has outperformed ASR correction~\cite{asrglue}, which explains why we focus on SNI.



%While it has distinct strength for making 


==> backup/240215/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
A widely used pipeline is leveraging PLMs subsequent to ASR transcribing audio inputs, where transcriptions are input to PLMs to facilitate downstream SLU tasks.
While the quality of transcriptions is critical in such pipeline,
ASR systems often incorrectly transcribe the spoken language into phonetically similar but semantically different words.
Our target problem is training SLU models to tolerate plausible ASR errors, by exposing to errors that are likely to be observed in ASR systems, which we denote as ASR-plausibility.
For such goal, we first augment pseudo transcription errors from  ASR$_i$,
which is inevitably conditional to a particular ASR$_i$, while a likely error in ASR$_i$
is not necessarily so in ASR$_j$.
To ensure SLU models not to be biased to ASR$_i$ used during augmentation,
we propose two phases: We first mitigate biases to  ASR$_i$, then we ensure our
augmentation to satisfy ASR-generic plausibility that holds for any ASR$_*$.
Our proposed approaches 
improve both the diversity and plausibility of the pseudo transcription, to eventually improve the robustness and generalizability of SLU models.
Experimental results and analysis show the effectiveness of our proposed methods.
\end{abstract}

==> backup/240215/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240215/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240215/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/240215/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs thus have gained widespread acceptance and employment within the realm of spoken language understanding (SLU) as applied in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
A concrete instance of this application involves a pipeline leveraging PLMs subsequent to the automatic speech recognition system (ASR) transcribing audio inputs. The resulting transcriptions are input to PLMs to facilitate downstream SLU tasks.


However, such pipeline would encounter challenges when confronted with inaccuracies stemming from ASR systems.
We denote such inaccuracy as ASR error words, which are phonetically akin yet semantically unrelated~\cite{ruan20_interspeech,9054689}.
%This inherent issue undermines the capacity of PLMs to discern meaningful semantics from such flawed transcriptions. 
To illustrate, consider Fig.~\ref{fig:example}, 
where ASR systems, confused between  ``cereal'' and ``serial'', ``quarry'' and ``carry'', may generate an incorrect transcription such as ``workers eat serial in the carry''.
These ASR error words, despite the phonetic resemblance, convey unintended meanings, thereby obstructing the semantics of the speech in the SLU tasks~\cite{belinkov2018synthetic}.




A well-known solution is annotating likely incorrect transcriptions, known as speech noise injection, or, SNI~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
An SLU corpus annotation typically starts from a corpus of written 
text as a ground-truth (GT), recorded into audio, then
transcribed into text using ASR systems.
A more efficient alternative is, skipping the recording and transcription,
to directly corrupt the written GT, to
 introduce noise to the original written sentence, creating a pseudo transcription that closely aligns with the expected output of an ASR system.
 Desirably, SNI noise should be ``ASR-plausible'', indicating the pseudo transcription is likely to be generated by ASR systems.

\input{figure_latex/figure1}


%However, by definition, ASR plausibility is 
%conditional to a particular ASR system~\cite{7178796}.
%%That is, an error plausible for one ASR system may be implausible in another ASR~\cite{different_error_distribution}.
%For example, the error of corrupting `c' to `s' made by ASR$_1$ would be implausible to ASR$_2$ which generates the correct transcript on `cerial' while confusing `%r' and generating the error word `walkers'. 
As ASR plausibility is conditional to a particular ASR system by definition~\cite{7178796}, previous methods mimic a particular ASR system.
Their first step is to collect the incorrect transcriptions of a particular ASR system.
Then, they generate pseudo transcripts similar to the collected incorrect transcriptions with confusion matrix~\cite{confusion_matrix, confusion_matrix2} or PLMs~\cite{noisygen}.
As a result of such mimicking, incorrect transcriptions from the ASR system, and pseudo transcripts have similar $P(z|x)$, the probability of whether the word $x$ is corrupted $(z=1)$ or not $(z=0)$.
In other words,  the word $x$ frequently corrupted by ASR$_i$ is also corrupted in pseudo transcripts.


However, ASR systems have different $P(z|x)$~\cite{different_error_distribution}, resulting SNI models to be used for ASR$_i$, even when they transcribe the identical audio.
For example, in Fig.~\ref{fig:example}, SNI with transcription by ASR$_1$ would corrupt the word `cue' and `ceiling' with character `c'.
Training with such pseudo-transcripts can only robustify against errors from ASR$_1$, but may fail to robustify against those from ASR$_2$.
To avoid such failure, each ASR$_i$ should build a robustified PLM$_i$.
However, recent trends in scaling PLMs make such robustification more exhaustive.


In contrast, to generate pseudo transcripts that generalize beyond a particular ASR system, our distinctions are two-fold: 
First, after generating noises conditional to ASR$_i$,
we debias its dependence on ASR$_i$. % adopting $do$-calculus.
%We generate ASR$_i$-plausible noises, by introducing a binary variable $z$, which determines whether the word $x$ in the written GT would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%Adopting do-calculus~\cite{glymour2016causal}, we propose to intervene in the effect of the word $x$ on $z$.
Specifically, $do$-calculus intervenes in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$.
It results in cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes. 
For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR 2 but not in ASR 1, in addition to the ones corrupted by baseline SNI.

%To implement do-calculus in SNI, we propose to adopt constrained decoding.
%Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-plausible noise words given the words in the written sentences, with do-calculus implemented by evenly corrupting the words in the written sentences.
%For example, as depicted in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR 2 but not in ASR 1, in addition to the ones corrupted by baseline SNI,  as a result of such diversification.

Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$, GT word and ASR noise word are phonetically similar~\cite{serai2022hallucination}.
We supervise and feed more information to aware of how words are pronounced.
Unaware of how words are pronounced, previous works generate ASR noise words plausible for no ASR system.  
For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
`serial'.
Mimicking ASR$_{1}$ unaware of pronunciation results in the replacement of c with s (or, replacing `cue' with `sue').
However, knowing that `c' can sound differently in other words, `cue' with k sound, ours can generate noise word `queue', which is plausible regardless of the ASR system used, or ASR$_*$-plausible.
 


Experiments are conducted in ASR zero-shot setting where SNI models are trained on ASR$_i$ and the SLU task is tested on another ASR$_j$ on DSTC10 Track2 and ASR GLUE benchmark.
Results show that our proposed methods are effective in ASR generalization with comparable or even outperforming performance compared to the in-domain setting where ASR$_j$ is used to train the SNI model.



==> backup/240215/2_prelim.tex <==
\section{Preliminaries}

Before we present our proposed Interventional SNI (ISNI), we formally define SNI then, briefly overview our ISNI and introduce related work as preliminaries.

\subsection{Problem Formulation}
SNI model can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
The resulting pseudo transcription, $T_i$, is used to train downstream SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ASR$_*$ plausible pseudo transcript $T_*$

\subsection{Overview of Our Proposed Approach}
\input{figure_latex/figure2}
In this section, we briefly overview the proposed ISNI in Fig.~\ref{fig:example2}.
%As we will detail in Sec.~\ref{interventional_sni}, to implement $do$-calculus, $P(z|x)$ should be explicitly controlled.
First, to debias the dependence on ASR$_i$ with $do$-calculus, we control $z$ by implementing SNI with constrained decoding following \citet{constdecoder}.
%The auto-regressive generation where $z$ of each token $x$ is implicitly determined by PLMs
In our approach, $z$ of each token is determined following $do$-calculus, enabling the corruption of the tokens rarely corrupted in ASR$_{i}$.  
The token $x$ with $z=1$, cue in Fig.~\ref{fig:example2}, is then fed to the constrained decoder to be corrupted.
Specifically, the constrained decoder outputs the noise word $t$ which replaces the token $x$.
Depending on the noise word $t$, the error type is determined.
If $t$ is only a special $<eos>$ token representing the end of the generation, $x$ is replaced with the empty string, which corresponds to the deletion error.
Substitution errors are modeled when $t$ is a new token and $<eos>$.
When $t$ includes new tokens in addition to $x$ and $<eos>$ as queue uh $<eos>$ in Fig.~\ref{fig:example2}, it corresponds to an insertion error.
These error types can happen synthetically as the generated examples of our ISNI show in Sec.~\ref{sec:pseudo_transcripts_examples}.

Second, to ensure that debiased noise to be ASR$_*$ plausible, during the generation of $t$, the phonetic information of $x$, kju in Fig.~\ref{fig:example2}, is fed to the constrained decoder.
The constrained decoder evaluates the generation probability based on the phonetic similarity that `c' is pronounced as the phoneme `k'.
As a result, the noise word 'queue` which is phonetically similar to 'cue` is generated.



\subsection{Related Work}
\subsubsection{SNI}
Previously proposed methods can be categorized in three categories. %, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation.%, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
First, TTS (Text-to-Speech)-ASR pipeline~\cite{tts_asr, tts_asr2} adopts the TTS engine, the reverse of ASR, to convert written text into audio, which, then, the ASR$_i$ transcribes into pseudo transcription. 
However, the human recording and TTS-generated audio differ in their error distributions, which makes the resulting pseudo transcriptions different~\cite{asrglue}. 
%The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
%During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
%However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
%The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 

Second is textual perturbation, replacing the words $x^k \in X$ to the noise word $t_{i}^{k}$ as follows:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix3, confusion_matrix5} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.

For comparison with the above two categories, we adopt TOD-DA as a baseline for the DSTC10 Track2 dataset which embodies both categories.
Due to its ignorance of the context, it is outperformed by the third method~\cite{noisygen, asrglue}.

Third is  the auto-regressive generation, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$ plausible noise words~\cite{noisygen}.

We adopt Noisy-Gen of the third category with the most competitive results in various spoken language tasks such as SLU and spoken language translation as our main baseline~\cite{noisygen,asrglue}.
Our distinction is, while auto-regressive generation is biased to ASR$_i$, % plausible noise words,
generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.% e a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
As an alternative, ASR correction 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT.
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperform ASR correction~\cite{asrglue}, which explains why we focus on SNI.






==> backup/240215/3_ours.tex <==
\section{Method}
We now formally define our ISNI, which aims to generate pseudo transcription that can robustify SLU tasks against ASR$_*$.
\subsection{Interventional SNI for Debiasing}
\label{interventional_sni}
For defining ISNI, we first formally introduce $do$-calculus.
%Our first step for such goal is to debias the dependence of SNI on ASR$_i$ with do-calculus.
%Before we explain our Interventional SNI, we introduce do-calculus.
Do-calculus aims to more robustly understand the causal effect of variable $X$ on another variable $Y$.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
That is, when a specific value of $X$ is strongly correlated to $z$ and has large $P(z|X)$, resulting $P(Y|X)$ would be influenced by the value of $P(Y|X,z)$, even when the other value of $X$ would have different $P(Y|X,z)$.
Do-calculus reduces such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer proof of transition between $P(z|do(X))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no longer influenced by $X$, thus the influence of $X$ on $Y$ through the mediator $z$ is mitigated.


%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Now, we first reveal that the SNI model depends on ASR$_i$ by introducing the variable $z$, which determines whether the word $x^k$ would be corrupted ($z=1$) or not ($z=0$) in the resulting pseudo transcript.
Using the variable $z$, the SNI process can be written as follows:
\begin{equation}
     P(t^{k}|x^{k}) = \sum_{z}P(t^{k}|x^{k},z)\cdot P(z|x^{k}).
     \label{eq:sni_definition}
\end{equation}
Then, the SNI model $P(t^{k}|x^{k})$ is biased to ASR$_i$ such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }




To debias the dependence on ASR$_i$, we propose to intervene $z$, so that the resulting pseudo transcript would contain diverse noise words even when they are rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
Specifically, we reduce any influence from the intervened variable, $x^k$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
As a result of the intervention in Eq.~\ref{eq:do-calculus}, whether or not to corrupt the words $x^k$ is determined independently from ASR$_i$ so that rarely corrupted words $x^k$ would be corrupted in the pseudo transcription.
Specifically, for each word $x^k$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$, which determines whether the word $x^k$ would be corrupted.
If $d^k\leq P(z)$, $z$ is set as 1, and $t^{k}$ would be a noise word and need to be generated.
Otherwise, $z$ is set to 0, and $t^{k}$ would be identical to $x^{k}$ as a simulation of the successful transcription.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x^{k}$, which we set as a hyperparameter.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t^{k}|x^{k},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.

To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ are word and position embeddings.

The transformer decoder~\cite{NIPS2017_3f5ee243} generates the noise word $t^{k}$ constrained on the written word $x^k$.
Specifically, the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E_{decoder}^{k}=M_{d}[e_{encoder}^{k}; bos],
    \label{eq:decoder_input}
\end{equation}
where  $M_d$ is the weight matrix of linear transformation.
The transformer decoder outputs the hidden representation $h^{k}$ as follows:
\begin{align}
    h^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K=E_{encoder},V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution $\textit{P}_{lm}(\hat{t}^{k})$ measures the probability of each token in vocabulary to be noise word $t^k$ as follows:
\begin{equation}
    \textit{P}_{lm}(\hat{t}^{k}) = softmax(M_{word} \cdot h^{k}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t^{k}$ as follows:
\begin{equation}
    l_{lm} =-\sum log(\textit{P}_{lm}(t^{k})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to ensure the noise word generation ASR$_*$-plausible.
The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
However, fed only words, not their pronunciation, auto-regressive SNI can generate noise words similar in character, not pronunciation.
To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
Toward our goal of ASR$_*$-plausible noise words, we propose to adjust the generation probability $\textit{P}_{lm}(\hat{t}^{k})$ with the phoneme-based generation probability $\textit{P}_{phoneme}(\hat{t}^{k})$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{equation}
    \textit{P}_{gen}(\hat{t}^{k}) = \textit{P}_{lm}(\hat{t}^{k}) \cdot \textit{P}_{phoneme}(\hat{t}^{k})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $\textit{P}_{phoneme}(\hat{t}^{k})$ is to provide phonetic information via phoneme embedding $M_{phoneme}$.
The main difficulty of evaluating $\textit{P}_{phoneme}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $M_{phoneme}$ is designed to have the phonetic information of each token in the vocabulary.
Thus, feeding the phoneme embedding $M_{phoneme}$ can deliver how each word in written sentences is pronounced.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{phoneme}(X)+M_{position}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^k$ to evaluate the phoneme based generation probability $\textit{P}_{phoneme}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{P}_{phoneme}(\hat{t}^{k}) = softmax(M_{phoneme} \cdot h^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $M_{phoneme}$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $M_{phoneme}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{phoneme}(\hat{t}^{k})$ can be evaluated based on the phonetic information.


Our second proposal for $\textit{P}_{phoneme}(\hat{t}^{k})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$-plausible noise words, $\textit{P}_{phoneme}(\hat{t}^{k})$ should evaluate how phonetically similar each word in the vocabulary is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{phoneme}(\hat{t}^{k})$.
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance $\textit{D}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{D}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{D}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. $S$ is computed based on articulatory features, thus, not equal to 1 as it is normally used when computing word error rates.


To supervise $\textit{P}_{phoneme}(\hat{t}^{k})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{phoneme}(\hat{t}^{k})$ is supervised by loss defined as follows:
 \begin{equation}
     l_{phoneme} = l_{KL}(\textit{P}_{phoneme}(\hat{t}^{k}),  \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $l_{KL}$ is the KL divergence loss.
Finally, our proposed ISNI model is optimized to jointly minimize the total loss $l_{tot}$ which is defined as follows:
\begin{equation}
    l_{tot} = l_{lm} + \lambda_{phoneme} \cdot l_{phoneme},
\end{equation}
where $\lambda_{phoneme}$ is the weight of $l_{phoneme}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{phoneme}(\hat{t}^k)$ can ensure the ASR$_*$-plausible noise words and $M_{phoneme}$ can contain phonetic information.
 

 




==> backup/240215/4_experiment.tex <==
\section{Experiments}
In this paper, we first experimentally confirm the validity of the ASR zero-shot setting, where SNI trained with ASR$_i$ cannot robustify against ASR$_j$ and the effectiveness of our proposed methods in the ASR zero-shot setting.
%For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.
Then, we show that our proposed methods can robustify various SLU tasks in the ASR zero-shot settings better than previous SNI methods.
\subsection{Dataset}

To test the ASR generalizability, we formulated an ASR zero-shot setting by adopting ASR systems with distinct architecture and training sets to transcribe SNI and downstream tasks. 
For training the SNI model, we used the Mozilla DeepSpeech~\cite{deepspeech}\footnote{https://github.com/mozilla/DeepSpeech}.
The audio of each downstream task, DSTC10 Track 2 and ASR GLUE benchmark, is transcribed by distinct ASR systems different from DeepSpeech.
We provide further details of ASR systems in Sec.~\ref{sec:asr_details}.

%\input{table/dataset_statistics}

For training the SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1, to collect ASR error transcriptions.
Specifically, we put the audio recordings of the above corpora into the DeepSpeech and get ASR transcriptions. 
Then, we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR error transcriptions would remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.



\input{table/asrglue_result}
ASR GLUE benchmark is an SLU version of the widely adopted NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which the DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.

DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken language.
We adopt the DSTC10 Track2 dataset as it contains various tasks in NLP in the dialogue domain where SLU is required frequently.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS), and Knowledge-grounded Response Generation (RG), where human responses are transcribed by an unknown ASR system.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a classification. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 





\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{NIPS2017_3f5ee243} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.
Also, we set $\lambda_{w}$ and $\lambda_{phoneme}$ as 0.5 to balance the semantic and phonetic information. 

Using the trained SNI model, the written GTs in DSTC10 Track2 dataset and ASR GLUE dataset are converted into pseudo transcripts.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset based on the validation set result of downstream SLU tasks.
As downstream task models, we adopted the GPT2-small for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}







\subsection{Baselines}
Our main baseline is Noisy-Gen, GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
Noisy-Gen is trained with a training set identical to ours.
Pseudo-transcriptions generated by Noisy-Gen are filtered by phoneme-based heuristics. 

For ASR GLUE benchmark, we adopt another baseline Noisy-Gen (In Domain)~\cite{asrglue}.
Noisy-Gen and Noisy-Gen (In Domain) are similar in that they are both GPT2-based SNI models.
However, Noisy-Gen (In Domain) uses the identical ASR system to transcribe the test set of ASR GLUE benchmark (TDNN LF-MMI), which is improbable in the ASR zero-shot setting.
Comparing with Noisy-Gen (In Domain) can show how SNI models are successful in ASR generalizability.

For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
TOD-DA encompasses both the TTS-ASR pipeline and
textual perturbation techniques.
It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
Also, it conducted character-level perturbation of substitution, insertion and deletion, and swap and split.








==> backup/240215/5_results.tex <==
\section{Results}


\input{table/dstc_result}
We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are our proposed methods in the ASR zero-shot setting?

%\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ2:} Can our proposed methods robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ3:} Does each of our proposed methods contribute to robustification?

\subsection{RQ1: Validity of ASR zero-shot setting and effectiveness of our proposed methods. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.


First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Noisy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.





%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ours showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
Specifically, ours outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can make SLU models ASR generalizable in the ASR zero-shot setting.


In addition, ours robustify against different noise levels.
Specifically, ours showed little degradation in performance as noise levels increased compared to baselines.
That is, as prior work suggests, phoneme confusions more frequently occur~\cite{wu2022phonetic,petkov2013maximizing} and ours can robustify even when such phoneme confusion increases.




%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.








\subsection{RQ2: Robustification of Our Proposed Methods on Various SLU Tasks.}
In this section, we show that our proposed methods can better robustify various SLU tasks over different SNI methods in ASR zero-shot setting.
%As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
Different from the previous observations where the identical ASR system is used for SNI and SLU tasks~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed the increase of the BLEU score by 2-3x times for RG.
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.



\subsection{RQ3: Importance of Each Proposed Method to the Robustification. }
To confirm that each of our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.

We report the result without the phoneme-aware generation in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme-aware generation showed a decreased score in every subtask, showing the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.
To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Decreased performance of the last row shows that the intervention itself contributes to robustification.


==> backup/240215/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we have addressed the challenge of ASR generalizability within the context of SNI. Specifically, our focus was on enhancing the robustness of downstream SLU models against ASR errors that may originate from diverse ASR systems. The existing SNI method is biased to a particular ASR system used for generating pseudo transcriptions.
To tackle the ASR generalizability issue, we introduce two key contributions: Interventional SNI and Phoneme-aware Generation. First, towards eliminating biases, Interventional SNI method significantly incorporates a wider range of ASR-plausible errors. However, such diversity should not interfere ASR-generic characteristcs, for which, our second step of Phoneme-aware Generation, leads to the generation of errors that are commonly plausible, or ASR$_*$ plausible.
Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/240216/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) as a pipeline where transcriptions from automatic speech recognition (ASR) systems are input to PLMs.
While the quality of transcriptions is critical in such pipeline,
ASR systems often incorrectly transcribe the spoken language into phonetically similar but semantically different words.
Our target problem is training SLU models to tolerate ASR errors, by exposing them to noises that are likely to be observed in ASR systems, which we denote as ASR plausible noises.
Speech noise injection (SNI) achieves such goal by introducing ASR plausible noises to the written text.
ASR plausible noises are inevitably conditional to a particular ASR, ASR$_i$, while it is not necessarily so in another ASR, ASR$_j$, biasing PLMs to be used for ASR$_i$.
To ensure SLU models not to be biased to ASR$_i$ used for SNI,
we propose two phases: We first mitigate biases to ASR$_i$, then we ensure our
augmentation to satisfy ASR-generic plausibility that holds for any ASR system, ASR$_*$.
Experimental results and analysis show the effectiveness of our proposed methods in improving the robustness and generalizability of SLU models against unseen ASR systems, by introducing more diverse and plausible ASR noises in advance.
\end{abstract}

==> backup/240216/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240216/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240216/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/240216/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs thus have gained widespread acceptance and employment within the realm of spoken language understanding (SLU) as applied in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
A concrete instance of this application involves a pipeline leveraging PLMs subsequent to the automatic speech recognition system (ASR) transcribing audio inputs. The resulting transcriptions are input to PLMs to facilitate downstream SLU tasks~\cite{asrglue}.


However, such pipeline would encounter challenges when confronted with inaccuracies stemming from ASR systems.
We denote such inaccuracy as ASR error words, which are phonetically akin yet semantically unrelated~\cite{ruan20_interspeech,9054689}.
To illustrate, consider Fig.~\ref{fig:example}, 
where ASR systems, confused between  ``cereal'' and ``serial'', ``quarry'' and ``carry'', may generate an incorrect transcription such as ``workers eat serial in the carry''.
Despite their phonetic resemblance, these ASR error words convey unintended meanings, thereby impeding the semantic understanding of speech in SLU tasks~\cite{belinkov2018synthetic}.




A well-known solution is annotating likely incorrect transcriptions, known as speech noise injection, or, SNI~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
An SLU corpus annotation typically starts from a corpus of written 
text as a ground truth (GT), recorded into audio, then
transcribed into text using ASR systems.
A more efficient alternative is, skipping the recording and transcription,
to directly corrupt the written GT, to
 introduce noise to the original written sentence, creating a pseudo transcript that closely aligns with the expected output of an ASR system.
 Desirably, SNI noise should be ``ASR-plausible'', indicating the pseudo transcript is likely to be generated by ASR systems.

\input{figure_latex/figure1}


 
By definition, as ASR plausibility is conditional to a particular ASR system, or ASR$_i$, previous methods have focused on mimicking the target ASR$_i$. 
To achieve this, these methods involve collecting the incorrect transcriptions generated by the target ASR$_i$ and subsequently corrupting the clean, written GTs into pseudo transcripts based on the errors observed~\cite{confusion_matrix, confusion_matrix2,noisygen}.
This process is designed to simulate the types of mistakes made by the target ASR$_i$. 
As a result, the probability of a word $x$ being corrupted $(z = 1)$ or not $(z = 0)$, denoted as $P(z|x)$, becomes closely aligned with the error patterns observed in both the real transcriptions produced by ASR$_i$ and the pseudo transcripts derived from this method. 
%For example, in Fig.~\ref{fig:example}, mimicking ASR 1 frequently corrupting `c', baseline SNI corrupts `cue' and `ceiling' in the pseudo transcripts.

However, ASR$_i$ and another ASR system, ASR$_j$, have different $P(z|x)$~\cite{different_error_distribution}, limiting SLU models trained with pseudo transcripts to be used for ASR$_i$.
For example, in Fig.~\ref{fig:example}, SNI with transcription by ASR$_1$ would corrupt the word `cue' and `ceiling' with character `c'.
Training with such pseudo transcripts can only robustify SLU models against errors from ASR$_1$, not ASR$_2$.
To avoid such failure, ASR$_i$ and ASR$_j$ and the other ASR systems should build their own SLU model.
However, recent trends in scaling PLMs make such robustification more exhaustive.


In contrast, to generate pseudo transcripts that generalize beyond ASR$_i$, our distinctions are two-fold: 
First, after generating noises conditional to ASR$_i$,
we debias its dependence on ASR$_i$.
Specifically, $do$-calculus intervenes in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$.
It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.


Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$, GT word and ASR noise word are phonetically similar~\cite{serai2022hallucination}.
Specifically, we supervise and feed how words are pronounced.
Unaware of how words are pronounced, previous works generate ASR noise words plausible for no ASR system.  
For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
`serial'.
Mimicking ASR$_{1}$ unaware of pronunciation results in replacing c with s (or, replacing `cue' with `sue').
However, knowing that `c' can sound differently in other words, k sound, ours can generate noise word `queue', which is plausible regardless of the ASR system used, or ASR$_*$-plausible.
 


Experiments are conducted in ASR zero-shot setting where SNI models are trained on ASR$_i$ and the SLU task is tested on another ASR$_j$ on DSTC10 Track2 and ASR GLUE benchmark.
Results show that our proposed methods are effective in ASR generalization with comparable or even outperforming performance compared to the in-domain setting where ASR$_j$ is used to train the SNI model.



==> backup/240216/2_prelim.tex <==
\section{Preliminaries}

Before we present our proposed Interventional SNI (ISNI), we formally define SNI then, briefly overview our ISNI and introduce related work as preliminaries.

\subsection{Problem Formulation}
SNI model can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
The resulting pseudo transcription, $T_i$, is used to train downstream SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ASR$_*$ plausible pseudo transcript $T_*$

\subsection{Overview of Our Proposed Approach}
\label{sec:overview}
\input{figure_latex/figure2}
In this section, we briefly overview the proposed ISNI in Fig.~\ref{fig:example2}.
%As we will detail in Sec.~\ref{interventional_sni}, to implement $do$-calculus, $P(z|x)$ should be explicitly controlled.
First, we debias the dependence on ASR$_i$ with $do$-calculus.
For such purpose, we control $z$ by implementing SNI with constrained decoding following \citet{constdecoder}.
%The auto-regressive generation where $z$ of each token $x$ is implicitly determined by PLMs
Determining $z$ following $do$-calculus, the tokens rarely corrupted in ASR$_{i}$ are noised in the pseudo transcripts.  
The token $x$ with $z=1$, `cue' in Fig.~\ref{fig:example2}, is fed to the constrained decoder.
Then, the constrained decoder generates the noise word $t$ which replaces $x$.

ISNI can noise the token $x$ into all conventional ASR error types, substitution/insertion/deletion~\cite{jurafsky2019speech}, depending on the output of the constrained decoder.
The most straightforward output is a new token that replaces $x$ and incurs a substitution error.
The constrained decoder can output new tokens in addition to $x$, queue uh in Fig.~\ref{fig:example2}.
Adding newly generated tokens, ISNI noises $x$ to an insertion error.
The constrained decoder can output an empty string which makes a deletion error.
These error types can happen synthetically as the generated examples of our ISNI show in Sec.~\ref{sec:pseudo_transcripts_examples}.

Second, we further generalize debiased noise to be ASR$_*$ plausible by discouraging the generation of phonetically different noise.
%Second, we ensure that debiased noise to be ASR$_*$ plausible by discouraging the generation of phonetically different noise.
For such purpose, we provide the phonetic information of $x$, `kju' in Fig.~\ref{fig:example2}, and make ISNI aware of how $x$ is pronounced.
Also, the constrained decoder evaluates the generation probability based on the phonetic similarity that `c' is pronounced as the phoneme `k'.
As a result, ISNI generates the ASR$_*$ plausible noise word `queue' which is phonetically similar to `cue'.



\subsection{Related Work}
\subsubsection{SNI}
Previously proposed methods can be categorized in three categories. %, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation.%, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
First, TTS (Text-to-Speech)-ASR pipeline~\cite{tts_asr, tts_asr2} adopts the TTS engine, the reverse of ASR, to convert written text into audio.
The ASR$_i$ transcribes it into pseudo transcription. 
However, the human recording and TTS-generated audio differ in their error distributions, which makes the resulting pseudo transcriptions different from ASR transcriptions~\cite{asrglue}. 
%The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
%During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
%However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
%The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 

Second is textual perturbation, replacing the words $x^k \in X$ to the noise word $t_{i}^{k}$ as follows:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix3, confusion_matrix5} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.

A representative of the above two categories is TOD-DA which embodies both categories. 
However, it ignores the context, thus it is outperformed by the third method~\cite{noisygen, asrglue}.

Third is  the auto-regressive generation, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$ plausible noise words~\cite{noisygen}.


Auto-regressive generation is biased to ASR$_i$, limiting the SLU model used for ASR$_i$.% plausible noise words,
Our distinction is generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.% e a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
As an alternative, ASR correction 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT.
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperform ASR correction~\cite{asrglue}.
Therefore, we focus on SNI.






==> backup/240216/3_ours.tex <==
\section{Method}
We now formally define our ISNI, which aims to generate pseudo transcription that can robustify SLU tasks against ASR$_*$.
\subsection{Interventional SNI for Debiasing}
\label{interventional_sni}
For defining ISNI, we formally introduce how $do$-calculus debiases conventional likelihood, and such debias can generalize SNI beyond a particular ASR.
%Our first step for such goal is to debias the dependence of SNI on ASR$_i$ with do-calculus.
%Before we explain our Interventional SNI, we introduce do-calculus.
Do-calculus aims to more robustly understand the causal effect of variable $X$ on another variable $Y$.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
Consider a specific value of $X$ strongly correlated to $z$, thus, has large $P(z|X)$. $P(Y|X)$ would be influenced by the value of $P(Y |X, z)$, even when the other value of $X$ would have different $P(Y |X, z)$.
Do-calculus reduces such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(X))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no longer influenced by $X$, thus the influence of $X$ on $Y$ through the mediator $z$ is mitigated.


%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Now, we formally reveal that the SNI model depends on ASR$_i$.
Using the variable $z$, the SNI process can be written as follows:
\begin{equation}
     P(t^{k}|x^{k}) = \sum_{z}P(t^{k}|x^{k},z)\cdot P(z|x^{k}).
     \label{eq:sni_definition}
\end{equation}
Then, the SNI model $P(t^{k}|x^{k})$ is biased to ASR$_i$ such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }




To debias the dependence on ASR$_i$, we propose to intervene $z$, so that the pseudo transcript would contain diverse noise words even when they are rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
Specifically, we reduce any influence from the intervened variable, $x^k$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
As a result of the intervention in Eq.~\ref{eq:do-calculus}, whether or not to corrupt the words $x^k$ is determined independently from ASR$_i$ so that rarely corrupted words $x^k$ would be corrupted in the pseudo transcription.
Specifically, for each word $x^k$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$, which determines whether the word $x^k$ would be corrupted.
If $d^k\leq P(z)$, $z$ is set as 1, and $t^{k}$ would be a noise word and need to be generated.
Otherwise, $z$ is set to 0, and $t^{k}$ would be identical to $x^{k}$ as a simulation of the successful transcription.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x^{k}$, which we set as a hyperparameter.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.

%The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
%Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
%Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.
To control the $z$, We model $P(t^{k}|x^{k},z)$ adopting constrained generation, where decoder is fed $x^{k}$ and outputs $t^{k}$.
To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ are word and position embeddings.
We note that dummy tokens are inserted between adjacent tokens in $X$ during the preprocessing step following \citet{constdecoder}.

The transformer decoder~\cite{NIPS2017_3f5ee243} generates $t^{k}$ constrained on $x^k$.
Specifically, the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E_{decoder}^{k}=M_{d}[e_{encoder}^{k}; bos],
    \label{eq:decoder_input}
\end{equation}
where  $M_d$ is the weight matrix of linear transformation.
The transformer decoder outputs the hidden representation $h^{k}$ as follows:
\begin{align}
    h^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K=E_{encoder},V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution $\textit{P}_{lm}(\hat{t}^{k}|x^{k})$ measures the probability of each token in vocabulary to be noise word $t^k$ as follows:
\begin{equation}
    \textit{P}_{lm}(\hat{t}^{k}|x^{k}) = softmax(M_{word} \cdot h^{k}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 
Here, we note that ISNI generates different error types depending on the output as we explained in Sec.~\ref{sec:overview}.

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t^{k}$ as follows:
\begin{equation}
    l_{lm} =-\sum log(\textit{P}_{lm}(t^{k}|x^{k})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to ensure the noise word generation ASR$_*$-plausible.
%The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
%To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
To reduce the bias of ASR$_i$ in $P(t^k|x^{k})$, we adjust the generation probability $\textit{P}_{lm}(\hat{t}^{k}|x^{k})$ with the phoneme-based generation probability $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{equation}
    \textit{P}_{gen}(\hat{t}^{k}|x^{k}) = \textit{P}_{lm}(\hat{t}^{k}|x^{k}) \cdot \textit{P}_{phoneme}(\hat{t}^{k}|x^{k})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ is to provide phonetic information via phoneme embedding $M_{phoneme}$.
%The main difficulty of evaluating $\textit{P}_{phoneme}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $M_{phoneme}$ is designed to have the phonetic information of each token in the vocabulary.
$M_{phoneme}$ can contain such information as tokens with identical phonetic codes have identical phoneme embedding. 
Thus, feeding the phoneme embedding $M_{phoneme}$ can deliver how each word in written sentences is pronounced.
The input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{phoneme}(X)+M_{position}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, the decoder would yield the hidden representation $h^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^k$ to evaluate the phoneme based generation probability $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ as follows:
\begin{equation}
    \textit{P}_{phoneme}(\hat{t}^{k}|x^{k}) = softmax(M_{phoneme} \cdot h^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $M_{phoneme}$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $M_{phoneme}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ can be evaluated based on the phonetic information.


Our second proposal for $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$-plausible noise words, $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ should evaluate how phonetically similar each token is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$.
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance $\textit{D}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{D}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{D}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 
It is noteworthy that $S$ is computed based on articulatory features, thus, not equal to 1 as it is normally used when computing word error rates.


To supervise $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ is supervised by loss defined as follows:
 \begin{equation}
     l_{phoneme} = l_{KL}(\textit{P}_{phoneme}(\hat{t}^{k}|x^{k}),  \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $l_{KL}$ is the KL divergence loss.
Finally, our proposed ISNI model is optimized to jointly minimize the total loss $l_{tot}$ which is defined as follows:
\begin{equation}
    l_{tot} = l_{lm} + \lambda_{phoneme} \cdot l_{phoneme},
\end{equation}
where $\lambda_{phoneme}$ is the weight of $l_{phoneme}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{phoneme}(\hat{t}^k|x^{k})$ can ensure the ASR$_*$-plausible noise words and $M_{phoneme}$ can contain phonetic information.
 

 




==> backup/240216/4_experiment.tex <==
\section{Experiments}
In this paper, we first experimentally confirm the validity of the ASR zero-shot setting, where SNI trained with ASR$_i$ cannot robustify against ASR$_j$ and the effectiveness of our proposed methods in the ASR zero-shot setting.
%For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.
Then, we show that our proposed methods can robustify various SLU tasks in the ASR zero-shot settings better than previous SNI methods.
\subsection{Dataset}
\label{sec:dataset}
To test the ASR generalizability, we formulated an ASR zero-shot setting by adopting ASR systems with distinct architecture and training sets to transcribe SNI and downstream tasks. 
For training the SNI model, we used the Mozilla DeepSpeech~\cite{deepspeech}\footnote{https://github.com/mozilla/DeepSpeech}.
The audio of each downstream task, DSTC10 Track 2 and ASR GLUE benchmark, is transcribed by distinct ASR systems different from DeepSpeech.
We provide further details of ASR systems in Sec.~\ref{sec:asr_details}.

%\input{table/dataset_statistics}

For training the SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1, to collect ASR error transcriptions.
Specifically, we put the audio recordings of the above corpora into the DeepSpeech and get ASR transcriptions. 
Then, we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR error transcriptions would remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.



\input{table/asrglue_result}
ASR GLUE benchmark is an SLU version of the widely adopted NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which the DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.

DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken language.
We adopt the DSTC10 Track2 dataset as it contains various tasks in NLP in the dialogue domain where SLU is required frequently.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS), and Knowledge-grounded Response Generation (RG), where human responses are transcribed by an unknown ASR system.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a classification. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 





\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{NIPS2017_3f5ee243} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our ISNI for 20 epochs with Adam optimizer with a learning rate of 0.00005.
Also, we set $\lambda_{w}$ and $\lambda_{phoneme}$ as 0.5 to balance the semantic and phonetic information. 

Using the trained ISNI, the written GTs in DSTC10 Track2 dataset and ASR GLUE dataset are converted into pseudo transcripts.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset based on the validation set result of downstream SLU tasks\footnote{Simply matching $P(z)$ to WER of the ASR system used for the SLU is seemingly straightforward but unfortunately inapplicable to ASR zero-shot setting where WER is unknown for unknown ASR. Also, training in arbitrary word error rates can cause the SLU model to be biased in certain ASR systems.}.
As downstream task models, we adopted the GPT2-small for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}







\subsection{Baselines}
%Our main baseline is Noisy-Gen, GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
We adopt Noisy-Gen, GPT2-based auto-regressive generation SNI model, as our main baseline.
It showed the most competitive results in various spoken language tasks such as SLU and spoken language translation~\cite{noisygen,asrglue}.
Noisy-Gen is trained with a training set identical to ours.
Pseudo-transcriptions generated by Noisy-Gen are filtered by phoneme-based heuristics. 

For ASR GLUE benchmark, we adopt another baseline Noisy-Gen (In Domain)~\cite{asrglue}.
Noisy-Gen and Noisy-Gen (In Domain) are similar in that they are both GPT2-based SNI models.
However, Noisy-Gen (In Domain) uses the identical ASR system to transcribe the test set of ASR GLUE benchmark (TDNN LF-MMI), which is improbable in the ASR zero-shot setting.
Comparing with Noisy-Gen (In Domain) can show how SNI models are successful in ASR generalizability.

For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
TOD-DA encompasses both the TTS-ASR pipeline and
textual perturbation techniques.
It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
Also, it conducted character-level perturbation of substitution, insertion and deletion, and swap and split.








==> backup/240216/5_results.tex <==
\section{Results}


\input{table/dstc_result}
We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are our proposed methods in the ASR zero-shot setting?

%\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ2:} Can our proposed methods robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ3:} Does each of our proposed methods contribute to robustification?

\subsection{RQ1: Validity of ASR zero-shot setting and effectiveness of our proposed methods. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.


First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Noisy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.





%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ours showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
Specifically, ours outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can make SLU models ASR generalizable in the ASR zero-shot setting.


In addition, ours robustify against different noise levels.
Specifically, ours showed little degradation in performance as noise levels increased compared to baselines.
That is, as prior work suggests, phoneme confusions more frequently occur~\cite{wu2022phonetic,petkov2013maximizing} and ours can robustify even when such phoneme confusion increases.




%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.








\subsection{RQ2: Robustification of Our Proposed Methods on Various SLU Tasks.}
In this section, we show that our proposed methods can better robustify various SLU tasks over different SNI methods in ASR zero-shot setting.
%As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
Different from the previous observations where the identical ASR system is used for SNI and SLU tasks~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed the increase of the BLEU score by 2-3x times for RG.
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.



\subsection{RQ3: Importance of Each Proposed Method to the Robustification. }
To confirm that each of our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.

We report the result without the phoneme-aware generation in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme-aware generation showed a decreased score in every subtask, showing the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.
To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
The last row of Table~\ref{tab:dstc_results} shows the increased performance of KTD. 
We suspect the degradation of KTD is due to its characteristic of text classification.
Previous work suggests that text classification in noisy text can decrease even when the noise in the training set is increased~\cite{4470224}.
The diversified noise of our proposed method, do-calculus, may contribute to an increase in the noise.
However, the performance is decreasing as expected in KS, which is our main consideration as it is largely influenced by lexical perturbation due to the ASR errors.
Such decrease is also observed in RG, showing that substituting the intervention contributes to the decreased performance in KS and RG.







==> backup/240216/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we have addressed the challenge of ASR generalizability within the context of SNI. Specifically, our focus was on enhancing the robustness of downstream SLU models against ASR errors that may originate from diverse ASR systems. The existing SNI method is biased to a particular ASR system used for generating pseudo transcriptions.
To tackle the ASR generalizability issue, we introduce two key contributions: Interventional SNI and Phoneme-aware Generation. First, towards eliminating biases, Interventional SNI method significantly incorporates a wider range of ASR-plausible errors. However, such diversity should not interfere ASR-generic characteristcs, for which, our second step of Phoneme-aware Generation, leads to the generation of errors that are commonly plausible, or ASR$_*$ plausible.
Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/240216/limitations.tex <==
\paragraph{Limitations.}
We make use of DeepSpeech ASR system, for the reason of its similarity in performance to many commercial ASR systems as we will discuss in Sec.~\ref{sec:asr_details}.
However, our ISNI may not well be trained with different ASR systems due to several reasons.
A notable reason is the scarcity of the training set due to rare ASR errors.
As we described in Sec.~\ref{sec:dataset}, we only use the erroneous transcriptions for training ISNI.
However, when the ASR system is too strong, it may make not enough erroneous transcriptions to train ISNI.
The most straightforward method is to use the other weaker ASR system for training, as our ISNI can generalize to different ASR systems.
Second, previous works suggest training the weaker version of the ASR system and using it for training SNI~\cite{dutta2022error}.





==> backup/240216_1745/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) as a pipeline where transcriptions from automatic speech recognition (ASR) systems are input to PLMs.
While the quality of transcriptions is critical in such pipeline,
ASR systems often incorrectly transcribe the spoken language into phonetically similar but semantically different words.
Our target problem is training SLU models to tolerate ASR errors, by exposing them to noises that are likely to be observed in ASR systems, which are denoted as ASR plausible noises.
Speech noise injection (SNI) achieves such goal by introducing ASR plausible noises to the written text.
ASR plausible noises are inevitably conditional to a particular ASR, ASR$_i$, while it is not necessarily so in another ASR, ASR$_j$, biasing PLMs to be used for ASR$_i$.
To ensure SLU models not to be biased to ASR$_i$ used for SNI,
we propose two phases: We first mitigate biases to ASR$_i$, then we ensure our
augmentation to satisfy ASR-generic plausibility that holds for any ASR system, ASR$_*$.
Experimental results and analysis show the effectiveness of our proposed methods in improving the robustness and generalizability of SLU models against unseen ASR systems, by introducing more diverse and plausible ASR noises in advance.
\end{abstract}

==> backup/240216_1745/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240216_1745/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240216_1745/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/240216_1745/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs thus have gained widespread acceptance and employment within the realm of spoken language understanding (SLU) as applied in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
A concrete instance of this application involves a pipeline leveraging PLMs subsequent to the automatic speech recognition system (ASR) transcribing audio inputs. The resulting transcriptions are input to PLMs to facilitate downstream SLU tasks~\cite{asrglue}.


However, such pipeline would encounter challenges when confronted with inaccuracies stemming from ASR systems.
We denote such inaccuracy as ASR error words, which are phonetically akin yet semantically unrelated~\cite{ruan20_interspeech,9054689}.
To illustrate, consider Fig.~\ref{fig:example}, 
where ASR systems, confused between  ``cereal'' and ``serial'', ``quarry'' and ``carry'', may generate an incorrect transcription such as ``workers eat serial in the carry''.
Despite their phonetic resemblance, these ASR error words convey unintended meanings, thereby impeding the semantic understanding of speech in SLU tasks~\cite{belinkov2018synthetic}.




A well-known solution is annotating likely incorrect transcriptions, known as speech noise injection, or, SNI~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
An SLU corpus annotation typically starts from a corpus of written 
text as a ground truth (GT), recorded into audio, then
transcribed into text using ASR systems.
A more efficient alternative is, skipping the recording and transcription,
to directly corrupt the written GT, to
 introduce noise to the original written sentence, creating a pseudo transcript that closely aligns with the expected output of an ASR system.
 Desirably, SNI noise should be ``ASR-plausible'', indicating the pseudo transcript is likely to be generated by ASR systems.

\input{figure_latex/figure1}


 
By definition, as ASR plausibility is conditional to a particular ASR system, or ASR$_i$, previous methods have focused on mimicking the target ASR$_i$. 
To achieve this, these methods involve collecting the incorrect transcriptions generated by the target ASR$_i$ and subsequently corrupting the clean, written GTs into pseudo transcripts based on the errors observed~\cite{confusion_matrix, confusion_matrix2,noisygen}.
This process is designed to simulate the types of mistakes made by the target ASR$_i$. 
As a result, the probability of a word $x$ being corrupted $(z = 1)$ or not $(z = 0)$, denoted as $P(z|x)$, becomes closely aligned with the error patterns observed in both the real transcriptions produced by ASR$_i$ and the pseudo transcripts derived from this method. 
%For example, in Fig.~\ref{fig:example}, mimicking ASR 1 frequently corrupting `c', baseline SNI corrupts `cue' and `ceiling' in the pseudo transcripts.

%However, ASR$_i$ and another ASR system, ASR$_j$, have different $P(z|x)$~\cite{different_error_distribution}, limiting SLU models trained with pseudo transcripts to be used for ASR$_i$.
%For example, in Fig.~\ref{fig:example}, SNI with transcription by ASR$_1$ would corrupt the word `cue' and `ceiling' with character `c'.
%Training with such pseudo transcripts can only robustify SLU models against errors from ASR$_1$, not ASR$_2$.
%To avoid such failure, ASR$_i$ and ASR$_j$ and the other ASR systems should build their own SLU model.
%However, recent trends in scaling PLMs make such robustification more exhaustive.
However, as different ASR systems have different probability distributions $P(z|x)$, the SLU model trained with pseudo transcripts with ASR$_i$ cannot robustly process the ASR errors produced by another system, ASR$_j$. 
To avoid such issues requires building several SLU models for their corresponding ASR systems. 
However, recent trends of scaling up PLMs make such process computationally more expensive.





%In contrast, to generate pseudo transcripts that generalize beyond ASR$_i$, our distinctions are two-fold: 
%First, after generating noises conditional to ASR$_i$,
%we debias its dependence on ASR$_i$.
%Specifically, $do$-calculus intervenes in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$.
%It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
%For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.
Our distinction is to generate pseudo transcripts that can generalize beyond a specific ASR system. 
For this purpose, we introduce two technical contributions: 1) interventional noise injection and 2) phoneme-aware generation. 
Specifically, we start by debiasing the dependence of noises to the specific ASR system, ASR$_i$, by applying \textit{do}-calculus in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$. 
It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.




%Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$, GT word and ASR noise word are phonetically similar~\cite{serai2022hallucination}.
%Specifically, we supervise and feed how words are pronounced.
%Unaware of how words are pronounced, previous works generate ASR noise words plausible for no ASR system.  
%For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
%`serial'.
%Mimicking ASR$_{1}$ unaware of pronunciation results in replacing c with s (or, replacing `cue' with `sue').
%However, knowing that `c' can sound differently in other words, k sound, ours can generate noise word `queue', which is plausible regardless of the ASR system used, or ASR$_*$-plausible.
Then, we ensure the debiased noises follow common characteristics shared by any ASR, namely ASR$_*$, such that GT words and ASR noises become phonetically similar~\cite{serai2022hallucination}. 
Specifically, along with the words as textual input, we feed how words are pronounced together. 
Being aware of how words are pronounced, we could introduce ASR noises plausible regardless of a specific ASR system used, namely ASR$_*$-plausible. 
 


Experiments are conducted in ASR zero-shot setting where SNI models are trained on ASR$_i$ and the SLU task is tested on another ASR$_j$ on DSTC10 Track2 and ASR GLUE benchmark.
Results show that our proposed methods are effective in ASR generalization with comparable or even outperforming performance compared to the in-domain setting where ASR$_j$ is used to train the SNI model.



==> backup/240216_1745/2_prelim.tex <==
\section{Preliminaries}

Before we present our proposed Interventional SNI (ISNI), we formally define SNI then, briefly overview our ISNI and introduce related work as preliminaries.

\subsection{Problem Formulation}
SNI model can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
The resulting pseudo transcription, $T_i$, is used to train downstream SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ASR$_*$ plausible pseudo transcript $T_*$

\subsection{Overview of Our Proposed Approach}
\label{sec:overview}
\input{figure_latex/figure2}
In this section, we briefly overview the proposed ISNI in Fig.~\ref{fig:example2}.
%As we will detail in Sec.~\ref{interventional_sni}, to implement $do$-calculus, $P(z|x)$ should be explicitly controlled.
First, we debias the dependence on ASR$_i$ with $do$-calculus.
For such purpose, we control $z$ by implementing SNI with constrained decoding following \citet{constdecoder}.
%The auto-regressive generation where $z$ of each token $x$ is implicitly determined by PLMs
Determining $z$ following $do$-calculus, the tokens rarely corrupted in ASR$_{i}$ are noised in the pseudo transcripts.  
The token $x$ with $z=1$, `cue' in Fig.~\ref{fig:example2}, is fed to the constrained decoder.
Then, the constrained decoder generates the noise word $t$ which replaces $x$.

ISNI can noise the token $x$ into all conventional ASR error types, substitution/insertion/deletion~\cite{jurafsky2019speech}, depending on the output of the constrained decoder.
The most straightforward output is a new token that replaces $x$ and incurs a substitution error.
The constrained decoder can output new tokens in addition to $x$, queue uh in Fig.~\ref{fig:example2}.
Adding newly generated tokens, ISNI noises $x$ to an insertion error.
Deletion errors are made when the constrained decoder outputs an empty string.
Our ISNI generates these error types synthetically as the generated examples in Sec.~\ref{sec:pseudo_transcripts_examples} show.

Second, we further generalize debiased noise to be ASR$_*$ plausible by discouraging the generation of phonetically different noise.
%Second, we ensure that debiased noise to be ASR$_*$ plausible by discouraging the generation of phonetically different noise.
For such purpose, we provide the phonetic information of $x$, `kju' in Fig.~\ref{fig:example2}, and make ISNI aware of how $x$ is pronounced.
Also, the constrained decoder evaluates the generation probability based on the phonetic similarity that `c' is pronounced as the phoneme `k'.
As a result, ISNI generates the ASR$_*$ plausible noise word `queue' which is phonetically similar to `cue'.



\subsection{Related Work}
\subsubsection{SNI}
Previously proposed methods can be categorized in three categories. %, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation.%, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
First, TTS (Text-to-Speech)-ASR pipeline~\cite{tts_asr, tts_asr2} adopts the TTS engine, the reverse of ASR, to convert written text into audio.
The ASR$_i$ transcribes it into pseudo transcription. 
However, the human recording and TTS-generated audio differ in their error distributions, which makes the resulting pseudo transcriptions different from ASR transcriptions~\cite{asrglue}. 
%The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
%During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
%However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
%The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 

Second is textual perturbation, replacing the words $x^k \in X$ to the noise word $t_{i}^{k}$ as follows:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix3, confusion_matrix5} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.

A representative of the above two categories is TOD-DA which embodies both categories. 
However, it ignores the context, thus it is outperformed by the third method~\cite{noisygen, asrglue}.

Third is  the auto-regressive generation, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$ plausible noise words~\cite{noisygen}.


Auto-regressive generation is biased to ASR$_i$, limiting the SLU model used for ASR$_i$.% plausible noise words,
Our distinction is generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.% e a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
As an alternative, ASR correction 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT.
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperform ASR correction~\cite{asrglue}.
Therefore, we focus on SNI.






==> backup/240216_1745/3_ours.tex <==
\section{Method}
We now formally define our ISNI, which aims to generate pseudo transcription that can robustify SLU tasks against ASR$_*$.
\subsection{Interventional SNI for Debiasing}
\label{interventional_sni}
For defining ISNI, we formally introduce how $do$-calculus debiases conventional likelihood, and such debias can generalize SNI beyond a particular ASR.
%Our first step for such goal is to debias the dependence of SNI on ASR$_i$ with do-calculus.
%Before we explain our Interventional SNI, we introduce do-calculus.
Do-calculus aims to more robustly understand the causal effect of variable $X$ on another variable $Y$.
Using Bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, the likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
Consider a specific value of $X$ strongly correlated to $z$, thus, has large $P(z|X)$. $P(Y|X)$ would be influenced by the value of $P(Y |X, z)$, even when the other value of $X$ would have different $P(Y |X, z)$.
Do-calculus reduces such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(X))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no longer influenced by $X$, thus the influence of $X$ on $Y$ through the mediator $z$ is mitigated.


%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Now, we formally reveal that the SNI model depends on ASR$_i$.
Using the variable $z$, the SNI process can be written as follows:
\begin{equation}
     P(t^{k}|x^{k}) = \sum_{z}P(t^{k}|x^{k},z)\cdot P(z|x^{k}).
     \label{eq:sni_definition}
\end{equation}
Then, the SNI model $P(t^{k}|x^{k})$ is biased to ASR$_i$ such that the word rarely corrupted by ASR$_i$, or, of large $P_i(z=0|x^k)$, yields large $P(t^k=x^k|x^k)$, the probability of leaving $x^k$ not noised.
Even though another ASR, ASR$_{j}$, may transcribe $x^k$ incorrectly, $P_i(z=1|x^k)$ would be low due to bias toward ASR$_i$. 
%such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }




To debias the dependence on ASR$_i$, we propose to intervene $z$, so that the pseudo transcript would contain diverse noise words even when they are rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
Specifically, we reduce any influence from the intervened variable, $x^k$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
As a result of the intervention in Eq.~\ref{eq:do-calculus}, whether or not to corrupt the words $x^k$ is determined independently from a specific ASR system, ASR$_i$, so that rarely corrupted words would be corrupted too in the pseudo transcripts. 
Specifically, for each word $x^k$, we sample random variable $a^k$ from the continuous uniform distribution of interval $[0,1]$, which determines whether the word $x^k$ would be corrupted.
If $a^k\leq P(z)$, $z$ is set as 1, and $t^{k}$ would be a noise word and need to be generated.
Otherwise, $z$ is set to 0, and $t^{k}$ would be identical to $x^{k}$ mimicking the successful transcription.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x^{k}$, which we set as a constant hyperparameter for pseudo transcript generation.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.

%The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
%Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
%Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.
As constrained generation outputs $t^{k}$ to input $x^{k}$, we adopt it to control the $z$ and remove the bias toward a specific ASR.
%Adopting constrained generation, we model $P(t^{k}|x^{k},z)$ and can control $z$, as 
%To control the $z$, we model $P(t^{k}|x^{k},z)$ adopting constrained generation, where decoder is fed $x^{k}$ and outputs $t^{k}$.
To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ are word and position embeddings.
%We note that dummy tokens are inserted between adjacent tokens in $X$ during the preprocessing step following \citet{constdecoder}.

The transformer decoder~\cite{NIPS2017_3f5ee243} generates $t^{k}$ constrained on $x^k$.
Specifically, the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E_{decoder}^{k}= H_{decoder} \cdot [e_{encoder}^{k}; bos],
    \label{eq:decoder_input}
\end{equation}
where $H_{decoder}$ is the weight matrix of the hidden layer.
The transformer decoder outputs the hidden representation $d^{k}$ as follows:
\begin{align}
    d^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K,V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, we measure the probability of each token in vocabulary to be noise word $t^k$, $P_{written}(\hat{t}^k|x^k)$, as follows:
\begin{equation}
    \textit{P}_{written}(\hat{t}^{k}|x^{k}) = softmax(M_{word} \cdot d^{k}+b_{written}),
    \label{eq:gen_prob}
\end{equation}
where $b_{written}$ are trained parameters. 
Here, we note that ISNI generates different error types depending on the output as we explained in Sec.~\ref{sec:overview}.

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t^{k}$ as follows:
\begin{equation}
    l_{written} =-\sum log(\textit{P}_{written}(t^{k}|x^{k})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to ensure the noise word generation ASR$_*$-plausible.
%The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
%To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
To reduce the bias of ASR$_i$ in $P(t^k|x^{k})$, we adjust the generation probability $\textit{P}_{lm}(\hat{t}^{k}|x^{k})$ with the phoneme-based generation probability $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{equation}
    \textit{P}_{gen}(\hat{t}^{k}|x^{k}) = \textit{P}_{written}(\hat{t}^{k}|x^{k}) \cdot \textit{P}_{phoneme}(\hat{t}^{k}|x^{k}).  
    \label{eq:phoneme_correction_prob}
\end{equation}
We here note that 

Our first proposal for $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ is to provide phonetic information via phoneme embedding $M_{phoneme}$.
%The main difficulty of evaluating $\textit{P}_{phoneme}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $M_{phoneme}$ is designed to have the phonetic information of each token in the vocabulary.
$M_{phoneme}$ can contain such information as tokens with identical phonetic codes have identical phoneme embedding. 
Thus, feeding the phoneme embedding $M_{phoneme}$ can deliver how each word in written sentences is pronounced.
Specifically, phoneme embedding is fed to the encoder with word and position embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{phoneme}(X)+M_{position}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, the decoder would yield the hidden representation $d^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we feed the hidden representation $d^k$ to classification head to evaluate the phoneme based generation probability $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ as follows:
\begin{equation}
    \textit{P}_{phoneme}(\hat{t}^{k}|x^{k}) = softmax(M_{phoneme} \cdot d^{k}+b_{phoneme}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where classification head has the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} for weight matrix and bias $b_{phoneme}$.
Using the phoneme embedding $M_{phoneme}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ can be evaluated based on the phonetic information.
%Then, we feed the hidden representation $h^k$ to classification head with weight matrix is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{phoneme}$  evaluate the phoneme based generation probability $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ as follows:


Our second proposal for $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$-plausible noise words, $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ should evaluate how phonetically similar each token is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$.
\begin{comment}
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance $\textit{D}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{D}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{D}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 
It is noteworthy that $S$ is computed based on articulatory features, thus, not equal to 1 as it is normally used when computing word error rates.
\end{comment}
pecifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance  $\textit{D}(w^{p}, w^{q})$ can measure how similar the word pair $(w^{p}, w^{q})$ is by measuring the minimum edit distance between the phonetic codes of the input word pair.
It is noteworthy that $\textit{D}(w^{p}, w^{q})$ is computed based on articulatory features, thus, it incrementally increases when the word pair is pronounced more similarly.
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 


To supervise $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})$ is supervised by loss defined as follows:
 \begin{equation}
     l_{phoneme} = KL(\textit{P}_{phoneme}(\hat{t}^{k}|x^{k})| \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $KL$ is the KL divergence loss.
Finally, our proposed ISNI model is optimized to jointly minimize the total loss $l_{tot}$ which is defined as follows:
\begin{equation}
    l_{tot} = l_{written} + \lambda_{phoneme} \cdot l_{phoneme},
\end{equation}
where $\lambda_{phoneme}$ is the weight of $l_{phoneme}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{phoneme}(\hat{t}^k|x^{k})$ can ensure the ASR$_*$-plausible noise words and $M_{phoneme}$ can contain phonetic information.
 

 




==> backup/240216_1745/4_experiment.tex <==
\section{Experiments}
In this paper, we first experimentally confirm the validity of the ASR zero-shot setting, where SNI trained with ASR$_i$ cannot robustify against ASR$_j$ and the effectiveness of our proposed methods in the ASR zero-shot setting.
%For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.
Then, we show that our proposed methods can robustify various SLU tasks in the ASR zero-shot settings better than previous SNI methods.
\subsection{Dataset}
\label{sec:dataset}
To test the ASR generalizability, we formulated an ASR zero-shot setting by adopting ASR systems with distinct architecture and training sets to transcribe SNI and downstream tasks. 
For training the SNI model, we used the Mozilla DeepSpeech~\cite{deepspeech}\footnote{https://github.com/mozilla/DeepSpeech}.
The audio of each downstream task, DSTC10 Track 2 and ASR GLUE benchmark, is transcribed by distinct ASR systems different from DeepSpeech.
We provide further details of ASR systems in Sec.~\ref{sec:asr_details}.

%\input{table/dataset_statistics}

For training the SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1, to collect ASR error transcriptions.
Specifically, we put the audio recordings of the above corpora into the DeepSpeech and get ASR transcriptions. 
Then, we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR error transcriptions would remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.



\input{table/asrglue_result}
ASR GLUE benchmark is an SLU version of the widely adopted NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which the DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.

DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken language.
We adopt the DSTC10 Track2 dataset as it contains various tasks in NLP in the dialogue domain where SLU is required frequently.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS), and Knowledge-grounded Response Generation (RG), where human responses are transcribed by an unknown ASR system.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a classification. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 





\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{NIPS2017_3f5ee243} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our ISNI for 20 epochs with Adam optimizer with a learning rate of 0.00005.
Also, we set $\lambda_{w}$ and $\lambda_{phoneme}$ as 0.5 to balance the semantic and phonetic information. 

Using the trained ISNI, the written GTs in DSTC10 Track2 dataset and ASR GLUE dataset are converted into pseudo transcripts.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset based on the validation set result of downstream SLU tasks\footnote{Simply matching $P(z)$ to WER of the ASR system used for the SLU is seemingly straightforward but unfortunately inapplicable to ASR zero-shot setting where WER is unknown for unknown ASR. Also, training in arbitrary word error rates can cause the SLU model to be biased in certain ASR systems.}.
As downstream task models, we adopted the GPT2-small for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}







\subsection{Baselines}
%Our main baseline is Noisy-Gen, GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
We adopt Noisy-Gen, GPT2-based auto-regressive generation SNI model, as our main baseline.
It showed the most competitive results in various spoken language tasks such as SLU and spoken language translation~\cite{noisygen,asrglue}.
Noisy-Gen is trained with a training set identical to ours.
Pseudo-transcriptions generated by Noisy-Gen are filtered by phoneme-based heuristics. 

For ASR GLUE benchmark, we adopt another baseline Noisy-Gen (In Domain)~\cite{asrglue}.
Noisy-Gen and Noisy-Gen (In Domain) are similar in that they are both GPT2-based SNI models.
However, Noisy-Gen (In Domain) uses the identical ASR system to transcribe the test set of ASR GLUE benchmark (TDNN LF-MMI), which is improbable in the ASR zero-shot setting.
Comparing with Noisy-Gen (In Domain) can show how SNI models are successful in ASR generalizability.

For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
TOD-DA encompasses both the TTS-ASR pipeline and
textual perturbation techniques.
It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
Also, it conducted character-level perturbation of substitution, insertion and deletion, and swap and split.








==> backup/240216_1745/5_results.tex <==
\section{Results}


\input{table/dstc_result}
We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are our proposed methods in the ASR zero-shot setting?

%\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ2:} Can our proposed methods robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ3:} Does each of our proposed methods contribute to robustification?

\subsection{RQ1: Validity of ASR zero-shot setting and effectiveness of our proposed methods. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.


First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Noisy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.





%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ours showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
Specifically, ours outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can make SLU models ASR generalizable in the ASR zero-shot setting.


In addition, ISNI robustifies SLU models against different noise levels.
Specifically, ours showed little degradation in performance as noise levels increased compared to baselines.
That is, as prior work suggests, phoneme confusions more frequently occur~\cite{wu2022phonetic,petkov2013maximizing} and ours can robustify even when such phoneme confusion increases.




%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.








\subsection{RQ2: Robustification of Our Proposed Methods on Various SLU Tasks.}
In this section, we show that our proposed methods can better robustify various SLU tasks over different SNI methods in ASR zero-shot setting.
%As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
Different from the previous observations where the identical ASR system is used for SNI and SLU tasks~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed the increase of the BLEU score by 2-3x times for RG.
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.



\subsection{RQ3: Importance of Each Proposed Method to the Robustification. }
To confirm that each of our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.

We report the result without the phoneme-aware generation in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme-aware generation showed a decreased score in every subtask, showing the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.
To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
The last row of Table~\ref{tab:dstc_results} shows the increased performance of KTD. 
We suspect such increase in KTD is due to its characteristic of text classification.
Previous work suggests that the text classification may fail robustification when the noises are abundant in the training set~\cite{4470224}, which our proposed method may contribute.
However, the performance is decreasing as expected in KS, which is our main consideration as it is largely influenced by lexical perturbation due to the ASR errors.
Such decrease is also observed in RG, showing that substituting the intervention contributes to the decreased performance in KS and RG.
%Previous work suggests that the abundance of noises in the training set may fail robustification in text classification \cite{4470224}.






==> backup/240216_1745/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we have addressed the challenge of ASR generalizability within the context of SNI. Specifically, our focus was on enhancing the robustness of downstream SLU models against ASR errors that may originate from diverse ASR systems. The existing SNI method is biased to a particular ASR system used for generating pseudo transcriptions.
To tackle the ASR generalizability issue, we introduce two key contributions: Interventional SNI and Phoneme-aware Generation. First, towards eliminating biases, Interventional SNI method significantly incorporates a wider range of ASR-plausible errors. However, such diversity should not interfere ASR-generic characteristcs, for which, our second step of Phoneme-aware Generation, leads to the generation of errors that are commonly plausible, or ASR$_*$ plausible.
Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/240216_1745/limitations.tex <==
\paragraph{Limitations.}
We make use of DeepSpeech ASR system, for the reason of its similarity in performance to many commercial ASR systems as we will discuss in Sec.~\ref{sec:asr_details}.
However, our ISNI may not well be trained with different ASR systems due to several reasons.
A notable reason is the scarcity of the training set due to rare ASR errors.
As we described in Sec.~\ref{sec:dataset}, we only use the erroneous transcriptions for training ISNI.
However, when the ASR system is too strong, it may make not enough erroneous transcriptions to train ISNI.
The most straightforward method is to use the other weaker ASR system for training, as our ISNI can generalize to different ASR systems.
Second, previous works suggest training the weaker version of the ASR system and using it for training SNI~\cite{dutta2022error}.





==> backup/240413/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) as a pipeline where transcriptions from automatic speech recognition (ASR) systems are input to PLMs.
While the quality of transcriptions is critical in such pipeline,
ASR systems often incorrectly transcribe the spoken language into phonetically similar but semantically different words.
Our target problem is training SLU models to tolerate ASR errors, by exposing them to noises that are likely to be observed in ASR systems, which are denoted as ASR plausible noises.
Speech noise injection (SNI) achieves such goal by introducing ASR plausible noises to the written text.
ASR plausible noises are inevitably conditional to a particular ASR system while it is not necessarily so in the other ASR systems, biasing PLMs to be used for a particular ASR system.
To ensure SLU models not to be biased to a particular ASR system used for SNI,
we propose two phases: We first mitigate biases to a particular ASR system, then we ensure our
augmentation to satisfy ASR-generic plausibility that holds for any ASR system.
Experimental results and analysis show the effectiveness of our proposed methods in improving the robustness and generalizability of SLU models against unseen ASR systems, by introducing more diverse and plausible ASR noises in advance.
\end{abstract}

==> backup/240413/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240413/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240413/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/240413/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs thus have gained widespread acceptance and employment within the realm of spoken language understanding (SLU) as applied in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
A concrete instance of this application involves a pipeline leveraging PLMs subsequent to the automatic speech recognition system (ASR) transcribing audio inputs. The resulting transcriptions are input to PLMs to facilitate downstream SLU tasks~\cite{asrglue}.


However, such pipeline encounter challenges when confronted with inaccuracies stemming from ASR systems.
We denote such inaccuracy as ASR error words, which are phonetically akin yet semantically unrelated~\cite{ruan20_interspeech,9054689}.
To illustrate, consider Fig.~\ref{fig:example}, 
where ASR systems, confused between  ``cereal'' and ``serial'', ``quarry'' and ``carry'', may generate an incorrect transcription such as ``workers eat serial in the carry''.
Despite their phonetic resemblance, these ASR error words convey unintended meanings, thereby impeding the semantic understanding of speech in SLU tasks~\cite{belinkov2018synthetic}.




A well-known solution is annotating likely incorrect transcriptions, known as speech noise injection, or, SNI~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
An SLU corpus annotation typically starts from a corpus of written 
text as a ground truth (GT), recorded into audio, then
transcribed into text using ASR systems.
A more efficient alternative is, skipping the recording and transcription,
to directly corrupt the written GT, to
 introduce noise to the original written sentence, creating a pseudo transcript that closely aligns with the expected output of an ASR system.
 Desirably, SNI noise should be ``ASR-plausible'', indicating the pseudo transcript is likely to be generated by ASR systems.



\input{figure_latex/figure1}

By definition, as ASR plausibility is conditional to a particular ASR system, or ASR$_i$, previous methods have focused on mimicking the target ASR$_i$. 
To achieve this, these methods involve collecting the incorrect transcriptions generated by the target ASR$_i$ and subsequently corrupting the clean, written GTs into pseudo transcripts based on the errors observed~\cite{confusion_matrix, confusion_matrix2,noisygen}.
This process is designed to simulate the types of mistakes made by the target ASR$_i$. 
As a result, the probability of a word $x$ being corrupted $(z = 1)$ or not $(z = 0)$, denoted as $P(z|x)$, becomes closely aligned with the error patterns observed in both the real transcriptions produced by ASR$_i$ and the pseudo transcripts derived from this method.



However, as different ASR systems have different probability distributions $P(z|x)$, the SLU model trained with pseudo transcripts with ASR$_i$ cannot robustly understand the semantics from the ASR errors produced by another system, ASR$_j$. 
To avoid such issues requires building several SLU models for their corresponding ASR systems. 
However, recent trends of scaling up PLMs make such process computationally more expensive.





%In contrast, to generate pseudo transcripts that generalize beyond ASR$_i$, our distinctions are two-fold: 
%First, after generating noises conditional to ASR$_i$,
%we debias its dependence on ASR$_i$.
%Specifically, $do$-calculus intervenes in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$.
%It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
%For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.
Our distinction is to generate pseudo transcripts that can generalize beyond a specific ASR system. 
For this purpose, we introduce two technical contributions: 1) interventional noise injection and 2) phoneme-aware generation. 
Specifically, we start by debiasing the dependence of noises to the specific ASR system, ASR$_i$, by applying \textit{do}-calculus in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$. 
It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.




%Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$, GT word and ASR noise word are phonetically similar~\cite{serai2022hallucination}.
%Specifically, we supervise and feed how words are pronounced.
%Unaware of how words are pronounced, previous works generate ASR noise words plausible for no ASR system.  
%For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
%`serial'.
%Mimicking ASR$_{1}$ unaware of pronunciation results in replacing c with s (or, replacing `cue' with `sue').
%However, knowing that `c' can sound differently in other words, k sound, ours can generate noise word `queue', which is plausible regardless of the ASR system used, or ASR$_*$-plausible.
\begin{comment}
Then, we ensure the debiased noises follow common characteristics shared by any ASR, namely ASR$_*$, such that GT words and ASR noises become phonetically similar~\cite{serai2022hallucination}. 
Specifically, along with the words as textual input, we feed how words are pronounced together. 
Being aware of how words are pronounced, we could introduce ASR noises plausible regardless of the specific ASR system used, namely ASR$_*$-plausible. 
\end{comment}
    
Then, we ensure the debiased noises to be plausible for any ASR, namely ASR$_*$, such that GT words and ASR noises become phonetically similar following the common characteristics shared by ASR$_*$~\cite{serai2022hallucination}. 
Specifically, along with the words as textual input, we feed how words are pronounced together. 
Being aware of how words are pronounced, we could introduce ASR noises plausible regardless of the specific ASR system used, namely ASR$_*$-plausible. 



Experiments are conducted in ASR zero-shot setting where SNI models are trained on ASR$_i$ and the SLU task is tested on another ASR$_j$ on DSTC10 Track2 and ASR GLUE benchmark.
Results show that our proposed methods are effective in ASR generalization with comparable or even outperforming performance compared to the in-domain setting where ASR$_j$ is used to train the SNI model.



==> backup/240413/2_prelim.tex <==
\section{Related Work}
\subsection{SNI}
Previously proposed methods can be categorized in three categories. %, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation.%, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
First, TTS (Text-to-Speech)-ASR pipeline~\cite{tts_asr, tts_asr2} adopts the TTS engine, the reverse of ASR, to convert written text into audio.
The ASR$_i$ transcribes it into pseudo transcription. 
However, the human recording and TTS-generated audio differ in their error distributions, which makes the resulting pseudo transcriptions different from ASR transcriptions~\cite{asrglue}. 
%The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
%During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
%However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
%The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 

Second is textual perturbation, replacing the words $x^k \in X$ to the noise word $t_{i}^{k}$ as follows:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix3, confusion_matrix5} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.

A representative of the above two categories is TOD-DA which embodies both categories. 
However, it ignores the context, thus it is outperformed by the third method~\cite{noisygen, asrglue}.

Third is  the auto-regressive generation, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$ plausible noise words~\cite{noisygen}.


Auto-regressive generation is biased to ASR$_i$, limiting the SLU model used for ASR$_i$.% plausible noise words,
Our distinction is generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.% e a noised version given the ground-truth transcription.

\subsection{ASR Correction}
As an alternative, ASR correction 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT.
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperform ASR correction~\cite{asrglue}.
Therefore, we focus on SNI.






==> backup/240413/3_ours.tex <==
\section{Method}
Before we define our ISNI, first formally define our problem of SNI.
Then, we overview our ISNI and provide detailed methods of ISNI which aims to generate pseudo transcription that can robustify SLU tasks against ASR$_*$.

\subsection{Problem Formulation}
SNI model can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
The resulting pseudo transcription, $T_i$, is used to train downstream SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ``ASR${_*}$ plausible'' pseudo transcript T$_*$, a pseudo transcript that is ASR plausible for ASR$_*$.

\subsection{Overview of Our Proposed Approach}
\label{sec:overview}
\input{figure_latex/figure2}
In this section, we briefly overview our proposed ISNI which can generate debiased ASR$_*$ noises of different error types, as illustrated in Fig.~\ref{fig:example2}.
%As we will detail in Sec.~\ref{interventional_sni}, to implement $do$-calculus, $P(z|x)$ should be explicitly controlled.

First, we debias the dependence on ASR$_i$ with $do$-calculus.
Second, we further generalize debiased noise to be ASR$_*$ plausible by discouraging the generation of phonetically different noise.



For debiasing, we control $z$ by implementing SNI with constrained decoding following \citet{constdecoder}.
%The auto-regressive generation where $z$ of each token $x$ is implicitly determined by PLMs
Determining $z$ following $do$-calculus, the tokens rarely corrupted in ASR$_{i}$ are noised in the pseudo transcripts.  
The token $x$ with $z=1$, such as `cue' in Fig.~\ref{fig:example2}, is fed to the constrained decoder.
Then, the constrained decoder generates the noise word $t$ which replaces $x$.

ISNI can noise the token $x$ into all conventional ASR error types, substitution/insertion/deletion~\cite{jurafsky2019speech}, depending on the output of the constrained decoder (see Eq~\ref{eq:decoder} in Section~\ref{sec:interventional_sni}).
The most straightforward output is a new token that replaces $x$, which incurs a substitution error.
However, when the constrained decoder  output new tokens in addition to $x$, such as queue uh in Fig.~\ref{fig:example2},
%Adding newly generated tokens, 
ISNI noises $x$ to an insertion error.
Similarly, deletion errors can be simulated when the constrained decoder outputs an empty string.
Our ISNI generates these error types synthetically as the generated examples in Sec.~\ref{sec:pseudo_transcripts_examples} show.

For ASR$_*$ plausibility, we provide the phonetic information of $x$, `kju' in Fig.~\ref{fig:example2}, and make ISNI aware of how $x$ is pronounced.
Also, the constrained decoder evaluates the generation probability based on the phonetic similarity that `c' is pronounced as the phoneme `k'.
As a result, ISNI generates the ASR$_*$ plausible noise word `queue' which is phonetically similar to `cue'.



\subsection{Interventional SNI for Debiasing}
\label{sec:interventional_sni}
For defining ISNI, we formally introduce how $do$-calculus debiases conventional likelihood, and such debias can generalize SNI beyond a particular ASR.
%Our first step for such goal is to debias the dependence of SNI on ASR$_i$ with do-calculus.
%Before we explain our Interventional SNI, we introduce do-calculus.
Do-calculus aims to more robustly understand the causal effect of variable $X$ on another variable $Y$.
Using Bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, the likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
Consider a specific value of $X$ strongly correlated to $z$, thus, has large $P(z|X)$. $P(Y|X)$ would be influenced by the value of $P(Y |X, z)$, even when the other value of $X$ would have different $P(Y |X, z)$.
Do-calculus reduces such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(X))$ and $P(z)$ to \citet{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no longer influenced by $X$, thus the influence of $X$ on $Y$ through the mediator $z$ is mitigated.


%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Now, we formally reveal that the SNI model depends on ASR$_i$.
Using the variable $z$, the SNI process can be written as follows:
\begin{equation}
     P(t^{k}|x^{k}) = \sum_{z}P(t^{k}|x^{k},z)\cdot P(z|x^{k}).
     \label{eq:sni_definition}
\end{equation}
Then, the SNI model $P(t^{k}|x^{k})$ is biased to ASR$_i$ such that the word rarely corrupted by ASR$_i$, or, of large $P_i(z=0|x^k)$, yields large $P(t^k=x^k|x^k)$, the probability of leaving $x^k$ not noised.
Even though another ASR, ASR$_{j}$, may transcribe $x^k$ incorrectly, $P_i(z=1|x^k)$ would be low due to bias toward ASR$_i$. 
%such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }




To debias the dependence on ASR$_i$, we propose to intervene $z$, so that the pseudo transcript would contain diverse noise words even when they are rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
Specifically, we reduce any influence from the intervened variable, $x^k$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
As a result of the intervention in Eq.~\ref{eq:do-calculus}, whether or not to corrupt the words $x^k$ is determined independently from a specific ASR system, ASR$_i$, so that rarely corrupted words would be corrupted too in the pseudo transcripts. 
Specifically, for each word $x^k$, we sample random variable $a^k$ from the continuous uniform distribution of interval $[0,1]$, which determines whether the word $x^k$ would be corrupted.
If $a^k\leq P(z)$, we set $z$ as 1 meaning that we will simulate incorrect transcription of $x^k$, thus, we generate its noise word $t^{k}$.
Otherwise, $z$ is set to 0, and $t^{k}$ would be identical to $x^{k}$ mimicking the successful transcription of $x^{k}$.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x^{k}$, which we set as a constant hyperparameter for pseudo transcript generation.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.

%The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
%Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
%Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.
As constrained generation outputs $t^{k}$ to input $x^{k}$, we adopt it to control the $z$ and remove the bias toward a specific ASR.
%Adopting constrained generation, we model $P(t^{k}|x^{k},z)$ and can control $z$, as 
%To control the $z$, we model $P(t^{k}|x^{k},z)$ adopting constrained generation, where decoder is fed $x^{k}$ and outputs $t^{k}$.
To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ are word and position embeddings.
%We note that dummy tokens are inserted between adjacent tokens in $X$ during the preprocessing step following \citet{constdecoder}.

The transformer decoder~\cite{NIPS2017_3f5ee243} generates $t^{k}$ constrained on $x^k$.
Specifically, the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E_{decoder}^{k}= H_{decoder} \cdot [e_{encoder}^{k}; bos],
    \label{eq:decoder_input}
\end{equation}
where $H_{decoder}$ is the weight matrix of the hidden layer.
The transformer decoder outputs the hidden representation $d^{k}$ as follows:
\begin{align}
    d^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K,V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, we measure the probability of each token in vocabulary to be noise word $t^k$, $P_{n}(\hat{t}^k|x^k)$, as follows:
\begin{equation}
    \textit{P}_{n}(\hat{t}^{k}|x^{k}) = softmax(M_{word} \cdot d^{k}+b_{n}),
    \label{eq:gen_prob}
\end{equation}
where $b_{n}$ are trained parameters. 
Here, we note that ISNI generates different error types depending on the output as we explained in Sec.~\ref{sec:overview}.

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t^{k}$ as follows:
\begin{equation}
    l_{n} =-\sum log(\textit{P}_{n}(t^{k}|x^{k})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to ensure the noise word generation ASR$_*$ plausible.
%The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
%To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
To reduce the bias of ASR$_i$ in $P(t^k|x^{k})$, we adjust the generation probability $\textit{P}_{n}(\hat{t}^{k}|x^{k})$ with the phoneme-based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{equation}
    \textit{P}_{gen}(\hat{t}^{k}|x^{k}) = \textit{P}_{n}(\hat{t}^{k}|x^{k}) \cdot \textit{P}_{ph}(\hat{t}^{k}|x^{k}).  
    \label{eq:phoneme_correction_prob}
\end{equation}

Our first proposal for $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ is to provide phonetic information via phoneme embedding $M_{ph}$.
%The main difficulty of evaluating $\textit{P}_{ph}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $M_{ph}$ is designed to have the phonetic information of each token in the vocabulary.
$M_{ph}$ can contain such information as tokens with identical phonetic codes have identical phoneme embedding. 
Thus, feeding the phoneme embedding $M_{ph}$ can deliver how each word in written sentences is pronounced.
Specifically, phoneme embedding is fed to the encoder with word and position embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{ph}(X)+M_{position}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, the decoder would yield the hidden representation $d^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we feed the hidden representation $d^k$ to classification head to evaluate the phoneme based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ as follows:
\begin{equation}
    \textit{P}_{ph}(\hat{t}^{k}|x^{k}) = softmax(M_{ph} \cdot d^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where classification head has the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} for weight matrix and bias $b_{ph}$.
Using the phoneme embedding $M_{ph}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ can be evaluated based on the phonetic information.
%Then, we feed the hidden representation $h^k$ to classification head with weight matrix is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$  evaluate the phoneme based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ as follows:


Our second proposal for $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$plausible noise words, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ should evaluate how phonetically similar each token is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$.
\begin{comment}
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance $\textit{D}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{D}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{D}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 
It is noteworthy that $S$ is computed based on articulatory features, thus, not equal to 1 as it is normally used when computing word error rates.
\end{comment}
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance  $\textit{D}(w^{p}, w^{q})$ can measure how similar the word pair $(w^{p}, w^{q})$ is by measuring the minimum edit distance between the phonetic codes of the input word pair.
It is noteworthy that $\textit{D}(w^{p}, w^{q})$ is computed based on articulatory features, thus, it incrementally increases when the word pair is pronounced more similarly.
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 


To supervise $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ is supervised by loss defined as follows:
 \begin{equation}
     l_{ph} = KL(\textit{P}_{ph}(\hat{t}^{k}|x^{k})| \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $KL$ is the KL divergence loss.
Finally, our proposed ISNI model is optimized to jointly minimize the total loss $l_{tot}$ which is defined as follows:
\begin{equation}
    l_{tot} = l_{n} + \lambda_{ph} \cdot l_{ph},
\end{equation}
where $\lambda_{ph}$ is the weight of $l_{ph}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{ph}(\hat{t}^k|x^{k})$ can ensure the ASR$_*$plausible noise words and $M_{ph}$ can contain phonetic information.
 

 




==> backup/240413/4_experiment.tex <==
\section{Experiments}
In this paper, we first experimentally confirm the validity of the ASR zero-shot setting, where SNI trained with ASR$_i$ cannot robustify against ASR$_j$ and the effectiveness of our proposed methods in the ASR zero-shot setting.
%For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.
Then, we show that our proposed methods can robustify various SLU tasks in the ASR zero-shot settings better than previous SNI methods.
\subsection{Dataset}
\label{sec:dataset}
To test the ASR generalizability, we formulated an ASR zero-shot setting by adopting ASR systems with distinct architecture and training sets to transcribe SNI and downstream tasks. 
For training the SNI model, we used the Mozilla DeepSpeech~\cite{deepspeech}\footnote{https://github.com/mozilla/DeepSpeech}.
The audio of each downstream task, DSTC10 Track 2 and ASR GLUE benchmark, is transcribed by distinct ASR systems different from DeepSpeech.
We provide further details of ASR systems in Sec.~\ref{sec:asr_details}.

%\input{table/dataset_statistics}

For training the SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1, to collect ASR error transcriptions.
Specifically, we put the audio recordings of the above corpora into the DeepSpeech and get ASR transcriptions. 
Then, we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR error transcriptions would remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.



\input{table/asrglue_result}
ASR GLUE benchmark is an SLU version of the widely adopted NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which the DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.

DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken language.
We adopt the DSTC10 Track2 dataset as it contains various tasks in NLP in the dialogue domain where SLU is required frequently.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS), and Knowledge-grounded Response Generation (RG), where human responses are transcribed by an unknown ASR system.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a classification. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 





\subsection{Experimental Settings}
\paragraph{SNI Training}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{NIPS2017_3f5ee243} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our ISNI for 20 epochs with Adam optimizer with a learning rate of 0.00005.
Also, we set $\lambda_{w}$ and $\lambda_{phoneme}$ as 0.5 to balance the semantic and phonetic information. 

\paragraph{SLU Training}
Using the trained ISNI, the written GTs in DSTC10 Track2 dataset and ASR GLUE dataset are converted into pseudo transcripts.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset based on the validation set result of downstream SLU tasks\footnote{Matching $P(z)$ to word error rate of the ASR system used for the SLU seems straightforward but unfortunately inapplicable to ASR zero-shot setting where WER is unknown for unknown ASR. Also, training in arbitrary word error rates can cause the SLU model to be biased in certain ASR systems.}.
As downstream task models, we adopted the GPT2-small for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}







\subsection{Baselines}
%Our main baseline is Noisy-Gen, GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
We adopt Noisy-Gen, GPT2-based auto-regressive generation SNI model, as our main baseline.
It showed the most competitive results in various spoken language tasks such as SLU and spoken language translation~\cite{noisygen,asrglue}.
Noisy-Gen is trained with a training set identical to ours.
Pseudo-transcriptions generated by Noisy-Gen are filtered by phoneme-based heuristics. 

For ASR GLUE benchmark, we adopt another baseline Noisy-Gen (In Domain)~\cite{asrglue}.
Noisy-Gen and Noisy-Gen (In Domain) are similar in that they are both GPT2-based SNI models.
However, Noisy-Gen (In Domain) uses the identical ASR system to transcribe the test set of ASR GLUE benchmark (TDNN LF-MMI), which is improbable in the ASR zero-shot setting.
Comparing with Noisy-Gen (In Domain) can show how SNI models are successful in ASR generalizability.

For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
TOD-DA encompasses both the TTS-ASR pipeline and
textual perturbation techniques.
It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
Also, it conducted character-level perturbation of substitution, insertion and deletion, and swap and split.








==> backup/240413/5_results.tex <==
\section{Results}


\input{table/dstc_result}
We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are our proposed methods in the ASR zero-shot setting?

%\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ2:} Can our proposed methods robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ3:} Does each of our proposed methods contribute to robustification?

\subsection{RQ1: Validity of ASR zero-shot setting and effectiveness of our proposed methods. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.


First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Noisy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.





%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ours showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
Specifically, ours outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can make SLU models ASR generalizable in the ASR zero-shot setting.


In addition, ISNI robustifies SLU models against different noise levels.
Specifically, ours showed little degradation in performance as noise levels increased compared to baselines.
That is, as prior work suggests, phoneme confusions more frequently occur~\cite{wu2022phonetic,petkov2013maximizing} and ours can robustify even when such phoneme confusion increases.




%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.








\subsection{RQ2: Robustification of Our Proposed Methods on Various SLU Tasks.}
In this section, we show that our proposed methods can better robustify various SLU tasks over different SNI methods in ASR zero-shot setting.
%As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
Different from the previous observations where the identical ASR system is used for SNI and SLU tasks~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed the increase of the BLEU score by 2-3 times for RG.
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.



\subsection{RQ3: Importance of Each Proposed Method to the Robustification. }
To confirm that each of our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.

We report the result without the phoneme-aware generation in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme-aware generation showed a decreased score in every subtask, showing the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.
To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Performance is decreasing as expected in KS, which is our main consideration as it is largely influenced by lexical perturbation due to the ASR errors.
Such decrease is also observed in RG, showing that substituting the intervention contributes to the decreased performance in KS and RG.
Unexpectedly, the last row of Table~\ref{tab:dstc_results} shows the increased performance of KTD. 
We suspect such increase in KTD is due to its characteristic of text classification.
Meanwhile, prior work suggests that even the text classification may still degrade,  when the noises are more abundant in the training set~\cite{4470224}, to which our proposed method may contribute.

%Previous work suggests that the abundance of noises in the training set may fail robustification in text classification \cite{4470224}.






==> backup/240413/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we have addressed the challenge of ASR generalizability within the context of SNI. Specifically, our focus was on enhancing the robustness of downstream SLU models against ASR errors that may originate from diverse ASR systems. The existing SNI method is biased to a particular ASR system used for generating pseudo transcriptions.
To tackle the ASR generalizability issue, we introduce two key contributions: Interventional SNI and Phoneme-aware Generation. First, towards eliminating biases, Interventional SNI method significantly incorporates a wider range of ASR-plausible errors. However, such diversity should not interfere ASR-generic characteristcs, for which, our second step of Phoneme-aware Generation, leads to the generation of errors that are commonly plausible, or ASR$_*$ plausible.
Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/240413/limitations.tex <==
\paragraph{Limitations.}
We make use of DeepSpeech ASR system, for the reason of its similarity in performance to many commercial ASR systems as we will discuss in Sec.~\ref{sec:asr_details}.
However, our ISNI may not well be trained with different ASR systems due to several reasons.
A notable reason is the scarcity of the training set due to rare ASR errors.
As we described in Sec.~\ref{sec:dataset}, we only use the erroneous transcriptions for training ISNI.
However, when the ASR system is too strong, it may make not enough erroneous transcriptions to train ISNI.
The most straightforward method is to use the other weaker ASR system for training, as our ISNI can generalize to different ASR systems.
Second, previous works suggest training the weaker version of the ASR system and using it for training SNI~\cite{dutta2022error}.





==> backup/240414/3_ours.tex <==
\section{Method}
Before we define ISNI, first formally define our problem of SNI.
Then, we overview ISNI and provide detailed methods of ISNI which aims to generate pseudo transcription that can robustify SLU tasks against ASR$_*$.

\subsection{Problem Formulation}
SNI model can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
The resulting pseudo transcription, $T_i$, is used to train downstream SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ``ASR${_*}$ plausible'' pseudo transcript T$_*$, a pseudo transcript that is ASR plausible for ASR$_*$.

\subsection{Overview of Our Proposed Approach}
\label{sec:overview}
\input{figure_latex/figure2}
In this section, we briefly overview our proposed ISNI which can generate debiased ASR$_*$ noises of different error types, as illustrated in Fig.~\ref{fig:example2}.
%As we will detail in Sec.~\ref{interventional_sni}, to implement $do$-calculus, $P(z|x)$ should be explicitly controlled.

First, we debias the dependence on ASR$_i$ with $do$-calculus.
Second, we further generalize debiased noise to be ASR$_*$ plausible by discouraging the generation of phonetically different noise.



For debiasing, we control $z$ by implementing SNI with constrained decoding following \citet{constdecoder}.
%The auto-regressive generation where $z$ of each token $x$ is implicitly determined by PLMs
Determining $z$ following $do$-calculus, the tokens rarely corrupted in ASR$_{i}$ are noised in the pseudo transcripts.  
The token $x$ with $z=1$, such as `cue' in Fig.~\ref{fig:example2}, is fed to the constrained decoder.
Then, the constrained decoder generates the noise word $t$ which replaces $x$.

ISNI can noise the token $x$ into all conventional ASR error types, substitution/insertion/deletion~\cite{jurafsky2019speech}, depending on the output of the constrained decoder (see Eq~\ref{eq:decoder} in Section~\ref{sec:interventional_sni}).
The most straightforward output is a new token that replaces $x$, which incurs a substitution error.
However, when the constrained decoder  output new tokens in addition to $x$, such as queue uh in Fig.~\ref{fig:example2},
%Adding newly generated tokens, 
ISNI noises $x$ to an insertion error.
Similarly, deletion errors can be simulated when the constrained decoder outputs an empty string.
ISNI generates these error types synthetically as the generated examples in Sec.~\ref{sec:pseudo_transcripts_examples} show.

For ASR$_*$ plausibility, we provide the phonetic information of $x$, `kju' in Fig.~\ref{fig:example2}, and make ISNI aware of how $x$ is pronounced.
Also, the constrained decoder evaluates the generation probability based on the phonetic similarity that `c' is pronounced as the phoneme `k'.
As a result, ISNI generates the ASR$_*$ plausible noise word `queue' which is phonetically similar to `cue'.



\subsection{Interventional SNI for Debiasing}
\label{sec:interventional_sni}
For defining ISNI, we formally introduce how $do$-calculus debiases conventional likelihood, and such debias can generalize SNI beyond a particular ASR.
%Our first step for such goal is to debias the dependence of SNI on ASR$_i$ with do-calculus.
%Before we explain our Interventional SNI, we introduce do-calculus.
Do-calculus aims to more robustly understand the causal effect of variable $X$ on another variable $Y$.
Using Bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, the likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
Consider a specific value of $X$ strongly correlated to $z$, thus, has large $P(z|X)$. $P(Y|X)$ would be influenced by the value of $P(Y |X, z)$, even when the other value of $X$ would have different $P(Y |X, z)$.
Do-calculus reduces such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer the proof of transition between $P(z|do(X))$ and $P(z)$ to \citet{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no longer influenced by $X$, thus the influence of $X$ on $Y$ through the mediator $z$ is mitigated.


%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Now, we formally reveal that the SNI model depends on ASR$_i$.
Using the variable $z$, the SNI process can be written as follows:
\begin{equation}
     P(t^{k}|x^{k}) = \sum_{z}P(t^{k}|x^{k},z)\cdot P(z|x^{k}).
     \label{eq:sni_definition}
\end{equation}
Then, the SNI model $P(t^{k}|x^{k})$ is biased to ASR$_i$ such that the word rarely corrupted by ASR$_i$, or, of large $P_i(z=0|x^k)$, yields large $P(t^k=x^k|x^k)$, the probability of leaving $x^k$ not noised.
Even though another ASR, ASR$_{j}$, may transcribe $x^k$ incorrectly, $P_i(z=1|x^k)$ would be low due to bias toward ASR$_i$. 
%such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }




To debias the dependence on ASR$_i$, we propose to intervene $z$, so that the pseudo transcript would contain diverse noise words even when they are rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
Specifically, we reduce any influence from the intervened variable, $x^k$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
As a result of the intervention specified in Eq.~\ref{eq:do-calculus}, the decision to corrupt the words $x^k$ in the pseudo transcripts is made independently of any specific ASR system, such as ASR$_i$. 
This approach ensures that words which are typically rarely corrupted by ASR$_i$ can also be corrupted.
Specifically, for each word $x^k$, we sample random variable $a^k$ from the continuous uniform distribution of interval $[0,1]$, which determines whether the word $x^k$ would be corrupted.
If $a^k\leq P(z)$, we set $z$ as 1 meaning that we will simulate incorrect transcription of $x^k$, thus, we generate its noise word $t^{k}$.
Otherwise, $z$ is set to 0, and $t^{k}$ would be identical to $x^{k}$ mimicking the successful transcription of $x^{k}$.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x^{k}$, which we set as a constant hyperparameter for pseudo transcript generation.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.

%The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
%Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
%Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.
As constrained generation outputs $t^{k}$ to input $x^{k}$, we adopt it to control the $z$ and remove the bias toward a specific ASR.
%Adopting constrained generation, we model $P(t^{k}|x^{k},z)$ and can control $z$, as 
%To control the $z$, we model $P(t^{k}|x^{k},z)$ adopting constrained generation, where decoder is fed $x^{k}$ and outputs $t^{k}$.
To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ are word and position embeddings.
%We note that dummy tokens are inserted between adjacent tokens in $X$ during the preprocessing step following \citet{constdecoder}.

The transformer decoder~\cite{NIPS2017_3f5ee243} generates $t^{k}$ constrained on $x^k$.
Specifically, the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E_{decoder}^{k}= H_{decoder} \cdot [e_{encoder}^{k}; bos],
    \label{eq:decoder_input}
\end{equation}
where $H_{decoder}$ is the weight matrix of the hidden layer.
The transformer decoder outputs the hidden representation $d^{k}$ as follows:
\begin{align}
    d^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K,V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, we measure the probability of each token in vocabulary to be noise word $t^k$, $P_{n}(\hat{t}^k|x^k)$, as follows:
\begin{equation}
    \textit{P}_{n}(\hat{t}^{k}|x^{k}) = softmax(M_{word} \cdot d^{k}+b_{n}),
    \label{eq:gen_prob}
\end{equation}
where $b_{n}$ are trained parameters. 
Here, we note that ISNI generates different error types depending on the output as we explained in Sec.~\ref{sec:overview}.

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t^{k}$ as follows:
\begin{equation}
    l_{n} =-\sum log(\textit{P}_{n}(t^{k}|x^{k})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is To reduce the bias of ASR$_i$ in $P(t^k|x^{k})$ and ensure the noise word generation ASR$_*$ plausible.
%The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
%To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
We adjust the generation probability $\textit{P}_{n}(\hat{t}^{k}|x^{k})$ with the phoneme-based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{equation}
    \textit{P}_{gen}(\hat{t}^{k}|x^{k}) = \textit{P}_{n}(\hat{t}^{k}|x^{k}) \cdot \textit{P}_{ph}(\hat{t}^{k}|x^{k}).  
    \label{eq:phoneme_correction_prob}
\end{equation}

Our first proposal for $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ is to provide phonetic information via phoneme embedding $M_{ph}$.
%The main difficulty of evaluating $\textit{P}_{ph}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $M_{ph}$ is designed to have the phonetic information of each token in the vocabulary.
$M_{ph}$ can contain such information as tokens with identical phonetic codes have identical phoneme embedding. 
Thus, feeding the phoneme embedding $M_{ph}$ can deliver how each word in written sentences is pronounced.
Specifically, phoneme embedding is fed to the encoder with word and position embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{ph}(X)+M_{position}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, the decoder would yield the hidden representation $d^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we feed the hidden representation $d^k$ to classification head to evaluate the phoneme based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ as follows:
\begin{equation}
    \textit{P}_{ph}(\hat{t}^{k}|x^{k}) = softmax(M_{ph} \cdot d^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where classification head has the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} for weight matrix and bias $b_{ph}$.
Using the phoneme embedding $M_{ph}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ can be evaluated based on the phonetic information.
%Then, we feed the hidden representation $h^k$ to classification head with weight matrix is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$  evaluate the phoneme based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ as follows:


Our second proposal for $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$plausible noise words, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ should evaluate how phonetically similar each token is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$.
\begin{comment}
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance $\textit{D}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{D}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{D}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 
It is noteworthy that $S$ is computed based on articulatory features, thus, not equal to 1 as it is normally used when computing word error rates.
\end{comment}
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance  $\textit{D}(w^{p}, w^{q})$ can measure how similar the word pair $(w^{p}, w^{q})$ is by measuring the minimum edit distance between the phonetic codes of the input word pair.
It is noteworthy that $\textit{D}(w^{p}, w^{q})$ is computed based on articulatory features, thus, it incrementally increases when the word pair is pronounced more similarly.
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 


To supervise $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ is supervised by loss defined as follows:
 \begin{equation}
     l_{ph} = KL(\textit{P}_{ph}(\hat{t}^{k}|x^{k})| \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $KL$ is the KL divergence loss.
Finally, our proposed ISNI model is optimized to jointly minimize the total loss $l_{tot}$ which is defined as follows:
\begin{equation}
    l_{tot} = l_{n} + \lambda_{ph} \cdot l_{ph},
\end{equation}
where $\lambda_{ph}$ is the weight of $l_{ph}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{ph}(\hat{t}^k|x^{k})$ can ensure the ASR$_*$plausible noise words and $M_{ph}$ can contain phonetic information.
 

 




==> backup/240613/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLMs) have been increasingly adopted in spoken language understanding (SLU). 
However, automatic speech recognition (ASR) systems frequently produce inaccurate transcriptions, leading to noisy inputs for SLU models, which can significantly degrade their performance. 
To address this, our objective is to train SLU models to withstand ASR errors by exposing them to noises commonly observed in ASR systems, referred to as ASR-plausible noises. 
Speech noise injection (SNI) achieves this goal by introducing ASR-plausible noises, which are inherently biased towards specific ASR systems. 
Our approach first mitigates these biases by cutting of the non-causal effect and then ensures that augmentation satisfies ASR-generic plausibility applicable to any ASR system. 
Experimental results and analyses demonstrate the effectiveness of our proposed methods in enhancing the robustness and generalizability of SLU models against unseen ASR systems by introducing more diverse and plausible ASR noises in advance. %Specifically, our methods improved SLU model accuracy by X% when tested on unseen ASR systems, showcasing their potential for broader application.
\end{abstract}
\begin{comment}
    Recently, pre-trained language models (PLMs) have been adopted in spoken language understanding (SLU). 
As automatic speech recognition (ASR) systems often transcribe spoken language inaccurately, noisy inputs are introduced to SLU models. 
Our goal is to train SLU models to tolerate these ASR errors by exposing them to noises that are likely to be observed in ASR systems, which are denoted as ASR-plausible noises.
Speech noise injection (SNI) achieves such goal by introducing ASR-plausible noises that are inevitably biased to a particular ASR system.
Our distinction is first to mitigate biases towards a particular ASR system, then ensure
that augmentation to satisfy ASR-generic plausibility applicable to any ASR system.
Experimental results and analyses show the effectiveness of our proposed methods in improving the robustness and generalizability of SLU models against unseen ASR systems by introducing more diverse and plausible ASR noises in advance.
\end{comment}

==> backup/240613/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240613/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/240613/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/240613/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLMs) have demonstrated a robust contextual understanding of language and the ability to generalize across different domains. 
Thus, PLMs have gained widespread acceptance and are employed within the realm of spoken language understanding (SLU), such as voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}. 
A concrete instance of this application involves a pipeline that leverages PLMs after an automatic speech recognition (ASR) system transcribes audio inputs. 
The resulting transcriptions are then fed to PLMs to facilitate downstream SLU tasks~\cite{asrglue}.



\input{figure_latex/figure1}
However, such pipelines encounter challenges when faced with inaccuracies from ASR systems. 
We refer to these inaccuracies as ASR error words, which are phonetically similar but semantically unrelated~\cite{ruan20_interspeech,9054689}. 
For instance, as shown in Fig.~\ref{fig:example}, ASR systems might confuse words like ``cereal'' and ``serial'' or ``quarry'' and ``carry'', resulting in incorrect transcriptions such as ``workers eat serial in the carry''. 
Despite their phonetic resemblance, these ASR error words convey unintended meanings, thereby impeding the semantic understanding of speech in SLU tasks~\cite{belinkov2018synthetic}.



A well-known solution to address these inaccuracies is speech noise injection (SNI)~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}. 
Typically, SLU corpus annotation begins with a written text corpus as ground truth (GT), which is then recorded into audio and transcribed using ASR systems. 
A more efficient alternative is to skip the recording and transcription steps and directly corrupt the written GT, introducing noise to the original text. 
This creates a pseudo transcript that closely aligns with the expected output of an ASR system. 
Ideally, SNI noise should be ASR-plausible, indicating that the pseudo transcript is likely to be generated by ASR systems.


\yj{
By definition, ASR-plausibility is conditional on a particular ASR system, or ASR$_i$. 
Previous methods have focused on mimicking the target ASR$_i$ by collecting its incorrect transcriptions and analyzing its error patterns. 
These methods then corrupt clean, written GTs into pseudo transcripts by replicating these observed error patterns~\cite{confusion_matrix, confusion_matrix2,noisygen}.} 

\yj{
During this process, correct transcriptions from ASR$_i$ are excluded because they lack the necessary noise patterns for training. 
Thus, the inclusion of written GTs in the collection is influenced by the presence of errors from the target ASR$_i$, leading to a biased dataset.
}


%\yj{
%However, this influence induces a non-causal effect that hinders the generalization of SLU models across different ASR systems. 
%To achieve generalization, pseudo transcripts should contain diverse phoneme noises, as different ASR systems have distinct error distributions~\cite{asr_pattern1}.
%The filtering process, however, introduces a reporting bias where the presence of errors dictates the inclusion of clean texts in the training set. 
As the errors in the pseudo transcripts are biased towards the error patterns of ASR$_i$.
SLU models trained on these biased pseudo transcripts fail to
generalize  to errors from other ASR systems, such as ASR$_j$. 
While building multiple SLU models for each ASR system could address this issue, the increasing costs associated with scaling up PLMs make this approach impractical.
%}



%In contrast, to generate pseudo transcripts that generalize beyond ASR$_i$, our distinctions are two-fold: 
%First, after generating noises conditional to ASR$_i$,
%we debias its dependence on ASR$_i$.
%Specifically, $do$-calculus intervenes in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$.
%It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
%For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.
\yj{
Our distinction is to generate pseudo transcripts that can generalize beyond a specific ASR system. 
To achieve this, we introduce two technical contributions: 1) interventional noise injection and 2) phoneme-aware generation. 
We begin by debiasing the dependence of noises on the specific ASR system, ASR$_i$, by applying \textit{do}-calculus, which cuts off the influence of errors from the target ASR$_i$ during filtering. 
Instead of replicating the error patterns of ASR$_i$, we intervene in the decision to corrupt the written GTs independently from ASR$_i$, thereby broadening the error patterns in the resulting pseudo transcripts. 
For instance, as shown in Fig.~\ref{fig:example}, our SNI model can corrupt the word `Read' with the phoneme '\textturnr', which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the errors introduced by baseline SNI.
}



%Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$, GT word and ASR noise word are phonetically similar~\cite{serai2022hallucination}.
%Specifically, we supervise and feed how words are pronounced.
%Unaware of how words are pronounced, previous works generate ASR noise words plausible for no ASR system.  
%For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
%`serial'.
%Mimicking ASR$_{1}$ unaware of pronunciation results in replacing c with s (or, replacing `cue' with `sue').
%However, knowing that `c' can sound differently in other words, k sound, ours can generate noise word `queue', which is plausible regardless of the ASR system used, or ASR$_*$-plausible.
\begin{comment}
Then, we ensure the debiased noises follow common characteristics shared by any ASR, namely ASR$_*$, such that GT words and ASR noises become phonetically similar~\cite{serai2022hallucination}. 
Specifically, along with the words as textual input, we feed how words are pronounced together. 
Being aware of how words are pronounced, we could introduce ASR noises plausible regardless of the specific ASR system used, namely ASR$_*$-plausible. 
\end{comment}
    
Next, we ensure that the debiased noises are plausible for any ASR system, referred to as ASR$_*$. 
This involves making GT words and ASR noises phonetically similar based on the common characteristics shared by ASR$_*$~\cite{serai2022hallucination}. 
Along with the textual input, we incorporate information on how words are pronounced. 
By being aware of pronunciation, we can introduce ASR noises that are plausible regardless of the specific ASR system used, making them ASR$_*$-plausible.



Experiments were conducted in an ASR zero-shot setting, where SNI models were trained on ASR$_i$ and tested on SLU tasks using another ASR system, ASR$_j$, on the DSTC10 Track2 and ASR GLUE benchmarks. 
Results show that our proposed methods effectively generalize across different ASR systems, with performance comparable to, or even exceeding, the in-domain setting where ASR$_j$ is used to train the SNI model.


==> backup/240613/2_prelim.tex <==
\section{Related Work}
\subsection{SNI}
Previously proposed methods can be categorized into three categories. %, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation.%, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
First, TTS (Text-to-Speech)-ASR pipeline~\cite{tts_asr, tts_asr2} adopts the TTS engine, the reverse of ASR, to convert written text into audio.
The ASR$_i$ transcribes it into pseudo transcription. 
However, the human recording and TTS-generated audio differ in their error distributions, which makes the resulting pseudo transcriptions different from ASR transcriptions~\cite{asrglue}. 
%The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
%During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
%However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
%The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 

Second is textual perturbation, replacing the words $x^k \in X$ to the noise word $t_{i}^{k}$ as follows:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix3, confusion_matrix5} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.

A representative of the above two categories is TOD-DA which embodies both categories. 
%Ignoring the context, thus it is outperformed by the third method~\cite{noisygen, asrglue}.

Third is  the auto-regressive generation, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$-plausible noise words~\cite{noisygen}.


Auto-regressive generation is biased to ASR$_i$, limiting the SLU model used for ASR$_i$.% plausible noise words,
Our distinction is generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.% e a noised version given the ground-truth transcription.

\subsection{ASR Correction}
As an alternative, ASR correction 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT. 
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart, chen2024hyporadise}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperform ASR correction~\cite{asrglue}.
In addition, it introduces additional latency in the SLU pipeline for ASR correction before the SLU model to conduct SLU tasks.
In voice assistant systems like Siri, such additional latency is crucial as the SLU pipeline should deliver responses with minimal delay to ensure real-time interaction.
Therefore, we focus on SNI for its effectiveness and minimal latency in SLU pipeline.






==> backup/240613/3_ours.tex <==
\section{Method}
Before introducing ISNI, we first formally define the problem of SNI and outline its causal diagram. 
Following this, we provide an overview of ISNI and detail the methods used to generate pseudo transcriptions that enhance the robustness of SLU tasks against ASR$_*$.

\subsection{Problem Formulation}
\yj{
The SNI model is defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$, which mimics the transcriptions of ASR$_i$.
Given the written ground truth (GT) $X=\{x^{k}\}_{k=1}^{n}$ with $n$ words, the SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i={t^{k}_{i}}{k=1}^{n}$, simulating the transcriptions produced by ASR$_i$. 
These pseudo transcriptions, $T_i$, are subsequently used to train SLU models. 
For each word $x^{k}$, $z^{k} \in Z$ indicates whether ASR$_i$ transcribed correctly ($z^{k}=0$, hence $x^{k}=t^{k}_{i}$) or incorrectly ($z^{k}=1$, hence $x^{k} \neq t^{k}_{i}$). 
However, errors generated by this model may not generalize well to another ASR system, ASR$_j$.
Therefore, we propose building an SNI model, $\textit{F}_*$, capable of generating ``ASR$_*$-plausible'' pseudo transcripts $T_*$, which are plausible for any ASR system, ASR$_*$.
}

\input{figure_latex/figure2}
\yj{
To achieve this, we compare the underlying causal relations between ASR transcription and SNI training data generation. 
During ASR transcription, $X$ is first spoken as audio $A$, which is then transcribed by ASR$_i$. 
Depending on the audio $A$, ASR$_i$ may make errors ($Z=1$) or not ($Z=0$) in the transcription $T$. 
These relations are depicted in Fig.~\ref{fig:fig2_subfig1}. 
While transcribing, $X$ influences $T$ through direct causal paths, forming only causal relations.}

\yj{
The resulting $X$ and $T$ are then filtered based on $Z$ since they do not exhibit the error patterns required for training.
However, such filtering induces a backdoor path and a non-causal relation in SNI. 
To further elucidate the causal relations in SNI training data generation depicted in Fig.~\ref{fig:fig2_subfig2}, we outline the causal influences as follows:
\begin{itemize}
\item $X \rightarrow T$: There is a direct causal relationship where the clean text $X$ influences the transcribed text $T$.
\item $Z \rightarrow T$: The variable $Z$ indicates whether an error occurs in the transcription $T$. 
If $z^{k} \in Z$ is 1 (an error occurs), it directly affects the corresponding transcription $t^{k}_{i}$, causing it to deviate from the clean text $x^{k}$.
\item $Z \rightarrow X$: During the training data collection process, $Z$ influences the inclusion of $X$.
Only instances where ASR$_i$ incorrectly transcribed, indicated by any $z^{k} \in Z$ being 1, are included, creating a dependency where the presence of errors influences which clean texts are selected.
\end{itemize}}


\subsection{$do$-calculus for ISNI}
\label{sec:do_calculus}
\yj{
Based on the above causal relations, we illustrate how non-causal relations affect SNI and how these relations can be removed by adopting $do$-calculus.}

\yj{
The backdoor path $X \leftarrow Z \rightarrow T$ introduces bias in previous SNI models based on conventional likelihood, defined as: 
\begin{equation}
P(t^{k}_{i}|x^{k})=\sum_{z^{k}}P(t^{k}_{i}|x^{k},z^{k})P(z^{k}|x^{k}).
\label{eq:likelihood}
\end{equation}
Here, the mediator $z^{k}$, instead of being merely a consequence of $x^{k}$, also influences $x^{k}$, thereby distorting the causal effect from $X$ to $T$. This backdoor path ensures that only instances where ASR$_i$ made errors are included, leading to a bias where SNI models generate pseudo transcripts containing only ASR$_i$-plausible noises.}


\yj{
Do-calculus removes this bias by cutting off the non-causal path $Z \rightarrow X$ using the $do$-operator, as shown in Fig.~\ref{fig:fig3}.
By eliminating this non-causal path from the causal graph, $X$ becomes independent of $Z$. Consequently, $P(z^{k}|x^{k})$ is replaced with $P(z^{k})$, allowing the SNI model to be estimated as follows:
\begin{equation}
    P(t^{k}|do(x^{k}))= \sum_{z^{k}}P(t^{k}|x^{k},z^{k})\cdot P(z^{k}).
    \label{eq:do}
\end{equation}
Compared to $P(t^{k}_{i}|x^{k})$ in Eq.\ref{eq:likelihood}, the term $X$ in Eq.~\ref{eq:likelihood}, $X$ in Eq.~\ref{eq:do} is independent of $Z$, effectively removing the influence of $Z$ on $X$.
We provide more detailed proof of Eq.~\ref{eq:do} in Sec.~\ref{sec:proof_do}.}

%Do-calculus aims to more robustly understand the causal effect %which is direct influence from variable $X$ to another variable $Y$.
%Using Bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
%\begin{equation}
%    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
%    \label{eq:likelihood}
%\end{equation}
%where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.


%However, $P(Y|X)$ can be easily biased by non-causal effects where %the mediator $Z$ influences $X$.
%That is, the mediator $Z$, rather than being just a consequence of $X$, might also be influencing $X$, thus distorting the causal effect from $X$ to $Y$.
%For example, SNI model is trained to generate the noise word $t^k$ given the word $x^k$, for which only $x^k$ such that $z=0$, an ASR incorrectly transcribed, is collected. 
%As an ASR is biased to make errors on specific phonemes, the collection of word $x^k$ for training the SNI model is affected by $z$.


%Do-calculus reduces such bias by reducing the non-causal effect, the influence of $z$ to $X$, using the $do$ operator to conventional likelihood as follows:
%\begin{align}
%    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
%    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
%    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
%    &= \sum_{z}P(Y|X,z)\cdot P(z).
%    \label{eq:do}
%\end{align}
%Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is independent of $X$, which cuts off the influence of $Z$ on $X$. 
%We refer the proof of transition between $P(z|do(X))$ and $P(z)$ to \citet{glymour2016causal}.

%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.

%such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }




\subsection{Overview of Our Proposed Approach}
\label{sec:overview}
\input{figure_latex/figure3}
\yj{
In this section, we briefly overview how ISNI can generate debiased ASR$_*$ noises of different error types, as illustrated in Fig.~\ref{fig:fig3}.
To achieve this, ISNI implements two distinct terms in Eq.~\ref{eq:do}, $P(z^{k})$ and $P(t^{k}|x^{k}, z^{k})$ for SNI.}


\yj{
For debiased noise generation $P(z^k)$, it is essential to cut off the influence of $x^k$ on $z^k$ so that $z^k$ becomes independent of $x^k$. 
ISNI explicitly controls $z^k$ and removes the dependence on $x^k$ by implementing SNI with constrained decoding, following \citet{constdecoder}.} 
By determining $z$ using $do$-calculus, tokens rarely corrupted in ASR$_i$ are included as noise in the pseudo transcripts. 
For example, the token $x$ with $z=1$, such as ‘cue’ in Fig.~\ref{fig:fig3}, is fed to the constrained decoder.
The constrained decoder then generates the noise word $t$ to replace $x$.

ISNI can introduce errors in the token $x$ through three conventional ASR error types: substitution, insertion, and deletion~\cite{jurafsky2019speech}. 
Substitution errors occur when the generated output is a new token that replaces $x$. 
Insertion errors occur when the constrained decoder outputs multiple tokens for $x$. 
For example, in Fig.~\ref{fig:fig3}, generating `the' in addition to $x^2$, `the', results in an insertion of the newly generated `the' is inserted.
Deletion errors occur when the constrained decoder outputs only the $eos$ token, representing the end of generation. 
If the generation ends without any tokens, as in $t^5$, the empty string replaces $x^5$. 
ISNI generates these error types synthetically, as demonstrated in the quantitative study in Sec.~\ref{sec:quantitiate_study} and the generated examples in Sec.~\ref{sec:pseudo_transcripts_examples}.

For ASR$_*$-plausible generation $P(t^{k}|x^{k},z)$, we provide the phonetic information of $x$, such as `kju' in Fig.~\ref{fig:fig3}, to ISNI to understand how $x$ is pronounced. 
The constrained decoder evaluates the generation probability based on phonetic similarity, recognizing that `c' is pronounced as the phoneme `k'. 
Consequently, ISNI generates the ASR$*$-plausible noise word `queue' which is phonetically similar to `cue'.







\subsection{Interventional SNI for Debiasing}
\label{sec:interventional_sni}
To debias the dependence on ASR$_i$, we propose to intervene in non-causal effect $X\leftarrow Z$ so that the pseudo transcripts contain diverse noise words, even those rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
We reduce the non-causal influence of $z$ on $x^k$ using do-calculus, as shown in Eq.~\ref{eq:do} resulting in the following model for SNI:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
This intervention ensures that the decision to corrupt the words $x^k$ in the pseudo transcripts is independent of any specific ASR system, such as ASR$_i$. Consequently, words typically rarely corrupted by ASR$_i$ can also be corrupted.

For each word $x^k$, we sample a random variable $a^k$ from a continuous uniform distribution over the interval $[0,1]$ to determine whether the word $x^k$ will be corrupted.
If $a^k \leq P(z)$, we set $z$ to 1, indicating an incorrect transcription of $x^k$ and generating its noise word $t^{k}$. 
Otherwise, $z$ is set to 0, and $t^{k}$ remains identical to $x^{k}$, mimicking a successful transcription. We set the prior probability $P(z)$ as a constant hyperparameter for pseudo transcript generation.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.

%The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
%Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
%Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.
As constrained generation outputs $t^{k}$ to input $x^{k}$, we adopt it to control the $z$ and remove the bias toward a specific ASR.
%Adopting constrained generation, we model $P(t^{k}|x^{k},z)$ and can control $z$, as 
%To control the $z$, we model $P(t^{k}|x^{k},z)$ adopting constrained generation, where decoder is fed $x^{k}$ and outputs $t^{k}$.
To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ are word and position embeddings.
%We note that dummy tokens are inserted between adjacent tokens in $X$ during the preprocessing step following \citet{constdecoder}.

The transformer decoder~\cite{NIPS2017_3f5ee243} generates $t^{k}$ constrained on $x^k$.
To replicate all ASR error types, we enable the transformer decoder to produce multiple tokens (see Section 3.2), denoted as $m$ tokens, $\{\Tilde{t}^{k}_{l}\}_{l=1}^{m}$, which will replace $x^k$ in the pseudo transcripts. The error type of $t^{k}$ is contingent on $m$:
$m=1$ corresponds to deletion, generating only eos is generated; $x^k$ is substituted by the empty string. 
If $m=2$, one token in addition to eos is generated; this token substitutes $x^k$.
When $m>2$,
 additional token will be inserted to $x^k$, to simulate insertion errors.


To generate $\Tilde{t}^{k}_{l}$, the input of the decoder is the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation and the tokens generated so far, $\{\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}\}$ as follows:%the special embedding vector $bos$ representing the beginning of the generation   
\begin{equation}
    E_{decoder}^{k}= H_{decoder} \cdot [e_{encoder}^{k}; bos,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}],
    \label{eq:decoder_input}
\end{equation}
where $H_{decoder}$ is the weight matrix of the hidden layer.
The transformer decoder outputs the hidden representation $d^{k}$ as follows:
\begin{align}
    d^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K,V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, we measure the probability of each token to be generated as $\Tilde{t}^{k}_{l}$, $P_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1})$, as follows:
\begin{equation}
    P_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = softmax(M_{word} \cdot d^{k}+b_{n}),
    \label{eq:gen_prob}
\end{equation}
where $b_{n}$ are trained parameters. 
Here, we note that ISNI generates different error types depending on the output as we explained in Sec.~\ref{sec:overview}.

We used the ASR transcription $T$ to train ISNI model.
ISNI is supervised to maximize the log-likelihood of the $l$-th token $\hat{t}^{k}_{l}$ from the ASR transcription as follows:
\begin{equation}
    \mathcal{L}_{n} =-\sum log(\textit{P}_{n}(\hat{t}^{k}_{l}|x^{k},\hat{t}^{k}_{0},..., \hat{t}^{k}_{l-1})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to reduce the bias of ASR$_i$ in $P(t^{k}|x^{k},z)$ and ensure the noise word generation ASR$_*$-plausible.
%The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
%To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
We adjust the generation probability $P_{n}$ with the phoneme-based generation probability $P_{ph}$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{multline}
    \textit{P}_{gen}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = \textit{P}_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) \\ \cdot \textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}).  
    \label{eq:phoneme_correction_prob}
\end{multline}

Our first proposal for $\textit{P}_{ph}$ is to provide phonetic information via phoneme embedding $M_{ph}$.
%The main difficulty of evaluating $\textit{P}_{ph}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $M_{ph}$ is designed to have the phonetic information of each token in the vocabulary.
$M_{ph}$ can contain such information as tokens with identical phonetic codes have identical phoneme embedding. 
Thus, feeding the phoneme embedding $M_{ph}$ can deliver how each word in written sentences is pronounced.
Phoneme embedding is fed to the encoder with word and position embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{ph}(X)+M_{position}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, the decoder would yield the hidden representation $d^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we feed the hidden representation $d^k$ to classification head to evaluate the phoneme based generation probability $\textit{P}_{ph}$ as follows:
\begin{equation}
    \textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = softmax(M_{ph} \cdot d^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where classification head has the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$.
Using the phoneme embedding $M_{ph}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ can be evaluated based on the phonetic information.
%Then, we feed the hidden representation $h^k$ to classification head with weight matrix is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$  evaluate the phoneme based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ as follows:


Our second proposal for $\textit{P}_{ph}$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$-plausible noise words, $\textit{P}_{ph}$ should evaluate how phonetically similar each token is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$.
\begin{comment}
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance $\textit{D}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{D}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{D}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 
It is noteworthy that $S$ is computed based on articulatory features, thus, not equal to 1 as it is normally used when computing word error rates.
\end{comment}
Phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance  $\textit{D}(w^{p}, w^{q})$ can measure how similar the word pair $(w^{p}, w^{q})$ is by measuring the minimum edit distance between the phonetic codes of the input word pair.
It is noteworthy that $\textit{D}(w^{p}, w^{q})$ is computed based on articulatory features, thus, it incrementally increases when the word pair is pronounced more similarly.
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 


To supervise $\textit{P}_{ph}$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{ph}$ is supervised by loss defined as follows:
 \begin{equation}
     \mathcal{L}_{ph} = KL(\textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1})| \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $KL$ is the KL divergence loss.
Finally, ISNI is optimized to jointly minimize the total loss $\mathcal{L}_{tot}$ which is defined as follows:
\begin{equation}
    \mathcal{L}_{tot} = \mathcal{L}_{n} + \lambda_{ph} \cdot \mathcal{L}_{ph},
    \label{eq:total_loss}
\end{equation}
where $\lambda_{ph}$ is the weight of $\mathcal{L}_{ph}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{ph}$ can ensure the ASR$_*$-plausible noise words and $M_{ph}$ can contain phonetic information.
 

 




==> backup/240613/4_experiment.tex <==
\section{Experiments}
In this section, we introduce the dataset and baselines for SNI and SLU, to ensure fair comparison of ISNI with baselines. 
Then, we explain ASR systems used for SNI training and SLU testing. 
We note that our experiments are conducted in ASR zero-shot setting where SNI models are trained on one ASR system (ASR$_i$), while SLU models are tested using a different ASR system (ASR$_j$).
Finally, we provide the experimental details.
%how we formulated the ASR zero-shot setting, where SNI models are trained on one ASR system (ASR$_i$), while SLU models are tested using a different ASR system (ASR$_j$), for SLU tasks, ASR GLUE and DSTC10 Track 2. 
%We also note that SLU models are trained with pseudo transcripts generated by SNI models.
%In this section, we thoroughly deliver experimental details SNI training and SLU testing.}
\subsection{Dataset}
\label{sec:dataset}
\paragraph{SNI Training} SNI training datasets are chosen to follow our main baseline, Noisy-Gen~\cite{noisygen}.
For training, 3 popular corpora, Common Voice, tatoeba audio, and LJSpeech-1.1 were used. MSLT corpus was used as validation set for SNI training.   %, which collected the ASR error transcriptions from popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1 for the training set and MSLT for the validation set. 
The audio recordings from such speech corpora are fed to DeepSpeech and the resulting transcription is collected if it contains the ASR errors. 
As a result, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\paragraph{SLU Testing} SLU datasets are chosen to show the ASR generalizability in diverse SLU tasks.
We adopt two distinct SLU benchmarks, ASR GLUE and DSTC10 Track 2.
ASR GLUE is an SLU version of the widely adopted NLU benchmark, GLUE.
We report the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST2.
DSTC10 Track 2 models spoken language dialogue systems, where SLU models are frequently adopted. % and consists of three successive subtasks of diverse kinds: Knowledge-seeking Turn Detection (KTD) of text classification, Knowledge Selection (KS) of textual retrieval, and Knowledge-grounded Response Generation (RG) of textual generation.
%We adopt the DSTC10 Track2 dataset as it covers various tasks in the dialogue domain.
It consists of three successive subtasks of diverse kinds: Knowledge-seeking Turn Detection (KTD) of text classification, Knowledge Selection (KS) of textual retrieval, and Knowledge-grounded Response Generation (RG) of textual generation.
%We report the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which were not covered in the DSTC10 Track 2.
We provide further details of the datasets for SNI training and SLU testing in Sec.~\ref{sec:dataset_details}.
%It provides the transcriptions of 3 noise levels spoken by 5 human speakers for the development set and test set.
%As the ground-truth label for the test set is unavailable, we report the results on the development set and sample the validation set from the pseudo transcripts generated from the training set.
%We provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which were not covered in the DSTC10 Track 2.


\subsection{Baselines}
%Our main baseline is Noisy-Gen, GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
In our study, we employed diverse SNI models as baselines, alongside consistent SLU models across all SNI methods, to verify the influence of SNI on SLU performance.
We adopt NoisyGen, GPT2-based auto-regressive generation SNI model, as our main baseline.
We adopted NoisyGen due to its competitive results in various spoken language tasks such as SLU and spoken language translation~\cite{noisygen,asrglue}.
%Noisy-Gen is trained with a training set identical to ours.
%Pseudo-transcriptions generated by Noisy-Gen are filtered by phoneme-based heuristics. 

For ASR GLUE benchmark, we adopt another baseline NoisyGen (In Domain)~\cite{asrglue},
Noisy-Gen and NoisyGen (In Domain) %are similar in that they 
are both GPT2-based SNI models, while
NoisyGen (In Domain) employs the same ASR system for both SNI training and SLU testing, which violates the ASR zero-shot setting. 
Thus,  the pseudo transcripts generated by NoisyGen (In Domain) would resemble the ASR transcripts for SLU testing, making robustification against ASR errors easier.
Thus, if SNI models can match or exceed the performance of NoisyGen(In Domain), SNI models can demonstrate their ASR-generalizability.
For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
We selected TOD-DA because it covers two distinct categories of SNI which were not covered by NoisyGen: TTS-ASR pipeline and textual perturbation. 
%It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
%Also, it conducted character-level perturbation of substitution, insertion and deletion, and swap and split.





\subsection{ASR system for SNI training and SLU testing}
We provide the ASR systems used for SNI training in Table~\ref{tab:SNI_ASR} and SLU testing in Table~\ref{tab:SLU_ASR}.
\paragraph{SNI Training}
We used the open-source commercial ASR system, Mozilla DeepSpeech~\cite{deepspeech}, for several reasons: 
Firstly, it aligns with our main baseline, NoisyGen, and other studies that utilize commercial ASR systems\footnote{We provide the comparison of commercial ASR systems in Sec.~\ref{sec:asr_details}.}. %like Google Translate’s speech-to-text API and IBM Watson Speech-to-text, demonstrating comparable word error rates on benchmarks such as Librispeech and CommonVoice. 
Secondly, despite being trained on DeepSpeech, ISNI showcases strong generalizability against the errors from the recent ASR systems, outperforming SNI models that use more recent ASR systems such as LF-MMI TDNN for NoisyGen (In Domain)~\cite{asrglue} and Wave2Vec for TOD-DA~\cite{yuan2017wave2vec}.


\input{table/sni_training_asr}
\paragraph{SLU Testing} To confirm the generalization of SNI over different ASR systems, we used different ASR systems for SLU testing, ASR GLUE and DSTC10 Track 2. 
In Table~\ref{tab:SLU_ASR}, we provide the ASR system used to transcribe the SLU test set.
For the ASR GLUE, the LF-MMI TDNN-based ASR system transcribed the test set.
For the DSTC 10 Track 2, an unknown ASR system is used to transcribe the validation and test set.

\input{table/slu_testing_asr}
\input{table/asrglue_result}



\subsection{Experimental Settings}
\paragraph{SNI Training}
To implement ISNI, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder and 1 Transformer decoder layer~\cite{NIPS2017_3f5ee243} following previous work~\cite{constdecoder}.
To balance the word embedding and phoneme embedding, $\lambda_{w}$ in Eq.~\ref{eq:phoneme_encoder} were set to 0.5.
For the weight of phoneme generation loss $\mathcal{L}$, $\lambda_{ph}$ in Eq.~\ref{eq:total_loss} were set to 0.5.
We provide further details in Sec.~\ref{sec:ISNI_model_detail}.

\paragraph{SLU Training}
Using the trained ISNI, the written GTs in SLU dataset are converted into pseudo transcripts.
We set the prior probability $P(z)$ as 0.15 for ASR GLUE and 0.21 for DSTC10 Track2 dataset based on the validation set result of downstream SLU tasks\footnote{Matching $P(z)$ to word error rate of the ASR system used for the SLU seems straightforward but unfortunately inapplicable to ASR zero-shot setting where WER is unknown for unknown ASR. Also, training in arbitrary word error rates can cause the SLU model to be biased in certain ASR systems.}.
For a fair comparison, PER, threshold phonetic similarity for filtering out phonetically dissimilar pseudo transcripts were tuned with the development sets as ISNI.
As downstream task models, we adopted BERT-base for ASR GLUE and GPT2-small for DSTC10 Track 2 following the settings from baseline results~\cite{dstc10_2,asrglue}.

















==> backup/240613/5_results.tex <==
\section{Results}


\input{table/dstc_result}
We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are ISNI in the ASR zero-shot setting?

%\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ2:} Can ISNI robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ3:} Does each of ISNI contribute to robustification?

\subsection{RQ1: Validity of ASR Zero-shot Setting and Effectiveness of ISNI. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.


First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Noisy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.





%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ISNI showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
ISNI outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST2 of the low noise level.
Also, ISNI always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that ISNI can make SLU models generalizable in the ASR zero-shot setting.


In addition, ISNI robustifies SLU models against different noise levels.
ISNI showed little degradation in performance as noise levels increased compared to baselines.
That is, as prior work suggests, phoneme confusions more frequently occur~\cite{wu2022phonetic,petkov2013maximizing} and ours can robustify even when such phoneme confusion increases.




%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.








\subsection{RQ2: Robustification of ISNI on Various SLU Tasks.}
We show that ISNI can better robustify various SLU tasks over different SNI methods in ASR zero-shot setting.
%As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, caused by ASR errors.

We present the results of ISNI methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
Different from the previous observations where the identical ASR system is used for SNI and SLU tasks~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of ISNI is not limited to KS.
Overall, ISNI outperformed baselines in every task and every metric with a large margin except P of KTD.
ISNI showed the increase of the BLEU score by 2-3 times for RG.
These results show that ISNI can robustify against ASR errors in various SLU tasks.



\subsection{RQ3: Importance of Each Proposed Method to the Robustification. }
To confirm that each of ISNI contributes to the robustification, we conducted the ablation studies  in Table~\ref{tab:dstc_results} by deducting each of the proposed methods.

We report the result without the phoneme-aware generation in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme-aware generation showed a decreased score in every subtask, showing the importance of ASR-plausibility of pseudo transcription to robustify against ASR errors.
To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
As the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:likelihood}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Performance is decreasing as expected in KS, which is our main consideration as it is largely influenced by lexical perturbation due to the ASR errors.
Such decrease is also observed in RG, showing that substituting the intervention contributes to the decreased performance in KS and RG.
Unexpectedly, the last row of Table~\ref{tab:dstc_results} shows the increased performance of KTD. 
We suspect such increase in KTD is due to its characteristic of text classification.
Meanwhile, prior work suggests that even the text classification may still degrade,  when the noises are more abundant in the training set~\cite{4470224}, to which ISNI may contribute.

%Previous work suggests that the abundance of noises in the training set may fail robustification in text classification \cite{4470224}.






==> backup/240613/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we have addressed the challenge of ASR generalizability within the context of SNI. Our focus was on enhancing the robustness of downstream SLU models against ASR errors that may originate from diverse ASR systems. The existing SNI method is biased to a particular ASR system used for generating pseudo transcriptions.
To tackle the ASR generalizability issue, we introduce two key contributions. First, towards eliminating biases, ISNI significantly incorporates a wider range of ASR-plausible errors. However, such diversity should not interfere ASR-generic characteristcs, for which, our second step leads to the generation of errors that are commonly plausible, or ASR$_*$-plausible.
Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/240613/limitations.tex <==
\paragraph{Limitations.}

As ISNI is trained with speech corpora collected for academic purposes, they may face challenges when adopted for real-world applications.
%We think ISNI would suffer from challenges similar to those encountered by ASR systems.
One example is handling diverse spoken language variations such as dialects and accents. 
These variations can introduce noises that are not phonetically similar, which are different from the speech data used during ISNI training. 
This discrepancy may fail ISNI to robustify SLU models as ISNI is not prepared to handle ASR errors from those speech variations.  %, potentially impacting its ability to robustify spoken language understanding (SLU) models across all speech variations. 
Addressing this limitation may require enlarging the training dataset of ISNI to include a wider array of noises due to such spoken language variation.
%ensuring it can effectively generalize across the diverse speech conditions found in practical applications.

%We make use of DeepSpeech ASR system, for the reason of its similarity in performance to many commercial ASR systems as we will discuss in Sec.~\ref{sec:asr_details}.


%However, our ISNI may not well be trained with different ASR systems due to several reasons.
%A notable reason is the scarcity of the training set due to rare ASR errors.
%As we described in Sec.~\ref{sec:dataset}, we only use the erroneous transcriptions for training ISNI.
%However, when the ASR system is too strong, it may make not enough erroneous transcriptions to train ISNI.
%The most straightforward method is to use the other weaker ASR system for training, as our ISNI can %generalize to different ASR systems.
%Second, previous works suggest training the weaker version of the ASR system and using it for training SNI~\cite{dutta2022error}.





==> backup/ARR_Apr_15/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU). 
As automatic speech recognition (ASR) systems often transcribe spoken language inaccurately, noisy inputs are introduced to SLU models. 
Our goal is to train SLU models to tolerate these ASR errors by exposing them to noises that are likely to be observed in ASR systems, which are denoted as ASR-plausible noises.
Speech noise injection (SNI) achieves such goal by introducing ASR-plausible noises that are inevitably biased to a particular ASR system.
Our distinction is first to mitigate biases to a particular ASR system, then ensure
augmentation to satisfy ASR-generic plausibility that holds for any ASR system.
Experimental results and analysis show the effectiveness of our proposed methods in improving the robustness and generalizability of SLU models against unseen ASR systems, by introducing more diverse and plausible ASR noises in advance.
\end{abstract}

==> backup/ARR_Apr_15/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/ARR_Apr_15/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/ARR_Apr_15/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/ARR_Apr_15/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs thus have gained widespread acceptance and employment within the realm of spoken language understanding (SLU) as applied in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
A concrete instance of this application involves a pipeline leveraging PLMs subsequent to the automatic speech recognition system (ASR) transcribing audio inputs. The resulting transcriptions are input to PLMs to facilitate downstream SLU tasks~\cite{asrglue}.


However, such pipeline encounter challenges when confronted with inaccuracies stemming from ASR systems.
We denote such inaccuracy as ASR error words, which are phonetically akin yet semantically unrelated~\cite{ruan20_interspeech,9054689}.
To illustrate, consider Fig.~\ref{fig:example}, 
where ASR systems, confused between  ``cereal'' and ``serial'', ``quarry'' and ``carry'', may generate an incorrect transcription such as ``workers eat serial in the carry''.
Despite their phonetic resemblance, these ASR error words convey unintended meanings, thereby impeding the semantic understanding of speech in SLU tasks~\cite{belinkov2018synthetic}.



A well-known solution is annotating likely incorrect transcriptions, known as speech noise injection, or, SNI~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
An SLU corpus annotation typically starts from a corpus of written 
text as a ground truth (GT), recorded into audio, then
transcribed into text using ASR systems.
A more efficient alternative is, skipping the recording and transcription,
to directly corrupt the written GT, to
 introduce noise to the original written sentence, creating a pseudo transcript that closely aligns with the expected output of an ASR system.
 Desirably, SNI noise should be ``ASR-plausible'', indicating the pseudo transcript is likely to be generated by ASR systems.



\input{figure_latex/figure1}

By definition, as ASR-plausibility is conditional to a particular ASR system, or ASR$_i$, previous methods have focused on mimicking the target ASR$_i$. 
To achieve this, these methods involve collecting the incorrect transcriptions generated by the target ASR$_i$ and subsequently corrupting the clean, written GTs into pseudo transcripts based on the errors observed~\cite{confusion_matrix, confusion_matrix2,noisygen}.
This method is designed to replicate the error patterns of a target  ASR$_i$. 
It does so by corrupting clean texts with errors observed in ASR$_i$ transcriptions, producing pseudo transcripts. 
In other words, both real and simulated outputs from ASR$_i$ have similar likelihood that a word $x$ will be misrecognized $(z = 1)$ or not $(z = 0)$, denoted as $P(z|x)$.

However, different ASR systems have distinct $P(z|x)$ and differ in the error pattern.
Such difference affects an SLU model trained on pseudo transcripts from one system (ASR$_i$) intoloerant to errors from another system (ASR$_j$). 
While avoiding such issues requires building several SLU models per each ASR system,
%for their corresponding ASR systems. 
%However, 
recent trends of scaling up 
PLMs make such processes too costly.




%In contrast, to generate pseudo transcripts that generalize beyond ASR$_i$, our distinctions are two-fold: 
%First, after generating noises conditional to ASR$_i$,
%we debias its dependence on ASR$_i$.
%Specifically, $do$-calculus intervenes in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$.
%It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
%For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.
Our distinction is to generate pseudo transcripts that can generalize beyond a specific ASR system. 
For this purpose, we introduce two technical contributions: 1) interventional noise injection and 2) phoneme-aware generation. 
We start by debiasing the dependence of noises to the specific ASR system, ASR$_i$, by applying \textit{do}-calculus in the effect of the word $x$ on $z$, replacing $P(z|x)$ into $P(z)$. 
It cuts off the corrupting probability of the frequently corrupted phonemes and increases that of the rarely corrupted phonemes. 
For example, in Fig.~\ref{fig:example}, our SNI model can corrupt the word `Read' with the phoneme `\textturnr'  which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the ones corrupted by baseline SNI.




%Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$, GT word and ASR noise word are phonetically similar~\cite{serai2022hallucination}.
%Specifically, we supervise and feed how words are pronounced.
%Unaware of how words are pronounced, previous works generate ASR noise words plausible for no ASR system.  
%For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
%`serial'.
%Mimicking ASR$_{1}$ unaware of pronunciation results in replacing c with s (or, replacing `cue' with `sue').
%However, knowing that `c' can sound differently in other words, k sound, ours can generate noise word `queue', which is plausible regardless of the ASR system used, or ASR$_*$-plausible.
\begin{comment}
Then, we ensure the debiased noises follow common characteristics shared by any ASR, namely ASR$_*$, such that GT words and ASR noises become phonetically similar~\cite{serai2022hallucination}. 
Specifically, along with the words as textual input, we feed how words are pronounced together. 
Being aware of how words are pronounced, we could introduce ASR noises plausible regardless of the specific ASR system used, namely ASR$_*$-plausible. 
\end{comment}
    
Then, we ensure the debiased noises to be plausible for any ASR, namely ASR$_*$, such that GT words and ASR noises become phonetically similar following the common characteristics shared by ASR$_*$~\cite{serai2022hallucination}. 
Along with the words as textual input, we feed how words are pronounced together. 
Being aware of how words are pronounced, we could introduce ASR noises plausible regardless of the specific ASR system used, namely ASR$_*$-plausible. 



Experiments are conducted in ASR zero-shot setting where SNI models are trained on ASR$_i$ and SLU tasks are tested on another ASR$_j$ on DSTC10 Track2 and ASR GLUE benchmark.
Results show that our proposed methods are effective in ASR generalization with comparable or even outperforming performance compared to the in-domain setting where ASR$_j$ is used to train the SNI model.



==> backup/ARR_Apr_15/2_prelim.tex <==
\section{Related Work}
\subsection{SNI}
Previously proposed methods can be categorized in three categories. %, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation.%, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
First, TTS (Text-to-Speech)-ASR pipeline~\cite{tts_asr, tts_asr2} adopts the TTS engine, the reverse of ASR, to convert written text into audio.
The ASR$_i$ transcribes it into pseudo transcription. 
However, the human recording and TTS-generated audio differ in their error distributions, which makes the resulting pseudo transcriptions different from ASR transcriptions~\cite{asrglue}. 
%The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
%During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
%However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
%The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 

Second is textual perturbation, replacing the words $x^k \in X$ to the noise word $t_{i}^{k}$ as follows:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix3, confusion_matrix5} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.

A representative of the above two categories is TOD-DA which embodies both categories. 
%Ignoring the context, thus it is outperformed by the third method~\cite{noisygen, asrglue}.

Third is  the auto-regressive generation, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$-plausible noise words~\cite{noisygen}.


Auto-regressive generation is biased to ASR$_i$, limiting the SLU model used for ASR$_i$.% plausible noise words,
Our distinction is generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.% e a noised version given the ground-truth transcription.

\subsection{ASR Correction}
As an alternative, ASR correction 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT. 
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart, chen2024hyporadise}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperform ASR correction~\cite{asrglue}.
In addition, it introduces additional latency in the SLU pipeline for ASR correction before the SLU model to conduct SLU tasks.
In voice assistant systems like Siri, such additional latency is crucial as the SLU pipeline should deliver responses with minimal delay to ensure real-time interaction.
Therefore, we focus on SNI for its effectiveness and minimal latency in SLU pipeline.






==> backup/ARR_Apr_15/3_ours.tex <==
\section{Method}
Before introducing ISNI, we first formally define our problem of SNI.
Then, we overview ISNI and provide detailed methods of ISNI which aims to generate pseudo transcription that can robustify SLU tasks against ASR$_*$.

\subsection{Problem Formulation}
SNI model can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
%\yj{Then, $t^{k}_{i}$ can be aligned with $x^k$ through three conventional types of ASR errors: insertions,  deletions, and substitutions following the ASR errors~\cite{6300437}.}
The resulting pseudo transcription, $T_i$, is used to train SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ``ASR${_*}$-plausible'' pseudo transcript T$_*$, a pseudo transcript that is ASR-plausible for ASR$_*$.

\subsection{Overview of Our Proposed Approach}
\label{sec:overview}
\input{figure_latex/figure2}
In this section, we briefly overview ISNI which can generate debiased ASR$_*$ noises of different error types, as illustrated in Fig.~\ref{fig:example2}.
%As we will detail in Sec.~\ref{interventional_sni}, to implement $do$-calculus, $P(z|x)$ should be explicitly controlled.


Using the variable $z$, the SNI process can be written as follows:
\begin{equation}
     P(t^{k}|x^{k}) = \sum_{z}P(t^{k}|x^{k},z)\cdot P(z|x^{k}),
     \label{eq:sni_definition}
\end{equation}
where $P(z|x^{k})$ determines whether $x^{k}$ will be corrupted and $P(t^{k}|x^{k},z)$ generates the noise word $t^k$.
Then, the SNI model $P(t^{k}|x^{k})$ is biased to ASR$_i$ such that the word rarely corrupted by ASR$_i$, or, of large $P(z=0|x^k)$, yields large $P(t^k=x^k|x^k)$, the probability of leaving $x^k$ not noised.
%Even though another ASR, ASR$_{j}$, may transcribe $x^k$ incorrectly, $P(z=1|x^k)$ would be low due to bias toward ASR$_i$. 
For the generalization beyond a specific ASR system, we propose the following two approaches:
First, we debias the dependence on ASR$_i$ in $P(z|x^{k})$ with $do$-calculus.
Second, we further generalize $P(t^{k}|x^{k},z)$ to be ASR$_*$-plausible by discouraging the generation of phonetically different noise.




For debiasing $P(z|x^{k})$ and control $z$, we implement SNI with constrained decoding following \citet{constdecoder}.
%The auto-regressive generation where $z$ of each token $x$ is implicitly determined by PLMs
By determining $z$ following $do$-calculus, the tokens rarely corrupted in ASR$_{i}$ are noised in the pseudo transcripts.  
The token $x$ with $z=1$, such as `cue' in Fig.~\ref{fig:example2}, is fed to the constrained decoder.
Then, the constrained decoder generates the noise word $t$ which replaces $x$.

ISNI can noise the token $x$ into all conventional ASR error types, 1) substitution, 2) insertion, and 3) deletion~\cite{jurafsky2019speech}.
%, \yj{by generating multiple tokens.}% (see Eq~\ref{eq:decoder} in Section~\ref{sec:interventional_sni}).
1) Substitution error occurs when the generated output is a new token that replaces $x$.
2) Insertion error occurs when the constrained decoder outputs multiple tokens per $x$.
For example, in Fig.~\ref{fig:example2}, generating `uh' in addition to $x$, `queue', newly generated `uh' is inserted.
%Adding newly generated tokens, 
3) Deletion error occurs when the constrained decoder outputs only $eos$ token representing the end of the generation.
As generation ends without any tokens, such output means that an empty string will replace $x$.
ISNI generates these error types synthetically as the quantitative study in Sec.~\ref{sec:quantitiate_study} and generated examples in Sec.~\ref{sec:pseudo_transcripts_examples} show.

For ASR$_*$-plausible generation $P(t^{k}|x^{k},z)$, we provide the phonetic information of $x$, `kju' in Fig.~\ref{fig:example2}, and notice ISNI of how $x$ is pronounced.
Also, the constrained decoder evaluates the generation probability based on the phonetic similarity that `c' is pronounced as the phoneme `k'.
As a result, ISNI generates the ASR$_*$-plausible noise word `queue' which is phonetically similar to `cue'.



\subsection{$do$-calculus for ISNI}
\label{sec:do_calculus}
Before defining ISNI, we briefly introduce $do$-calculus and how it removes the bias.
Do-calculus aims to more robustly understand the causal effect which is direct influence from variable $X$ to another variable $Y$.
Using Bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.


However, $P(Y|X)$ can be easily biased by non-causal effects where the mediator $Z$ influences $X$.
That is, the mediator $Z$, rather than being just a consequence of $X$, might also be influencing $X$, thus distorting the causal effect from $X$ to $Y$.
For example, SNI model is trained to generate the noise word $t^k$ given the word $x^k$, for which only $x^k$ such that $z=0$, an ASR incorrectly transcribed, is collected. 
As an ASR is biased to make errors on specific phonemes, the collection of word $x^k$ for training the SNI model is affected by $z$.


Do-calculus reduces such bias by reducing the non-causal effect, the influence of $z$ to $X$, using the $do$ operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is independent of $X$, which cuts off the influence of $Z$ on $X$. 
We refer the proof of transition between $P(z|do(X))$ and $P(z)$ to \citet{glymour2016causal}.

%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.

%such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }



\subsection{Interventional SNI for Debiasing}
\label{sec:interventional_sni}
To debias the dependence on ASR$_i$, we propose to intervene $P(z|x^{k})$, so that the pseudo transcript would contain diverse noise words even when they are rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
We reduce non-causal influence from $z$ to $x^k$ using do-calculus as in Eq.~\ref{eq:do} and we have the SNI modeled as follows:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
As a result of the intervention specified in Eq.~\ref{eq:do-calculus}, the decision to corrupt the words $x^k$ in the pseudo transcripts is made independently of any specific ASR system, such as ASR$_i$. 
This approach ensures that words which are typically rarely corrupted by ASR$_i$ can also be corrupted.
For each word $x^k$, we sample random variable $a^k$ from the continuous uniform distribution of interval $[0,1]$, which determines whether the word $x^k$ would be corrupted.
If $a^k\leq P(z)$, we set $z$ as 1 meaning that we will simulate incorrect transcription of $x^k$, thus, we generate its noise word $t^{k}$.
Otherwise, $z$ is set to 0, and $t^{k}$ would be identical to $x^{k}$ mimicking the successful transcription of $x^{k}$.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x^{k}$, which we set as a constant hyperparameter for pseudo transcript generation.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.

%The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
%Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
%Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.
As constrained generation outputs $t^{k}$ to input $x^{k}$, we adopt it to control the $z$ and remove the bias toward a specific ASR.
%Adopting constrained generation, we model $P(t^{k}|x^{k},z)$ and can control $z$, as 
%To control the $z$, we model $P(t^{k}|x^{k},z)$ adopting constrained generation, where decoder is fed $x^{k}$ and outputs $t^{k}$.
To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ are word and position embeddings.
%We note that dummy tokens are inserted between adjacent tokens in $X$ during the preprocessing step following \citet{constdecoder}.

The transformer decoder~\cite{NIPS2017_3f5ee243} generates $t^{k}$ constrained on $x^k$.
To replicate all ASR error types, we enable the transformer decoder to produce multiple tokens (see Section 3.2), denoted as $m$ tokens, $\{\Tilde{t}^{k}_{l}\}_{l=1}^{m}$, which will replace $x^k$ in the pseudo transcripts. The error type of $t^{k}$ is contingent on $m$:
$m=1$ corresponds to deletion, generating only eos is generated; $x^k$ is substituted by the empty string. 
If $m=2$, one token in addition to eos is generated; this token substitutes $x^k$.
When $m>2$,
 additional token will be inserted to $x^k$, to simulate insertion errors.


To generate $\Tilde{t}^{k}_{l}$, the input of the decoder is the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation and the tokens generated so far, $\{\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}\}$ as follows:%the special embedding vector $bos$ representing the beginning of the generation   
\begin{equation}
    E_{decoder}^{k}= H_{decoder} \cdot [e_{encoder}^{k}; bos,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}],
    \label{eq:decoder_input}
\end{equation}
where $H_{decoder}$ is the weight matrix of the hidden layer.
The transformer decoder outputs the hidden representation $d^{k}$ as follows:
\begin{align}
    d^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K,V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, we measure the probability of each token to be generated as $\Tilde{t}^{k}_{l}$, $P_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1})$, as follows:
\begin{equation}
    P_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = softmax(M_{word} \cdot d^{k}+b_{n}),
    \label{eq:gen_prob}
\end{equation}
where $b_{n}$ are trained parameters. 
Here, we note that ISNI generates different error types depending on the output as we explained in Sec.~\ref{sec:overview}.

We used the ASR transcription $T$ to train ISNI model.
ISNI is supervised to maximize the log-likelihood of the $l$-th token $\hat{t}^{k}_{l}$ from the ASR transcription as follows:
\begin{equation}
    \mathcal{L}_{n} =-\sum log(\textit{P}_{n}(\hat{t}^{k}_{l}|x^{k},\hat{t}^{k}_{0},..., \hat{t}^{k}_{l-1})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to reduce the bias of ASR$_i$ in $P(t^{k}|x^{k},z)$ and ensure the noise word generation ASR$_*$-plausible.
%The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
%To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
We adjust the generation probability $P_{n}$ with the phoneme-based generation probability $P_{ph}$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{multline}
    \textit{P}_{gen}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = \textit{P}_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) \\ \cdot \textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}).  
    \label{eq:phoneme_correction_prob}
\end{multline}

Our first proposal for $\textit{P}_{ph}$ is to provide phonetic information via phoneme embedding $M_{ph}$.
%The main difficulty of evaluating $\textit{P}_{ph}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $M_{ph}$ is designed to have the phonetic information of each token in the vocabulary.
$M_{ph}$ can contain such information as tokens with identical phonetic codes have identical phoneme embedding. 
Thus, feeding the phoneme embedding $M_{ph}$ can deliver how each word in written sentences is pronounced.
Phoneme embedding is fed to the encoder with word and position embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{ph}(X)+M_{position}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, the decoder would yield the hidden representation $d^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we feed the hidden representation $d^k$ to classification head to evaluate the phoneme based generation probability $\textit{P}_{ph}$ as follows:
\begin{equation}
    \textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = softmax(M_{ph} \cdot d^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where classification head has the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$.
Using the phoneme embedding $M_{ph}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ can be evaluated based on the phonetic information.
%Then, we feed the hidden representation $h^k$ to classification head with weight matrix is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$  evaluate the phoneme based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ as follows:


Our second proposal for $\textit{P}_{ph}$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$-plausible noise words, $\textit{P}_{ph}$ should evaluate how phonetically similar each token is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$.
\begin{comment}
Specifically, phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance $\textit{D}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{D}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{D}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 
It is noteworthy that $S$ is computed based on articulatory features, thus, not equal to 1 as it is normally used when computing word error rates.
\end{comment}
Phonetic similarity $\textit{S}$ is evaluated using the phoneme edit distance $\textit{D}$~\cite{9662078}.
The phoneme edit distance  $\textit{D}(w^{p}, w^{q})$ can measure how similar the word pair $(w^{p}, w^{q})$ is by measuring the minimum edit distance between the phonetic codes of the input word pair.
It is noteworthy that $\textit{D}(w^{p}, w^{q})$ is computed based on articulatory features, thus, it incrementally increases when the word pair is pronounced more similarly.
Then, phonetic similarity $\textit{S}$ can be defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{S}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different. 


To supervise $\textit{P}_{ph}$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{ph}$ is supervised by loss defined as follows:
 \begin{equation}
     \mathcal{L}_{ph} = KL(\textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1})| \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $KL$ is the KL divergence loss.
Finally, ISNI is optimized to jointly minimize the total loss $\mathcal{L}_{tot}$ which is defined as follows:
\begin{equation}
    \mathcal{L}_{tot} = \mathcal{L}_{n} + \lambda_{ph} \cdot \mathcal{L}_{ph},
\end{equation}
where $\lambda_{ph}$ is the weight of $\mathcal{L}_{ph}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{ph}$ can ensure the ASR$_*$-plausible noise words and $M_{ph}$ can contain phonetic information.
 

 




==> backup/ARR_Apr_15/4_experiment.tex <==
\section{Experiments}
In this section, we introduce the dataset and baselines for SNI and SLU. 
Then, we explain ASR systems used for SNI training and SLU testing. 
We note that our experiments are conducted in ASR zero-shot setting where SNI models are trained on one ASR system (ASR$_i$), while SLU models are tested using a different ASR system (ASR$_j$).
Finally, we provide the experimental details.
%how we formulated the ASR zero-shot setting, where SNI models are trained on one ASR system (ASR$_i$), while SLU models are tested using a different ASR system (ASR$_j$), for SLU tasks, ASR GLUE and DSTC10 Track 2. 
%We also note that SLU models are trained with pseudo transcripts generated by SNI models.
%In this section, we thoroughly deliver experimental details SNI training and SLU testing.}
\subsection{Dataset}
\label{sec:dataset}
\paragraph{SNI Training} We followed our main baseline, Noisy-Gen~\cite{noisygen}, and used 3 speech corpora for training and 1 speech corpus for validation. %, which collected the ASR error transcriptions from popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1 for the training set and MSLT for the validation set. 
The audio recordings from speech corpora are fed to DeepSpeech and the resulting transcription is collected if it contains the ASR errors. 
%As a result, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.

\paragraph{SLU Testing}
To show the ASR generalizability of the SNI models, we adopt two distinct SLU benchmarks, ASR GLUE and DSTC10 Track 2.
ASR GLUE is an SLU version of the widely adopted NLU benchmark, GLUE.
We report the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST2.
DSTC10 Track 2 models spoken language dialogue systems. % and consists of three successive subtasks of diverse kinds: Knowledge-seeking Turn Detection (KTD) of text classification, Knowledge Selection (KS) of textual retrieval, and Knowledge-grounded Response Generation (RG) of textual generation.
%We adopt the DSTC10 Track2 dataset as it covers various tasks in the dialogue domain.
It consists of three successive subtasks of diverse kinds: Knowledge-seeking Turn Detection (KTD) of text classification, Knowledge Selection (KS) of textual retrieval, and Knowledge-grounded Response Generation (RG) of textual generation.
%We report the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which were not covered in the DSTC10 Track 2.
We provide further details of the datasets for SNI training and SLU testing in Sec.~\ref{sec:dataset_details}.
%It provides the transcriptions of 3 noise levels spoken by 5 human speakers for the development set and test set.
%As the ground-truth label for the test set is unavailable, we report the results on the development set and sample the validation set from the pseudo transcripts generated from the training set.
%We provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which were not covered in the DSTC10 Track 2.


\subsection{Baselines}
%Our main baseline is Noisy-Gen, GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
In our study, we employed diverse SNI models as baselines, alongside consistent SLU models across all SNI methods, to verify the influence of SNI on SLU performance.
We adopt NoisyGen, GPT2-based auto-regressive generation SNI model, as our main baseline.
We adopted NoisyGen due to its competitive results in various spoken language tasks such as SLU and spoken language translation~\cite{noisygen,asrglue}.
%Noisy-Gen is trained with a training set identical to ours.
%Pseudo-transcriptions generated by Noisy-Gen are filtered by phoneme-based heuristics. 

For ASR GLUE benchmark, we adopt another baseline NoisyGen (In Domain)~\cite{asrglue},
Noisy-Gen and NoisyGen (In Domain) %are similar in that they 
are both GPT2-based SNI models, while
NoisyGen (In Domain) employs the same ASR system for both SNI training and SLU testing, which violates the ASR zero-shot setting. 
Thus,  the pseudo transcripts generated by NoisyGen (In Domain) would resemble the ASR transcripts for SLU testing, making robustification against ASR errors easier.
Thus, if SNI models can match or exceed the performance of NoisyGen(In Domain), SNI models can demonstrate their ASR-generalizability.
For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
We selected TOD-DA because it covers two distinct categories of SNI which were not covered by NoisyGen: TTS-ASR pipeline and textual perturbation. 
%It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
%Also, it conducted character-level perturbation of substitution, insertion and deletion, and swap and split.





\subsection{ASR system for SNI training and SLU testing}
We provide the ASR systems used for SNI training in Table~\ref{tab:SNI_ASR} and SLU testing in Table~\ref{tab:SLU_ASR}.
\paragraph{SNI Training}
We used the open-source commercial ASR system, Mozilla DeepSpeech~\cite{deepspeech}, for several reasons: 
Firstly, it aligns with our main baseline, NoisyGen, and other studies that utilize commercial ASR systems\footnote{We provide the comparison of commercial ASR systems in Sec.~\ref{sec:asr_details}.}. %like Google Translate’s speech-to-text API and IBM Watson Speech-to-text, demonstrating comparable word error rates on benchmarks such as Librispeech and CommonVoice. 
Secondly, despite being trained on DeepSpeech, ISNI showcases strong generalizability against the errors from the recent ASR systems, outperforming SNI models that use more recent ASR systems such as LF-MMI TDNN for NoisyGen (In Domain)~\cite{asrglue} and Wave2Vec for TOD-DA~\cite{yuan2017wave2vec}.


\input{table/sni_training_asr}
\paragraph{SLU Testing} To confirm the generalization of SNI over different ASR systems, we used different ASR systems for SLU tasks, ASR GLUE and DSTC10 Track 2. 
In Table~\ref{tab:SLU_ASR}, we provide the ASR system used to transcribe the SLU test set.
For the ASR GLUE, the LF-MMI TDNN-based ASR system transcribed the test set.
For the DSTC 10 Track 2, an unknown ASR system is used to transcribe the validation and test set.

\input{table/slu_testing_asr}
\input{table/asrglue_result}



\subsection{Experimental Settings}
\paragraph{SNI Training}
For ISNI, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder and 1 Transformer decoder layer~\cite{NIPS2017_3f5ee243} for ISNI following previous work~\cite{constdecoder}.
We provide further details in Sec.~\ref{sec:ISNI_model_detail}.

\paragraph{SLU Training}
Using the trained ISNI, the written GTs in SLU dataset are converted into pseudo transcripts.
We set the prior probability $P(z)$ as 0.15 for ASR GLUE and 0.21 for DSTC10 Track2 dataset based on the validation set result of downstream SLU tasks\footnote{Matching $P(z)$ to word error rate of the ASR system used for the SLU seems straightforward but unfortunately inapplicable to ASR zero-shot setting where WER is unknown for unknown ASR. Also, training in arbitrary word error rates can cause the SLU model to be biased in certain ASR systems.}.
As downstream task models, we adopted BERT-base for ASR GLUE and GPT2-small for DSTC10 Track 2 following the settings from baseline results~\cite{dstc10_2,asrglue}.

















==> backup/ARR_Apr_15/5_results.tex <==
\section{Results}


\input{table/dstc_result}
We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are ISNI in the ASR zero-shot setting?

%\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ2:} Can ISNI robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ3:} Does each of ISNI contribute to robustification?

\subsection{RQ1: Validity of ASR Zero-shot Setting and Effectiveness of ISNI. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.


First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Noisy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.





%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ISNI showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
ISNI outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST2 of the low noise level.
Also, ISNI always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that ISNI can make SLU models generalizable in the ASR zero-shot setting.


In addition, ISNI robustifies SLU models against different noise levels.
ISNI showed little degradation in performance as noise levels increased compared to baselines.
That is, as prior work suggests, phoneme confusions more frequently occur~\cite{wu2022phonetic,petkov2013maximizing} and ours can robustify even when such phoneme confusion increases.




%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.








\subsection{RQ2: Robustification of ISNI on Various SLU Tasks.}
We show that ISNI can better robustify various SLU tasks over different SNI methods in ASR zero-shot setting.
%As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, caused by ASR errors.

We present the results of ISNI methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
Different from the previous observations where the identical ASR system is used for SNI and SLU tasks~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of ISNI is not limited to KS.
Overall, ISNI outperformed baselines in every task and every metric with a large margin except P of KTD.
ISNI showed the increase of the BLEU score by 2-3 times for RG.
These results show that ISNI can robustify against ASR errors in various SLU tasks.



\subsection{RQ3: Importance of Each Proposed Method to the Robustification. }
To confirm that each of ISNI contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results} and \ref{tab:ablation_rte} by deducting each of the proposed methods.

We report the result without the phoneme-aware generation in the fourth row of Table~\ref{tab:dstc_results} and ~\ref{tab:ablation_rte}.
Deducting the phoneme-aware generation showed a decreased score in every subtask of DSTC10 Track2 and high and medium noise levels of RTE, showing the importance of ASR-plausibility of pseudo transcription to robustify against ASR errors.
To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
As the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the fifth row of Table~\ref{tab:dstc_results} and ~\ref{tab:ablation_rte}. 
Performance is decreasing as expected in KS, which is our main consideration as it is largely influenced by lexical perturbation due to the ASR errors.
Such decrease is also observed in RG, showing that substituting the intervention contributes to the decreased performance in KS and RG.
Unexpectedly, the last row of Table~\ref{tab:dstc_results} shows the increased performance of KTD. 
We suspect such increase in KTD is due to its characteristic of text classification.
Meanwhile, prior work suggests that even the text classification may still degrade,  when the noises are more abundant in the training set~\cite{4470224}, to which ISNI may contribute.

%Previous work suggests that the abundance of noises in the training set may fail robustification in text classification \cite{4470224}.






==> backup/ARR_Apr_15/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we have addressed the challenge of ASR generalizability within the context of SNI. Our focus was on enhancing the robustness of downstream SLU models against ASR errors that may originate from diverse ASR systems. The existing SNI method is biased to a particular ASR system used for generating pseudo transcriptions.
To tackle the ASR generalizability issue, we introduce two key contributions. First, towards eliminating biases, ISNI significantly incorporates a wider range of ASR-plausible errors. However, such diversity should not interfere ASR-generic characteristcs, for which, our second step leads to the generation of errors that are commonly plausible, or ASR$_*$-plausible.
Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/ARR_Apr_15/limitations.tex <==
\paragraph{Limitations.}

As ISNI is trained with speech corpora collected for academic purposes, they may face challenges when adopted for real-world applications.
%We think ISNI would suffer from challenges similar to those encountered by ASR systems.
One example is handling diverse spoken language variations such as dialects and accents. 
These variations can introduce noises that are not phonetically similar, which are different from the speech data used during ISNI training. 
This discrepancy may fail ISNI to robustify SLU models as ISNI is not prepared to handle ASR errors from those speech variations.  %, potentially impacting its ability to robustify spoken language understanding (SLU) models across all speech variations. 
Addressing this limitation may require enlarging the training dataset of ISNI to include a wider array of noises due to such spoken language variation.
%ensuring it can effectively generalize across the diverse speech conditions found in practical applications.

%We make use of DeepSpeech ASR system, for the reason of its similarity in performance to many commercial ASR systems as we will discuss in Sec.~\ref{sec:asr_details}.


%However, our ISNI may not well be trained with different ASR systems due to several reasons.
%A notable reason is the scarcity of the training set due to rare ASR errors.
%As we described in Sec.~\ref{sec:dataset}, we only use the erroneous transcriptions for training ISNI.
%However, when the ASR system is too strong, it may make not enough erroneous transcriptions to train ISNI.
%The most straightforward method is to use the other weaker ASR system for training, as our ISNI can %generalize to different ASR systems.
%Second, previous works suggest training the weaker version of the ASR system and using it for training SNI~\cite{dutta2022error}.





==> backup/ARR_Dec_15/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLM) have been adopted in spoken language understanding (SLU) with automatic speech recognition (ASR) systems.
A widely used pipeline is leveraging PLMs subsequent to ASR transcribing audio inputs, where transcriptions are input to PLMs to facilitate downstream SLU tasks.
While the quality of transcriptions is critical in such pipeline,
ASR systems often incorrectly transcribe the spoken language into phonetically similar but semantically different words.
Our target problem is training SLU models to tolerate plausible ASR errors, by exposing to errors that are likely to be observed in ASR systems, which we denote as ASR-plausibility.
For such goal, we first augment pseudo transcription errors from  ASR$_i$,
which is inevitably conditional to a particular ASR$_i$, while a likely error in ASR$_i$
is not necessarily so in ASR$_j$.
To ensure SLU models not to be biased to ASR$_i$ used during augmentation,
we propose two phases: We first mitigate biases to  ASR$_i$, then we ensure our
augmentation to satisfy ASR-generic plausibility that holds for any ASR$_*$.
Our proposed approaches 
improve both the diversity and plausibility of the pseudo transcription, to eventually improve the robustness and generalizability of SLU models.
Experimental results and analysis show the effectiveness of our proposed methods.
\end{abstract}

==> backup/ARR_Dec_15/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/ARR_Dec_15/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/ARR_Dec_15/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/ARR_Dec_15/1_intro_short.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs thus have gained widespread acceptance and employment within the realm of spoken language understanding (SLU) as applied in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
A concrete instance of this application involves a pipeline leveraging PLMs subsequent to the automatic speech recognition system (ASR) transcribing audio inputs. The resulting transcriptions are input to PLMs to facilitate downstream SLU tasks.


However, such pipeline would encounter challenges when confronted with inaccuracies stemming from ASR systems incorrectly transcribing speech into phonetically akin yet semantically unrelated terms~\cite{ruan20_interspeech,9054689}, which we denote as, ASR error words.
This inherent issue undermines the capacity of PLMs to discern meaningful semantics from such flawed transcriptions. To illustrate, consider Fig.~\ref{fig:example}, 
where ASR systems, confused between  ``cereal'' and ``serial'', ``quarry'' and ``carry'', may generate an incorrect transcription such as ``workers eat serial in the carry''.
These ASR error words, despite the phonetic resemblance, convey unintended meanings, thereby obstructing the coherent semantics of the spoken content in the downstream SLU tasks~\cite{belinkov2018synthetic}.




A well-known solution is annotating likely incorrect transcriptions, known as speech noise injection, or, SNI~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
An SLU corpus annotation typically starts from a corpus of written 
text as a ground-truth (GT), recorded into audio, then
transcribed into text using ASR systems.
A more efficient alternative is, skipping the recording and transcription,
to directly corrupt the written GT, to
 introduce noise to the original written sentence, creating a pseudo transcription that closely aligns with the expected output of an ASR system.
 Desirably, SNI noise should be ``ASR-plausible'', indicating the pseudo transcription is likely to be generated by ASR systems.

\input{figure_latex/figure1}


However, by definition, ASR plausibility is 
conditional to a particular ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may be implausible in another ASR~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR$_1$ would be implausible to ASR$_2$ which generates the correct transcript on `cerial' while confusing `r' and generating the error word `walkers'. 
In contrast,
we propose to generate pseudo transcription  that
generalizes beyond a particular ASR system.


Our distinctions are two steps: 
First, after generating noises conditional to ASR$_i$,
we debias its dependence on ASR$_i$.
We generate  ASR$_i$-plausible noises, by introducing a binary variable $z$, which determines whether the word $x$ in the written GT would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR$_1$ would corrupt the word `cue' and `ceiling' with character `c',
and training with such pseudo transcripts
can only robustify against errors from ASR$_1$,
but may fail to robustify against those from ASR$_2$.
To mitigate such bias,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 

To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-plausible noise words given the words in the written sentences, with do-calculus implemented by evenly corrupting the words in the written sentences.
For example, as depicted in Fig.~\ref{fig:example}, our SNI model can corrupt the word `reading' with the phoneme `\textturnr'  which was corrupted in ASR 2 but not in ASR 1, in addition to the ones corrupted by baseline SNI,  as a result of such diversification.



Then, we ensure debiased noises follow common characteristics shared by any ASR, or, ASR$_*$.
For example, in Figure~\ref{fig:example}, ASR$_1$ plausible noises would be transcribing `c' from `cereal' as
`serial'.
However, `c' can sound differently in another word, `cue' with k sound,
where replacing c with s (or, replacing `cue' with `sue') is not plausible for any ASR system.
To ensure noise generation to aware of such ASR-generic characteristics, we provide additional phoneme information that `c' is pronounced as the phoneme `k' and evaluate the noise generation probability according to such phoneme information,
to more ASR-plausible word `queue', regardless of the ASR system used, or ASR$_*$-plausible.


Experiments are conducted in ASR zero-shot setting where SNI models are trained on ASR$_i$ and the SLU task is tested on another ASR$_j$ on DSTC10 Track2 and ASR GLUE benchmark.
Results show that our proposed methods are effective in ASR generalization with comparable or even outperforming performance compared to the in-domain setting where ASR$_j$ is used to train the SNI model.



==> backup/ARR_Dec_15/2_prelim.tex <==
\section{Preliminaries}

Before we present our proposed Interventional SNI (ISNI), we formally define SNI and introduce related work as preliminaries

\subsection{Problem Formulation}
SNI model can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$ which is expected to mimic ASR$_i$. %, including its error.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with  $n$ words, SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, which ASR$_i$ would transcribe into.
The resulting pseudo transcription, $T_i$, is used to train downstream SLU models.
However, as errors obtained from this model may not generalize to ASR$_j$, we propose to build the SNI model $\textit{F}_*$ which can generate ASR$_*$ plausible pseudo transcript $T_*$


\subsection{Related Work}
\subsubsection{SNI}
Previously proposed methods can be summarized as three categories. %, TTS(Text-To-Speech)-ASR pipeline,  textual perturbation, and auto-regressive generation.%, which differ in how to generate the noise word $t^{k}_i$ given the word $x^k$ and ASR$_i$.
First, TTS (Text-to-Speech)-ASR pipeline~\cite{tian2021tod-da, asrglue} adopts the TTS engine, the reverse of ASR, to convert written text into audio, which, then, the ASR$_i$ transcribes into pseudo transcription. 
However, the human recording and TTS-generated audio differ in their error distributions, which makes the resulting pseudo transcriptions different~\cite{asrglue}. 
%The most intuitive method of SNI is the TTS-ASR pipeline~\cite{tian2021tod-da, asrglue}, where a TTS engine converts the written text into audio, then an ASR$_i$ transcribes the audio. 
%During the conversion between the text and audio, ASR$_i$ would incorrectly transcribe the written word $x^{k}$ into the ASR$_i$ plausible noise word $t_{i}^{k}$.
%However, due to different error distributions between the human recording and the audio generated by TTS, the resulting pseudo transcription would have a different error distribution from the ASR transcription~\cite{asrglue}.
%The exhaustive cost of the TTS engine and ASR system makes such methods hard to adopt for large-scale corpora. 

Second, textual perturbation replaces the words $x^k \in X$ to the noise word $t_{i}^{k}$ as follows:
\begin{equation}
   t^{k}_i = argmax_{w \in W} \textit{S}_i(w|x^{k}),
\end{equation}
where $\textit{S}_i(w|x^{k})$ evaluates the score that ASR$_i$ would corrupt the written word $x^k$ into each word $w \in W$ in the vocabulary set $W$.
A widely adopted type of $\textit{S}_i(w|x^{k})$ is a confusion matrix built from the paired written and ASR transcribed corpora~\cite{confusion_matrix, confusion_matrix2} or phonetic similarity function~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}.
%Despite the efficiency of these textual perturbation methods, 
Due to its ignorance of the context, it is outperformed by third method~\cite{noisygen}.

Third is  the auto-regressive generation, where
auto-regressive PLMs such as GPT-2 or BART are supervised to maximize the likelihood of the ASR transcription $T_i$ given its written text $X$. 
Adopting PLMs, the auto-regressive generation can consider contextual information and generate more ASR$_i$ plausible noise words~\cite{noisygen}.

We adopt the third category with the most competitive results in various SLU tasks as our baseline~\cite{noisygen,asrglue}.
Our distinction is, while auto-regressive generation is biased to ASR$_i$, % plausible noise words,
generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.% e a noised version given the ground-truth transcription.

\subsubsection{ASR Correction}
As an alternative, ASR correction 
aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT.
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperform ASR correction~\cite{asrglue}, which explains why we focus on SNI.






==> backup/ARR_Dec_15/3_ours.tex <==
\section{Methods}
We now propose our SNI model, which aims to generate pseudo transcription that can robustify SLU tasks against ASR$_*$.
\subsection{Interventional SNI for Debiasing}
\label{interventional_sni}
Our first step for such goal is to debias the dependence of SNI on ASR$_i$ with do-calculus.
Before we explain our Interventional SNI, we introduce do-calculus.
Do-calculus aims to more robustly understand the causal effect of variable $X$ on another variable $Y$.
Using bayes rule, conventional likelihood $P(Y|X)$ can be written as follows:
\begin{equation}
    P(Y|X) = \sum_{z\in Z}P(Y|X,z)\cdot P(z|X),
    \label{eq:likelihood}
\end{equation}
where $Z$ is the mediator, which is influenced by $X$ and influences to $Y$.
However, likelihood $P(Y|X)$ can be easily biased when $X$ is correlated to the mediator $Z$.
That is, when a specific value of $X$ is strongly correlated to $z$ and has large $P(z|X)$, resulting $P(Y|X)$ would be influenced by the value of $P(Y|X,z)$, even when the other value of $X$ would have different $P(Y|X,z)$.
Do-calculus reduces such bias by intervening in the influence of $X$ on $z$, using do operator to conventional likelihood as follows:
\begin{align}
    P(Y|do(X)) &= \sum_{z}P(Y,z|do(X))\\
    &= \sum_{z}P(Y|do(X),z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z|do(X))\\
    &= \sum_{z}P(Y|X,z)\cdot P(z).
    \label{eq:do}
\end{align}
We refer proof of transition between $P(z|do(X))$ and $P(z)$ to the book~\cite{glymour2016causal}.
Compared to $P(z|X)$ in Eq.~\ref{eq:likelihood}, $P(z)$ in Eq.~\ref{eq:do} is no longer influenced by $X$, thus the influence of $X$ on $Y$ through the mediator $z$ is mitigated.


%To debias the dependence, we propose to intervene in the variable $z$, which determines whether the word $x^k$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
Now, we first reveal that the SNI model depends on ASR$_i$ by introducing the variable $z$, which determines whether the word $x^k$ would be corrupted ($z=1$) or not ($z=0$) in the resulting pseudo transcript.
Using the variable $z$, the SNI process can be written as follows:
\begin{equation}
     P(t^{k}|x^{k}) = \sum_{z}P(t^{k}|x^{k},z)\cdot P(z|x^{k}).
     \label{eq:sni_definition}
\end{equation}
Then, the SNI model $P(t^{k}|x^{k})$ is biased to ASR$_i$ such that the word $x^k$ would have large $P(z|x^{k})$ if $x^k$ is frequently corrupted by ASR$_i$, while that of others would be low.
%As a result, the word $x^k$ with frequently corrupted by ASR$_i$ would be corrupted in the pseudo transcriptions.

%From the formulation of SNI in Eq.~\ref{eq:sni_definition}, we argue that $P$
%For such goal, we introduce the variable $z_i$, which determines whether the word $x_i \in X$ would be corrupted ($z_i=1$) or not ($z_i=0$) in the resulting pseudo transcript.
%An ASR system would frequently generate incorrect transcription, thus, $x_i$ with specific phonemes tend to have large $P(z_{i}|x_{i})$, while that of others would be low.
%Mimicking the ASR system, the SNI model would have a similar distribution of $P(z_{i}|x_{i})$.


%\sw{our contribution is adopting do-calculus to represent intervention }




To debias the dependence on ASR$_i$, we propose to intervene $z$, so that the resulting pseudo transcript would contain diverse noise words even when they are rarely corrupted by ASR$_i$.
%Intervening $z$, we aim to manipulate $P(z|x^k)$ so that $P(z|x^{k})$ of rarely corrupted phonemes would be increased while that of frequently corrupted phonemes would be decreased. 
%As a result of such manipulation, the words $x^k$ rarely corrupted by ASR$_i$.
Specifically, we reduce any influence from the intervened variable, $x^k$, on $z$ using do-calculus and we have the SNI modeled as follows:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
As a result of the intervention in Eq.~\ref{eq:do-calculus}, whether or not to corrupt the words $x^k$ is determined independently from ASR$_i$ so that rarely corrupted words $x^k$ would be corrupted in the pseudo transcription.
Specifically, for each word $x^k$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$, which determines whether the word $x^k$ would be corrupted.
If $d^k\leq P(z)$, $z$ is set as 1, and $t^{k}$ would be a noise word and need to be generated.
Otherwise, $z$ is set to 0, and $t^{k}$ would be identical to $x^{k}$ as a simulation of the successful transcription.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
The prior probability $P(z)$ can be considered as the probability of corrupting the word $x^{k}$, which we set as a hyperparameter.

%In Eq.~\ref{eq:do-calculus},  whether or not to corrupt the word $x_i$ is determined independent of the word $x_i$.
%To implement Eq.~\ref{eq:do-calculus}, we propose to determine whether or not to corrupt the word $x^k$ explicitly. 
%Specifically, for each word $x_i$, we sample random variable $d^k$ from the continuous uniform distribution of interval $[0,1]$.
%Then, the value of $z$ is determined as 1 if $d^k\leq P(z)$ else 0.
%If $z$ is set to 0, $t^{k}$ would be identical to $x^{k}$ which simulates the successful transcription of the ASR system.
%If $z$ is set to 1, $t^{k}$ would be a noise word and need to be generated.
%Removing the bias from following individual ASR error distribution, the resulting pseudo-ASR would have diverse ASR error patterns and can better robustify downstream task models.

%When $x_{i}$ is determined to be corrupted, the noise word $t_{i}$ should be generated as modeled by $P(t_{i}|x_{i},z)$.
We propose to model $P(t^{k}|x^{k},z)$ adopting constrained generation~\cite{constdecoder}.
The key characteristic of ASR error is that the ASR error word $t^{k} \in T$ is phonetically similar to its cleanly written form $x^{k} \in X$.
%Modeling $P(t_{i}|x_{i},z)$ can use such characteristic by generating $t_i$ constrained on $x_i$. 
Generated under the constraint on $x^{k}$, the noise word $t^{k}$ is phonetically similar to the cleanly written word $x^{k}$.
Replacing $x^{k}$ to the generated noise word $t^{k}$, $X$ is corrupted into pseudo transcription $T$.

To implement constrained decoding~\cite{constdecoder}, we use BERT~\cite{devlin-etal-2019-bert} to encode the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(WE(X)+PE(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $WE$ and $PE$ are word and position embeddings.

The transformer decoder~\cite{NIPS2017_3f5ee243} is used to generate the noise word $t^{k}$ constrained on the written word $x^k$.
Specifically, the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ representing the beginning of the generation is formulated as input of the decoder as follows:     
\begin{equation}
    E_{decoder}^{k}=M_{d}[e_{encoder}^{k}; bos],
    \label{eq:decoder_input}
\end{equation}
where  $M_d$ is the weight matrix of linear transformation.
The transformer decoder outputs the hidden representation $h^{k}$ as follows:
\begin{align}
    h^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K=E_{encoder},V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ is used as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability distribution $\textit{P}_{lm}(\hat{t}^{k})$ measures the probability of each token in vocabulary to be noise word $t^k$ as follows:
\begin{equation}
    \textit{P}_{lm}(\hat{t}^{k}) = softmax(WE \cdot h^{k}+b_{d}),
    \label{eq:gen_prob}
\end{equation}
where $b_{d}$ are trained parameters. 

We used the ASR transcription $T$ to train our interventional SNI model.
Specifically, our SNI model is supervised to maximize the log-likelihood of the ASR error word $t^{k}$ as follows:
\begin{equation}
    l_{lm} =-\sum log(\textit{P}_{lm}(t^{k})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to ensure the noise word generation ASR$_*$-plausible.
The common characteristic of ASR$_*$ is that any incorrect transcription is phonetically similar to its written GT.
However, fed only words, not their pronunciation, auto-regressive SNI can generate noise words similar in character, not pronunciation.
To ensure ASR$_*$-plausibility, we propose to discourage the generation of phonetically different noise words.
Toward our goal of ASR$_*$-plausible noise words, we propose to adjust the generation probability $\textit{P}_{lm}(\hat{t}^{k})$ with the phoneme-based generation probability $\textit{P}_{phoneme}(\hat{t}^{k})$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{equation}
    \textit{P}_{gen}(\hat{t}^{k}) = \textit{P}_{lm}(\hat{t}^{k}) \cdot \textit{P}_{phoneme}(\hat{t}^{k})  
    \label{eq:phoneme_correction_prob}
\end{equation}


Our first proposal for $\textit{P}_{phoneme}(\hat{t}^{k})$ is to provide phonetic information via phoneme embedding $PHE$.
The main difficulty of evaluating $\textit{P}_{phoneme}(\hat{t}^{k})$ is that PLMs are not aware of how the written sentences are pronounced.
Our proposed phoneme embedding $PHE$ is designed to have the phonetic information of each token in the vocabulary.
Thus, feeding the phoneme embedding $PHE$ can deliver how each word in written sentences is pronounced.
Specifically, the input for the encoder is formulated using the phoneme embedding as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot WE(X)\\+(1-\lambda_{w})\cdot PHE(X)+PE(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is the weight to balance the word embedding and phoneme embedding.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, then, the decoder would yield the hidden representation $h^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we use the hidden representation $h^k$ to evaluate the phoneme based generation probability $\textit{P}_{phoneme}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{P}_{phoneme}(\hat{t}^{k}) = softmax(PHE \cdot h^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where $PHE$ is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and $b_{ph}$ is trainable parameter.
Using the phoneme embedding $PHE$ instead of the word embedding $WE$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{phoneme}(\hat{t}^{k})$ can be evaluated based on the phonetic information.


Our second proposal for $\textit{P}_{phoneme}(\hat{t}^{k})$ is to supervise the phonetic information using phonetic similarity.
To generate ASR$_*$-plausible noise words, $\textit{P}_{phoneme}(\hat{t}^{k})$ should evaluate how phonetically similar each word in the vocabulary is to the $x^{k}$.
As phonetic similarity can satisfy such goal by measuring the difference of phonetic code, we adopt it to supervise $\textit{P}_{phoneme}(\hat{t}^{k})$.
Specifically, phonetic similarity $\textit{PS}$ is evaluated using the phoneme edit distance $\textit{PD}$~\cite{9662078}.
The phoneme edit distance $\textit{PD}$ measures the difference of the phonetic code between the given two words $w^{p}$ and $w^{q}$.
First, two words are converted into phonetic code $C^p=\{c_{r}^{p}\}_{r=1}^{|C^p|}$ and $C^q=\{c_{r}^{q}\}_{r=1}^{|C^q|}$, where each characters represents how the word is pronounced.
Then, the phoneme edit distance $\textit{PD}(w^{p}, w^{q})$ is Levenshtein distance, the minimum edit distance, between the phonetic codes which is evaluated as follows:
\begin{equation}
    \textit{PD}(w^{p}, w^{q}) = Levenshtein(C^p,C^q).
    \label{eq:phoneme_edit_distance}
\end{equation}
Then, phonetic similarity $\textit{PS}$ can be defined as follows:
\begin{equation}
    \textit{PS}(w^{p}, w^{q}) = max(|C_p|-\textit{PD}(w^{p}, w^{q}), 0),
\end{equation}
so that $\textit{PS}(w^{p}, w^{q})$ is larger when $w^p$ and $w^q$ are phonetically similar and 0 when they are phonetically different.

To supervise $\textit{P}_{phoneme}(\hat{t}^{k})$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{PS}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{PS}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{phoneme}(\hat{t}^{k})$ is supervised by loss defined as follows:
 \begin{equation}
     l_{phoneme} = \textit{D}_{KL}(\textit{P}_{phoneme}(\hat{t}^{k}),  \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $\textit{D}_{KL}$ is the KL divergence loss.
Finally, our proposed ISNI model is optimized to jointly minimize the total loss $l_{tot}$ which is defined as follows:
\begin{equation}
    l_{tot} = l_{lm} + \lambda_{phoneme} \cdot l_{phoneme},
\end{equation}
where $\lambda_{phoneme}$ is the weight of $l_{phoneme}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{phoneme}(\hat{t}^k)$ can ensure the ASR$_*$-plausible noise words and $PHE$ can contain phonetic information.
 

 




==> backup/ARR_Dec_15/4_experiment.tex <==
\section{Experiments}
In this paper, we first experimentally confirm the validity of the ASR zero-shot setting, where SNI trained with ASR$_i$ cannot robustify against ASR$_j$ and the effectiveness of our proposed methods in the ASR zero-shot setting.
%For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.
Then, we show that our proposed methods can robustify various SLU tasks in the ASR zero-shot settings better than previous SNI methods.
\subsection{Dataset}

To test the ASR generalizability, we formulated an ASR zero-shot setting by adopting ASR systems with distinct architecture and training sets to transcribe SNI and downstream tasks. 
For training the SNI model, we used the Mozilla DeepSpeech\footnote{https://github.com/mozilla/DeepSpeech}.
The audio of each downstream task, DSTC10 Track 2 and ASR GLUE benchmark, is transcribed by distinct ASR systems different from DeepSpeech.
We provide further details of ASR systems in Sec.~\ref{sec:asr_details}.

%\input{table/dataset_statistics}

For training the SNI model, we followed the settings from our main baseline, Noisy-Gen~\cite{noisygen}, which used popular speech corpora, Common Voice, tatoeba audio, and LJSpeech-1.1, to collect ASR error transcriptions.
Specifically, we put the audio recordings of the above corpora into the DeepSpeech and get ASR transcriptions. 
Then, we compare ASR transcription with ground-truth transcription, ignoring punctuation and casing errors, so that only ASR error transcriptions would remain. 
Finally, we obtain about 930k pairs of ground-truth transcription and the ASR-noised transcription pair.



\input{table/asrglue_result}
ASR GLUE benchmark is an SLU version of the widely adopted NLU benchmark, GLUE.
The key reason for adopting the ASR GLUE benchmark is that it provides the diverse transcription of 3 noise levels spoken by 5 distinct human annotators.
Among various subtasks, we provide the results of two NLI tasks, QNLI and RTE, and 1 sentiment classification task, SST, which the DSTC10 Track2 dataset does not contain.
As the ground-truth label for the test set is unavailable, we explicitly organized the validation set from the train set and report the results on the development set.

DSTC10 Track2 dataset models task-oriented dialogue systems with unstructured knowledge access in a spoken language.
We adopt the DSTC10 Track2 dataset as it contains various tasks in NLP in the dialogue domain where SLU is required frequently.
Specifically, it consists of three successive subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS), and Knowledge-grounded Response Generation (RG), where human responses are transcribed by an unknown ASR system.
First, KTD aims to determine whether the dialogue turn requires external knowledge access or not as a classification. 
Once determined to require external knowledge, the second step is KS, which aims to retrieve the appropriate knowledge snippet by estimating the relevance between the given dialogue context and each knowledge snippet in the knowledge base.
Finally, the response is generated in RG, based on the dialogue context and the selected knowledge snippet. 





\subsection{Experimental Settings}
For SNI, we trained our SNI model with collected ground-truth transcription and the ASR-noised transcription pair.
Specifically, we adopted BERT-base~\cite{devlin-etal-2019-bert} as an encoder for our SNI model following previous work~\cite{constdecoder}.
We used Transformer decoder~\cite{NIPS2017_3f5ee243} with 1 layer which has 12 attention heads and 768 hidden layer dimensions, identical to BERT-base.
We trained our SNI model for 20 epochs with Adam optimizer with a learning rate of 0.00005.
Also, we set $\lambda_{w}$ and $\lambda_{phoneme}$ as 0.5 to balance the semantic and phonetic information. 

Using the trained SNI model, the written GTs in DSTC10 Track2 dataset and ASR GLUE dataset are converted into pseudo transcripts.
We set the prior probability $P(z)$ as 0.21 for DSTC10 Track2 dataset and 0.15 for ASR GLUE dataset based on the validation set result of downstream SLU tasks.
As downstream task models, we adopted the GPT2-small for DSTC10 Track2 and BERT-base for ASR GLUE following the settings from baseline results~\cite{dstc10_2,asrglue}







\subsection{Baselines}
Our main baseline is NoisyGen, GPT2-based auto-regressive generation SNI model~\cite{noisygen}. 
NoisyGen is trained with a training set identical to ours.
Pseudo-transcriptions generated by NoisyGen are filtered by phoneme-based heuristics. 

For ASR GLUE benchmark, we adopt another baseline Noisy-Gen (In Domain)~\cite{asrglue}.
NoisyGen and NoisyGen (In Domain) are similar in that they are both GPT2-based SNI models.
However, NoisyGen (In Domain) uses the identical ASR system to transcribe the test set of ASR GLUE benchmark, which is improbable in the ASR zero-shot setting.
Comparing with NoisyGen (In Domain) can show how SNI models are successful in ASR generalizability.

For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
TOD-DA encompasses both the TTS-ASR pipeline and
textual perturbation techniques.
It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
Also, it conducted character-level perturbation of substitution, insertion and dele

==> backup/ARR_Dec_15/5_results.tex <==
\section{Results}


We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are our proposed methods in the ASR zero-shot setting?

\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ3:} Can our proposed methods robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ4:} Does each of our proposed methods contribute to robustification?

\subsection{RQ1: Validity of ASR zero-shot setting and effectiveness of our proposed methods. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To show the ASR generalizability of SNI models, we compare them with Noisy-Gen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Different from Noisy-Gen and ours tested in the ASR zero-shot setting, the training set of Noisy-Gen (In Domain) used the ASR system identical to the test set, which is improbable in the ASR zero-shot setting.


First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
If different ASR models are highly correlated and have similar error distributions, existing auto-regressive generation SNI models can well generalize in an ASR zero-shot setting.
However, Noisy-Gen which is trained with a larger training corpus, is outperformed by Noisy-Gen (In Domain) in every task.
Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Nosiy-Gen in the medium noise level.
This result shows the validity of the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize.

%\sw{zero-shot, trained in i, test in j, In Domain}
In contrast, ours showed comparable or even outperforming results to Noisy-Gen (In Domain), in the ASR zero-shot setting.
Specifically, ours outperformed Noisy-Gen (In Domain) in QNLI of the high and medium noise levels and in SST of the low noise level.
Also, ours always outperformed Noisy-Gen with ASR errors in every subtask.
These results show that our proposed methods can make SLU models ASR generalizable in the ASR zero-shot setting.






%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.

\subsection{RQ2:Phoneme-aware generation for ASR$_*$-plausiblity. }
\input{table/phoneme_edit_distance}
\input{table/dstc_result}
In this section, we show that PLMs are insufficient to generate the ASR$_*$-plausible pseudo transcriptions.
The noise words would be ASR$_*$-plausible if it is phonetically similar to its written form as an ASR system would incorrectly transcribe into phonetically similar noise words.
Therefore, we compared the phoneme edit distance defined in Eq.~\ref{eq:phoneme_edit_distance} between the written GT and the pseudo transcriptions.
For a fair comparison, we set identical $P(z)$ for the noise word generation to ensure that the identical words are corrupted.

Table~\ref{tab4:phoneme_edit_distance} shows that the pseudo transcriptions without phoneme-aware generation show 17\% larger phonetic distance.
This result shows that PLMs are not enough to generate the ASR$_*$-plausible pseudo transcriptions and ignorance of phonetic information is the obstacle to generating ASR$_*$-plausible pseudo transcriptions.






\subsection{RQ3: Robustification of Our Proposed Methods on Various SLU Yasks.}
In this section, we show that our proposed methods can better robustify various SLU tasks over different SNI methods in ASR zero-shot setting.
%As DSTC10 Track 2 dataset requires the correct recognition of the entity such as hotels~\cite{dstc10_2}, which is largely influenced by ASR errors, we mainly considered DSTC10 Track 2 dataset to show the effectiveness in robustification.
Among different subtasks, we mainly considered KS as the retrieval task is largely influenced by lexical perturbation~\cite{ir_error_robustness1, ir_error_robustness2}, which can be caused by ASR errors.

We present the results of our proposed methods and baselines on DSTC 10 Track 2 dataset in Table~\ref{tab:dstc_results}.
We can observe that baselines struggle to robustify SLU tasks against ASR errors in the ASR zero-shot setting, showing R@1 score below 60.
Different from the previous observations where the identical ASR system is used for SNI and SLU tasks~\cite{asrglue,noisygen}, Noisy-Gen showed inferior results than TOD-DA. 
In contrast, ours outperforms baselines in every metric in KS by a large margin, showing that ours can robustify against ASR errors made by an unknown ASR system.

Results in Table~\ref{tab:dstc_results} show that the robustification of our proposed methods is not limited to KS.
Overall, ours outperformed baselines in every task and every metric with a large margin except P of KTD.
Specifically, ours showed the increase of the BLEU score by 2-3x times for RG.
These results highlight that our proposed methods can robustify against ASR errors for various downstream SLU tasks.



\subsection{RQ4: Importance of Each Proposed Method to the Robustification. }
To confirm that each of our proposed methods contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results}.
Specifically, we deducted our proposed methods in turn.

We report the result without the phoneme-aware generation in the fourth row in Table~\ref{tab:dstc_results}.
Deducting the phoneme-aware generation showed a decreased score in every subtask, showing the importance of ASR plausibility of pseudo transcription to robustify against ASR errors.
To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
Specifically, as the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:sni_definition}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
Decreased performance of the last row shows that the intervention itself contributes to robustification.


==> backup/ARR_Dec_15/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we have addressed the challenge of ASR generalizability within the context of SNI. Specifically, our focus was on enhancing the robustness of downstream SLU models against ASR errors that may originate from diverse ASR systems. The existing SNI method is biased to a particular ASR system used for generating pseudo transcriptions.
To tackle the ASR generalizability issue, we introduce two key contributions: Interventional SNI and Phoneme-aware Generation. First, towards eliminating biases, Interventional SNI method significantly incorporates a wider range of ASR-plausible errors. However, such diversity should not interfere ASR-generic characteristcs, for which, our second step of Phoneme-aware Generation, leads to the generation of errors that are commonly plausible, or ASR$_*$ plausible.
Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/ARR_June/0_abs.tex <==
\begin{abstract}
Recently, pre-trained language models (PLMs) have been increasingly adopted in spoken language understanding (SLU). 
However, automatic speech recognition (ASR) systems frequently produce inaccurate transcriptions, leading to noisy inputs for SLU models, which can significantly degrade their performance. 
To address this, our objective is to train SLU models to withstand ASR errors by exposing them to noises commonly observed in ASR systems, referred to as ASR-plausible noises. 
Speech noise injection (SNI) methods have pursued this objective by introducing ASR-plausible noises, but we argue that these methods are inherently biased towards specific ASR systems, or ASR-specific noises.
In this work, we propose a novel and less biased augmentation method of introducing the noises that are plausible to any ASR system, by cutting off the non-causal effect of noises.
Experimental results and analyses demonstrate the effectiveness of our proposed methods in enhancing the robustness and generalizability of SLU models against unseen ASR systems by introducing more diverse and plausible ASR noises in advance. %Specifically, our methods improved SLU model accuracy by X% when tested on unseen ASR systems, showcasing their potential for broader application.
\end{abstract}
\begin{comment}
    Recently, pre-trained language models (PLMs) have been adopted in spoken language understanding (SLU). 
As automatic speech recognition (ASR) systems often transcribe spoken language inaccurately, noisy inputs are introduced to SLU models. 
Our goal is to train SLU models to tolerate these ASR errors by exposing them to noises that are likely to be observed in ASR systems, which are denoted as ASR-plausible noises.
Speech noise injection (SNI) achieves such goal by introducing ASR-plausible noises that are inevitably biased to a particular ASR system.
Our distinction is first to mitigate biases towards a particular ASR system, then ensure
that augmentation to satisfy ASR-generic plausibility applicable to any ASR system.
Experimental results and analyses show the effectiveness of our proposed methods in improving the robustness and generalizability of SLU models against unseen ASR systems by introducing more diverse and plausible ASR noises in advance.
\end{comment}

==> backup/ARR_June/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/ARR_June/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> backup/ARR_June/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.

==> backup/ARR_June/1_intro_short.tex <==
\section{Introduction}
\input{figure_latex/figure1}
Pre-trained language models (PLMs) have demonstrated a robust contextual understanding of language and the ability to generalize across different domains. 
Thus, PLMs have gained widespread acceptance and been employed within the realm of spoken language understanding (SLU), such as voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}. 
A concrete instance of this application is a pipeline where an automatic speech recognition (ASR) system first transcribes audio inputs, and the transcriptions are then processed by PLMs for downstream SLU tasks~\cite{asrglue}.



However, such pipelines encounter challenges when faced with inaccuracies from ASR systems. 
We refer to these inaccuracies as ASR error words, which are phonetically similar but semantically unrelated~\cite{ruan20_interspeech,9054689}. 
For instance, as shown in Fig.~\ref{fig:example}, ASR systems might confuse words like ``cereal'' and ``serial'' or ``quarry'' and ``carry'', resulting in incorrect transcriptions such as ``workers eat serial in the carry''. 
Despite their phonetic resemblance, these ASR error words convey unintended meanings, thereby impeding the semantic understanding of speech in SLU tasks~\cite{belinkov2018synthetic}.





A well-known solution is speech noise injection (SNI) which generates likely incorrect transcriptions, namely pseudo transcriptions, then exposes PLMs to the generated pseudo transcriptions while training SLU tasks~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Thus, the injected noises should be ASR-plausible, being likely to be generated by ASR systems from real audio input, for which the traditional methods attempted to replicate the ASR errors from written text. However, their ASR-plausibility is conditional on a particular ASR system, or ASR$_i$, where the error distribution from the collected transcriptions follows only the observed error distribution~\cite{confusion_matrix,confusion_matrix2,noisygen}.


However, different ASR systems have distinct error distributions~\cite{asr_pattern1}, which hinders the trained SLU models to be used with other ASR systems, ASR$_j$.
A straightforward solution to this issue might be to employ multiple ASR systems or to build multiple SLU models, but this approach incurs significant overheads and cannot account for the diversity of real-world ASR errors, \eg, errors due to environmental sounds. %\hist{environmental sounds 는 ASR errors 의 원인이지 그 종류처럼 언급되면 안 될 것 같은데요?}
Instead, we investigate a novel but easier solution of introducing better generalizable noises from a single ASR system.


For this purpose, we first identify the gap between the ASR transcription in SLU and SNI
%purpose 
from a causality perspective.
First, SLU tasks aim to handle real audio input, where written GTs are recorded as audio by humans, such that ASR errors are causally affected by recorded audio, as shown in Figure~\ref{fig:fig2_subfig1}. 
However, SNI,
%methods reverse the causal relationships, as they try to 
when replicating error patterns, may discard the correctly transcripted texts, biased towards the observed errors.
%We argue that this results in SNI being biased toward the observed error distributions, generating ASR$_i$-plausible noises. 
Inspired by causality literature, we introduce two technical contributions: 1) interventional noise injection and 2) phoneme-aware generation. 
Specifically, we adopt $do$-calculus to intervene the ``revised'' in SNI to
%causal relations and enforce deviating 
deviate rom the observed error distribution, thereby broadening the error patterns in the resulting pseudo transcripts.
For instance, as shown in Fig.~\ref{fig:example}, our SNI model can corrupt the word `Read' with the phoneme `\textturnr', which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the errors introduced by baseline SNI.
%our distinction is to generate pseudo transcripts that can generalize beyond a specific ASR system. 
%To achieve this, we introduce two technical contributions: 1) interventional noise injection and 2) phoneme-aware generation. 
%We begin by debiasing the dependence of noises on the specific ASR system, ASR$_i$, by applying \textit{do}-calculus. 
%Mimicking only the observed error distribution, causal relations in SNI are reversed from that of SLU.
%In SLU where the ASR systems generate from real audio input, ASR errors are causally affected by written GTs through recording written GTs into speech, then, ASR errors are made while transcribing recorded audio.
%In contrast, in SNI, ASR errors affect the observance of written GTs, reversed from SLU, as written GTs without incurring ASR errors lack the error patterns that SNI tries to replicate.
%\hist{Mimicking 문장부터 여기까지가 contributions 이전에 좀 설명이 되어야 할 것 같은데. For this purpose, we first identify the gap between SLU task definition and SNI purpose in causality perspective? Firstly, SLU tasks aim to handle real audio input, where written GTs are recorded as audio by human, such that ASR errors are causally affected by recorded audio, as shown in Figure~\ref{fig:fig2_subfig1}. However, SNI methods reverse the causal relationships, as they try to replicate error patterns, discarding the correctly transcripted texts. We argue that this is problematic ... Inspired by causality literature, we introduce two technical contributions: 1) interventional noise injection and 2) phoneme-aware generation. Specifically, we ... $do$-calculus ...}
%$do$-calculus intervenes in such reversed causal relations and enforces to deviate from the observed error distribution, thereby broadening the error patterns in the resulting pseudo transcripts. %\hist{$do$ 는 항상 너무 심오해서... 대체 뭘 한다는 걸까 싶네요ㅎ devlbert 논문 처럼 친절해야 좀 이해가 될 듯}\yj{일단 여기 고치고 3장 다시 고쳐보겠습니다}
%For instance, as shown in Fig.~\ref{fig:example}, our SNI model can corrupt the word `Read' with the phoneme `\textturnr', which was corrupted in ASR$_2$ but not in ASR$_1$, in addition to the errors introduced by baseline SNI.




    
Next, we ensure that the debiased noises are plausible for any ASR system, referred to as ASR$_*$. 
This involves making GT words and ASR noises phonetically similar based on the common characteristics shared by ASR$_*$~\cite{serai2022hallucination}. 
Along with the textual input, we incorporate information on how words are pronounced. 
By being aware of pronunciation, we can introduce ASR noises that are plausible regardless of the specific ASR system used, making them ASR$_*$-plausible.



Experiments were conducted in an ASR zero-shot setting, where SNI models were trained on ASR$_i$ and tested on SLU tasks using another ASR system, ASR$_j$, on the DSTC10 Track2 and ASR GLUE benchmarks. 
Results show that our proposed methods effectively generalize across different ASR systems, with performance comparable to, or even exceeding, the in-domain setting where ASR$_j$ is used to train the SNI model.


==> backup/ARR_June/2_prelim.tex <==
\section{Related Work}

\subsection{SNI}
Previously proposed methods can be broadly categorized into three main approaches. 
The first, a Text-to-Speech (TTS)-ASR pipeline~\cite{tts_asr, tts_asr2}, uses a TTS engine to convert text into audio, which is then transcribed by an ASR system into pseudo transcriptions. 
However, this method struggles due to different error distributions between human and TTS-generated audio, making the pseudo transcriptions less representative of actual ASR errors. 
The second approach, textual perturbation, involves replacing words in text with noise words using a scoring function that estimates how likely an ASR system is to misrecognize the words, often employing confusion matrices~\cite{confusion_matrix3, confusion_matrix5} or phonetic similarity functions~\cite{li-specia-2019-improving,tsvetkov-etal-2014-augmenting}. 
The third method, auto-regressive generation, utilizes PLMs like GPT-2 or BART to generate text that mimics the likelihood of ASR errors in a contextually aware manner, producing more plausible ASR-like noise~\cite{noisygen}. 


We consider auto-regressive noise generation as our main baseline as it has shown superior performance over other categories~\cite{asrglue,dstc10_2}
However, auto-regressive noise generation is biased to ASR$_i$, limiting the SLU model used for ASR$_i$. % plausible noise words.
Our distinction is generalizing SNI so that the SLU tasks can be conducted with ASR$_*$.
We provide a more detailed explanation of each category in Appendix~\ref{sec:rel_work}.
% e a noised version given the ground-truth transcription.

%As an alternative, ASR correction 
%aims to map (possibly noisy) ASR transcription $T_i$ to $X$. %,which can be considered as an inverse functional mapping of SNI $\textit{F}_i$, $\textit{F}_i^{-1} : T_i \rightarrow X$.
%In the SLU pipeline, the ASR transcription is fed to the ASR correction model beforehand, which is then fed to downstream models trained with the written GT. 
\subsection{ASR Correction}
As an alternative to SNI, ASR correction
aims to denoise (possibly noisy) ASR transcription $T_i$ into $X$:
Due to its similarity to SNI, similar methods, such as
 textual perturbation~\cite{leng-etal-2021-fastcorrect-2} and auto-regressive generation~\cite{robart, chen2024hyporadise}, were used.
Also, PLMs showed impressive results~\cite{robart}, as the ASR noise words can be easily detected by PLMs due to their semantic irrelevance.
Using such characteristics, the constrained decoding method which first detects ASR errors, then corrects detected ASR errors is proposed~\cite{constdecoder}.
However, the innate robustness of PLMs~\cite{heigold-etal-2018-robust} makes SNI outperforms ASR correction~\cite{asrglue}.
In addition, it introduces additional latency in the SLU pipeline for ASR correction before the SLU model to conduct SLU tasks.
In voice assistant systems like Siri, such additional latency is crucial as the SLU pipeline should deliver responses with minimal delay to ensure real-time interaction.
Therefore, we focus on SNI for its effectiveness and minimal latency in SLU pipeline.






==> backup/ARR_June/3_ours.tex <==
\section{Method}
Before introducing ISNI, we first formally define the problem of SNI and outline its causal diagram. 
Following this, we provide an overview of ISNI and detail the methods used to generate pseudo transcriptions that enhance the robustness of SLU tasks against ASR$_*$.

\subsection{Problem Formulation}
To robustify PLMs against ASR errors in SLU, the SNI model mimics the transcriptions of ASR$_i$ which can be defined as a functional mapping $\textit{F}_i: X \rightarrow T_i$.
Given the written GT $X=\{x^{k}\}_{k=1}^{n}$ with $n$ words, the SNI model $\textit{F}_i$ outputs the pseudo transcription $T_i=\{t^{k}_{i}\}_{k=1}^{n}$, simulating the transcriptions produced by ASR$_i$. 
These pseudo transcriptions, $T_i$, are subsequently used to train SLU models. 
For each word $x^{k}$, $z^{k} \in Z$ indicates whether ASR$_i$ make errors ($z^{k}=1$, hence $x^{k} \neq t^{k}_{i}$) or not ($z^{k}=0$, hence $x^{k}=t^{k}_{i}$). %\hist{whether .. correctly 인데 1일때는 incorrectly 인게 어색하네요}
However, noises generated by this model differ from those of the other ASR system, ASR$_j$, and SLU model trained with generated noises struggles with the errors from ASR$_j$.
Therefore, we propose building an SNI model, $\textit{F}_*$, capable of generating ``ASR$_*$-plausible'' pseudo transcripts $T_*$, which are plausible for any ASR system, ASR$_*$.

\subsection{Causality in SNI}
\input{figure_latex/figure2}
To achieve this, we compare the underlying causal relations between the transcription process in SLU and SNI training data generation, which are depicted in Fig.~\ref{fig:fig2_subfig1}. 
During ASR transcription, written GT $X$ is first spoken as audio $A$, which is then transcribed as transcription $T$ by ASR$_i$.
Depending on the audio $A$, ASR$_i$ may make errors ($Z=1$) or not ($Z=0$) in the transcription $T$. 
While transcribing, $X$ influences $Z$ through causal paths where every edge in the path is directed toward $Z$.

In SNI, the $X$ and $T$ transcribed by ASR$_i$ are filtered based on $Z$ since they do not exhibit the error patterns required for training.
However, such filtering induces a backdoor path and a non-causal relation in SNI. 
To further elucidate the causal relations in SNI training data generation depicted in Fig.~\ref{fig:fig2_subfig2}, we outline the causal influences as follows:
\begin{itemize}
\item $X \rightarrow T$: There is a direct causal relationship where the clean text $X$ influences the transcribed text $T$.
\item $Z \rightarrow T$: If $z^{k} \in Z$ is 1 (an error occurs), it directly affects the corresponding transcription $t^{k}_{i}$, causing it to deviate from the clean text $x^{k}$.
\item $Z \rightarrow X$: In the SNI training data collection process, $Z$ determines if $X$ is included. This means that only when the ASR system makes a mistake, indicated by any value $z^k \in Z$ being 1, the corresponding text is included in the training data. So, errors by the ASR system decide which clean texts are chosen.
\end{itemize}
The backdoor path $X \leftarrow Z \rightarrow T$, while ensuring that only instances where ASR$_i$ made errors are included, introduces bias in previous SNI models based on conventional likelihood, defined as: 
\begin{equation}
P(t^{k}_{i}|x^{k})=\sum_{z^{k}}P(t^{k}_{i}|x^{k},z^{k})P(z^{k}|x^{k}).
\label{eq:likelihood}
\end{equation}
Here, the mediator $z^{k}$, instead of being merely a consequence of $x^{k}$, also influences $x^{k}$.
Thus, the influence of $x^k$ to $t^k$ is drawn from $z^k$, not from $x^k$, thereby distorting the causal effect from $X$ to $T$. 
Such distortion skews the prior probability $P(z^{k}|x^{k})$ so that texts frequently incorrectly transcribed by ASR$_i$ are also noised by SNI.


\subsection{$do$-calculus for ISNI}
\label{sec:do_calculus}

To mitigate biases in SNI toward the ASR$_i$, we propose interventional SNI (ISNI) where the non-causal relations are cut off by adopting $do$-calculus.
Adopting $do$-calculus for conventional likelihood in Eq.~\ref{eq:likelihood}, ISNI can be formulated as follows:
\begin{equation}
    P(t^{k}|do(x^{k}))= \sum_{z^{k}}P(t^{k}|x^{k},z^{k})\cdot P(z^{k}).
    \label{eq:do}
\end{equation}  
Compared to Eq.\ref{eq:likelihood},  the prior probability $P(z^{k}|x^{k})$ is replaced with $P(z^{k})$.
This difference implies that the non-causal path $Z \rightarrow X$ is cut off, as the influence of $x^k$ on $t^k$ is not drawn from $z^k$ in Eq.~\ref{eq:do} as prior probability $P(z^k)$ is estimated independently from the non-causal path $Z \rightarrow X$. %\hist{confounder?}\yj{네 근데 confounder 단어를 쓰면 또 정의해줘야할 것 같아서 이렇게 설명하고 넘어가려고 합니다} 
Thus, the influence of $x^k$ to $t^k$ is induced solely from $x^k$.
We provide more detailed proof of Eq.~\ref{eq:do} in Appendix~\ref{sec:proof_do}.



\subsection{Overview of Our Proposed Approach}
\label{sec:overview}
\input{figure_latex/figure3}

In this section, we briefly overview how ISNI is implemented to generate ASR$_*$-plausible noises of different error types, as illustrated in Fig.~\ref{fig:fig3}.
%To achieve this, ISNI implements two distinct terms in Eq.~\ref{eq:do}, $P(z^{k})$ and $P(t^{k}|x^{k}, z^{k})$ for SNI.
To achieve this, ISNI implements two distinct terms in Eq.~\ref{eq:do}: $P(z^{k})$ and $P(t^{k}|x^{k}, z^{k})$.



For debiased noise generation $P(z^k)$, it is essential to cut off the influence of $x^k$ on $z^k$ so that $z^k$ becomes independent of $x^k$. 
ISNI explicitly controls $z^k$ and removes the dependence on $x^k$ by implementing SNI with constrained decoding, following \citet{constdecoder}.
Specifically, by utilizing do-calculus to determine $z$, ISNI introduces corruption in tokens that  ASR$_i$ transcribes correctly but ASR$_j$ may mistranscribe, thereby adding these as noise in the pseudo transcripts.
For example, the token $x$ with $z=1$, such as `cue' in Fig.~\ref{fig:fig3}, is fed to the constrained decoder.
The constrained decoder then generates the noise word $t$ to replace $x$.

\begin{comment}
    Specifically, by utilizing do-calculus to determine $z$, ISNI introduces corruption in tokens that  ASR$_i$ transcribes correctly but ASR$_j$ may mistranscribe, thereby adding these as noise in the pseudo transcripts.
\end{comment}


The noise word $t$ can be categorized as three conventional ASR error types: substitution, insertion, and deletion~\cite{jurafsky2019speech}, which is determined by the generation output of ISNI.
Substitution errors occur when the generated output is a new token that replaces $x$. 
Insertion errors occur when the constrained decoder outputs multiple tokens for $x$. 
For example, in Fig.~\ref{fig:fig3}, the constrained decoder outputs two `the' words for $x^2$, which means the insertion of the newly generated `the' beside the given word `the'. 
Deletion errors occur when the constrained decoder outputs only the $eos$ token, representing the end of generation. 
If the generation ends without any tokens, as in $t^5$, the empty string replaces $x^5$. 
ISNI generates these error types synthetically, as demonstrated in the quantitative study in Appendix~\ref{sec:quantitiate_study} and the generated examples in Appendix~\ref{sec:pseudo_transcripts_examples}.

For ASR$_*$-plausible generation $P(t^{k}|x^{k},z)$, we provide the phonetic information of $x$, such as `kju' in Fig.~\ref{fig:fig3}, to ISNI to understand how $x$ is pronounced. 
The constrained decoder evaluates the generation probability based on phonetic similarity, recognizing that `c' is pronounced as the phoneme `k'. 
Consequently, ISNI generates the ASR$*$-plausible noise word `queue' which is phonetically similar to `cue'.







\subsection{Interventional SNI for Debiasing}
\label{sec:interventional_sni}
To mitigate bias from dependence on ASR$_i$, we propose an intervention on the non-causal effect $X \leftarrow Z$.   
This approach diversifies the noise words in the pseudo transcripts, including those rarely corrupted by ASR$_i$. 
By applying do-calculus as shown in Eq.~\ref{eq:do}, we derive a following equation for SNI:
\begin{equation}
    P(t^{k}|do(x^{k})) = \sum_{z}P(t^{k}|x^{k},z) \cdot P(z).
                                \label{eq:do-calculus}
\end{equation}
This intervention ensures that the corruption of words $x^k$ in the pseudo transcripts does not depend on any particular ASR system. 
Consequently, it allows for the corruption of words that are typically less susceptible to errors under ASR$_i$.

For each word $x^k$,  the prior probability $P(z)$ in Eq.~\ref{eq:do-calculus} represents the probability that any given word $x^k$ will be corrupted.
To simulate $P(z)$, we sample a random variable $a^k$ for each word $x^k$ from a continuous uniform distribution over the interval $[0,1]$.
If $a^k \leq P(z)$, we set $z$ to 1, indicating an incorrect transcription of $x^k$ and generating its noise word $t^{k}$. 
Otherwise, $z$ is set to 0, and $t^{k}$ remains identical to $x^{k}$, mimicking an accurate transcription. 
We set the prior probability $P(z)$ as a constant hyperparameter for pseudo transcript generation.


To generate a noise word $t^k$ whose corruption variable $z^k$ is determined independently of any biases, we adopt a constrained generation technique that outputs $t^{k}$ to input $x^{k}$~\cite{constdecoder}.
To implement constrained generation, we use BERT~\cite{devlin-etal-2019-bert} for encoding the written GT $X$ into the vector representation $E$ as follows:
\begin{equation}
    E_{encoder} = \textit{BERT}(M_{word}(X)+M_{pos}(X)),
    \label{eq:encoder}
\end{equation}
where $e_{encoder}^{k} \in E_{encoder}$ is the encoder representation of the token $x^{k}\in X$ and $M_{word}$ and $M_{pos}$ denote word and position embeddings.


The transformer decoder~\cite{NIPS2017_3f5ee243} generates $t^{k}$ constrained on $x^k$.
To encompass all ASR error types, the transformer decoder generates multiple tokens (see Section~\ref{sec:overview}), denoted as $m$ tokens, $\{\Tilde{t}^{k}_{l}\}_{l=1}^{m}$.  
These tokens replace $x^k$ in the pseudo transcripts. 
 The error type of $t^{k}$ is contingent on $m$:
 \begin{itemize}
     \item $m=1$ corresponds to deletion, generating only eos is generated; $x^k$ is substituted by the empty string. 
    \item If $m=2$, one token in addition to eos is generated; this token substitutes $x^k$.
    \item When $m>2$, additional token will be inserted to $x^k$, to simulate insertion errors.
 \end{itemize}


To generate $\Tilde{t}^{k}_{l}$, the input of the decoder comprises the encoder representation of the written word $e_{encoder}^{k}$ and the special embedding vector $bos$ (beginning of sequence) and the tokens generated so far, $\{\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}\}$ as follows:
\begin{equation}
    E_{decoder}^{k}= H_{decoder} \cdot [e_{encoder}^{k}; bos,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}],
    \label{eq:decoder_input}
\end{equation}
where $H_{decoder}$ is the weight matrix of the hidden layer in the decoder.
The transformer decoder then computes the hidden representation $d^{k}$ by processing the input through its layers as follows:
\begin{align}
    d^{k}= TransformerDecoder(Q,K,V),\\
    Q=E_{decoder}^{k},K,V=E_{encoder},
    \label{eq:decoder}
\end{align}
where $E_{decoder}^{k}$ serves as query $Q$, and $E_{encoder}$ is used for both key $K$ and value $V$ in the transformer decoder.
Finally, the probability of generating each token $\Tilde{t}^{k}_{l}$ is calculated using a softmax function applied to the product of the word embedding matrix $M_{word}$ and the hidden representation $d^{k}$ added to the trained bias $b_{n}$:
\begin{equation}
    P_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = softmax(M_{word} \cdot d^{k}+b_{n}),
    \label{eq:gen_prob}
\end{equation}
where $b_{n}$ are trained parameters. 
Here, we note that ISNI generates different error types depending on the output as we explained in Sec.~\ref{sec:overview}.

We used the ASR transcription $T$ to train ISNI model.
ISNI is supervised to maximize the log-likelihood of the $l$-th token $\hat{t}^{k}_{l}$ from the ASR transcription as follows:
\begin{equation}
    \mathcal{L}_{n} =-\sum log(\textit{P}_{n}(\hat{t}^{k}_{l}|x^{k},\hat{t}^{k}_{0},..., \hat{t}^{k}_{l-1})).
\end{equation}


\subsection{Phoneme-aware Generation for Generalizability}
\label{phoneme_head}

The next step is to ensure the noise word generation $P(t^{k}|x^{k},z)$ ASR$_*$-plausible.
We adjust the generation probability $P_{n}$ with the phoneme-based generation probability $P_{ph}$ so that the ASR$_*$-plausible noise words can be generated as followed:
\begin{multline}
    \textit{P}_{gen}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = \textit{P}_{n}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) \\ \cdot \textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}).  
    \label{eq:phoneme_correction_prob}
\end{multline}

Our first proposal for $\textit{P}_{ph}$ is to provide the phonetic characteristics of each token via phoneme embedding $M_{ph}$.
%Our proposed phoneme embedding $M_{ph}$ is designed to have the phonetic information of each token in the vocabulary.
$M_{ph}$ assigns identical embeddings to tokens sharing phonetic codes, thereby delivering how each word is pronounced.
Phoneme embedding $M_{ph}$ is incorporated into the input alongside word and position embeddings as follows:
\begin{multline}
     E_{encoder} = BERT(\lambda_{w}\cdot M_{word}(X)\\+(1-\lambda_{w})\cdot M_{ph}(X)+M_{pos}(X)),
    \label{eq:phoneme_encoder}
\end{multline}
where $\lambda_{w}$ is a hyperparameter that balances the influence of word embeddings and phoneme embeddings.
The input for the decoder is formulated similarly to Eq.~\ref{eq:decoder_input}.


Fed both the word and phoneme embedding, the decoder then can understand the phonetic information of both the encoder and decoder input.
Aggregating such information, the decoder would yield the hidden representation $d^{k}$ as in Eq.~\ref{eq:decoder}.
Then, we feed the hidden representation $d^k$ to classification head to evaluate the phoneme based generation probability $\textit{P}_{ph}$ as follows:
\begin{equation}
    \textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1}) = softmax(M_{ph} \cdot d^{k}+b_{ph}),
    \label{eq:phoneme_gen_prob}
\end{equation}
where classification head has the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$.
Using the phoneme embedding $M_{ph}$ instead of the word embedding $M_{word}$ in Eq.~\ref{eq:gen_prob}, $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ can be evaluated based on the phonetic information.
%Then, we feed the hidden representation $h^k$ to classification head with weight matrix is the phoneme embedding matrix same as in Eq.~\ref{eq:phoneme_encoder} and bias $b_{ph}$  evaluate the phoneme based generation probability $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$ as follows:


Our second proposal for $\textit{P}_{ph}$ involves supervising the phonetic information using phonetic similarity.
This approach aims to generate ASR$_*$-plausible noise words by assessing the phonetic resemblance of each token to $x^k$.
$\textit{P}_{ph}$ should evaluate how phonetically similar each token is to the $x^{k}$.
Phonetic similarity is advantageous as it quantifies the differences in phonetic codes, thereby allowing for objective supervision of $\textit{P}_{ph}(\hat{t}^{k}|x^{k})$.
We utilize the phoneme edit distance $D$, as outlined in \citet{9662078}, to calculate phonetic similarity. 
The phoneme edit distance $\textit{D}(w^{p}, w^{q})$ measures the minimum edit distance between the phonetic codes of two words, reflecting how closely one word is pronounced to another. 
Notably, $\textit{D}(w^{p}, w^{q})$ leverages articulatory features to compute similarity, which incrementally increases as the phonetic resemblance between the word pair enhances.

Phonetic similarity, $S$, is defined as follows:
\begin{equation}
    \textit{S}(w^{p}, w^{q}) = max(|C_p|-\textit{D}(w^{p}, w^{q}), 0),
\end{equation}
where $|C_p|$ is the length of the phonetic code of the word $w^p$.
This formulation ensures that $\textit{S}(w^{p}, w^{q})$ attains higher values when $w^p$ and $w^q$ are phonetically similar, and approaches zero when there is no phonetic resemblance.


To supervise $\textit{P}_{ph}$, phonetic similarity should be formulated as a probability distribution. 
For such purpose, we normalize phonetic similarity and compute the supervision $\textit{R}(\hat{t}^{k})$ as follows:
\begin{equation}
    \textit{R}(\hat{t}^{k}) = \frac{\textit{S}(t^{k},w)}{\sum_{w^{\prime}\in W}\textit{S}(t^{k},w^{\prime} )}.
 \end{equation}
Then, $\textit{P}_{ph}$ is supervised by loss defined as follows:
 \begin{equation}
     \mathcal{L}_{ph} = KL(\textit{P}_{ph}(\Tilde{t}^{k}_{l}|x^k,\Tilde{t}^{k}_{0},..., \Tilde{t}^{k}_{l-1})| \textit{R}(\hat{t}^{k})),
 \end{equation}
 where $KL$ is the KL divergence loss.
Finally, ISNI is optimized to jointly minimize the total loss $\mathcal{L}_{tot}$ which is defined as follows:
\begin{equation}
    \mathcal{L}_{tot} = \mathcal{L}_{n} + \lambda_{ph} \cdot \mathcal{L}_{ph},
    \label{eq:total_loss}
\end{equation}
where $\lambda_{ph}$ is the weight of $\mathcal{L}_{ph}$.
Supervised to evaluate the generation probability based on the phoneme information, the phoneme generation probability $\textit{P}_{ph}$ ensures the ASR$_*$-plausible noise words and $M_{ph}$ contains phonetic information.
 

 




==> backup/ARR_June/4_experiment.tex <==
\section{Experiments}
In this section, we delineate our experimental setup, datasets, and baseline, for SNI and SLU.
Our experiments, conducted in an ASR zero-shot setting, train SNI models on one ASR system (ASR$_i$) and test SLU models on another (ASR$_j$), to evaluate generalizability across different ASR systems.
\begin{comment}
In this section, we outline the datasets and baselines for evaluating SNI and SLU models, alongside descriptions of ASR systems used for SNI training and SLU testing. 
Our experiments are conducted in ASR zero-shot setting, where SNI models trained on one ASR system (ASR$_i$) and SLU models are tested on another (ASR$_j$), evaluating model generalizability across different ASR systems. Comprehensive experimental details follow to elucidate our methodology.

Our experiments, conducted in an ASR zero-shot setting, train SNI models on one ASR system (ASR$_i$) and test SLU models on another (ASR$_j$), to evaluate generalizability across different ASR systems.
\end{comment}

%how we formulated the ASR zero-shot setting, where SNI models are trained on one ASR system (ASR$_i$), while SLU models are tested using a different ASR system (ASR$_j$), for SLU tasks, ASR GLUE and DSTC10 Track 2. 
%We also note that SLU models are trained with pseudo transcripts generated by SNI models.
%In this section, we thoroughly deliver experimental details SNI training and SLU testing.}
\subsection{Dataset}
\label{sec:dataset}
\paragraph{SNI Training} For SNI training, we selected datasets consistent with our primary baseline, Noisy-Gen~\cite{noisygen}, utilizing three popular corpora: Common Voice, Tatoeba audio, and LJSpeech-1.1, with the MSLT corpus serving as the validation set. Audio recordings from these sources were processed using DeepSpeech to collect transcriptions that exhibit ASR errors. This approach yielded approximately 930,000 pairs of ground-truth and ASR-noised transcriptions.

\paragraph{SLU Training} To demonstrate ASR generalizability across diverse SLU tasks, we utilize two benchmarks: ASR GLUE and DSTC10 Track 2. 
ASR GLUE, an adaptation of the widely recognized NLU benchmark GLUE, includes two natural language inference tasks, QNLI and RTE, and one sentiment classification task, SST2. 
To simulate real-world background noises, ASR GLUE benchmark randomly injected background noise audios into speech.  
Noises are injected in 4 levels, high and medium, low and clean.
Randomly injected noises introduce ASR errors across a broader range of phonemes.
DSTC10 Track 2, tailored for spoken language dialogue systems, comprises three subtasks: Knowledge-seeking Turn Detection (KTD), Knowledge Selection (KS), and Knowledge-grounded Response Generation (RG). 
Details of the datasets for SNI training and SLU testing are available in Appendix~\ref{sec:dataset_details}.


\subsection{Baselines}
In our study, we utilized diverse SNI models, including the GPT2-based auto-regressive SNI model, NoisyGen, as our primary baseline, given its proven efficacy in various spoken language tasks~\cite{noisygen,asrglue}. 
For the ASR GLUE benchmark, we also included NoisyGen (In Domain)~\cite{asrglue}, another GPT2-based SNI model that, unlike our standard approach, uses the same ASR system for both training and testing, thereby not adhering to the ASR zero-shot setting.
Also, PLMs trained only with written GT are used to show the necessity of exposure to ASR noises.
Demonstrating that SNI models can match or surpass NoisyGen (In Domain) will confirm their ASR generalizability.

Additionally, for the DSTC10 Track 2, we incorporated the state-of-the-art TOD-DA~\cite{tian2021tod-da} as a baseline, selected for its inclusion of both TTS-ASR pipeline and textual perturbation techniques, which are absent in NoisyGen.
For DSTC10 Track2, we adopted state-of-the-art baseline TOD-DA~\cite{tian2021tod-da}.
We selected TOD-DA because it covers two distinct categories of SNI which were not covered by NoisyGen: TTS-ASR pipeline and textual perturbation. 
%It implements the TTS-ASR pipeline with the TTS engine from Google Translate and the wave2vec ASR.
%Also, it conducted character-level perturbation of substitution, insertion and deletion, and swap and split.





\subsection{ASR system for SNI training and SLU testing}
We provide the ASR systems used for SNI training and SLU testing in Table~\ref{tab:ASRs}.
\paragraph{SNI Training}
We selected the open-source commercial Mozilla DeepSpeech ASR system~\cite{deepspeech} primarily because it aligns with our main baseline, NoisyGen, and other studies involving commercial ASR systems\footnote{For a detailed comparison of commercial ASR systems, see Appendix\ref{sec:asr_details}}\hist{missing period (.)} \hist{+ 여기 글이 좀 이해가 안 되는데, NoisyGen 은 Mozilla DeepSpeech ASR 을 쓰고 다른 놈들은 commercial ASR 을 썼는데, 우리 메인 베이스라인은 NoisyGen 이니까 Mozilla DeepSpeech 를 썼다는 걸까요?}
Furthermore, despite being trained on DeepSpeech, our ISNI model demonstrates substantial generalizability, outperforming SNI models that rely on newer ASR systems, such as LF-MMI TDNN for NoisyGen (In Domain)~\cite{asrglue} and Wave2Vec for TOD-DA~\cite{yuan2017wave2vec}.\hist{왜 실험 결과같은 내용이 여기에?}

\input{table/asr_setting_merged}
%\input{table/ASR_setting_subtable}
%\input{table/sni_training_asr}
\paragraph{SLU Testing} To evaluate the generalizability of SNI across various ASR systems, we employed distinct ASR systems for SLU testing in the ASR GLUE and DSTC10 Track 2 benchmarks.
As detailed in Table~\ref{tab:ASRs}, the ASR GLUE test set was transcribed using an LF-MMI TDNN-based ASR system, while an unknown ASR system was used for the DSTC10 Track 2 validation and test sets.

%\input{table/slu_testing_asr}
\input{table/asrglue_result}



\subsection{Experimental Settings}
\paragraph{SNI Training}
For ISNI implementation, we utilized BERT-base~\cite{devlin-etal-2019-bert} as an encoder and a single Transformer decoder layer~\cite{NIPS2017_3f5ee243}, aligning with established methodologies~\cite{constdecoder}.
The balance between word and phoneme embeddings was set with $\lambda_{w}$ at 0.5 in Eq.~\ref{eq:phoneme_encoder}, and the phoneme generation loss weight $\lambda_{ph}$ was also adjusted to 0.5 (Eq.~\ref{eq:total_loss}).
We provide further details in Appendix~\ref{sec:ISNI_model_detail}.

\paragraph{SLU Training}
Utilizing the trained ISNI, we convert the written GTs into pseudo transcripts. 
During the generation of pseudo transcripts, we set the prior probability $P(z)$ for ASR GLUE at 0.15 and for DSTC10 Track2, at 0.21, based on validation set result of downstream SLU tasks\footnote{Directly matching $P(z)$ to the word error rate (WER) of the ASR system is not feasible in an ASR zero-shot setting where WER for unknown ASR systems is not available. Additionally, training with arbitrary word error rates might bias the SLU model towards certain ASR systems.}. 
To ensure a fair comparison, we set phonetic similarity thresholds in our baseline, NoisyGen, for filtering out dissimilar pseudo transcripts, based on the validation set result of downstream SLU tasks. 
In terms of downstream task models, we implemented BERT-base for ASR GLUE and GPT2-small for DSTC10 Track 2, consistent with baseline configurations~\cite{dstc10_2,asrglue}.

















==> backup/ARR_June/5_results.tex <==
\section{Results}


\input{table/dstc_result}
We now present our experimental results, 
aiming to address each of the following research questions:
\noindent \textbf{RQ1:} Is the ASR zero-shot setting valid and how effective are ISNI in the ASR zero-shot setting?

%\noindent \textbf{RQ2:} Can ASR$_*$-plauisible pseudo transcriptions be generated without phonetic information?

\noindent \textbf{RQ2:} Can ISNI robustify the various SLU tasks in the ASR zero-shot setting?

\noindent \textbf{RQ3:} Does each of methods contribute to robustification?

\subsection{RQ1: Validity of ASR Zero-shot Setting and Effectiveness of ISNI. }
%Then, we now study the ASR generalizability of our proposed methods with the ASR GLUE benchmark.
%We report the results on the ASR GLUE benchmark in Table~\ref{tab:asrglue_result}.
To demonstrate the ASR generalizability of SNI models, we compare them with NoisyGen (In Domain) on ASR GLUE in Table~\ref{tab:asrglue_result}.
Unlike Noisy-Gen and our models tested in an ASR zero-shot setting, NoisyGen (In Domain) was trained and tested using the identical ASR system, which is incompatible with the ASR zero-shot setting.


%First, we show that existing auto-regressive generation SNI models are not generalizable across ASR systems.
Our findings indicate that auto-regressive SNI lacks generalizability for diverse ASR systems.
If different ASR systems have similar error distributions, existing auto-regressive generation SNIs would generalize in an ASR zero-shot setting.
However, NoisyGen is consistently outperformed by NoisyGen (In Domain) in every task.
%Interestingly, in QNLI, the accuracy of Noisy-Gen (In Domain) in the high noise level was higher than that of Noisy-Gen in the medium noise level.
This result validates the ASR zero-shot setting where existing auto-regressive generation-based SNI models struggle to generalize in the other ASR systems.




Results of ISNI suggest that ISNI can robustify SLU model in the ASR zero-shot setting.
ISNI surpassed NoisyGen in every task in every noise level even NoisyGen (In Domain) in high and medium noise levels for QNLI and in low noise levels for SST2.
Such result might be attributed to the diversified ASR errors in the ASR GLUE benchmark, which ISNI is specifically designed to target.



ISNI demonstrated robust performance across varying noise levels compared to baselines, maintaining its efficacy as noise levels escalated.
This result highlights that ISNI can better robustify against phoneme confusions, which increase under noisy conditions~\cite{wu2022phonetic,petkov2013maximizing}.
%That is, as prior work suggests, phoneme confusions more frequently occur~\cite{wu2022phonetic,petkov2013maximizing} and ours can robustify even when such phoneme confusion increases.




%For the knowledge selection subtask, our method achieved a significantly higher MRR@5 of 71.12\% compared to the baseline methods, where the TOD-DA followed ours with 67.29\% and such tendency was also confirmed in other metrics of R@1,5. 
%This demonstrates the effectiveness of our approach in accurately selecting the relevant knowledge for the given dialogue context. 
%Specifically, the improvement in knowledge selection shows that our SNI method can better robustify the PLMs on retrieval task where lexical similarity is largely considered.


%In the response generation subtask, our method outperformed the baseline methods in every metric. 
%However, different from the knowledge selection subtask, on the other hand, noisygen followed ours.
%This indicates that our SNI method can better robustify the PLMs on generation task.


%Regarding the knowledge turn detection subtask, our method achieved comparable results to the baseline methods, noisygen. 
%The precision, recall, and F1-score of our method were similar to those of the baselines, indicating that our approach effectively detects the points in the dialogue where knowledge-seeking turns occur. 
%This is crucial for identifying the moments when the dialogue context requires accessing specific knowledge.








\subsection{RQ2: Robustification of ISNI on Various SLU Tasks.}
We demonstrate that ISNI significantly enhances robustness across various SLU tasks in an ASR zero-shot setting, particularly in KS, where lexical perturbation heavily influences retrieval~\cite{ir_error_robustness1, ir_error_robustness2}.

Results from the DSTC10 Track 2 dataset, in Table~\ref{tab:dstc_results}, 
reveal that while baseline models struggle in the ASR zero-shot setting, showing R@1 score below 60, ISNI consistently outperforms these models across all metrics.
This superior performance, especially notable in KS, validates ISNI's effectiveness against errors from unknown ASR systems, unlike previous models that require identical ASR systems for both training and testing~\cite{asrglue,noisygen}.


Additionally, the robustification of ISNI extends beyond KS.
ISNI excels across all evaluated tasks, markedly improving the BLEU score by 2-3 times for Response Generation (RG). 
These findings affirm ISNI's capacity to substantially mitigate the impact of ASR errors across diverse SLU tasks.



\subsection{RQ3: Importance of Each Proposed Method to the Robustification. }
To confirm that each of ISNI contributes to the robustification, we conducted the ablation studies in Table~\ref{tab:dstc_results} by deducting each of the proposed methods.
Performance drops gradually as each of our methods is ablated as expected in KS and RG showing the contribution of phoneme-aware generation and intervention.
Due to space limit, we leave the detailed analysis of ablations in Appendix~\ref{sec:ablation_studies}.



\begin{comment}


To conduct the ablation on the intervention itself, we trained a constrained decoding-based SNI model without do-calculus-based random corruption as in Eq.~\ref{eq:do-calculus}.
As the constrained decoding method in ASR correction~\cite{constdecoder}, the corruption module, which determines whether the word $x^k$ will be corrupted, is jointly learned with the generation decoder.
Such module can be considered as implementing $P(z|x^k)$ in Eq.~\ref{eq:likelihood}.
The result is shown in the last row of Table~\ref{tab:dstc_results}. 
%Performance drops as expected in KS, which is our main consideration as it is 
being largely influenced by lexical perturbation due to the ASR errors.
Such decrease is also observed in RG, showing that substituting the intervention contributes to the decreased performance in KS and RG.
Unexpectedly, the last row of Table~\ref{tab:dstc_results} shows the improved performance of KTD. 
We suspect such increase in KTD is due to its characteristic of text classification.
Meanwhile, prior work suggests that even the text classification may still degrade,  when the noises are more abundant in the training set~\cite{4470224}, to which ISNI may contribute.

\end{comment}
%Previous work suggests that the abundance of noises in the training set may fail robustification in text classification \cite{4470224}.






==> backup/ARR_June/6_conclusion.tex <==
\section{Conclusion}
\begin{comment}
In this paper, we tackled the problem of ASR generalizability in SNI, where training the SLU task with pseudo transcription generated by SNI model cannot robustify the downstream SLU models against ASR error generated by different ASR systems.
To solve the problem of ASR generalizability in SNI, we proposed the interventional SNI and phoneme correction.
The interventional SNI contributes to the diversity in generated pseudo transcription, so that it contains the ASR plausible errors of diverse phonemes.
The phoneme correction increases the plusiblity of generated pseudo transcription, which results in generating phonetically similar ASR plausible errors.
Then, we showed that our proposed methods are effective in robustifying the downstream SLU tasks against ASR errors while generalizing across different ASR systems.
\end{comment}
In this paper, we address the challenge of ASR generalizability within the context of SNI. 
We focus on enhancing the robustness of SLU models against ASR errors from diverse ASR systems. 
Our contributions are two-fold: Firstly, ISNI significantly broadens the spectrum of plausible ASR errors, thereby reducing biases. 
Second, not to lose the generality to any ASR, we generate noises that are universally plausible, or ASR$_*$-plausible,
which is empirically validated through extensive experiments across multiple ASR systems.
%Our empirical results validate the effectiveness of our proposed approaches. Through extensive experiments, we demonstrate how our methods substantially bolster the resilience of downstream SLU tasks against ASR errors, even when confronted with variations across different ASR systems.


==> backup/ARR_June/limitations.tex <==
\paragraph{Limitations.}

As ISNI is trained with speech corpora collected for academic purposes, they may face challenges when adopted for real-world applications, including
%We think ISNI would suffer from challenges similar to those encountered by ASR systems.
%One example is handling 
diverse spoken language variations such as dialects and accents. 
These variations can introduce noises that are not phonetically similar, which are different from the speech data used during ISNI training. 
This discrepancy may fail ISNI to robustify SLU models as ISNI is not prepared to handle ASR errors from those speech variations.  %, potentially impacting its ability to robustify spoken language understanding (SLU) models across all speech variations. 
Addressing this limitation may require enlarging the training dataset for ISNI
to cover the diverse noises
%to include a wider array of noises due to such 
from spoken language variations.
%ensuring it can effectively generalize across the diverse speech conditions found in practical applications.

%We make use of DeepSpeech ASR system, for the reason of its similarity in performance to many commercial ASR systems as we will discuss in Sec.~\ref{sec:asr_details}.


%However, our ISNI may not well be trained with different ASR systems due to several reasons.
%A notable reason is the scarcity of the training set due to rare ASR errors.
%As we described in Sec.~\ref{sec:dataset}, we only use the erroneous transcriptions for training ISNI.
%However, when the ASR system is too strong, it may make not enough erroneous transcriptions to train ISNI.
%The most straightforward method is to use the other weaker ASR system for training, as our ISNI can %generalize to different ASR systems.
%Second, previous works suggest training the weaker version of the ASR system and using it for training SNI~\cite{dutta2022error}.





==> table/ASR_setting_subtable.tex <==
\begin{table}[ht]
    \centering
    \begin{subtable}[t]{0.45\textwidth}
        \centering
        \caption{First subtable}
\scalebox{0.7}{
\begin{tabular}{l|c|c|c|c}
\hline
SNI & \multicolumn{1}{l|}{ISNI} & NoisyGen & NoisyGen (In Domain) & TOD-DA   \\ \hline
ASR & \multicolumn{2}{l|}{DeepSpeech}      & LF-MMI TDNN          & Wave2Vec \\ \hline
\end{tabular}
}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.45\textwidth}
        \centering
        \caption{Second subtable}
\scalebox{0.7}{
\begin{tabular}{l|c|c}
\hline
    & DSTC Track2 & ASR GLUE    \\ \hline
ASR & Unknown     & LF-MMI TDNN \\ \hline
\end{tabular}
}
    \end{subtable}
\caption{Main caption for the table collection}
\end{table}

==> table/asr_cer.tex <==
\begin{table}[h]
\centering
\scalebox{1.0}{
\begin{tabular}{c|c|c}
\hline
ASR1& ASR2 & CER \\ \hline
Ground Truth & DeepSpeech        &         39.71                \\
Ground Truth  & Leopard &      35.80                  \\
DeepSpeech & Leopard   &    22.01                   \\ \hline
\end{tabular}
}
\caption{Character Error Rate (CER) between different ASR models.}
\label{tab:cer}
\end{table}

==> table/asr_dataset.tex <==
\begin{table}[h]
\scalebox{0.8}{
\begin{tabular}{l|cc|c|c}
\hline
SNI                & \multicolumn{1}{c|}{Ours} & NoisyGen & NoisyGen (Kaldi) & TOD-DA \\ \hline
ASR                & \multicolumn{2}{c|}{DeepSpeech}      & Kaldi            & gTTS   \\ \hline
Identical to Test? & \multicolumn{2}{c|}{}                & \checkmark               &        \\ \hline
\end{tabular}}
\caption{ASR systems used for training SNI models.}
\label{tab:asr_dataset}
\end{table}

==> table/dataset_statistics.tex <==
\begin{table}[h]
\centering
\scalebox{1.0}{
\begin{tabular}{cccc}
\hline
Name & Hours & Recordings & Language \\ \hline
Common Voice & 1488 & 854,444        &        En                \\
tatoeba audio & - & 300,076        &        En                      \\
LJSpeech-1.1 & 24 & 13,100        &        En                       \\ \hline
\end{tabular}
}
\caption{Statistics of speech corpora used for SNI training.}
\label{tab:dataset_stat}
\end{table}

==> table/slu_testing_asr.tex <==
\begin{table}[h]
\centering
\scalebox{0.7}{
\begin{tabular}{l|c|c}
\hline
    & DSTC Track2 & ASR GLUE    \\ \hline
ASR & Unknown     & LF-MMI TDNN \\ \hline
\end{tabular}
}
\caption{ASR systems for testing SLU models.}
\label{tab:SLU_ASR}
\end{table}

==> table/sni_training_asr.tex <==
\begin{table}[h]
\centering
\scalebox{0.7}{
\begin{tabular}{l|c|c|c|c}
\hline
SNI & \multicolumn{1}{l|}{ISNI} & NoisyGen & NoisyGen (In Domain) & TOD-DA   \\ \hline
ASR & \multicolumn{2}{l|}{DeepSpeech}      & LF-MMI TDNN          & Wave2Vec \\ \hline
\end{tabular}
}
\caption{ASR systems for training SNI models.}

\label{tab:SNI_ASR}
\end{table}

==> tex/1_intro.tex <==
\section{Introduction}
Pre-trained language models (PLM) are shown to have a contextual understanding of language and generalization ability across different domains.
PLMs are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842}.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription is fed into PLMs to conduct downstream SLU tasks. 



%As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
As ASR systems incorrectly transcribe the speech into phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689} or, ASR error words, PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.



%Though training PLMs with incorrect transcription can adapt them to SLU, collecting SLU corpora with such incorrect transcriptions requires additional human annotations.
A well-known solution is annotating likely incorrect transcriptions, in addition to correct ground-truth.
Specifically, an SLU corpus requires two additional steps following after collecting the written corpus. 
The collected written language corpus is first recorded in audio by human annotators.
Then they are transcribed into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.


To reduce these additional annotations of recording and transcription, an automated data augmentation method of corrupting the written sentence similar to the ASR transcription, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.  

\input{figure_latex/figure1}
However, we argue that ASR plausibility is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error plausible for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

%As different ASR systems can be used in SLU pipeline~\cite{blackbox1},
For PLMs to be used with arbitrary ASR systems,
we propose to generate pseudo transcription such that 
1) not exactly ASR plausible for an individual ASR system,
while 2) generally ASR plausible.


First, we propose not to exactly follow an individual ASR system.
As SNI models are supervised to maximize the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model would exactly mimic an individual ASR transcript and corrupt the phonemes that were frequently corrupted by such ASR system.
To show such mimicking explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
For example, in Fig.~\ref{fig:example}, SNI trained with transcription by ASR 1 would only corrupt the word `cue', following the ASR 1.
Training with such pseudo transcripts would only robustify against the errors by ASR 1.
Therefore, our proposed SNI model would have a corrupting probability $P(z|x)$ different from an individual ASR system. 

Second, we argue that the pseudo transcripts that are not ASR plausible for one ASR system can still be ASR plausible for the other ASR systems.
While different ASR systems would make errors on the words of different phonemes, such errors would be common in that they are phonetically similar to their ground truth words.
For example, while ASR 1 and 2 would confuse different phonemes, `c' for ASR 1 and `r' for ASR 2, they are converted into similarly pronounced phonemes such as `cereal' to `serial' and `workers' to `walkers'.
Similarly, pseudo transcripts can still be ASR plausible by the other ASR systems, unless they are phonetically similar to their written sentences.

%we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
%For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.

%However, due to the supervision of maximizing the likelihood of the ASR transcription given its written sentence~\cite{asrglue, noisygen}, the SNI model is biased to mimic an individual ASR system.
%Such bias results in the following two problems blocking the generalization of ASR probability:
%1) Distribution bias: Only the limited range of phonemes that are favored in error distribution of an individual ASR system would be covered.
% 1) Narrowed noise problem where only the narrow range of phonemes that are frequently incorrectly transcribed by an individual ASR system would be corrupted in the resulting pseudo transcription.
%To show such bias explicitly, we introduce a binary variable $z$, which determines whether the word $x$ in the written sentence would be corrupted, where $P(z|x)$ is the probability of corrupting $x$ to the noise word.
%For example, as depicted in Fig.~\ref{fig:example}, one ASR system would make errors of corrupting `c' to `s' such as `cereal' to `serial' and `cease' to `sees'.
%Trained to follow such ASR errors, SNI is biased that $P(z|x)$ is high for the word $x$ containing `c' while it is low for the words with `r'.
%Due to such bias, SNI model would corrupt only the word `cue' containing the  `c'.
%2) ASR improbable noise problem: The generated noise words may be ASR-improbable as the SNI model is blinded to the phonetic information.
% 2) ASR improbable noise problem where the generated noise words would be ASR-improbable as the SNI model is blinded to the phonetic information.
%Blinded to the phonetic information that `c' in the word `cue' corresponds to the phoneme `k', `c' is considered to be pronounced similarly to the `c' in the `cereal' and `cease' as the phoneme `s'.
%As a result of bias to an individual ASR system and blindness to phonetic information, the resulting pseudo transcription would contain narrow and ASR-improbable noise words. 



For such goal: we propose Interventional Speech Noise Injection (ISNI). 
To generate pseudo transcripts not exactly ASR plausible for an individual ASR system,
we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
Do-calculus enables diversification by replacing $P(z|x)$ into $P(z)$ which results in the cutting off the corrupting probability of the frequently corrupted phonemes and increasing for the rarely corrupted phonemes as depicted in Fig~\ref{fig:example}. 
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, our constrained decoding generates only the ASR-probable noise words given the words in the written sentences.
Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, where chosen words are corrupted to noise words by constrained decoding. 
For example, our SNI corrupts words with distinct phonemes such as `reading' and `cue' as depicted in Fig.~\ref{fig:example} as a result of such diversification.



Second, to generate generally ASR plausible pseudo transcripts, we propose to correct the generation of phonetically different noise words. 
The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
However, previous models are ignorant of such phonetic information.
We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
For example in Fig.~\ref{fig:example}, the ASR system frequently generates incorrect transcription of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR improbable noise word `sue'.
To remedy such ignorance, we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR probable, noise word `queue'.
Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR-probable.




Our major contributions to ASR-generalizable SNI are threefold:
1) propose an interventional method to generate pseudo transcript such that not exactly ASR plausible for an individual ASR system
2) propose phoneme correction which generates generally ASR plausible pseudo transcripts
and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> tex/1_intro_alt.tex <==

\section{Introduction}

Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 


However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

A well-known solution is \ {robustifying the PLMs to such errors, by augmenting the data.
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
This requires two additional steps following after collecting the written corpus-- recording in audio by human annotators, and transcribing into text using ASR systems.
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus and converts the written corpus into pseudo transcription using the trained language model.
% of corrupting the written sentence similar to the ASR transcription,
% Specifically, SNI noises the given written sentence into pseudo transcription which the ASR system would probably transcribe into.
% In order to generate pseudo transcription, a ground-truth word in the written sentence should be phonetically similar, which ASR systems would probably confuse the ground-truth word into.

\input{figure_latex/figure1}
However, we disclose two blind spots of such assumption of ASR plausibility.
First, language models trained with a corpus from a single ASR system are prone to \textit{character confusables}. 
Since the characters of the written corpus are fed to the language models, not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face character confusables-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).


Second, language models trained with a single-ASR-generated corpus have \textit{distribution bias}.
Different ASR systems (e.g. Siri, Cortana, etc.) can be used in SLU pipeline~\cite{blackbox1}, yielding different errors.
Ideally, speech noises generated from the true ASR error distribution should contain all of these errors. 
However, current SNI models are biased to an individual ASR error distribution~\cite{different_error_distribution}.
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution (Fig. \ref{fig:example}).
Only when this bias is resolved, the generated corpus would be closer to the true ASR-noise distribution. 
The PLMs trained against true ASR error distribution would be robust to diverse ASR systems, even on newly-developed unseen ASR systems.


In this paper, we propose Interventional Speech Noise Injection (ISNI), to overcome such deficiencies.
On the one hand, to resolve the character confusables, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

On the other hand, to alleviate the distribution bias, we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}).
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r' (Fig.~\ref{fig:example}). This helps the PLMs trained on such words be robust to different ASR systems also.


Experiments on DSTC10 Track2 and ASR GLUE benchmark show that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.

Our major contributions to ASR-generalizable SNI are \ {as follows}:

\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: character confusables, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove character confusables.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
\end{itemize}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.


==> tex/1_intro_merge.tex <==

\section{Introduction}
\jslee{
Pre-trained language models (PLMs) are widely adopted for spoken language understanding (SLU) in voice assistants~\cite{broscheit-etal-2022-distributionally, 8907842},
due to their contextual understanding of language and generalization ability across different domains.
}
For example, after the automatic speech recognition system (ASR) transcribes the audio, the resulting transcription can be fed into PLMs to conduct downstream SLU tasks. 

\jslee{
However, since ASR systems incorrectly transcribe the speech into ASR error words-- phonetically similar but semantically irrelevant words~\cite{ruan20_interspeech,9054689}-- 
PLMs suffer to understand semantics from such erroneous transcription.
}
For example, in Fig.~\ref{fig:example}, confusing between  ``cereal'' and ``serial'', ASR systems may generate an incorrect transcription of ``workers eat serial in the cay''  as depicted in Fig.~\ref{fig:example}.
ASR errors words, despite the phonetic similarity, represent unintended meanings and in turn hinder the semantics of the speech from the resulting incorrect transcription.
As a result of such corruption, PLMs cannot robustly understand the semantics of the original speech and make incorrect predictions on SLU~\cite{belinkov2018synthetic}.

While a well-known solution is \jslee{to robustify the PLMs by training with such incorrect transcriptions or pseudo transcription, automatically generated incorrect transcription, the recent trend of scaling PLMs makes hard .
One can manually annotate} likely incorrect transcriptions, in addition to correct ground-truth.
\jslee{This requires two additional steps following after collecting the written corpus: Recording in audio by human annotators, and transcribing into text using ASR systems.}
Such additional annotation steps obstruct collecting the large-scale SLU corpora.

To reduce these additional annotations of recording and transcription, an automated data augmentation method, speech noise injection (SNI), is proposed~\cite{heigold-etal-2018-robust,di-gangi-etal-2019-robust}.
SNI assumes the generated corpus from a single ASR system would well-define ASR plausible words. It trains another language model with the generated corpus, and augment the SLU corpora \jslee{by generating} with trained language model.

However, we argue that ASR plausiblity defined by a single ASR system is limited to individual ASR systems, which hinders PLM to be used with different ASR systems. 
As ASR systems have different error distributions, such as phonemes or accents, ASR probability is specific to ASR system~\cite{7178796}.
That is, an error probable for one ASR system may not be probable for other ASR systems~\cite{different_error_distribution}.
For example, the error of corrupting `c' to `s' made by ASR 1 would be improbable to ASR 2 which generates the correct transcript on `serial' while confusing `r' and generating the error word `walkers'. 
Due to the difference in ASR probability, PLMs robust against ASR1 would be fragile to the errors made by ASR 2.

As different ASR systems can be used in SLU pipeline~\cite{blackbox1}, we propose to generalize the notion of ASR probability, so that PLMs can be used generally with arbitrary ASR systems.
For such goal, PLMs should be exposed to ASR errors probable for diverse ASR systems.


\input{figure_latex/figure1}
\jslee{However, we disclose two blind spots of such assumption of ASR plausibility.}
First, language models trained with a corpus from a single ASR system are prone to \textit{hard-negatives}. 
Since the language models rely on only syntatic information, and not to the phonetic information, they may generate ASR-implausible words.
For example, since `c' in the `cereal' and `cease' is considered to be pronounced as the phoneme `s', the ASR-noise tends to change `c' into `s'. Trained with such corpora, if language models face hard-negatives-- For example, `c' in `cue' which corresponds to the phoneme `k', not `s'-- they generate ASR-implausible word, such as `sue' (Fig \ref{fig:example}).

Second, language models trained with a single-ASR-generated corpus has \textit{distribution bias}.
Different ASR makes different errors~\cite{different_error_distribution}, but language models may not be able to generate diverse errors, resulting in low robustness of PLMs.
\jslee{
For example, while ASR1 makes the error of corrupting `c' to `s', it may rarely generate noise on `r', which is a plausible noise in the true ASR-noise distribution.
}
% Due to the difference in ASR plausibility, 
% PLMs robust against ASR1 would be fragile to the errors made by ASR2.
\jslee{
By solving this problem, the noise words will be closer to the true ASR-noise distribution, and the PLMs will be robust to various ASR systems.
}

In this paper, we propose ISNI, to overcome such deficiencies.
\jslee{
On the one hand, to resolve the hard-negatives, 
% we propose to correct the generation of phonetically different noise words. 
% The key characteristic of ASR error words is that the ASR systems incorrectly transcribe into phonetically similar words such as `cue' to `queue'.
% However, previous models are ignorant of such phonetic information.
% We argue that such ignorance biases the SNI model to blindly follow the error distribution of the individual ASR systems.
% To remedy such ignorance, 
we propose to feed the phonetic information and evaluate another phoneme-based generation probability.
}
\jslee{
For example in Fig.~\ref{fig:example}, ASR1 frequently generates error of corrupting `c'  to `s'.
}
Fed only the words, not their phonetic information, previous SNI models confuse `c' in the word `cue' to be pronounced as `s' and generate the ASR implausible noise word `sue'.
Aware of the phonetic information that `c' is pronounced as phoneme `k', our SNI model corrupts into the phonetically similar, thus ASR plausible, noise word `queue'.
% Understanding phonemes, the resulting pseudo transcription becomes more phonetically similar to cleanly written sentences and more ASR plausible.

\jslee{On the other hand, to alleviate the distribution bias,} we propose to intervene SNI based on do-calculus~\cite{glymour2016causal} to diversify the noises in the pseudo transcripts.
% Adopting do-calculus in SNI, we intervene in the effect of the word $x$ on $z$.
% Do-calculus enables diversification by 
\jslee{Do-calculus replaces $P(z|x)$ into $P(z)$, which reduces the corrupting probability of the frequently corrupted phonemes and increases the rarely corrupted phonemes (Fig~\ref{fig:example}). }
To implement do-calculus in SNI, we propose to adopt constrained decoding.
Different from previous works generating the whole pseudo transcription given the written sentences, 
our constrained decoding generates only the ASR plausible noise words given the words in the written sentences.
% Using constrained decoding, do-calculus in SNI is implemented by evenly corrupting the words in the written sentences, 
% where chosen words are corrupted to noise words by constrained decoding. 
\jslee{As a result of such diversification, our SNI model trained with ASR1-generated corpus successfully corrupts words the phoneme `r'. This helps the PLMs trained on such words be robust to different ASR systems also (Fig.~\ref{fig:example}).}

\jslee{
Experiments on DSTC10 Track2 and ASR GLUE benchmark shows that ISNI is truly effective-- the BLEU score increases by 2-3x times for response generation, and ISNI even provides significant gains for the unseen ASR systems also.
}

Our major contributions to ASR-generalizable SNI are \jslee{as follows}:
\jslee{
	\begin{itemize}
		\item We point out two blind spots from the ASR plausibility of the conventionally generated speech noise: hard-negatives, and distribution bias.
		\item We devise to provide phonetic information to SNI model, to remove hard-negatives.
		\item We propose to intervene SNI based on do-calculus, to alleviate distribution bias.
		\item Experiments shows that our SNI model, ISNI, significantly increases the performance, even on unseen ASR systems.
	\end{itemize}
}
% 1) propose an interventional method for ASR generalizable SNI
% 2) propose phoneme correction which corrects the generation of ASR implausible noise words
% and 3) show that the proposed methods improve the ASR-generalizability of downstream models.
